Safe Edges: A Study of Triangulation in Fill-in and Tree-Width Problems

This paper considers two well-studied problems \textsc{Minimum Fill-In} (\textsc{Min Fill-In}) and \textsc{Treewidth}. Since both problems are \textsf{NP}-hard, various reduction rules simplifying an input graph have been intensively studied to better understand the structural properties relevant to these problems. Bodlaender at el. introduced the concept of a safe edge that is included in a solution of the \textsc{Minimum Fill-In} problem and showed some initial results. In this paper, we extend their result and prove a new condition for an edge set to be safe. This in turn helps us to construct a novel reduction tool for \textsc{Min Fill-In} that we use to answer other questions related to the problem. In this paper, we also study another interesting research question: Whether there exists a triangulation that answers both problems \textsc{Min Fill-In} and \textsc{Treewidth}. To formalise our study, we introduce a new parameter reflecting a distance of triangulations optimising both problems. We present some initial results regarding this parameter and study graph classes where both problems can be solved with one triangulation.

==> content/grids.tex <==
\section{$\tau$ Parameter and Minimum Fill-In of Grids}\label{sec:tfm:gridsMinusRook}


% retracted (Intro)
\iffalse{
This section is mainly dedicated to showing that $\tau(G)=0$ given a grid graph $G$ with at most four rows and an arbitrarily large number of columns.

% grid
{
First, let us begin with a definition of grids.
An $m\times n$ \textit{gird}, written as $P_m\square P_n$, is the Cartesian product of two paths $P_m,P_n$ on $m,n$ vertices, respectively.
Given a $P_m\square P_n$ grid $G=(V,E)$, for $m,n\geq 2$, we refer to the copies of $P_m$ as the \textit{rows} and the copies of $P_n$ as the columns of $G$.
Additionally, we let $v_{r,c}\in V$ for $r\in \{1,\dots,m\}$ and $c\in \{1,\dots,n\}$ be the vertex in the row $r$ and column $c$ of $G$.
Then, formally, we define:
\begin{multline*}
E=\{v_{r,c}v_{r,c+1}| 
r\in\{1,\dots,m\},
c\in\{1,\dots,n-1\}\}
\, \cup \\
\{v_{r,c}v_{r+1,c}|
r\in\{1,\dots,m-1\},
c\in\{1,\dots,n\}\}\}
\end{multline*}
}
}
\fi

In this section, we extend the results about the parameter $\tau$ equal to 0 also for grid graphs with at most four rows and any number of columns.

Formally, for any $m, n\geq 1$, the $m\times n$ \textit{grid} graph $P_m\square P_n$ is the Cartesian product of two paths $P_m =(v_1, \dots, v_m), P_n=(v_1, \dots, v_n)$.
$P_m\square P_n$ contains all the vertices $v_{r,c}$ where $r\in \{1,\dots,m\}$, $c\in \{1,\dots,n\}$.
For every edge $v_r v_{r+1}$ in $P_m$, $r\in\{1,\dots,m\}$, $P_m\square P_n$ includes the edge $v_{r,c} v_{r+1,c}$ and similarly for every edge $v_c v_{c+1}$ in $P_n$, $c\in\{1,\dots,n\}$, $P_m\square P_n$  has the edge $v_{r,c}, v_{r,c+1}$.

% 2 grid 
{
Grids with a single row, $P_1\square P_n$, or a single column, $P_m\square P_1$  are paths, therefore chordal and obviously have $\tau=0$.
Hence,  we can start by discussing grids with two rows and at least 2 columns.
% Furthermore, we point out that $\textit{mfi}(G)=4n-3$ (as determined in the proof of the aforementioned lemma).

\begin{lemma}\label{lem:2grid2king2hex2tria}
Let $G$ be a $P_2\square P_n$ for $n\geq 2$. 
Then $\tau(G)=0$ and $\textit{mfi}(G)=4n-3$.
\end{lemma}
\begin{proof}
It is shown in \cite{janka} that $\textit{tw}(G)=2$ and obviously $\kappa(G)=2$.
Then by \cref{lem:tw<=2}, $\tau(G)=0$.
$\textit{mfi}(G)=4n-3$ follows from \cref{lem:tw=kConnected} and the fact that the graph $G=P_2\square P_n$, for $n\geq 2$, has $\textit{tw}(G)=\kappa(G)=2$.
\end{proof}
}

% 3xn grids
Using the technique introduced in \cref{sec:safe} we will extend our results to $3\times n$ grid graphs for $n\geq 2$.

\begin{lemma}\label{lem:3grid}
Let $G=(V,E)$ be a $P_3\square P_n$ for $n\geq 2$.
Then $\tau(G)=0$.
\end{lemma}
\begin{proof}

{
\tikzset{
invisible/.style={draw=white, inner sep=0pt, text width=4mm,  align=center}}
\tikzset{
mystyle/.style={draw=black,rectangle, inner sep=0pt, text width=4.7mm, text height=1.75 mm,  align=right}}
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.4\textwidth}
    \begin{tikzpicture}[scale=0.35,every node/.style={draw=black, rectangle, inner sep=0pt, text width=8mm, text height=1.75 mm,  align=right}]
    \node [mystyle] [ label=left:{\scriptsize 5$\rightarrow$}] (v21) at (0,0) {\tiny{$v_{2,1}$}};
    \node [mystyle] (v32) at (2,-2) {\tiny{$v_{3,2}$}};
    \node [mystyle] (v12) at (2,2) {\tiny{$v_{1,2}$}};
    \node [mystyle] (v22) at (2,0) {\tiny{$v_{2,2}$}};
    \node [mystyle] (v33) at (4,-2) {\tiny{$v_{3,3}$}};
    \node [mystyle] (v13) at (4,2) {\tiny{$v_{1,3}$}};
    \node [mystyle] (v24) at (4,0) {\tiny{$v_{2,3}$}};
    
    \node (v3n-1) at (7.5,-2) {\tiny{$v_{3,n-1}$}};
    \node (v1n-1) at (7.5,2) {\tiny{$v_{1,n-1}$}};
    \node (v2n-1) at (7.5,0) {\tiny{$v_{2,n-1}$}};
    \node [mystyle] (v2n) at (10,0) {\tiny{$v_{2,n}$}};
    \draw[-] 
    (v3n-1) to (v2n-1)
    (v1n-1) to (v2n-1)
    (v1n-1) to (v2n)
    (v2n-1) to (v2n)
    (v3n-1) to (v2n);
    \draw[-] 
    (v21) to (v22)
    (v32) to (v22)
    (v12) to (v22)
    (v21) to (v32)
    (v21) to (v12)
    (v22) to (v24)
    (v33) to (v24)
    (v13) to (v24)
    (v32) to (v33)
    (v12) to (v13)
    (v33) to (5,-2)
    (v24) to (5,0)
    (v13) to (5,2)
    (v3n-1) to (5.75,-2)
    (v2n-1) to (5.75,0)
    (v1n-1) to (5.75,2);
    \draw[dashed, draw=red]
    (v12) to[out=0, in=0, looseness=0.3] (v32);
    ;
    \draw[dotted]
    (5.2,-2) to (5.7,-2)
    (5.2,0) to (5.7,0)
    (5.2,2) to (5.7,2);
    \draw[dashed]
    ;
    \end{tikzpicture}
    \caption{$G_4$}
    \label{fig:3grid:G'0}   
  \end{subfigure}
  \begin{subfigure}[b]{0.2\textwidth}
    \begin{tikzpicture}[scale=0.35,every node/.style={draw=black, rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
    \node [mystyle] (v32) at (2,-2) {\tiny{$v_{3,2}$}};
    \node [mystyle] (v12) at (2,2) {\tiny{$v_{1,2}$}};
    \node [mystyle] [label=left:{\scriptsize 6$\rightarrow$}](v22) at (2,0) {\tiny{$v_{2,2}$}};
    \node [mystyle] (v33) at (4,-2) {\tiny{$v_{3,3}$}};
    \node [mystyle] (v13) at (4,2) {\tiny{$v_{1,3}$}};
    \node [mystyle] (v24) at (4,0) {\tiny{$v_{2,3}$}};
    \draw[-] 
    (v32) to (v22)
    (v12) to (v22)
    (v22) to (v24)
    (v33) to (v24)
    (v13) to (v24)
    (v32) to (v33)
    (v12) to (v13)
    (v33) to (5,-2)
    (v24) to (5,0)
    (v13) to (5,2);
    \draw[dotted]
    (5.1,-2) to (5.6,-2)
    (5.1,0) to (5.6,0)
    (5.1,2) to (5.6,2);
    \draw[draw=MyColorOne, line width=0.5mm]
    (v12) to[out=0, in=0, looseness=0.5] (v32);
    \end{tikzpicture}   
    \caption{$G_5$}
    \label{fig:3grid:G'1}   
  \end{subfigure}
    \vspace{0.25cm}
  \begin{subfigure}[b]{0.2\textwidth}
    \begin{tikzpicture}[scale=0.35,every node/.style={draw=black, rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
    \node [mystyle] (v32) at (2,-2) {\tiny{$v_{3,2}$}};
    \node [mystyle] [label=left:{\scriptsize 7$\rightarrow$}] (v12) at (2,2) {\tiny{$v_{1,2}$}};
    \node [mystyle] (v33) at (4,-2) {\tiny{$v_{3,3}$}};
    \node [mystyle] (v13) at (4,2) {\tiny{$v_{1,3}$}};
    \node [mystyle] (v24) at (4,0) {\tiny{$v_{2,3}$}};
    \draw[-]
    (v33) to (v24)
    (v13) to (v24)
    (v32) to (v33)
    (v12) to (v13)
    (v33) to (5,-2)
    (v24) to (5,0)
    (v13) to (5,2);
    \draw[dotted]
    (5.1,-2) to (5.6,-2)
    (5.1,0) to (5.6,0)
    (5.1,2) to (5.6,2);
    \draw[draw=MyColorOneDark, line width=0.5mm]
    (v12) -- (v32);
    \draw[draw=MyColorOne, line width=0.5mm]
    (v32) -- (v24)
    (v12)--(v24);
    \draw[dashed,draw=red]
    (v13)--(v32)
    ;
    \end{tikzpicture}   
    \caption{$G_6$}
    \label{fig:3grid:G'2}   
  \end{subfigure}
  \begin{subfigure}[b]{0.225\textwidth}
    \begin{tikzpicture}[scale=0.35,every node/.style={draw=black, rectangle, inner sep=0pt, text width=5mm, text height=1.75 mm,  align=right}]
        \node [mystyle] [label=left:{\scriptsize 8$\rightarrow$}] (v32) at (2,-2) {\tiny{$v_{3,2}$}};
        \node [mystyle] (v33) at (4,-2) {\tiny{$v_{3,3}$}};
        \node [mystyle] (v13) at (4,2) {\tiny{$v_{1,3}$}};
        \node [mystyle] (v24) at (4,0) {\tiny{$v_{2,3}$}};
        \draw[-]
        (v32) to (v33)
        (v33) to (v24)
        (v13) to (v24)
        (v33) to (5,-2)
        (v24) to (5,0)
        (v13) to (5,2);
        \draw[dotted]
        (5.1,-2) to (5.6,-2)
        (5.1,0) to (5.6,0)
        (5.1,2) to (5.6,2);
        
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (v32) to (v24)
        ;
        \draw[draw=MyColorOne, line width=0.5mm]
        (v32) to (v13)
        ;
        \draw[dashed, draw=red]
        (v13) to[out=0, in=0, looseness=0.5] (v33)
        ;
    \end{tikzpicture}  
    \caption{$G_7$}
    \label{fig:3grid:G'3}   
  \end{subfigure}
  \begin{subfigure}[b]{0.125\textwidth}
    \begin{tikzpicture}[scale=0.35,every node/.style={draw=black, rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (v33) at (4,-2) {\tiny{$v_{3,3}$}};
        \node [mystyle] (v13) at (4,2) {\tiny{$v_{1,3}$}};
        \node [mystyle] [label=left:{\scriptsize 9$\rightarrow$}] (v24) at (4,0) {\tiny{$v_{2,3}$}};
        \draw[-] 
        (v33) to (v24)
        (v13) to (v24)
        (v33) to (5,-2)
        (v24) to (5,0)
        (v13) to (5,2);
        \draw[dotted]
        (5.1,-2) to (5.5,-2)
        (5.1,0) to (5.5,0)
        (5.1,2) to (5.5,2);
        \draw[draw=black,style=ultra thick,dotted]
        (7.25,0) to (8.2,0);
        \draw[draw=MyColorOne, line width=0.5mm]
        (v13) to[out=0, in=0, looseness=0.5] (v33);
    \end{tikzpicture}
    \caption{$G_8$}
    \label{fig:3grid:G'4}   
  \end{subfigure}
  \hspace{0.5cm}
  \begin{subfigure}[b]{0.2\textwidth}
    \begin{tikzpicture}[scale=0.35,every node/.style={draw=black, rectangle, inner sep=0pt, text width=8mm, text height=1.75 mm,  align=right}]
        \node [invisible] (x) at (2,0) {};
        \node (v33) at (4,-2) {\tiny{$v_{3,n-1}$}};
        \node (v13) at (4,2) {\tiny{$v_{1,n-1}$}};
        \node (v23) at (4,0) {\tiny{$v_{2,n-1}$}};
        \node [mystyle] (v2n) at (6.5,0) {\tiny{$v_{2,n}$}};
        \draw[-] 
        (v33) to (v23)
        (v13) to (v23)
        (v13) to (v2n)
        (v23) to (v2n)
        (v33) to (v2n);
        \draw[draw=MyColorOne, line width=0.5mm]
        (v13) to[out=0, in=0, looseness=0.35] (v33);
    \end{tikzpicture}
    \caption{$G_{|V|-4}$}
    \label{fig:3grid:G'V-4}   
  \end{subfigure}
  % \caption{
  %   (a)-(e) demonstrate the graph $G_i$ obtained at steps $i\in\{4,\dots,8\}$, of $\alpha$.
  %   For every graph $G_i$, the vertex $\alpha(i+1)$ is pointed out with its label, the edges added by elimination of $\alpha(i)$ are drawn in light green while the previously added edges are shown in dark green.
  %   Additionally, the edges from $F^{\alpha(i+1)}$ are shown with dashed red lines.
  %   Notice that the process of elimination shown in (b)-(d) can be repeated on $G_8$.
  %   Also note that in every step, the vertex $\alpha(i+1)$ in the graph $G_{i}\oplus F^{\alpha(i+1)}$ is either simplicial or it is almost simplicial and $\textit{deg}_{G_i}(\alpha(i+1))=\kappa(G_{i})=3$.
  %   (f) the graph $G_{|V|-4}$ is a $K_4$.
  %   }
  \label{fig:3grid}
\end{figure}
}% fig
Since the $3\times 2$ grid graph is isomorphic to the $2\times 3$ grid, the statement of the lemma follows from \cref{lem:2grid2king2hex2tria} for the case where $n=2$.
So let's consider the case where $n\geq 3$.\unsure{updated}
To show that $\tau(G)=0$, we define a minimum elimination ordering $\alpha$ over $G$ in which $\max_{v\in V}|\textit{madj}^+_\alpha(v)|=\textit{tw}(G)$.

Let $X$ be the set of all degree 2 vertices of $G$, then ${X=\{v_{1,1},v_{1,n},v_{3,1},v_{3,n}\}}$.
Begin by letting $\alpha(1)=v_{1,1}$.
Obviously, $N(\alpha(1))$ is a minimal separator in $G$, separating $\alpha(1)$ from the rest of the graph, that has only one missing edge.
Using Algorithm~\ref{alg:Fv} we have that $F^{\alpha(1)}=\textit{fill}(N(\alpha(1)))$ and hence $\alpha(1)$ is a simplicial vertex in the graph $G\oplus F^{\alpha(1)}$.
Consequently, $\alpha(1)$ satisfies condition (A) from \cref{lem:safeVertexRepeatedly}.

Next, given the graph $G_1$ obtained by eliminating $\alpha(1)$, we define $\alpha(2)=v_{1,n}$ and observe that since $\alpha(1)\notin N_G(\alpha(2))$, by \cref{cor:madjNonAdjacent} we have $N_{G_1}(\alpha(2))=N_G(\alpha(2))$.
Since $F^{\alpha(2)}=\textit{fill}_{G_1}(N_{G_1}(\alpha(2)))$ and $\alpha(2)$ is simplicial in $G_1\oplus F^{\alpha(2)}$, $\alpha(2)$ satisfies condition (A) from \cref{lem:safeVertexRepeatedly}.
Likewise, during the steps $i\in\{3,4\}$ we eliminate $v_{3,1}$, $v_{3,n}$ respectively, and we point out that, as in the first two steps, $\alpha(i)$ is simplicial in the graph $G_{i-1}\oplus F^{\alpha(i)}$.
Thus, we can summarize by stating that during steps $i\in\{1,\dots,4\}$, $\alpha(i)$ satisfies condition (A) from \cref{lem:safeVertexRepeatedly}.

The graph $G_4$ obtained from $G$ by eliminating every vertex of $X$, has a vertex connectivity of 3 (i.e. $\kappa(G_4)=3$).
Then \cref{cor:tw=kConnected} implies that $\kappa(G_i)\geq 3$ for every step $i\in\{4,\dots,|V|-4\}$ regardless of how $\alpha$ is defined during these steps.
Additionally, by the same corollary, $G_{|V|-4}$ is a complete graph on 4 vertices.

In the next step, we define $\alpha(5)=v_{2,1}$.
Notice that $v_{1,2}v_{3,2}$ is the only missing edge of the minimal separator $N_{G_4}(\alpha(5))=\{v_{1,2},v_{2,2},v_{3,2}\}$, hence we have
$F^{\alpha(5)}=\textit{fill}_{G_4}\,(N_{G_4}(\alpha(5)))$. 
Therefore, $\alpha(5)$ is a simplicial vertex in the graph $G_4\oplus F^{\alpha(5)}$ satisfying condition (A) from \cref{lem:safeVertexRepeatedly}.

During the steps $i\in\{6,\dots,|V|-4\}$ we define $\alpha$ to eliminate the vertices of every column $c$, starting with column index 2 to $n-2$ in the following order: $v_{2,c}$, $v_{1,c}$, $v_{3,c}$.
Below, we show that during these steps, the vertices eliminated by $\alpha$ satisfy one of the conditions (A) or (B) of \cref{lem:safeVertexRepeatedly}.

For every fixed column $c\in\{2,\dots,n-2\}$, let $i_r=\alpha^{-1}(v_{r,c})$ for every $r\in\{1,2,3\}$, i.e.,\ $i_r$ is the step at which the vertex $v_{r, c}$ is eliminated.
Obviously, $v_{2,c}$ is an almost simplicial vertex in the graph $G_{i_2-1}$ with $\textit{deg}_{G_{i_2-1}}(v_{2,c})=\kappa(G_{i_2-1})=3$.
This satisfies condition (B) from \cref{lem:safeVertexRepeatedly}.
Also, by Algorithm~\ref{alg:Fv}, the vertices $v_{1,c},v_{3,c}$ are simplicial in the graphs $G_{i_1-1}\oplus F^{v_{1,c}}$ and $G_{i_3-1}\oplus F^{v_{3,c}}$, therefore satisfying condition (A) of \cref{lem:safeVertexRepeatedly}.
We also point out that $\textit{deg}_{G_{i-1}}(\alpha(i))=3$ for every step $i\in\{5,\dots,|V|-4\}$.

% The graph $G_{|V|-4}$ is a complete graph, so we let $\alpha$ be any elimination ordering over $G_{|V|-4}$ in the remaining steps $i\in\{|V|-3,\dots,|V|\}$.
% Note that as a result, $\alpha$ is a minimum elimination ordering over $G_{|V|-4}$.
% To summarize, $\alpha$ during steps $i\in\{1,\dots,|V|-4\}$ satisfies condition (1) and for $i\in\{|V|-3,\dots,|V|\}$, $\alpha$ satisfies condition (2) of \cref{lem:safeVertexRepeatedly}. 
% We know that $\textit{tw}(G)=3$ (as shown in \cite{janka}) and by our construction $\max_{v\in V}|\textit{madj}^+_\alpha(v)|=3$ (satisfying condition (3) of \cref{lem:safeVertexRepeatedly}).
% In conclusion, we can state that $\tau(G)=0$ as desired.

The graph $G_{|V|-4}$ is a complete graph, so we let $\alpha$ be any elimination ordering over $G_{|V|-4}$.
To summarise, the vertices eliminated by $\alpha$ during steps $i\in\{1,\dots,|V|-4\}$ satisfy condition (1) and the rest of the eliminated vertices satisfy condition (2) of \cref{lem:safeVertexRepeatedly}.
% (as well as \cref{lem:safeVertexRepeatedly}). 
% As a result, $\alpha$ is a minimum elimination ordering over $G$.
It is known that $\textit{tw}(G)=3$ (\cite{janka}) and by our construction $\alpha$ is a minimum elimination ordering over $G$ with $\max_{v\in V}|\textit{madj}^+_\alpha(v)|=3$, hence $\tau(G)=0$ as desired.
\end{proof}

% 3xn mfi
{
The elimination ordering defined in the proof of 
\cref{lem:3grid} helps us to state the following statement about the minimum fill-in value of the $P_3\square P_n$ grid graphs for $n\geq 3$.

\begin{corollary}\label{cor:3grid:mfi}
Let $G$ be a $P_3\square P_n$ for $n\geq 2$.
Then $\textit{mfi}(G)=5+4(n-3)$ if $n\geq 3$ and $\textit{mfi}(G)=9$ when $n=2$.
\end{corollary}
\begin{proof}

% fig
{
\tikzset{
mystyle/.style={draw=black,rectangle, inner sep=0pt, text width=5mm, text height=1.75 mm,  align=right}
}
\begin{figure}
\centering
    \begin{tikzpicture}
        [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=8mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (13) at (4,2) {\tiny{$v_{1,1}\,\,$}};
        \node [mystyle] (23) at (4,0) {\tiny{$v_{2,1}\,\,$}};
        \node [mystyle] (33) at (4,-2) {\tiny{$v_{3,1}\,\,$}};
        
        \node [mystyle] (14) at (6,2) {\tiny{$v_{1,2}\,\,$}};
        \node [mystyle] (24) at (6,0) {\tiny{$v_{2,2}\,\,$}};
        \node [mystyle] (34) at (6,-2) {\tiny{$v_{3,2}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,3}\,\,$}};
        \node [mystyle] (25) at (8,0) {\tiny{$v_{2,3}\,\,$}};
        \node [mystyle] (35) at (8,-2) {\tiny{$v_{3,3}\,\,$}};
        
        \node (1n-2) at (11.5,2)    {\tiny{$v_{1,n-1}$}};
        \node (2n-2) at (11.5,0)  {\tiny{$v_{2,n-1}$}};
        \node (3n-2) at (11.5,-2) {\tiny{$v_{3,n-1}$}};
        
        \node [mystyle] (1n-1) at (13.5,2)    {\tiny{$v_{1,n}$}};
        \node [mystyle] (2n-1) at (13.5,0)  {\tiny{$v_{2,n}$}};
        \node [mystyle] (3n-1) at (13.5,-2) {\tiny{$v_{3,n}$}};
        \draw[-] 
        {
        (13)--(23)
        (23)--(33)
        (13)--(14)
        (23)--(24)
        (33)--(34)
        
        (14)--(24)
        (24)--(34)
        (14)--(15)
        (24)--(25)
        (34)--(35)
        
        (15)--(25)
        (25)--(35)
        (15)--(9.25,2)   
        (25)--(9.25,0) 
        (35)--(9.25,-2)
        
        (1n-2)--(2n-2)
        (1n-2)--(1n-1)
        (2n-2)--(3n-2)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        (1n-2)--(10.25,2)    
        (2n-2)--(10.25,0)  
        (3n-2)--(10.25,-2)
        
        (1n-1)--(2n-1)
        (2n-1)--(3n-1)
        }
        ;
        \draw[draw=black,style=thick,dotted]
        (9.5,2)--(10,2)   
        (9.5,0)--(10,0) 
        (9.5,-2)--(10,-2)
        ;
        
        \draw[draw=green]
        (23)--(14)
        (23)--(34)
        (14)to[out=180,in=180,looseness=0.25](34)
        
        (14)--(25)
        (34)--(25)
        (34)--(15)
        (15)to[out=180,in=180,looseness=0.25](35)
        
        (1n-2)to[out=180,in=180,looseness=0.25](3n-2)
        (1n-2)--(2n-1)
        (3n-2)--(2n-1)
        ;
    \end{tikzpicture}
    \vspace{0.5cm}
\caption
{
The minimum triangulation $G^+_\alpha$ of the $P_3\square P_n$ graph $G$.
The green lines represent the edges added by $\alpha$.
} 
\label{fig:3gridTriangulation}
\end{figure}
}

The case where $n=2$ follows from \cref{lem:2grid2king2hex2tria} so let's consider the case where $n\geq 3$.
Let $\alpha$ be the elimination ordering over $G$ defined in the proof of \cref{lem:3grid}.
By selection, $\alpha$ is a minimum elimination ordering, as it satisfies both conditions (1) and (2) of \cref{lem:safeVertexRepeatedly}.
Therefore, the number of edges added during $\alpha$ is $\textit{mfi}(G)$.
It is easy to verify that $\alpha$ adds 5 edges when eliminating the vertex set of columns 1, $n-1$ and $n$ in $G$ (see \cref{fig:3gridTriangulation} for a demonstration).
Note that the edge $v_{1,n-1}v_{3,n-1}$ is added in $G^+_\alpha$ when the vertex $v_{3,n-2}$ is eliminated.
For every other column index $c$, $c\in \{2,\dots,n-2\}$, $\alpha$ adds 4 edges when eliminating vertices $v_{1,c},\dots,v_{3,c}$ thus showing that $\textit{mfi}(G)=5+4(n-3)$ as desired.
\end{proof}
}

Our results can also be extended to $P_4\square P_n$, hexagonal and triangular grids, as well as King's graphs.
\unsure[inline]{
Is it OK to note this here?
The next result from thesis ($\tau$ and minimum fill-in of $P_4\square P_n$ is even longer than the one above.
I highly doubt we can fit that one to a paper under 12 pages long.
}
\todo[inline]{This last sentence about extension of the results should be placed after Corollary 2, but the question is whether we want to mention it here?
One option would be to  include P4 x Pn still here and write the second paper about these other graphs or any combination. It may be better to discuss. Any idea how long would be the proof for  P4 x Pn?}
\unsure[inline]{
I have included the proof below.
It does include multiple large pictures but with this latex template, it currently takes 7 pages (with its mfi result).
}
\todo[inline]{OK, thanks. There are lots of references missing and a question is how much this proof can be shortened...in between we can go through this proof carefully anyway and we can discuss whether the proof will be included here or not sometime next week, if there is a time window.   }
\unsure[inline]{
I will fix them.
Is there a journal that you have in mind and if so when is the submission date on it?
I am slightly busy in the next 3 weeks but have more time (and no marking) afterwards.
}
\todo[inline]{No worries, there is no deadline for the journals. I am think about Discrete Mathematics (https://www.sciencedirect.com/journal/discrete-mathematics). One option is to take a risk and try to send only Chapters 1-4 in one paper and to put the other results in the second paper. If the 1st paper would be accepted, we have still enough results for the 2nd paper. If if it is not accepted - we can change the strategy. Let's just discuss it when we see each other on campus. Now I am more inclined to include only Chap 1-4 in the first paper - some slight modifications of the soft text/the abstract will be needed, but it should not take too much time and we would have at least a feedback and time to work on the 2nd paper.}

==> content/grids4n.tex <==

% 4
{
% 4xn grid helper def
{
Before discussing grids and grid-like graphs with 4 rows, we need to introduce the following notation.
Let $G=(V,E)$ be a graph, $\alpha$ any elimination ordering over $G$ and $k=\kappa(G)$.
By \cref{cor:tw=kConnected}, the graph $G_{|V|-(k+1)}$ obtained at step $|V|-(k+1)$ of $\alpha$ is a complete graph on $k+1$ vertices.
Hence, we necessarily have that $\textit{deg}_{G_{|V|-(k+1)}}(\alpha(|V|-k))=|\textit{madj}^+_\alpha(\alpha(|V|-k)))|=\kappa(G)$.

The following function, given any integer $c\geq 1$, returns the set of vertices eliminated with degree $c$ in $\alpha$ before step $|V|-c$:

\begin{definition}\label{def:f}
Let $G=(V,E)$ be a graph and $c$ be an integer, $c\geq 1$.
Given an elimination ordering $\alpha$ over $G$ define $\mathcal{V}_G(\alpha,c)$ to be the set of vertices $v\in V$, eliminated through all steps $i\in\{1,\dots,|V|-(c+1)\}$ where $|\textit{madj}^+_\alpha(v)|=c$.
\end{definition}

}

% 4xn grid
{
The following lemma determines the value of the $\tau$ parameter for $P_4\square P_n$ graphs, for $n\geq 4$.

% 4 lemma main
{
\begin{lemma}
\label{lem:4grid}
Let $G=(V,E)$ be a $P_4\square P_n$ for $n\geq 4$, then $\tau(G)=0$.
\end{lemma}
\begin{proof}
% It is known that $\textit{tw}(G)=4$ (as shown in \cite{janka}).
To prove that $\tau(G)=0$, we construct an elimination ordering $\alpha$ over $G$ satisfying the condition of \cref{lem:tau0Elim}.

Notice that $\kappa(G)=2$.
Define $X=\{v_{1,1},v_{1,n},v_{4,1},v_{4,n}\}$ to be the set of degree 2 vertices of $G$.
Let $\alpha$ be an elimination ordering over $G$ that eliminates the vertices of $X$ in the following order within its first 4 steps: $v_{1,1},v_{1,n},v_{4,1},v_{4,n}$.
As discussed in the proof of \cref{lem:3grid}, the fact that the vertices from $X$ are pairwise non-adjacent combined with \cref{cor:madjNonAdjacent} imply that $N_{G_{i-1}}(\alpha(i))=N_G(\alpha(i))$ for every step $i\in \{1,\dots,4\}$.
Therefore, $\alpha(i)$ during these steps is simplicial in the graph $G_{i-1}\oplus F^{\alpha(i)}$ satisfying condition (A) from \cref{lem:tau0Elim}.
Additionally, note that $|\textit{madj}^+_\alpha(\alpha(i))|=2$ for $i\in \{1,\dots,4\}$.

The resulting graph $G_4$ is demonstrated in \cref{fig:4grid:G4} (ignoring the dashed red line).
It is easy to see that $\kappa(G_4)=3$.
Then by \cref{cor:tw=kConnected}, regardless of how $\alpha$ is defined over the steps $i\in\{5,\dots,|V|-4\}$ we have $\kappa(G_{i-1})\geq 3$.
Additionally, by the same corollary, the graph $G_{|V|-4}$ obtained at step $|V|-4$ of $\alpha$ is a $K_4$.
We will need these facts later in our proof.
Define the subset $X'\subset V_{G_4}$ as:
\[
    X'= 
    \begin{cases}
        \{v_{2,1},v_{4,3},v_{2,4},v_{1,3}\},& \text{if } n=4\\
        \{v_{2,1},v_{1,2},v_{4,2},v_{4,n-1},v_{2,n},v_{1,n-1}\},& \text{if } n\geq 5
    \end{cases}
\]

We point out that in the case where $n\geq 5$, $X'$ includes 2 additional vertices $v_{1,2}$ and $v_{4,2}$.
During the steps $i\in\{5,\dots,|X'|+4\}$ we let $\alpha$ eliminate all vertices from $X'$ in the same order that is written above.

By construction, $\alpha(i)$ is an almost simplicial vertex in the graph $G_{i-1}$ with degree equal to $\kappa(G_{i-1})=3$ for every step $i\in\{5,\dots,|X'|+4\}$ (see \cref{fig:4grid}).
Therefore, the vertices eliminated by $\alpha$ during these steps satisfying condition (B) of \cref{lem:tau0Elim}.
We also need to point out that $|\textit{madj}^+_\alpha(\alpha(i))|=3$ for every step $i\in \{5,\dots,|X'|+4\}$.
    
Next, consider the graph $G_{|X'|+4}$ as demonstrated in \cref{fig:4grid:G10}.
Below we consider 2 complementary cases and show that in both cases $\tau(G)=0$.

% figs
{
\tikzset{
mystyle/.style={draw=black,rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}
}
\tikzset{
invisible/.style={draw=white,circle, inner sep=0pt, text width=5mm, text height=1.75mm, align=right, opacity=0}
}
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \begin{tikzpicture}
    [scale=0.45,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6.5mm, text height=1.75 mm,  align=right}]
        \node [label=left:{\scriptsize 5$\rightarrow$}] [mystyle] (21) at (-0.5,0.6) {\tiny{$v_{2,1}$}};
        \node [mystyle] (31) at (-0.5,-0.6) {\tiny{$v_{3,1}$}};
        
        \node [mystyle] (12) at (2,2) {\tiny{$v_{1,2}$}};
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}$}};
        \node [mystyle] (42) at (2,-2) {\tiny{$v_{4,2}$}};
        
        \node [mystyle] (13) at (4,2)   {\tiny{$v_{1,3}$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}$}};
        \node [mystyle] (43) at (4,-2)   {\tiny{$v_{4,3}$}};
        
        \node (1n-2) at (6.5,2) {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (6.5,0.6) {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (6.5,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (6.5,-2) {\tiny{$v_{4,n-2}$}};
        
        \node (1n-1) at (9.25,2)   {\tiny{$v_{1,n-1}$}};
        \node (2n-1) at (9.25,0.6) {\tiny{$v_{2,n-1}$}};
        \node (3n-1) at (9.25,-0.6) {\tiny{$v_{3,n-1}$}};
        \node (4n-1) at (9.25,-2)   {\tiny{$v_{4,n-1}$}};
        
        \node [mystyle] (2n) at (12,0.6) {\tiny{$v_{2,n}$}};
        \node [mystyle] (3n) at (12,-0.6) {\tiny{$v_{3,n}$}};
        
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (21)--(12)
        (31)--(42)
        (1n-1)--(2n)
        ;
        
        
        \draw[draw=MyColorOne, line width=0.5mm]
        (4n-1)--(3n)
        ;
        % \draw[draw=red, dashed]
        % (31)--(12)
        % (31)--(22)
        % ;
        \draw[-]
        (21)--(31)
        (21)--(22)
        (31)--(32)
        
        (12)--(22)
        (22)--(32)
        (32)--(42)
        (12)--(13)
        (22)--(23)
        (32)--(33)
        (42)--(43)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(4.75,2)   
        (23)--(4.75,0.6) 
        (33)--(4.75,-0.6)
        (43)--(4.75,-2)
        
        (5.35,2)--(1n-2)   
        (5.35,0.6)--(2n-2)
        (5.35,-0.6)--(3n-2)
        (5.35,-2)--(4n-2)
        
        (1n-2)--(2n-2)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (1n-2)--(1n-1)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        (4n-2)--(4n-1)
        
        (1n-1)--(2n-1)
        (2n-1)--(3n-1)
        (3n-1)--(4n-1)
        (2n-1)--(2n)
        (3n-1)--(3n)
        
        (2n)--(3n)
        ;
        \draw[dotted]
        (4.85,2)--(5.3,2)
        (4.85,0.6)--(5.3,0.6)
        (4.85,-0.6)--(5.3,-0.6)
        (4.85,-2)--(5.3,-2)
        ;
        
        \draw[draw=red]
        ;
    \end{tikzpicture}
    \caption{$G_4$}
    \label{fig:4grid:G4}   
  \end{subfigure}
  \hspace{0.4cm}
  \vspace{0.7cm}
  \begin{subfigure}[b]{0.45\textwidth}
    \begin{tikzpicture}
    [scale=0.45,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6.5mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (31) at (-0.5,-0.6) {\tiny{$v_{3,1}$}};
        
        \node [label=left:{\scriptsize 6$\rightarrow$}] [mystyle] (12) at (2,2) {\tiny{$v_{1,2}$}};
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}$}};
        \node [mystyle] (42) at (2,-2) {\tiny{$v_{4,2}$}};
        
        \node [mystyle] (13) at (4,2)   {\tiny{$v_{1,3}$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}$}};
        \node [mystyle] (43) at (4,-2)   {\tiny{$v_{4,3}$}};
        
        \node (1n-2) at (6.5,2) {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (6.5,0.6) {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (6.5,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (6.5,-2) {\tiny{$v_{4,n-2}$}};
        
        \node (1n-1) at (9.25,2)   {\tiny{$v_{1,n-1}$}};
        \node (2n-1) at (9.25,0.6) {\tiny{$v_{2,n-1}$}};
        \node (3n-1) at (9.25,-0.6) {\tiny{$v_{3,n-1}$}};
        \node (4n-1) at (9.25,-2)   {\tiny{$v_{4,n-1}$}};
        
        \node [mystyle] (2n) at (12,0.6) {\tiny{$v_{2,n}$}};
        \node [mystyle] (3n) at (12,-0.6) {\tiny{$v_{3,n}$}};
        
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (31)--(42)
        (1n-1)--(2n)
        (4n-1)--(3n)
        ;
        \draw[draw=MyColorOne, line width=0.5mm]
        (31)--(22)
        (31)--(12)
        ;
        % \draw[draw=red, dashed]
        % (31) to[out=45, in=180, looseness=0.35] (13)
        % (22)--(13)
        % ;
        \draw[-]
        (31)--(32)
        
        (12)--(22)
        (22)--(32)
        (32)--(42)
        (12)--(13)
        (22)--(23)
        (32)--(33)
        (42)--(43)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(4.75,2)   
        (23)--(4.75,0.6) 
        (33)--(4.75,-0.6)
        (43)--(4.75,-2)
        
        (5.35,2)--(1n-2)   
        (5.35,0.6)--(2n-2)
        (5.35,-0.6)--(3n-2)
        (5.35,-2)--(4n-2)
        
        (1n-2)--(2n-2)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (1n-2)--(1n-1)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        (4n-2)--(4n-1)
        
        (1n-1)--(2n-1)
        (2n-1)--(3n-1)
        (3n-1)--(4n-1)
        (2n-1)--(2n)
        (3n-1)--(3n)
        
        (2n)--(3n)
        ;
        \draw[dotted]
        (4.85,2)--(5.3,2)
        (4.85,0.6)--(5.3,0.6)
        (4.85,-0.6)--(5.3,-0.6)
        (4.85,-2)--(5.3,-2)
        ;
    \end{tikzpicture}
    \caption{$G_5$}
    \label{fig:4grid:G5} 
  \end{subfigure}
  \begin{subfigure}[b]{0.4\textwidth}
    \begin{tikzpicture}
    [scale=0.45,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6.5mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (31) at (-0.5,0) {\tiny{$v_{3,1}$}};
        
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}$}};
        \node [label=left:{\scriptsize 7$\rightarrow$}] [mystyle] (42) at (2,-2) {\tiny{$v_{4,2}$}};
        
        \node [mystyle] (13) at (4,2)   {\tiny{$v_{1,3}$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}$}};
        \node [mystyle] (43) at (4,-2)   {\tiny{$v_{4,3}$}};
        
        \node (1n-2) at (6.5,2) {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (6.5,0.6) {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (6.5,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (6.5,-2) {\tiny{$v_{4,n-2}$}};
        
        \node (1n-1) at (9.25,2)   {\tiny{$v_{1,n-1}$}};
        \node (2n-1) at (9.25,0.6) {\tiny{$v_{2,n-1}$}};
        \node (3n-1) at (9.25,-0.6) {\tiny{$v_{3,n-1}$}};
        \node (4n-1) at (9.25,-2)   {\tiny{$v_{4,n-1}$}};
        
        \node [mystyle] (2n) at (12,0.6) {\tiny{$v_{2,n}$}};
        \node [mystyle] (3n) at (12,-0.6) {\tiny{$v_{3,n}$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (31)--(42)
        (1n-1)--(2n)
        (4n-1)--(3n)
        (31)--(22)
        ;
        \draw[draw=MyColorOne, line width=0.5mm]
        (31)--(13)
        (22)--(13)
        ;
        
        
        % \draw[draw=red, dashed]
        % % (31) to[out=45, in=180, looseness=0.35] (43)
        % (31) -- (43)
        % (32)--(43)
        % ;
        
        
        \draw[-]
        (31)--(32)
        
        (22)--(32)
        (32)--(42)
        (22)--(23)
        (32)--(33)
        (42)--(43)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(4.75,2)   
        (23)--(4.75,0.6) 
        (33)--(4.75,-0.6)
        (43)--(4.75,-2)
        
        (5.35,2)--(1n-2)   
        (5.35,0.6)--(2n-2)
        (5.35,-0.6)--(3n-2)
        (5.35,-2)--(4n-2)
        
        (1n-2)--(2n-2)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (1n-2)--(1n-1)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        (4n-2)--(4n-1)
        
        (1n-1)--(2n-1)
        (2n-1)--(3n-1)
        (3n-1)--(4n-1)
        (2n-1)--(2n)
        (3n-1)--(3n)
        
        (2n)--(3n)
        ;
        \draw[dotted]
        (4.85,2)--(5.3,2)
        (4.85,0.6)--(5.3,0.6)
        (4.85,-0.6)--(5.3,-0.6)
        (4.85,-2)--(5.3,-2)
        ;
    \end{tikzpicture}
    \caption{$G_6$}
    \label{fig:4grid:G6}  
  \end{subfigure}
  \hspace{0.4cm}
  \vspace{0.5cm}
  \begin{subfigure}[b]{0.4\textwidth}
    \begin{tikzpicture}
    [scale=0.45,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6.5mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (31) at (-0.5,0) {\tiny{$v_{3,1}$}};
        
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}$}};
        
        \node [mystyle] (13) at (4,2)   {\tiny{$v_{1,3}$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}$}};
        \node [mystyle] (43) at (4,-2)   {\tiny{$v_{4,3}$}};
        
        \node (1n-2) at (6.5,2) {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (6.5,0.6) {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (6.5,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (6.5,-2) {\tiny{$v_{4,n-2}$}};
        
        \node (1n-1) at (9.25,2)   {\tiny{$v_{1,n-1}$}};
        \node (2n-1) at (9.25,0.6) {\tiny{$v_{2,n-1}$}};
        \node (3n-1) at (9.25,-0.6) {\tiny{$v_{3,n-1}$}};
        \node (4n-1) at (9.25,-2)   {\tiny{$v_{4,n-1}$}};
        
        \node [label={[label distance=-0.2cm]0:\scriptsize{$\leftarrow$8}}] [mystyle] (2n) at (12,0.6) {\tiny{$v_{2,n}$}};
        \node [mystyle] (3n) at (12,-0.6) {\tiny{$v_{3,n}$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (1n-1)--(2n)
        (4n-1)--(3n)
        (31)--(22)
        (31)--(13)
        (22)--(13)
        
        ;
        \draw[draw=MyColorOne, line width=0.5mm]
        (31)--(43)
        (32)--(43)
        ;
        % \draw[draw=red, dashed]
        % % (31) to[out=45, in=180, looseness=0.35] (43)
        % (1n-1)--(3n)
        % (2n-1)--(3n)
        % ;
        \draw[-]
        (31)--(32)
        
        (22)--(32)
        (22)--(23)
        (32)--(33)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(4.75,2)   
        (23)--(4.75,0.6) 
        (33)--(4.75,-0.6)
        (43)--(4.75,-2)
        
        (5.35,2)--(1n-2)   
        (5.35,0.6)--(2n-2)
        (5.35,-0.6)--(3n-2)
        (5.35,-2)--(4n-2)
        
        (1n-2)--(2n-2)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (1n-2)--(1n-1)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        (4n-2)--(4n-1)
        
        (1n-1)--(2n-1)
        (2n-1)--(3n-1)
        (3n-1)--(4n-1)
        (2n-1)--(2n)
        (3n-1)--(3n)
        
        (2n)--(3n)
        ;
        \draw[dotted]
        (4.85,2)--(5.3,2)
        (4.85,0.6)--(5.3,0.6)
        (4.85,-0.6)--(5.3,-0.6)
        (4.85,-2)--(5.3,-2)
        ;
        
    \end{tikzpicture}
    \caption{$G_7$}
    \label{fig:4grid:G7} 
  \end{subfigure}
  \begin{subfigure}[b]{0.4\textwidth}
    \begin{tikzpicture}
    [scale=0.45,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6.5mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (31) at (-0.5,0) {\tiny{$v_{3,1}$}};
        
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}$}};
        
        \node [mystyle] (13) at (4,2)   {\tiny{$v_{1,3}$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}$}};
        \node [mystyle] (43) at (4,-2)   {\tiny{$v_{4,3}$}};
        
        \node (1n-2) at (6.5,2) {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (6.5,0.6) {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (6.5,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (6.5,-2) {\tiny{$v_{4,n-2}$}};
        
        \node [label={[label distance=-0.2cm]0:\scriptsize{$\leftarrow$9}}] (1n-1) at (9.25,2)   {\tiny{$v_{1,n-1}$}};
        \node (2n-1) at (9.25,0.6) {\tiny{$v_{2,n-1}$}};
        \node (3n-1) at (9.25,-0.6) {\tiny{$v_{3,n-1}$}};
        \node (4n-1) at (9.25,-2)   {\tiny{$v_{4,n-1}$}};
        
        \node [mystyle] (3n) at (12,-0.6) {\tiny{$v_{3,n}$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (4n-1)--(3n)
        (31)--(22)
        (31)--(13)
        (22)--(13)
        
        (31)--(43)
        (32)--(43)
        
        ;
        
        
        \draw[draw=MyColorOne, line width=0.5mm]
        (3n)--(1n-1)
        (3n)--(2n-1)
        ;
        
        % \draw[draw=red, dashed]
        % (3n) to[out=135, in=0, looseness=0.35] (1n-2)
        % (2n-1)--(1n-2)
        % ;
        \draw[-]
        (31)--(32)
        
        (22)--(32)
        (22)--(23)
        (32)--(33)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(4.75,2)   
        (23)--(4.75,0.6) 
        (33)--(4.75,-0.6)
        (43)--(4.75,-2)
        
        (5.35,2)--(1n-2)   
        (5.35,0.6)--(2n-2)
        (5.35,-0.6)--(3n-2)
        (5.35,-2)--(4n-2)
        
        (1n-2)--(2n-2)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (1n-2)--(1n-1)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        (4n-2)--(4n-1)
        
        (1n-1)--(2n-1)
        (2n-1)--(3n-1)
        (3n-1)--(4n-1)
        (3n-1)--(3n)
        ;
        \draw[dotted]
        (4.85,2)--(5.3,2)
        (4.85,0.6)--(5.3,0.6)
        (4.85,-0.6)--(5.3,-0.6)
        (4.85,-2)--(5.3,-2)
        ;
    \end{tikzpicture}
    \caption{$G_8$}
    \label{fig:4grid:G8} 
  \end{subfigure}
  \hspace{0.4cm}
  \vspace{0.5cm}
  \begin{subfigure}[b]{0.4\textwidth}
    \begin{tikzpicture}
    [scale=0.45,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6.5mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (31) at (-0.5,0) {\tiny{$v_{3,1}$}};
        
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}$}};
        
        \node [mystyle] (13) at (4,2)   {\tiny{$v_{1,3}$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}$}};
        \node [mystyle] (43) at (4,-2)   {\tiny{$v_{4,3}$}};
        
        \node (1n-2) at (6.5,2) {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (6.5,0.6) {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (6.5,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (6.5,-2) {\tiny{$v_{4,n-2}$}};
        
        \node (2n-1) at (9.25,0.6) {\tiny{$v_{2,n-1}$}};
        \node (3n-1) at (9.25,-0.6) {\tiny{$v_{3,n-1}$}};
        \node [label={[label distance=0cm]0:\scriptsize{$\leftarrow$10}}] (4n-1) at (9.25,-2)   {\tiny{$v_{4,n-1}$}};
        
        \node [mystyle] (3n) at (13,0) {\tiny{$v_{3,n}$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (4n-1)--(3n)
        (31)--(22)
        (31)--(13)
        (22)--(13)
        
        (31)--(43)
        (32)--(43)
        
        (3n)--(2n-1)
        
        ;
        
        \draw[draw=MyColorOne, line width=0.5mm]
        (3n)--(1n-2)
        (2n-1)--(1n-2)
        ;
        % \draw[draw=red, dashed]
        % (3n)--(4n-2)
        % (3n-1)--(4n-2)
        % ;
        \draw[-]
        (31)--(32)
        
        (22)--(32)
        (22)--(23)
        (32)--(33)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(4.75,2)   
        (23)--(4.75,0.6) 
        (33)--(4.75,-0.6)
        (43)--(4.75,-2)
        
        (5.35,2)--(1n-2)   
        (5.35,0.6)--(2n-2)
        (5.35,-0.6)--(3n-2)
        (5.35,-2)--(4n-2)
        
        (1n-2)--(2n-2)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        (4n-2)--(4n-1)
        
        (2n-1)--(3n-1)
        (3n-1)--(4n-1)
        (3n-1)--(3n)
        ;
        \draw[dotted]
        (4.85,2)--(5.3,2)
        (4.85,0.6)--(5.3,0.6)
        (4.85,-0.6)--(5.3,-0.6)
        (4.85,-2)--(5.3,-2)
        ;
    \end{tikzpicture}
    \caption{$G_9$}
    \label{fig:4grid:G9} 
  \end{subfigure}
  \begin{subfigure}[b]{0.6\textwidth}
    \begin{tikzpicture}
    [scale=0.55,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
    \node [mystyle] (31) at (-0.75,0) {\tiny{$v_{3,1}\,\,$}};
    
    \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}\,\,$}};
    \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}\,\,$}};
    
    \node [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
    \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}\,\,$}};
    \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}\,\,$}};
    \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
    
    \node [mystyle] (14) at (6,2) {\tiny{$v_{1,4}\,\,$}};
    \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
    \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
    \node [mystyle] (44) at (6,-2) {\tiny{$v_{4,4}\,\,$}};
    
    \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
    \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
    \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
    \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
    
    \node (1n-2) at (10.5,2)    {\tiny{$v_{1,n-2}$}};
    \node (2n-2) at (10.5,0.6)  {\tiny{$v_{2,n-2}$}};
    \node (3n-2) at (10.5,-0.6) {\tiny{$v_{3,n-2}$}};
    \node (4n-2) at (10.5,-2)   {\tiny{$v_{4,n-2}$}};
    
    \node (2n-1) at (12.5,0.6) {\tiny{$v_{2,n-1}$}};
    \node (3n-1) at (12.5,-0.6) {\tiny{$v_{3,n-1}$}};
    
    \node [mystyle] (3n) at (15.25,0) {\tiny{$v_{3,n}\,\,$}};
    \draw[draw=MyColorOneDark, line width=0.5mm]
    (31)--(13)
    (31)--(22)
    (31)--(43)
    (22)--(13)
    (32)--(43)
    (1n-2)--(3n)
    (1n-2)--(2n-1)
    (2n-1)--(3n)
    ;
    \draw[draw=MyColorOne, line width=0.5mm]
    (4n-2)--(3n)
    (4n-2)--(3n-1)
    ;
    \draw[-] 
    (31)--(32)
    
    (22)--(32)
    (22)--(23)
    (32)--(33)
    
    (13)--(23)
    (23)--(33)
    (33)--(43)
    (13)--(14)
    (23)--(24)
    (33)--(34)
    (43)--(44)
    
    (14)--(24)
    (24)--(34)
    (34)--(44)
    (14)--(15)
    (24)--(25)
    (34)--(35)
    (44)--(45)
    
    (15)--(25)
    (25)--(35)
    (35)--(45)
    (15)--(8.8,2)   
    (25)--(8.8,0.6) 
    (35)--(8.8,-0.6)
    (45)--(8.8,-2)  
    
    (1n-2)--(2n-2)
    
    (2n-2)--(3n-2)
    (3n-2)--(4n-2)
    (2n-2)--(2n-1)
    (3n-2)--(3n-1)
    
    (1n-2)--(9.6,2)    
    (2n-2)--(9.6,0.6)  
    (3n-2)--(9.6,-0.6) 
    (4n-2)--(9.6,-2)   
    
    (2n-1)--(3n-1)
    (3n-1)--(3n)
    ;
    \draw[dotted]
    (9,2)--(9.4,2)   
    (9,0.6)--(9.4,0.6) 
    (9,-0.6)--(9.4,-0.6) 
    (9,-2)--(9.4,-2)    
    ;
\end{tikzpicture}
    \caption{$G_{10}$}
    \label{fig:4grid:G10} 
  \end{subfigure}
    \caption
    {
    The elimination ordering $\alpha$ over the $P_4\square P_n$ graph $G$, for $n\geq 7$.
    (a)-(f) demonstrate the graph $G_i$ obtained at steps $i\in\{4,\dots,9\}$ of $\alpha$.
    For each graph $G_i$, the vertex $\alpha(i+1)$ is pointed out with its label,
    the edges added by elimination of $\alpha(i)$ are drawn in light green, and the edges added in the previous steps are shown in dark green.
    Notice that for every step $i\in\{4,\dots,9\}$, $F^{\alpha(i)}=\emptyset$ (that is the set of missing edges defined using Algorithm \ref{alg:Fv}) and that the vertex $\alpha(i+1)$ is almost simplicial in $G_i$ with $\textit{deg}_{G_{i}}(\alpha(i+1))=\kappa(G_{i})$.
    (g) the resulting graph $G_{10}$.
    } 
    \label{fig:4grid} 
\end{figure}

\tikzset{
mystyle/.style={draw=black,rectangle, inner sep=0pt, text width=5mm, text height=1.75 mm,  align=right}
}
\tikzset{
invisible/.style={draw=white,circle, inner sep=0pt, text width=5mm, text height=1.75mm, align=right, opacity=0}
}
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.7\textwidth}
    \begin{tikzpicture}
        [scale=0.55,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
        \node [label={[label distance=0.4cm]180:\scriptsize{$q+$11$\rightarrow$}}] [mystyle] (31) at (-0.75,0) {\tiny{$v_{3,1}\,\,$}};
        
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}\,\,$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}\,\,$}};
        
        \node [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}\,\,$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}\,\,$}};
        \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        
        \node (1n-2) at (10.5,2)    {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (10.5,0.6)  {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (10.5,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (10.5,-2)   {\tiny{$v_{4,n-2}$}};
        
        \node (2n-1) at (12.5,0.6) {\tiny{$v_{2,n-1}$}};
        \node (3n-1) at (12.5,-0.6) {\tiny{$v_{3,n-1}$}};
        
        \node [mystyle] (3n) at (15.25,0) {\tiny{$v_{3,n}\,\,$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (31)--(13)
        (31)--(22)
        (31)--(43)
        
        (22)--(13)
        (32)--(43)
        
        (13)--(15)
        (13)--(24)
        (24)--(15)
        
        (43)--(45)
        (43)--(34)
        (34)--(45)
        
        (1n-2)--(2n-1)
        (2n-1)--(3n)
        (1n-2)--(3n)
        
        (4n-2)--(3n-1)
        (4n-2)--(3n)
        ;
        \draw[-] 
        
        (3n-1)--(3n)
        (31)--(32)
        
        (22)--(32)
        (22)--(23)
        (32)--(33)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (23)--(24)
        (33)--(34)
        
        (24)--(34)
        (24)--(25)
        (34)--(35)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(8.6,2)   
        (25)--(8.6,0.6) 
        (35)--(8.6,-0.6)
        (45)--(8.6,-2)  
        
        (1n-2)--(2n-2)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        (1n-2)--(9.5,2)    
        (2n-2)--(9.5,0.6)  
        (3n-2)--(9.5,-0.6) 
        (4n-2)--(9.5,-2)   
        
        (2n-1)--(3n-1)
        ;
        \draw[dotted]
        (8.8,2)--(9.4,2)   
        (8.8,0.6)--(9.4,0.6) 
        (8.8,-0.6)--(9.4,-0.6) 
        (8.8,-2)--(9.4,-2)    
        ;
    \end{tikzpicture}
    \caption{$G_{q+10}$}
    \label{fig:4grid2:G10}   
  \end{subfigure}\vspace{0.25cm}\vspace{0.25cm}
  \begin{subfigure}[b]{0.325\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
        \node [label={[label distance=0.6cm]180:\scriptsize{$q+$12$\rightarrow$}}] [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}\,\,$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}\,\,$}};
        
        \node [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}\,\,$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}\,\,$}};
        \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (22)--(13)
        (32)--(43)
        
        (13)--(15)
        (13)--(24)
        (24)--(15)
        
        (43)--(45)
        (43)--(34)
        (34)--(45)
        ;
        \draw[draw=MyColorOneDark, line width=0.5mm]
        ;
        
        \draw[-] 
        (22)--(32)
        (22)--(23)
        (32)--(33)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (23)--(24)
        (33)--(34)
        
        (24)--(34)
        (24)--(25)
        (34)--(35)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(8.75,2)   
        (25)--(8.75,0.6) 
        (35)--(8.75,-0.6)
        (45)--(8.75,-2) 
        ;
        \draw[dotted]
        (8.85,2)--(9.25,2)   
        (8.85,0.6)--(9.25,0.6)  
        (8.85,-0.6)--(9.25,-0.6)
        (8.85,-2)--(9.25,-2)
        ;
        
        \draw[draw=MyColorOne, line width=0.5mm]
        (22)--(43)
        (32)--(13)
        (13)to[out=0, in=0, looseness=0.5](43)
        ;
    \end{tikzpicture}
    \caption{$G_{q+11}$}
    \label{fig:4grid2:G11}
  \end{subfigure}
  \vspace{0.5cm}
  \hspace{0.4cm}
  \begin{subfigure}[b]{0.325\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
        \node [label={[label distance=0.6cm]180:\scriptsize{$q+$13$\rightarrow$}}] [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}\,\,$}};
        
        \node [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}\,\,$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}\,\,$}};
        \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (32)--(43)
        
        (13)--(15)
        (13)--(24)
        (24)--(15)
        
        (43)--(45)
        (43)--(34)
        (34)--(45)
        
        (32)--(13)
        (13)to[out=0, in=0, looseness=0.5](43)
        ;
        \draw[-]
        (32)--(33)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (23)--(24)
        (33)--(34)
        
        (24)--(34)
        (24)--(25)
        (34)--(35)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(8.75,2)   
        (25)--(8.75,0.6) 
        (35)--(8.75,-0.6)
        (45)--(8.75,-2) 
        ;
        \draw[dotted]
        (8.85,2)--(9.25,2)   
        (8.85,0.6)--(9.25,0.6)  
        (8.85,-0.6)--(9.25,-0.6)
        (8.85,-2)--(9.25,-2)
        ;
        
        \draw[draw=MyColorOne, line width=0.5mm]
        (32)--(23)
        (23)to[out=0, in=0, looseness=0.5](43)
        ;
    \end{tikzpicture}
    \caption{$G_{q+12}$}
    \label{fig:4grid2:G12} 
  \end{subfigure}
  \vspace{0.25cm}
  \hspace{0.4cm}
  \begin{subfigure}[b]{0.25\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
        \node [label={[label distance=0.6cm]180:\scriptsize{$q+$14$\rightarrow$}}] [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}\,\,$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}\,\,$}};
        \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (13)--(15)
        (13)--(24)
        (24)--(15)
        
        (43)--(45)
        (43)--(34)
        (34)--(45)
        
        (13)to[out=0, in=0, looseness=0.6](43)
        (23)to[out=0, in=0, looseness=0.4](43)
        ;
        \draw[-]
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (23)--(24)
        (33)--(34)
        
        (24)--(34)
        (24)--(25)
        (34)--(35)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(8.75,2)   
        (25)--(8.75,0.6) 
        (35)--(8.75,-0.6)
        (45)--(8.75,-2) 
        ;
        \draw[dotted]
        (8.85,2)--(9.25,2)   
        (8.85,0.6)--(9.25,0.6)  
        (8.85,-0.6)--(9.25,-0.6)
        (8.85,-2)--(9.25,-2)
        ;
        
        \draw[draw=MyColorOne, line width=0.5mm]
        (13)to[out=0, in=0, looseness=0.4](33)
        ;
    \end{tikzpicture}
    \caption{$G_{q+13}$}
    \label{fig:4grid2:G13} 
  \end{subfigure}
  \begin{subfigure}[b]{0.25\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
        \node [label={[label distance=0.6cm]180:\scriptsize{$q+$15$\rightarrow$}}] [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}\,\,$}};
        \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (13)--(15)
        (13)--(24)
        (24)--(15)
        
        (43)--(45)
        (43)--(34)
        (34)--(45)
        
        (13)--(33)
        (13)to[out=0, in=0, looseness=0.4](43)
        ;
        \draw[-]
        (33)--(43)
        (33)--(34)
        
        (24)--(34)
        (24)--(25)
        (34)--(35)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(8.75,2)   
        (25)--(8.75,0.6) 
        (35)--(8.75,-0.6)
        (45)--(8.75,-2) 
        ;
        \draw[dotted]
        (8.85,2)--(9.25,2)   
        (8.85,0.6)--(9.25,0.6)  
        (8.85,-0.6)--(9.25,-0.6)
        (8.85,-2)--(9.25,-2)
        ;
        
        \draw[draw=MyColorOne, line width=0.5mm]
        (24)--(33)
        (24)--(43)
        ;
    \end{tikzpicture}
    \caption{$G_{q+14}$}
    \label{fig:4grid2:G14} 
  \end{subfigure}
  \hspace{0.5cm}
  \begin{subfigure}[b]{0.25\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
        \node [label={[label distance=0.6cm]180:\scriptsize{$q+$16$\rightarrow$}}] [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
        \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (13)--(15)
        (13)--(24)
        (24)--(15)
        
        (43)--(45)
        (43)--(34)
        (34)--(45)
        
        (13)--(43)
        (24)--(43)
        ;
        \draw[-]
        (24)--(34)
        (24)--(25)
        (34)--(35)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(8.75,2)   
        (25)--(8.75,0.6) 
        (35)--(8.75,-0.6)
        (45)--(8.75,-2) 
        ;
        \draw[dotted]
        (8.85,2)--(9.25,2)   
        (8.85,0.6)--(9.25,0.6)  
        (8.85,-0.6)--(9.25,-0.6)
        (8.85,-2)--(9.25,-2)
        ;
        
        \draw[draw=MyColorOne, line width=0.5mm]
        (13)--(34)
        %(13)to[out=0, in=0, looseness=0.4](43)
        ;
    \end{tikzpicture}
    \caption{$G_{q+15}$}
    \label{fig:4grid2:G15} 
  \end{subfigure}
  \hspace{0.5cm}
  \vspace{0.5cm}
  \begin{subfigure}[b]{0.25\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
        \node [label={[label distance=0.6cm]180:\scriptsize{$q+$17$\rightarrow$}}] [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (24)--(15)
        
        (43)--(45)
        (43)--(34)
        (34)--(45)
        
        (24)--(43)
        ;
        \draw[-]
        (24)--(34)
        (24)--(25)
        (34)--(35)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(8.75,2)   
        (25)--(8.75,0.6) 
        (35)--(8.75,-0.6)
        (45)--(8.75,-2) 
        ;
        \draw[dotted]
        (8.85,2)--(9.25,2)   
        (8.85,0.6)--(9.25,0.6)  
        (8.85,-0.6)--(9.25,-0.6)
        (8.85,-2)--(9.25,-2)
        ;
        
        \draw[draw=MyColorOne, line width=0.5mm]
        (34)--(15)
        (43)to[out=90, in=180, looseness=0.8](15)
        ;
    \end{tikzpicture}
    \caption{$G_{q+16}$}
    \label{fig:4grid2:G16}  
  \end{subfigure}
  \vspace{0.5cm}
  \begin{subfigure}[b]{0.2\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
        \node [label={[label distance=0.6cm]180:\scriptsize{$q+$18$\rightarrow$}}] [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (24)--(15)
        
        (34)--(45)
        
        (34)--(15)
        ;
        \draw[-]
        (24)--(34)
        (24)--(25)
        (34)--(35)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(8.75,2)   
        (25)--(8.75,0.6) 
        (35)--(8.75,-0.6)
        (45)--(8.75,-2) 
        ;
        \draw[dotted]
        (8.85,2)--(9.25,2)   
        (8.85,0.6)--(9.25,0.6)  
        (8.85,-0.6)--(9.25,-0.6)
        (8.85,-2)--(9.25,-2)
        ;
        \draw[draw=MyColorOne, line width=0.5mm]
        (24)--(45)
        (15)to[out=0, in=0, looseness=0.3](45)
        ;
    \end{tikzpicture}
    \caption{$G_{q+17}$}
    \label{fig:4grid2:G17}    
  \end{subfigure}
  \hspace{1.25cm}
  \begin{subfigure}[b]{0.225\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
        \node [label={[label distance=0.6cm]180:\scriptsize{$q+$19$\rightarrow$}}] [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (34)--(45)
        
        (34)--(15)
        (15)to[out=0, in=0, looseness=0.5](45)
        ;
        \draw[-]
        (34)--(35)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(8.75,2)   
        (25)--(8.75,0.6) 
        (35)--(8.75,-0.6)
        (45)--(8.75,-2) 
        ;
        \draw[dotted]
        (8.85,2)--(9.25,2)   
        (8.85,0.6)--(9.25,0.6)  
        (8.85,-0.6)--(9.25,-0.6)
        (8.85,-2)--(9.25,-2)
        ;
        \draw[draw=MyColorOne, line width=0.5mm]
        
        (25)to[out=0, in=0, looseness=0.3](45)
        (25)--(34)
        ;
    \end{tikzpicture}
    \caption{$G_{q+18}$}
    \label{fig:4grid2:G18}    
  \end{subfigure}
  \hspace{1.25cm}
  \begin{subfigure}[b]{0.1\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=4mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (15)to[out=180, in=180, looseness=0.7](45)
        
        (25)to[out=180, in=180, looseness=0.4](45)
        ;
        \draw[-]
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(8.75,2)   
        (25)--(8.75,0.6) 
        (35)--(8.75,-0.6)
        (45)--(8.75,-2) 
        ;
        \draw[dotted]
        (8.85,2)--(9.25,2)   
        (8.85,0.6)--(9.25,0.6)  
        (8.85,-0.6)--(9.25,-0.6)
        (8.85,-2)--(9.25,-2)
        ;
        \draw[draw=MyColorOne, line width=0.5mm]
        (15)to[out=180, in=180, looseness=0.4](35)
        ;
    \end{tikzpicture}
    \caption{$G_{q+19}$}
    \label{fig:4grid2:G19}    
  \end{subfigure}
  \hspace{0.5cm}
  \begin{subfigure}[b]{0.35\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
        \node [invisible] at (-2,2) {};
        \node (1n-2) at (0,2)    {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (0,0.6)  {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (0,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (0,-2)   {\tiny{$v_{4,n-2}$}};
        
        \node (2n-1) at (2.25,0.6) {\tiny{$v_{2,n-1}$}};
        \node (3n-1) at (2.25,-0.6) {\tiny{$v_{3,n-1}$}};
        
        \node [label=right:{\mbox{\scriptsize{$\leftarrow|V|-6$}}}] [mystyle] (3n) at (5.75,0) {\tiny{$v_{3,n}\,\,$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (1n-2)--(2n-1)
        (2n-1)--(3n)
        (1n-2)--(3n)
        
        (4n-2)--(3n-1)
        (4n-2)--(3n)
        
        (1n-2)to[out=180,in=180,looseness=0.7](4n-2)
        (2n-2)to[out=180,in=180,looseness=0.5](4n-2)
        ;
        \draw[-]
        
        (3n-1)--(3n)
        (1n-2)--(2n-2)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        
        (2n-1)--(3n-1)
        ;
        \draw[draw=MyColorOne, line width=0.5mm]
        (1n-2)to[out=180,in=180,looseness=0.5](3n-2)
        ;
    \end{tikzpicture}
    \caption{$G_{|V|-7}$}
    \label{fig:4grid2:GV-7}   
  \end{subfigure}
  \begin{subfigure}[b]{0.25\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
        \node [invisible] at (-2,2) {};
        \node (1n-2) at (0,2)    {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (0,0.6)  {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (0,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (0,-2)   {\tiny{$v_{4,n-2}$}};
        
        \node [label=right:{\mbox{\scriptsize{$\leftarrow|V|-5$}}}] (2n-1) at (2.25,0.6) {\tiny{$v_{2,n-1}$}};
        \node (3n-1) at (2.25,-0.6) {\tiny{$v_{3,n-1}$}};
        \draw[draw=MyColorOneDark, line width=0.5mm]
        (1n-2)--(2n-1)
        
        (4n-2)--(3n-1)
        
        (1n-2)to[out=180,in=180,looseness=0.5](3n-2)
        (2n-2)to[out=180,in=180,looseness=0.5](4n-2)
        (1n-2)to[out=180,in=180,looseness=0.7](4n-2)
        ;
        \draw[-]
        (1n-2)--(2n-2)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        
        (2n-1)--(3n-1)
        ;
        \draw[draw=MyColorOne, line width=0.5mm]
        (2n-1)--(4n-2)
        (3n-1)--(1n-2)
        ;
    \end{tikzpicture}
    \caption{$G_{|V|-6}$}
    \label{fig:4grid2:GV-6}    
  \end{subfigure}
  \begin{subfigure}[b]{0.25\textwidth}
    \begin{tikzpicture}
    [scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
        \node [invisible] at (-2,2) {};
        \node (1n-2) at (0,2)    {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (0,0.6)  {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (0,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (0,-2)   {\tiny{$v_{4,n-2}$}};
        
        \node (3n-1) at (2.25,-0.6) {\tiny{$v_{3,n-1}$}};
        
        \draw[draw=MyColorOne, line width=0.5mm]
        (3n-1)--(2n-2)
        ;
        \draw[-]
        (1n-2)--(2n-2)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (3n-2)--(3n-1)
        ;
        \draw[draw=MyColorOneDark, line width=0.5mm]
        
        (4n-2)--(3n-1)
        (3n-1)--(1n-2)
        (1n-2)to[out=180,in=180,looseness=0.5](3n-2)
        (2n-2)to[out=180,in=180,looseness=0.5](4n-2)
        (1n-2)to[out=180,in=180,looseness=0.7](4n-2)
        ;
    \end{tikzpicture}
    \caption{$G_{|V|-5}$}
    \label{fig:4grid2:GV-5}    
  \end{subfigure}
  \caption{
    The elimination ordering $\alpha$ over the $P_4\square P_n$ graph $G$, where $n\geq7$ and $q=2\ceil*{(n-6)/2}$ for short.
    (a) demonstrates the graph $G_{q+10}$ obtained at step $q+10$.
    (a)-(h) show the graph $G_i$ for $i\in\{q+10,\dots,q+17\}$ where the vertex $\alpha(i+1)$ is pointed out with its label, the edges added by elimination of $\alpha(i)$ are drawn in light green and the edges added in the previous steps are in dark green.
    We point out that $\alpha(i+1)$ has a degree of 4 in $G_i$.
    Also observe that the process of elimination shown in (b)-(g) can be repeated on $G_{q+17}$.
    (i),(j) demonstrate the graph $G_i$ and vertex $\alpha(i+1)$ for $i\in \{|V|-7,|V|-6\}$.
    (k) the graph $G_{|V|-5}$ is a $K_5$.
    } 
  \label{fig:4grid2}
\end{figure}
}

\begin{mycases}
    \case 
    {
    Suppose that $n\geq 7$.
    In this case, $|X'|=6$ and $\kappa(G_{|X'|+4})=3$.
    We first define $\alpha$ during steps $i\in\{11,\dots,|V|\}$ and then show that $\alpha$ is a minimum elimination ordering over the graph $G_{10}$.
    Ultimately, we prove that $\alpha$, in this case, satisfies all the conditions from \cref{lem:tau0Elim}.
    
    Begin with defining the vertex set $Y''\subset V_{G_{10}}$ as $Y''=\{v_{r,c}|r\in \{1,4\}, c\in \{4,\dots,n-3\}\}$  therefore $|Y''|=2(n-6)$.
    Note that $Y''$ is the set of all degree 3 vertices of $G_{10}$ (as seen in \cref{fig:4grid:G10}).
    Since $\kappa(G_{10})=3$, every separator of size 3 in $G_{10}$ is also a minimum separator of $G_{10}$.
    Then the neighbourhood of every vertex $v\in Y''$ is a minimum separator in $G_{10}$. 
    In fact, it is easy to confirm that the set of all minimum separators of $G_{10}$ (i.e.,\ $\mathcal{S}^*_{G_{10}}$) is exactly the set of neighbourhoods for all vertices from $Y''$.
    Formally
    $\mathcal{S}^3_{G_{10}}=\mathcal{S}^*_{G_{10}}=\{N_{G_{10}}(v)|v\in Y''\}$ and since $|Y''|=2(n-6)$, we have that $|\mathcal{S}^*_{G_{10}}|=2(n-6)$.
    Additionally note that for every minimum separator $S\in \mathcal{S}^*_{G_{10}}$, the number of its connected components $|\mathcal{C}_{G_{10}}(S)|=2$.
    We will be using the above facts in order to prove that $\alpha$ is a minimum elimination ordering over $G_{10}$.
    
    Define the subset of vertex $X''\subset V_{G_{10}}$ as 
    $$X''=\{v_{r,c}|
    r\in\{1,4\}, c\in\{4,\dots,n-3\} \,\textit{and }c \textit{ is even }\}$$
    By definition $X''$ contains $\ceil*{(n-6)/2}$ vertices from $\{v_{1,4},\dots,v_{1,n-3}\}$ and the same number of vertices from $\{v_{4,4},\dots,v_{4,n-3}\}$. 
    Consequently, we get that $|X''|=2\ceil*{(n-6)/2}$ and let us define $q=|X''|$ as a shorthand.
    We point out that $q\geq 2$, and it is an even number.
    
    During the steps $i\in\{11,\dots,10+\frac{q}{2}\}$, let $\alpha(i)=v_{1,c}$ and for $i\in\{11+\frac{q}{2},\dots,q+10\}$ let $\alpha(i)=v_{4,c}$ where $c$ is an even column index starting from 4 to $n-3$.
    Notice that by \cref{cor:madjNonAdjacent} and the fact that the vertices of $X''$ are pairwise non-adjacent vertices of degree 3 in $G_{10}$, we have $|\textit{madj}^+_\alpha(\alpha(i))|=3$ for every step $i\in\{11,\dots,q+10\}$.

    The graph $G_{q+10}$ (shown in \cref{fig:4grid2:G10}) has vertex connectivity of 4, i.e.,\ $\kappa(G_{q+10})=4$.
    Also note that in the graph $G_{q+10}$, for every $c\in \{1,\dots,\ceil{\frac{n-4}{2}}\}$ the column $2c$ has 2 vertices: $v_{2,2c},v_{3,2c}$ and the column $2c+1$ contains 4 vertices: $v_{1,2c+1},\dots,v_{4,2c+1}$.
    Let $\alpha$ eliminates the vertices of $G_{q+10}$ as described below.
    
    Begin by letting $\alpha(q+11)=v_{3,1}$.
    Next, starting with $c=2$ to $2\ceil{\frac{n-4}{2}}$, eliminate the vertices of column $c$ in the following order:
    Given that $c$ is even eliminate $v_{2,c},v_{3,c}$ and for odd $c$ eliminate $v_{2,c},v_{3,c},v_{1,c},v_{4,c}$.
    This elimination process is demonstrated in \cref{fig:4grid2}.
    Note that in the case where $n$ is odd, our elimination process already covers column $n-3$ of the graph $G_{q+10}$.
    Thus in the case where $n$ is even we let $\alpha$ eliminate the vertices of column $n-3$ (that has 4 vertices) in the following order $v_{1,n-3},v_{2,n-3},v_{3,n-3},v_{4,n-3}$.
    By construction, every eliminated vertex has degree of exactly 4 during the above specified steps $i\in\{q+11,\dots,|V|-6\}$ (see \cref{fig:4grid2}) as a result $\max_{i\in\{1,\dots,|V|-6\}}|\textit{madj}^+_\alpha(\alpha(i))|=4$.

    
    \cref{fig:4grid2:GV-7} demonstrates the resulting graph $G_{|V|-7}$.
    Let $\alpha(|V|-6)$ and $\alpha(|V|-5)$ be $v_{3,n}$ and $v_{2,n-1}$ respectively.
    Since $\kappa(G_{q+10})=4$, by \cref{cor:tw=kConnected}, the graph $G_{|V|-5}$ is a $K_5$ (as seen in \cref{fig:4grid2:GV-5}).
    So let $\alpha$ be any elimination ordering over $G_{|V|-5}$ in the final steps.
    Notice that by our construction, $\max_{v\in V}|\textit{madj}^+_\alpha(v)|=4$.
    We also point out that $\mathcal{V}_{G_{10}}(\alpha,3)=X''$ by \cref{def:f}.
    Therefore, $|\mathcal{V}_{G_{10}}(\alpha,3)|=q$.
    

    We claim that $\alpha$ is a minimum elimination ordering over the graph $G_{10}$.
    By construction, $\alpha$ eliminates $q$ vertices from the graph $G_{10}$ with degree 3 and then $|\textit{madj}^+_\alpha(\alpha(i))|=4$ for every step $i\in\{q+11,\dots,|V|-4\}$.
    Finally, at step $|V|-4$ the graph $G_{|V|-4}$ is a $K_4$.
    To summarize $\sum_{v\in V_{G_{10}}}|\textit{madj}^+_\alpha(v)|= 3q+4(|V_{G_{10}}|-(q+4))+6$.
    
    Suppose for a contradiction that $\alpha$ is not minimum elimination ordering.
    By construction of $\alpha$ and \cref{lem:safeVertexRepeatedly}, there must exist a minimum elimination ordering $\beta$ over $G$ s.t.\ $\beta(i)=\alpha(i)$ for every step $i\in\{1,\dots,10\}$ and $\beta$ is a minimum elimination ordering over the graph $G_{10}$.
    By this selection, when comparing the number of edges added by $\alpha$ and $\beta$ eliminating the vertices of $G_{10}$, we can safely ignore the first 10 steps of both elimination orderings.
    
    Combining \cref{cor:tw=kConnected} and the fact that $\kappa(G_{10})=3$, the graph $G^\beta_{|V|-4}$ is a $K_4$ (same as $G^\alpha_{|V|-4}$).
    Then similarly we can ignore the final 4 steps in both elimination orderings.
    Formally, we must have:
    $$
        \sum\nolimits_{i\in\{11,\dots,|V|-4\}}
        |\textit{madj}^+_\beta(\beta(i))|
        < \sum\nolimits_{i\in\{11,\dots,|V|-4\}}
        |\textit{madj}^+_\alpha(\alpha(i))|
        = 3q+4(|V_{G_{10}}|-(q+4))
    $$
    
    Also, by \cref{cor:tw=kConnected} we have that $|\textit{madj}^+_\beta(\beta(i))|\geq 3$ for every step $i\in\{11,\dots,|V|-4\}$.
    Recall that $\alpha$ eliminated $q$ vertices of degree 3 from $G_{10}$ before step $|V|-4$ (and the reaming vertices had degree 4).
    Therefore, we can conclude by saying that: 
    \begin{equation}\label{eq:4nGridVBetaVsAlpha}
        |\mathcal{V}_{G_{10}}(\beta,3)|>|\mathcal{V}_{G_{10}}(\alpha,3)|=q
    \end{equation}

    Before determining an upperbound for $|\mathcal{V}_{G_{10}}(\beta,3)|$ let us make some general observations.
    It is previously shown that 
    $\mathcal{S}^3_{G_{10}}= 
    \{N_{G_{10}}(v_{r,c}) | r\in\{1,4\}, c\in\{4,\dots,n-3\}\}$.
    For every step $t\in\{11,\dots,|V|-4\}$ in $\beta$ where $|\textit{madj}^+_\beta(\beta(t))|=3$, we clearly have that $N_{G^\beta_{t-1}}(\beta(t))$ is a separator of size 3 in the graph $G^\beta_{t-1}$.
    This combined with \cref{cor:numberofMinimumSeparators} implies that for every such step $t\in\{11,\dots,|V|-4\}$:
    \begin{equation}\label{eq:4grid:1}
        \mathcal{S}^3_{G^\beta_{t-1}}\subseteq 
        \mathcal{S}^3_{G_{10}}=
        \{N_{G_{10}}(v_{r,c}) | r\in\{1,4\}, c\in\{4,\dots,n-3\}\}
    \end{equation}
    
    Below, we will show that the following statements are correct.
    This will then result in a contradiction with \cref{eq:4nGridVBetaVsAlpha} implying that $\alpha$ is a minimum triangulation over $G_{10}$ as needed.
    
    \begin{itemize}
        \item[(a)] 
        {
        Every vertex $v\in\mathcal{V}_{
        G_{10}}(\beta,3)$ can be mapped to a unique vertex set from $\{N_{G_{10}}(v_{r,c}) | r\in\{1,4\}, c\in\{4,\dots,n-3\}\}$.
        Furthermore, given that $\beta^{-1}(v)\leq |V|-5$, we neccessarily have that $\beta(t)=v_{r,c}$ for some $r\in\{1,4\}, c\in\{4,\dots,n-3\}$.
        }
       
        \item[(b)]
        {
        % Any elimination ordering can use at most $q$ vertex sets from $\{N_{G_{10}}(v_{r,c}) |r\in\{1,4\},  c\in\{4,\dots,n-3\}\}$ as separator of size 3 for vertices of $\mathcal{V}_{G_{10}}(\beta,3)$.
        At most $q$ vertex sets from
        $\{N_{G_{10}}(v_{r,c}) |r\in\{1,4\},  c\in\{4,\dots,n-3\}\}$ can have a vertex from $\mathcal{V}_{G_{10}}(\beta,3)$ mapped to it.
        }
    \end{itemize}
    
    %a
    {
    In order to prove statement (a),
    fix a vertex $v^*\in\mathcal{V}_{G_{10}}(\beta,3)$ and let $t^*=\beta^{-1}(v^*)$.
    By selection of vertex $v^*$, $N_{G^\beta_{t^*-1}}(v^*)$ is a minimal separator of size 3 in the graph $G^\beta_{t^*-1}$.
    Then by \cref{eq:4grid:1} we have that $N_{G^\beta_{t^*-1}}(v^*)\in  \mathcal{S}^3_{G_{10}}$ and hence $N_{G^\beta_{t^*-1}}(v^*)= N_{G_{10}}(v_{r^*,c^*})$ for some $c^*\in\{4,\dots,n-3\}$ and $r^*\in\{1,4\}$.
    By a repeated application of \cref{lem:numberofMinimumSeparatorComponents} from step $10$ to $t^*-1$ we have $|\mathcal{C}_{G^\beta_{t^*-1}}\,(N_{G_{10}}(v_{r^*,c^*}))|\leq  |\mathcal{C}_{G_{10}}\,(N_{G_{10}}(v_{r^*,c^*}))|=2$.
    Since $N_{G^\beta_{t^*-1}}(v^*)=N_{G_{10}}(v_{r^*,c^*})$ is still a separator at step $t^*-1$ we have that $G^\beta_{t^*-1}- N_{G_{10}}(v_{r^*,c^*})$ has 2 components: $G^\beta_{t^*-1}\,[\{v^*\}]$ and 
    $G^\beta_{t^*-1}-(N_{G_{10}}(v_{r^*,c^*})\cup \{v^*\})$.
    We will use this fact shortly.
    
    By elimination of vertex $v^*$ we get $|\mathcal{C}_{G^\beta_{t^*-1}}\,(N_{G_{10}}(v_{r^*,c^*}))|=1$, in other words $N_{G_{10}}(v_{r^*,c^*})$ is no longer a separator in the graph $G^\beta_{t^*}$.
    By \cref{cor:numberofMinimumSeparators} we can state that $N_{G_{10}}(v_{r^*,c^*})\notin \mathcal{S}^3_{G^\beta_{t-1}}$ for every later step $t\in\{t^*+1,\dots,|V_G|-4\}$.
    Then $N_{G_{10}}(v_{r^*,c^*})$ is the unique separator corresponding to the vertex
    $v^*\in \mathcal{V}_{G_{10}}(\beta,3)$.
    This proves the first part of statement (a).
    
    To prove the second part of this statement further, assume that $v^*$ is selected s.t.\ $t^*\leq |V_G|-5$ and suppose for a contradiction $\beta(t^*)\neq v_{r^*,c^*}$.
    $G_{10}\,[\{v_{r^*,c^*}\}]$ is one of the 2 components of 
    $G_{10}- N_{G_{10}}(v_{r^*,c^*})$ and obviously by elimination of $v_{r^*,c^*}$, $N_{G_{10}}(v_{r^*,c^*})$ will no longer be a separator.
    It is previously shown that $G^\beta_{t^*-1}- N_{G_{10}}(v_{r^*,c^*})$ has 2 components $G^\beta_{t^*-1}\,[\{v^*\}]$ and 
    $G^\beta_{t^*-1}-(N_{G_{10}}(v_{r^*,c^*})\cup \{v^*\})$.
    Combining these two observations, we have that 
    $V_{G^\beta_{t^*-1}}- (N_{G_{10}}(v_{r^*,c^*})\cup \{v^*\}) =\{v_{r^*,c^*}\}$.
    Since $|N_{G_{10}}(v_{r^*,c^*})|=3$ we have that $|V_{G^\beta_{t^*-1}}|=5$ and so $|V_{G^\beta_{t^*}}|=4$, i.e.,\ $t^*=|V_G|-4$.
    This contradicts the assumption that $t^*\leq |V_G|-5$ thus proving the second part of statement (a).
    }
    
    % b
    {
    Statement (b) is easy to see from (a) in the case where $n=7$, as $q=2\ceil{\frac{n-6}{2}}=2$ and 
    $|\{N_{G_{10}}(v_{r,c}) |r\in\{1,4\}, c\in\{4,\dots,n-3\}\}|=2$.
    Therefore, suppose that $n\geq 8$ and fix row and column index 
    $r\in\{1,4\}, c\in\{4,\dots,n-3\}$ s.t.\ 
    $N_{G_{10}}(v_{r,c})=N_{G^\beta_{t}}(\beta(t))$ for a step $t\in\{11,\dots,|V_G|-4\}$.
    There exists at most two column indices $c'\in\{4,\dots,n-3\}\setminus\{c\}$ s.t.\ $|c-c'|=1$ and $N_{G_{10}}\,(v_{r,c'})\in\mathcal{S}^3_{G^\beta_{t-1}}$.
    We claim that $N_{G_{10}}\,(v_{r,c'})\notin\mathcal{S}^3_{G^\beta_{t}}$ for every such column index $c'$.
    
    By statement (a), given that $t\leq|V_G|-5$ we have that $\beta(t)=v_{r,c}$.
    Then in this case we clearly have that $N_{G_{10}}\,(v_{r,c'})\notin\mathcal{S}^3_{G^\beta_{t}}$ as
    $v_{r,c}\in N_{G_{10}}\,(v_{r,c'})$ and
    $v_{r,c}\notin V_{G^\beta_{t}}$.
    Moreover in the case where $t=|V_G|-4$, the graph $G^\beta_{t}$ is clearly a $K_4$ which implies that ${S}^3_{G^\beta_{t}}=\emptyset$ proving our claim.
    Hence, we can thus conclude that $N_{G_{10}}\,(v_{r,c'})\notin\mathcal{S}^3_{G^\beta_{t}}$.
    
    To recap, by elimination of vertex $\beta(t)$,
    $\mathcal{S}^3_{G^\beta_{t-1}}\setminus \mathcal{S}^3_{G^\beta_{t}}$ contains
    $N_{G_{10}}(v_{r,c})$ as well as $N_{G_{10}}(v_{r,c'})$ for every column index $c'\in\{4,\dots,n-3\}\setminus\{c\}$ with $|c-c'|=1$.
    Then given the row index $r=1$, for at most $\ceil{\frac{n-6}{2}}$ indices $c\in\{4,\dots,n-6\}$, the separator $N_{G_{10}}(v_{r,c})$ has a vertex $v\in\mathcal{V}_{G_{10}}(\beta,3)$ mapped to it.
    The case where $r=4$ is symmetric.
Therefore, at most $2\ceil{\frac{n-6}{2}}=q$ vertex sets in $\{N_{G_{10}}(v_{r,c}) |r\in\{1,4\},  c\in\{4,\dots,n-3\}\}$ can have a vertex from $\mathcal{V}_{G_{10}}(\beta,3)$ mapped to them, proving statement (b).
    }
    
    
    By combining statements (a) and (b) we can state that $|\mathcal{V}_{G_{10}}(\beta,3)|\leq q$ contradicting \cref{eq:4nGridVBetaVsAlpha}.
    This proves our claim that $\alpha$ is a minimum elimination ordering over $G_{10}$.
    By our construction, $\max_{v\in V}|\textit{madj}^+_\alpha(v)|=4=\textit{tw}(G)$.
    Additionally, for $i\in\{1,\dots,10\}$, $\alpha(i)$ satisfies one of the conditions (A) or (B) from \cref{lem:tau0Elim} and $\alpha$ is a minimum elimination ordering over the graph $G_{10}$.
    As a result, we can conclude that $\tau(G)=0$.
    }
    
    \case 
    {
    Suppose that $4\leq n\leq 6$.
    By construction, for $i\in\{1,\dots, |X'|+4\}$,
    $\alpha(i)$ is an almost simplicial vertex in the graph $G_{i-1}$ and
    $\max_{i\in\{1,\dots,|X'|+4\}} \textit{deg}_{G_{i-1}}(\alpha(i))=3$.
    Then by \cref{cor:safeTw}, $\textit{tw}(G_{|X'|+4})\leq \textit{tw}(G)=4$.
    Since $\delta(G_{|X'|+4})=4$ we have that $\textit{tw}(G_{|X'|+4})=4$ by \cref{lem:twSubgraph}.
    This, combined with the fact that $\kappa(G_{|X'|+4})=4$ implies that there exists a minimum triangulation of the graph $G_{|X'|+4}$ with treewidth of 4 (as shown in the proof of \cref{lem:tw=kConnected}).
    So let $\alpha$ be one such minimum elimination ordering over $G_{|X'|+4}$ where $\max_{v\in V_{G_{|X'|+4}}}|\textit{madj}^+_\alpha(v)|
    =\textit{tw}(G)=4$.
    
    To conclude $\alpha(i)$ for $i\in\{1,\dots,|X'|+4\}$ satisfies one of the conditions (A) or (B) from \cref{lem:tau0Elim} and by selection $\alpha$ is a minimum elimination ordering over the graph $G_{|X'|+4}$.
    Condition (3) from \cref{lem:tau0Elim} is also satisfied as $\max_{v\in V}|\textit{madj}^+_\alpha(v)|=4=\textit{tw}(G)$ thus showing that $\tau(G)=0$.
    }
\end{mycases}
\end{proof}
}
}
% 4n main

% 4xn grid mfi
{
As a corollary to \cref{lem:4grid} we can state the following about the minimum fill-in value of the $P_4\square P_n$ grid graphs for $n\geq 4$.

\begin{corollary}\label{cor:4grid:nton+2}
Let $G$ be a $P_4\square P_n$ for $n\geq 4$.
Then we have:
\[
\textit{mfi}(P_4\square P_n)= 
\begin{cases}
    18+8(n-4) & \text{if } n \text{ is even}\\
    25+8(n-5) & \text{if } n \text{ is odd}
\end{cases}
\]
\end{corollary}

\begin{proof}

% fig
{
\tikzset{
mystyle/.style={draw=black,rectangle, inner sep=0pt, text width=5mm, text height=1.75 mm,  align=right}
}
\begin{figure}
\centering
  \begin{subfigure}[b]{0.25\textwidth}
    \begin{tikzpicture}
        [scale=0.55,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (11) at (0,2) {\tiny{$v_{1,1}\,\,$}};
        \node [mystyle] (21) at (0,0.6) {\tiny{$v_{2,1}\,\,$}};
        \node [mystyle] (31) at (0,-0.6) {\tiny{$v_{3,1}\,\,$}};
        \node [mystyle] (41) at (0,-2) {\tiny{$v_{4,1}\,\,$}};
        
        \node [mystyle] (12) at (2,2) {\tiny{$v_{1,2}\,\,$}};
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}\,\,$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}\,\,$}};
        \node [mystyle] (42) at (2,-2) {\tiny{$v_{4,2}\,\,$}};
        
        \node [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}\,\,$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}\,\,$}};
        \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (14) at (6,2) {\tiny{$v_{1,4}\,\,$}};
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        \node [mystyle] (44) at (6,-2) {\tiny{$v_{4,4}\,\,$}};
        \draw[-] 
        {
        (11)--(21)
        (21)--(31)
        (31)--(41)
        (11)--(12)
        (21)--(22)
        (31)--(32)
        (41)--(42)
        
        (12)--(22)
        (22)--(32)
        (32)--(42)
        (12)--(13)
        (22)--(23)
        (32)--(33)
        (42)--(43)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(14)
        (23)--(24)
        (33)--(34)
        (43)--(44)
        
        (14)--(24)
        (24)--(34)
        (34)--(44)
        }
        ;
        
        
        \draw[draw=MyColorOneDark, line width=0.35mm]
        (12)--(21)
        (31)--(42)
        (34)--(43)
        (13)--(24)
        % 4
        ;
        \draw[draw=MyColorOne, line width=0.35mm]
        (31)--(22)
        (31)--(12)
        
        (42)--(33)
        (42)--(34)
        
        (34)--(23)
        (34)--(13)
        
        (12)--(23)
        (12)to[out=0, in=90, looseness=0.45](34)
        % 8
        ;
        \draw[draw=MyColorTwo, line width=0.35mm]
        (42)--(23)
        (12)--(33)
        (12)to[out=180,in=180,looseness=0.35](32)
        (22)to[out=180,in=180,looseness=0.2](42)
        (12)to[in=0,out=0,looseness=0.2](42)
        
        (33)--(22)
        ;
    \end{tikzpicture}
    \caption{$n=4$}
    \label{fig:4grid:44}
  \end{subfigure}
  \hspace{1.5cm}
  \begin{subfigure}[b]{0.35\textwidth}
    \begin{tikzpicture}
        [scale=0.55,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (11) at (0,2) {\tiny{$v_{1,1}\,\,$}};
        \node [mystyle] (21) at (0,0.6) {\tiny{$v_{2,1}\,\,$}};
        \node [mystyle] (31) at (0,-0.6) {\tiny{$v_{3,1}\,\,$}};
        \node [mystyle] (41) at (0,-2) {\tiny{$v_{4,1}\,\,$}};
        
        \node [mystyle] (12) at (2,2) {\tiny{$v_{1,2}\,\,$}};
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}\,\,$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}\,\,$}};
        \node [mystyle] (42) at (2,-2) {\tiny{$v_{4,2}\,\,$}};
        
        \node [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}\,\,$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}\,\,$}};
        \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (14) at (6,2) {\tiny{$v_{1,4}\,\,$}};
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        \node [mystyle] (44) at (6,-2) {\tiny{$v_{4,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        \draw[-] 
        {
        (11)--(21)
        (21)--(31)
        (31)--(41)
        (11)--(12)
        (21)--(22)
        (31)--(32)
        (41)--(42)
        
        (12)--(22)
        (22)--(32)
        (32)--(42)
        (12)--(13)
        (22)--(23)
        (32)--(33)
        (42)--(43)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(14)
        (23)--(24)
        (33)--(34)
        (43)--(44)
        
        (14)--(24)
        (24)--(34)
        (34)--(44)
        (14)--(15)
        (24)--(25)
        (34)--(35)
        (44)--(45)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        }
        ;
        
        
        \draw[draw=MyColorOneDark, line width=0.35mm]
        (12)--(21)
        (31)--(42)
        
        (35)--(44)
        (14)--(25)
        % 4
        ;
        \draw[draw=MyColorOne, line width=0.35mm]
        (31)--(22)
        (31)--(12)
        
        (31)to[out=45, in=180, looseness=0.45](13)
        (13)--(22)
        
        (43)--(32)
        (43)--(31)
        
        (43)--(34)
        (43)--(35)
        
        (35)--(24)
        (35)--(14)
        
        (13)--(24)
        (13)to[out=0, in=135, looseness=0.45](35)
        % 12
        ;
        \draw[draw=MyColorTwo, line width=0.35mm]
        (22)--(43)
        (32)--(13)
        (13)to[in=0,out=0,looseness=0.2](43)
        
        (13)--(34)
        (43)--(24)
        (13)to[out=180,in=180,looseness=0.35](33)
        (23)to[out=180,in=180,looseness=0.2](43)
        
        (32)--(23)
        (23)--(34)
        % 9 
        ;
    \end{tikzpicture}
    \caption{$n=5$}
    \label{fig:4grid:45}
  \end{subfigure}
  \hfill\\
  \hfill\\
  \begin{subfigure}[b]{0.4\textwidth}
    \begin{tikzpicture}
        [scale=0.55,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (11) at (0,2) {\tiny{$v_{1,1}\,\,$}};
        \node [mystyle] (21) at (0,0.6) {\tiny{$v_{2,1}\,\,$}};
        \node [mystyle] (31) at (0,-0.6) {\tiny{$v_{3,1}\,\,$}};
        \node [mystyle] (41) at (0,-2) {\tiny{$v_{4,1}\,\,$}};
        
        \node [mystyle] (12) at (2,2) {\tiny{$v_{1,2}\,\,$}};
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}\,\,$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}\,\,$}};
        \node [mystyle] (42) at (2,-2) {\tiny{$v_{4,2}\,\,$}};
        
        \node [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}\,\,$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}\,\,$}};
        \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (14) at (6,2) {\tiny{$v_{1,4}\,\,$}};
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        \node [mystyle] (44) at (6,-2) {\tiny{$v_{4,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        
        \node [mystyle] (16) at (10,2) {\tiny{$v_{1,6}\,\,$}};
        \node [mystyle] (26) at (10,0.6) {\tiny{$v_{2,6}\,\,$}};
        \node [mystyle] (36) at (10,-0.6) {\tiny{$v_{3,6}\,\,$}};
        \node [mystyle] (46) at (10,-2) {\tiny{$v_{4,6}\,\,$}};
        \draw[-] 
        {
        (11)--(21)
        (21)--(31)
        (31)--(41)
        (11)--(12)
        (21)--(22)
        (31)--(32)
        (41)--(42)
        
        (12)--(22)
        (22)--(32)
        (32)--(42)
        (12)--(13)
        (22)--(23)
        (32)--(33)
        (42)--(43)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(14)
        (23)--(24)
        (33)--(34)
        (43)--(44)
        
        (14)--(24)
        (24)--(34)
        (34)--(44)
        (14)--(15)
        (24)--(25)
        (34)--(35)
        (44)--(45)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(16)
        (25)--(26)
        (35)--(36)
        (45)--(46)
        
        (16)--(26)
        (26)--(36)
        (36)--(46)
        }
        ;
        
        
        \draw[draw=MyColorOneDark, line width=0.35mm]
        (12)--(21)
        (31)--(42)
        
        (36)--(45)
        (15)--(26)
        % 4
        ;
        \draw[draw=MyColorOne, line width=0.35mm]
        (31)--(22)
        (31)--(12)
        
        (31)to[out=45, in=180, looseness=0.45](13)
        (13)--(22)
        
        (43)--(32)
        (43)--(31)
        
        (44)--(35)
        (44)--(36)
        
        (36)--(25)
        (36)--(15)
        
        (14)--(25)
        (14)to[out=0, in=135, looseness=0.45](36)
        % 12
        ;
        \draw[draw=MyColorTwo, line width=0.35mm]
        (22)--(43)
        (32)--(13)
        (13)to[in=0,out=0,looseness=0.2](43) 
        
        (13)to[out=180,in=180,looseness=0.2](33)
        (23)to[out=180,in=180,looseness=0.2](43)
        (32)--(23) 
        
        (14)--(35)
        (44)--(25)
        (14)to[out=180,in=180,looseness=0.2](34)
        (24)to[out=180,in=180,looseness=0.2](44)
        (14)to[in=0,out=0,looseness=0.2](44) 
        
        (24)--(35) 
        
        (14)--(23)
        (14)--(33)
        (14)--(43) 
        
        (43)--(34)
        (43)--(24) 
        
        (33)--(24) 
        % 18
        ;
    \end{tikzpicture}
    \caption{$n=6$}
    \label{fig:4grid:46}
  \end{subfigure}
  \hfill\\
  \hfill\\
  \begin{subfigure}[b]{0.6\textwidth}
    \begin{tikzpicture}
        [scale=0.55,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (11) at (0,2) {\tiny{$v_{1,1}\,\,$}};
        \node [mystyle] (21) at (0,0.6) {\tiny{$v_{2,1}\,\,$}};
        \node [mystyle] (31) at (0,-0.6) {\tiny{$v_{3,1}\,\,$}};
        \node [mystyle] (41) at (0,-2) {\tiny{$v_{4,1}\,\,$}};
        
        \node [mystyle] (12) at (2,2) {\tiny{$v_{1,2}\,\,$}};
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}\,\,$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}\,\,$}};
        \node [mystyle] (42) at (2,-2) {\tiny{$v_{4,2}\,\,$}};
        
        \node [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}\,\,$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}\,\,$}};
        \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (14) at (6,2) {\tiny{$v_{1,4}\,\,$}};
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        \node [mystyle] (44) at (6,-2) {\tiny{$v_{4,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        
        \node (1n-2) at (11.5,2)    {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (11.5,0.6)  {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (11.5,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (11.5,-2)   {\tiny{$v_{4,n-2}$}};
        
        \node (1n-1) at (13.5,2)    {\tiny{$v_{1,n-1}$}};
        \node (2n-1) at (13.5,0.6)  {\tiny{$v_{2,n-1}$}};
        \node (3n-1) at (13.5,-0.6) {\tiny{$v_{3,n-1}$}};
        \node (4n-1) at (13.5,-2)   {\tiny{$v_{4,n-1}$}};
        
        \node [mystyle] (1n) at (15.5,2)    {\tiny{$v_{1,n}\,\,$}};
        \node [mystyle] (2n) at (15.5,0.6)  {\tiny{$v_{2,n}\,\,$}};
        \node [mystyle] (3n) at (15.5,-0.6) {\tiny{$v_{3,n}\,\,$}};
        \node [mystyle] (4n) at (15.5,-2)   {\tiny{$v_{4,n}\,\,$}};
        \draw[-] 
        {
        (11)--(21)
        (21)--(31)
        (31)--(41)
        (11)--(12)
        (21)--(22)
        (31)--(32)
        (41)--(42)
        
        (12)--(22)
        (22)--(32)
        (32)--(42)
        (12)--(13)
        (22)--(23)
        (32)--(33)
        (42)--(43)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(14)
        (23)--(24)
        (33)--(34)
        (43)--(44)
        
        (14)--(24)
        (24)--(34)
        (34)--(44)
        (14)--(15)
        (24)--(25)
        (34)--(35)
        (44)--(45)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(9.25,2)   
        (25)--(9.25,0.6) 
        (35)--(9.25,-0.6)
        (45)--(9.25,-2)  
        
        (1n-2)--(2n-2)
        (1n-2)--(1n-1)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        (4n-2)--(4n-1)
        (1n-2)--(10.25,2)    
        (2n-2)--(10.25,0.6)  
        (3n-2)--(10.25,-0.6) 
        (4n-2)--(10.25,-2)   
        
        (1n-1)--(2n-1)
        (2n-1)--(3n-1)
        (3n-1)--(4n-1)
        (1n-1)--(1n)
        (2n-1)--(2n)
        (3n-1)--(3n)
        (4n-1)--(4n)
        
        (1n)--(2n)
        (2n)--(3n)
        (3n)--(4n)
        }
        ;
        \draw[draw=black,style=thick,dotted]
        (9.5,2)--(10,2)   
        (9.5,0.6)--(10,0.6) 
        (9.5,-0.6)--(10,-0.6) 
        (9.5,-2)--(10,-2)
        ;
        \draw[draw=MyColorOneDark, line width=0.35mm]
        (12)--(21)
        (31)--(42)
        
        (3n)--(4n-1)
        (1n-1)--(2n)
        % 4
        ;
        \draw[draw=MyColorOne, line width=0.35mm]
        (31)--(22)
        (31)--(12)
        
        (31)to[out=45, in=180, looseness=0.45](13)
        (13)--(22)
        
        (43)--(32)
        (43)--(31)
        
        (4n-2)--(3n-1)
        (4n-2)--(3n)
        
        (3n)--(2n-1)
        (3n)--(1n-1)
        
        (1n-2)--(2n-1)
        (1n-2)to[out=0, in=135, looseness=0.45](3n)
        % 12
        ;
        
        \draw[draw=cyan, line width=0.35mm]
        (13)--(24)
        (24)--(15)
        (13)to[out=90,in=90,looseness=0.2](15)
        
        (43)--(34)
        (34)--(45)
        (43)to[out=270,in=270,looseness=0.2](45)
        ;
        
        \draw[draw=MyColorTwo, line width=0.35mm]
        (22)--(43)
        (32)--(13)
        
        (13)to[in=0,out=0,looseness=0.2](43) 
        (13)to[out=180,in=180,looseness=0.2](33)
        (23)to[out=180,in=180,looseness=0.2](43)
        
        (32)--(23) 
        
        (1n-2)--(3n-1)
        (4n-2)--(2n-1)
        (1n-2)to[out=180,in=180,looseness=0.2](3n-2)
        (2n-2)to[out=180,in=180,looseness=0.2](4n-2)
        (1n-2)to[in=0,out=0,looseness=0.2](4n-2) 
        
        (2n-2)--(3n-1) 
        
        (15)to[in=0,out=0,looseness=0.2](45) 
        (15)to[out=180,in=180,looseness=0.2](35)
        (25)to[out=180,in=180,looseness=0.2](45)
        
        (13)--(24)
        (24)--(15)
        
        (43)--(34)
        (34)--(45)
        
        (24)--(33)
        (24)--(43)
        (13)--(34)
        
        (24)--(35)
        (24)--(45)
        (34)--(15)
        % 
        ;
        
    \end{tikzpicture}
    \caption{$n\geq 7$ and $n$ is odd}
    \label{fig:4grid:triangulationOdd}
  \end{subfigure}
  \hfill\\
  \hfill\\
  \begin{subfigure}[b]{0.7\textwidth}
    \begin{tikzpicture}
        [scale=0.55,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (11) at (0,2) {\tiny{$v_{1,1}\,\,$}};
        \node [mystyle] (21) at (0,0.6) {\tiny{$v_{2,1}\,\,$}};
        \node [mystyle] (31) at (0,-0.6) {\tiny{$v_{3,1}\,\,$}};
        \node [mystyle] (41) at (0,-2) {\tiny{$v_{4,1}\,\,$}};
        
        \node [mystyle] (12) at (2,2) {\tiny{$v_{1,2}\,\,$}};
        \node [mystyle] (22) at (2,0.6) {\tiny{$v_{2,2}\,\,$}};
        \node [mystyle] (32) at (2,-0.6) {\tiny{$v_{3,2}\,\,$}};
        \node [mystyle] (42) at (2,-2) {\tiny{$v_{4,2}\,\,$}};
        
        \node [mystyle] (13) at (4,2) {\tiny{$v_{1,3}\,\,$}};
        \node [mystyle] (23) at (4,0.6) {\tiny{$v_{2,3}\,\,$}};
        \node [mystyle] (33) at (4,-0.6) {\tiny{$v_{3,3}\,\,$}};
        \node [mystyle] (43) at (4,-2) {\tiny{$v_{4,3}\,\,$}};
        
        \node [mystyle] (14) at (6,2) {\tiny{$v_{1,4}\,\,$}};
        \node [mystyle] (24) at (6,0.6) {\tiny{$v_{2,4}\,\,$}};
        \node [mystyle] (34) at (6,-0.6) {\tiny{$v_{3,4}\,\,$}};
        \node [mystyle] (44) at (6,-2) {\tiny{$v_{4,4}\,\,$}};
        
        \node [mystyle] (15) at (8,2) {\tiny{$v_{1,5}\,\,$}};
        \node [mystyle] (25) at (8,0.6) {\tiny{$v_{2,5}\,\,$}};
        \node [mystyle] (35) at (8,-0.6) {\tiny{$v_{3,5}\,\,$}};
        \node [mystyle] (45) at (8,-2) {\tiny{$v_{4,5}\,\,$}};
        
        \node (1n-3) at (11.5,2)    {\tiny{$v_{1,n-3}$}};
        \node (2n-3) at (11.5,0.6)  {\tiny{$v_{2,n-3}$}};
        \node (3n-3) at (11.5,-0.6) {\tiny{$v_{3,n-3}$}};
        \node (4n-3) at (11.5,-2)   {\tiny{$v_{4,n-3}$}};
        
        
        \node (1n-2) at (13.5,2)    {\tiny{$v_{1,n-2}$}};
        \node (2n-2) at (13.5,0.6)  {\tiny{$v_{2,n-2}$}};
        \node (3n-2) at (13.5,-0.6) {\tiny{$v_{3,n-2}$}};
        \node (4n-2) at (13.5,-2)   {\tiny{$v_{4,n-2}$}};
        
        \node (1n-1) at (15.5,2)    {\tiny{$v_{1,n-1}$}};
        \node (2n-1) at (15.5,0.6)  {\tiny{$v_{2,n-1}$}};
        \node (3n-1) at (15.5,-0.6) {\tiny{$v_{3,n-1}$}};
        \node (4n-1) at (15.5,-2)   {\tiny{$v_{4,n-1}$}};
        
        \node [mystyle] (1n) at (17.5,2)    {\tiny{$v_{1,n}\,\,$}};
        \node [mystyle] (2n) at (17.5,0.6)  {\tiny{$v_{2,n}\,\,$}};
        \node [mystyle] (3n) at (17.5,-0.6) {\tiny{$v_{3,n}\,\,$}};
        \node [mystyle] (4n) at (17.5,-2)   {\tiny{$v_{4,n}\,\,$}};
        \draw[-] 
        {
        (11)--(21)
        (21)--(31)
        (31)--(41)
        (11)--(12)
        (21)--(22)
        (31)--(32)
        (41)--(42)
        
        (12)--(22)
        (22)--(32)
        (32)--(42)
        (12)--(13)
        (22)--(23)
        (32)--(33)
        (42)--(43)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(14)
        (23)--(24)
        (33)--(34)
        (43)--(44)
        
        (14)--(24)
        (24)--(34)
        (34)--(44)
        (14)--(15)
        (24)--(25)
        (34)--(35)
        (44)--(45)
        
        (15)--(25)
        (25)--(35)
        (35)--(45)
        (15)--(9.25,2)   
        (25)--(9.25,0.6) 
        (35)--(9.25,-0.6)
        (45)--(9.25,-2)  
        
        
        (1n-3)--(10.25,2)    
        (2n-3)--(10.25,0.6)  
        (3n-3)--(10.25,-0.6) 
        (4n-3)--(10.25,-2)  
        
        (1n-3)--(2n-3)
        (2n-3)--(3n-3)
        (3n-3)--(4n-3)
        
        (1n-3)--(1n-2)
        (2n-3)--(2n-2)
        (3n-3)--(3n-2)
        (4n-3)--(4n-2)
        
        (1n-2)--(2n-2)
        (1n-2)--(1n-1)
        (2n-2)--(3n-2)
        (3n-2)--(4n-2)
        (2n-2)--(2n-1)
        (3n-2)--(3n-1)
        (4n-2)--(4n-1) 
        
        (1n-1)--(2n-1)
        (2n-1)--(3n-1)
        (3n-1)--(4n-1)
        (1n-1)--(1n)
        (2n-1)--(2n)
        (3n-1)--(3n)
        (4n-1)--(4n)
        
        (1n)--(2n)
        (2n)--(3n)
        (3n)--(4n)
        }
        ;
        \draw[draw=black,style=thick,dotted]
        (9.5,2)--(10,2)   
        (9.5,0.6)--(10,0.6) 
        (9.5,-0.6)--(10,-0.6) 
        (9.5,-2)--(10,-2)
        ;
        \draw[draw=MyColorOneDark, line width=0.35mm]
        (12)--(21)
        (31)--(42)
        
        (3n)--(4n-1)
        (1n-1)--(2n)
        % 4
        ;
        \draw[draw=MyColorOne, line width=0.35mm]
        (31)--(22)
        (31)--(12)
        
        (31)to[out=45, in=180, looseness=0.45](13)
        (13)--(22)
        
        (43)--(32)
        (43)--(31)
        
        (4n-2)--(3n-1)
        (4n-2)--(3n)
        
        (3n)--(2n-1)
        (3n)--(1n-1)
        
        (1n-2)--(2n-1)
        (1n-2)to[out=0, in=135, looseness=0.45](3n)
        % 12
        ;
        
        \draw[draw=cyan, line width=0.35mm]
        (13)--(24)
        (24)--(15)
        (13)to[out=90,in=90,looseness=0.2](15)
        
        (43)--(34)
        (34)--(45)
        (43)to[out=270,in=270,looseness=0.2](45)
        ;
        
        \draw[draw=MyColorTwo, line width=0.35mm]
        (22)--(43)
        (32)--(13)
        
        (13)to[in=0,out=0,looseness=0.2](43) 
        (13)to[out=180,in=180,looseness=0.2](33)
        (23)to[out=180,in=180,looseness=0.2](43)
        
        (32)--(23) 
        
        (1n-2)--(3n-1)
        (4n-2)--(2n-1)
        (1n-2)to[out=180,in=180,looseness=0.2](3n-2)
        (2n-2)to[out=180,in=180,looseness=0.2](4n-2)
        (1n-2)to[in=0,out=0,looseness=0.2](4n-2) 
        
        (2n-2)--(3n-1) 
        
        (15)to[in=0,out=0,looseness=0.2](45) 
        (15)to[out=180,in=180,looseness=0.2](35)
        (25)to[out=180,in=180,looseness=0.2](45)
        
        (13)--(24)
        (24)--(15)
        
        (43)--(34)
        (34)--(45)
        
        (24)--(33)
        (24)--(43)
        (13)--(34)
        
        (24)--(35)
        (24)--(45)
        (34)--(15)
        
        (1n-3)to[out=180,in=180,looseness=0.2](3n-3)
        (2n-3)to[out=180,in=180,looseness=0.2](4n-3)
        (1n-3)to[in=0,out=0,looseness=0.2](4n-3) 
        
        (1n-2)--(2n-3)
        (1n-2)--(3n-3)
        (1n-2)--(4n-3) 
        
        (4n-3)--(3n-2)
        (4n-3)--(2n-2) 
        
        (3n-3)--(2n-2) 
        % 
        ;
        
    \end{tikzpicture}
    \caption{$n\geq 7$ and $n$ is even}
    \label{fig:4grid:triangulationEven}
  \end{subfigure}
\vspace{0.5cm}
\caption
{
The triangulation $G^+_\alpha$ obtained from $P_4\square P_n$ graph $G$ using the elimination ordering defined in the proof of \cref{lem:4grid}.
The edges in light green are added first, after the elimination of vertices $X$.
Next the edges in dark green are added in $\alpha$, when the vertices in $X'$ are eliminated.
Afterwards, we add the light blue edges, done after we eliminate the vertices in $X''$ (this is only the case when $n\geq 7$).
Finally we add the dark blue edges, that is during the steps in $\alpha$ where the intermideate graphs have vertex connectivity of 4.
(a)-(c) depict $G^+_\alpha$ for $n\in\{4,5,6\}$.
(d),(e) show the complementary cases when $n\geq 7$.
} 
\label{fig:4Grid:Mfi}
\end{figure}
}

Let $\alpha$ be the elimination ordering over $G$ defined in the proof of \cref{lem:4grid}.
$\alpha$ is a minimum elimination ordering over $G$ as it satisfies both conditions (1) and (2) from \cref{lem:safeVertexRepeatedly}.
Then $\alpha$ adds $\textit{mfi}(G)$ edges while eliminating the vertex set of $G$.

$\alpha$ begins by eliminating the vertices of $X=\{v_{1,1},v_{1,n},v_{4,1},v_{4,n}\}$.
Clearly, 1 edge is added in $G^+_\alpha$ by elimination of every vertex $v\in X$.
Next $\alpha$ eliminates vertices of the set $X'$ which is defined depending on the following cases:
given that $n=4$, $X'=\{v_{2,1},v_{4,3},v_{2,4},v_{1,3}\}$ and for $n\geq 5$ we have 
$X'=\{v_{2,1},v_{1,2},v_{4,2},v_{4,n-1},v_{2,n},v_{1,n-1}\}$.
% n=4: 3×4+3+2+1 = 18
% n>=5: 2×6
Similarly, 2 edges are added in $G^+_\alpha$ by elimination of every vertex $v\in X'$.
At this stage, let us consider the following cases:
\begin{mycases}
    \case
    {
    Suppose that $n\leq 6$.
    We first define $\alpha$ over the graph $G_{|X|+|X'|}$ and then define the value of $\textit{mfi}(G)$ depending on the following subcases:
    
    \begin{subcases}
        \subcase
        {
        Suppose that $n=4$.
        After elimination of vertices $X\cup X'$, we have that
        $\textit{tw}(G_{|X'|+4})=\kappa(G_{|X'|+4})=4$.
        Let $\alpha$ eliminate the following vertices (in this order) during the steps $i\in\{9,\dots,12\}$:
        $ v_{3,1}, v_{3,2}, v_{2,2}, v_{1,2} $.
        It is easy to see that all above vertices are eliminated with degree of 4 and that the resulting graph, $G_{12}$, is a $K_4$.
        Therefore, by \cref{cor:tw=kConnected}, $\alpha$ is a minimum elimination ordering over $G_8$ and by our construction it is easy to confirm that $\textit{mfi}(G)=18$ in this case (see \cref{fig:4grid:44}).
        }
        
        \subcase
        {
        Suppose that $n=5$.
        During the steps $i\in\{11,\dots,16\}$ let $\alpha$ eliminate the following vertices:
        $ v_{3,1}, v_{2,2}, v_{3,2}, v_{3,3}, v_{2,3}, v_{1,3}$.
        All above vertices are eliminated with degree 4 thus $\alpha$ is a minimum elimination ordering over $G_{10}$.
        Then in this case $\textit{mfi}(G)=25$ (see \cref{fig:4grid:45}).
        }
        
        \subcase
        {
        Finally, suppose that $n=6$.
        During the steps $i\in\{11,\dots,20\}$ let $\alpha$ eliminate the following vertices in the specified order:
        $v_{3,1}, v_{2,2}, v_{3,2}, v_{1,3}, v_{2,3}, v_{3,3}, v_{4,3}, v_{3,4}, v_{2,4}, v_{1,4}$.
        $\alpha$ is a minimum elimination ordering over $G_{10}$ as every one of the above vertices are eliminated with degree of 4.
        Then in this case $\textit{mfi}(G)=34$ (see \cref{fig:4grid:46}).
        % 4×2+6×3+10×4+3+2+1-((4-1)*6+(6-1)*4)=34
        }
    \end{subcases}
    }
    
    \case
    {
    Suppose that $n\geq 7$.
    There are 14 edges added in $\alpha$ by elimination of the vertices in columns 1 and 2.
    Observe that the 3 missing edges turning the vertices of column 3 into a clique are among the above-mentioned edges.
    
    Let us consider how many edges are added in $G^+_\alpha$ when eliminating the vertices of columns $c$ and $c+1$ for every odd column index $c\in\{3,\dots,n-4\}$.
    The vertices of column $c$ become a clique after the elimination of the vertices from columns $c-1$ and $c-2$ (see \cref{fig:4grid2:G13} for an example).
    Therefore, we do not count the added edges between the vertices of column $c$.
    $\alpha$ adds 3 edges by elimination of $v_{1,c+1}$ and the same number of edges are added when $v_{4,c+1}$ is eliminated (these vertices belong to the vertex set $X''$ discussed in the proof of \cref{lem:4grid}).
    By elimination of every other vertex from columns $c$ and $c+1$, $\alpha$ adds 10 edges, including the set of missing edges turning the vertices of column $c+2$ into a clique.
    As a demonstration, when $c=3$, these added edges are highlighted in bright green in \cref{fig:4grid2:G14} to \cref{fig:4grid2:G19}.
    Therefore, we can conclude that $\alpha$ adds a total of 16 edges while eliminating the vertices of
    $\{v_{r,c}, v_{r,c+1}, |r\in\{1,\dots,4\}\}$.
    Next, let us consider the following subcases:
    \begin{subcases}
        \subcase
        {
        Suppose that $n$ is odd.
        We have thus far considered the number of added edges when $\alpha$ eliminates the vertices of columns 1 to $n-3$.
        Note that vertex set of column $n-2$ is a clique at this stage.
        There are 11 added edges in $G^+_\alpha$ by elimination of the vertices in columns $n-2$, $n-1$ and $n$.
        Putting all this together, we can see that $G^+_\alpha$ has $14+16(\frac{n-5}{2})+11$ added edges (see \cref{fig:4grid:triangulationOdd}).
        As a result, $\textit{mfi}(G)=25+8(n-5)$.
        }
        
        \subcase
        {
        Suppose that $n$ is even.
        Thus far, we have considered the number of added edges by $\alpha$ when eliminating the vertices of columns 1 to $n-4$.
        At this stage, the vertex set of column $n-3$ is a clique.
        There are 20 added edges in $G^+_\alpha$ when the vertices of columns $n-3$ to $n$ are eliminated.
        Then by combining our above observations, we have that $G^+_\alpha$ has $14+16(\frac{n-6}{2})+20$ added edges (see \cref{fig:4grid:triangulationEven}).
        Consequently, in this case, $\textit{mfi}(G)=18+8(n-4)$.
        }
    \end{subcases}
    }
\end{mycases}

This concludes the statement of the corollary as desired.
\end{proof}
}

==> content/rook.tex <==
\section{Minimum Fill-In and $\tau$ Parameter: Rook's graph}\label{sec:tfm:rook}


% rook def
{
The $m\times n$ \textit{rook's graph}, written as $K_m\square K_n$, is the Cartesian product of two cliques $K_m,K_n$ respectively on $m,n$ vertices.
Informally, the $m\times n$ rook's graph represents all legal moves of the rook chess piece on an $m\times n$ chessboard.
We point out that every vertex in an $m\times n$ rook's graph $G$ has degree of $m+n-2$ and that $\kappa(G)=m+n-2$.\unsure{Is this needed?}
}


% rook
{
% rook helper
{

In this section, we will study the parameters $\tau$ and $\textit{mfi}$ of rook's graphs.
While doing this, we will also prove some properties of rook's graphs.
The structure of these graphs and hence our approach to them differs significantly from what was discussed in \cref{sec:grid:grid}.
We will show in this section that there exists a rook's graph $G$, with relatively small dimensions, where $\tau(G)>0$.
To simplify our discussion, we begin by introducing some shorthands and a general lemma concerning elimination ordering of rook's graphs.

Given an elimination ordering $\alpha$ over the graph $G=(V,E)$ and two steps $i,j$, $1\leq i<j\leq |V|$, define the set of vertices $\alpha[i,j]=\{\alpha(t)|t\in\{i,\dots,j\}\}$. 
Also let $\textit{comp}_\alpha(i)$ be the connected component of $G[\alpha[1,i]]$ containing the vertex $\alpha(i)$.

Let $G=(V,E)$ be a $K_m\square K_n$ (rook's) graph, for $m,n\geq 2$.
For $c\in\{1,\dots,n\}$ let $L_c=\{v_{r,c}| r\in\{1,\dots,m\}\}$ and for $r\in\{1,\dots,m\}$ let $M_r=\{v_{r,c}| c\in\{1,\dots,n\}\}$.
Simply put, $L_c,M_r$ are respectively the vertices of the column number $c$ and row number $r$ of $G$.
Given an elimination ordering $\alpha$ over the rook's graph $G$ and a step $i\in \{1,\dots,|V|\}$, let $\mathcal{M}_\alpha(i)$ be the set of row indices spanned by $\textit{comp}_\alpha(i)$ and $\mathcal{L}_\alpha(i)$ the set of column indices spanned by $\textit{comp}_\alpha(i)$.

Formally 
$\mathcal{M}_\alpha(i)=\{r|r\in \{1, \dots, m\}, M_r\cap V_{\textit{comp}_\alpha(i)}\neq\emptyset\}$ and 
$\mathcal{L}_\alpha(i)=\{c|c\in\{1,\dots,n\}, L_c\cap V_{\textit{comp}_\alpha(i)}\neq\emptyset\}$.
The next lemma shows the relationship between
$\textit{madj}^+_\alpha(\alpha(i))$ and $\textit{comp}_\alpha(i)$.

\begin{lemma}\label{rmk:madjRooks}
Let $G=(V,E)$ be a $K_m\square K_n$ for $n,m\geq 2$ and $\alpha$ an elimination ordering over $G$.
For a step $i\in \{1,\dots,|V|\}$ of the elimination ordering $\alpha$ we have:

$$
\textit{madj}^+_\alpha(\alpha(i))=
\{v_{r,c}| 
c\in \mathcal{L}_\alpha(i) \textit{ \,or\, } r\in \mathcal{M}_\alpha(i)\}
\setminus \alpha[1,i]
$$
\end{lemma}

\begin{proof}
%figure
{
\tikzset{
mystyle/.style={draw=black,rectangle, inner sep=0pt, text width=5mm, text height=1.75 mm,  align=right, fill=white}
}
\tikzset{
madj/.style={draw=black,rectangle, inner sep=0pt, text width=5mm, text height=1.75 mm,  align=right,  fill=MyColorOne}
}
\tikzset{
elim/.style={draw=black,rectangle, inner sep=0pt, text width=5mm, text height=1.75 mm,  align=right,  fill=red!80}
}
\tikzset{
current/.style={draw=black,rectangle, line width=0.47mm,  inner sep=0.5pt, text width=5mm, text height=1.75 mm,  align=right,  fill=red!80}
}
\tikzset{
comp/.style={draw=black,circle, inner sep=0pt, text width=7mm, text height=2 mm,  align=right,  fill=yellow, opacity=0.5}
}
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.25\textwidth}
  \begin{tikzpicture}[scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
    \node [elim] (11) at (0,3) {\tiny{$v_{1,1}\,\, $ }};
    \node [elim] (21) at (0.25,1.5) {\tiny{$v_{2,1}\,\, $ }};
    \node [madj] (31) at (-0.25,0) {\tiny{$v_{3,1}\,\, $ }};
    \node [madj] (41) at (0,-1.5) {\tiny{$v_{4,1}\,\, $ }};
    
    
    \node [current] (12) at (2,3.25) {\tiny{$v_{1,2}\,\, $ }};
    \node [madj] (22) at (2.25,1.75) {\tiny{$v_{2,2}\,\, $ }};
    \node [madj] (32) at (1.75,0.25) {\tiny{$v_{3,2}\,\, $ }};
    \node [madj] (42) at (2,-1.25) {\tiny{$v_{4,2}\,\, $ }};
    
    
    \node [madj] (13) at (4,2.75) {\tiny{$v_{1,3}\,\, $ }};
    \node [madj] (23) at (4.25,1.25) {\tiny{$v_{2,3}\,\, $ }};
    \node [mystyle] (33) at (3.75,-0.25) {\tiny{$v_{3,3}\,\, $ }};
    \node [mystyle] (43) at (4,-1.75) {\tiny{$v_{4,3}\,\, $ }};
    
    
    \node [madj] (14) at (6,3) {\tiny{$v_{1,4}\,\, $ }};
    \node [madj] (24) at (6.25,1.5) {\tiny{$v_{2,4}\,\, $ }};
    \node [mystyle] (34) at (5.75,-0) {\tiny{$v_{3,4}\,\, $ }};
    \node [mystyle] (44) at (6,-1.5) {\tiny{$v_{4,4}\,\, $ }};
    
    \begin{scope}[on background layer]
    {
    \draw[-] 
        (11)--(12)
        (12)--(13)
        (13)--(14)
        (11)--(13)
        (11)--(14)
        (12)--(14)
        
        (21)--(22)
        (22)--(23)
        (23)--(24)
        (21)--(23)
        (21)--(24)
        (22)--(24)
        
        (31)--(32)
        (32)--(33)
        (33)--(34)
        (31)--(33)
        (31)--(34)
        (32)--(34)
        
        (41)--(42)
        (42)--(43)
        (43)--(44)
        (41)--(43)
        (41)--(44)
        (42)--(44)
        
        
        (11)--(21)
        (21)--(31)
        (31)--(41)
        (11)--(31)
        (11)--(41)
        (21)--(41)
        
        (12)--(22)
        (22)--(32)
        (32)--(42)
        (12)--(32)
        (12)--(42)
        (22)--(42)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(33)
        (13)--(43)
        (23)--(43)
        
        (14)--(24)
        (24)--(34)
        (34)--(44)
        (14)--(34)
        (14)--(44)
        (24)--(44)
        ;
        }
    \node [comp] (11comp) at (0,3) {};
    \node [comp] (21comp) at (0.25,1.5) {};
    \node [comp] (12comp) at (2,3.25) {};
    \end{scope}
    \end{tikzpicture}
    \caption{$i=3,\alpha(i)=v_{1,2}$}
    \label{fig:RookMadjDemo0}   
  \end{subfigure}
  \hspace{1.15em}
  \vspace{0.5em}
  \begin{subfigure}[b]{0.25\textwidth}
  \begin{tikzpicture}[scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
    \node [elim] (11) at (0,3) {\tiny{$v_{1,1}\,\, $ }};
    \node [elim] (21) at (0.25,1.5) {\tiny{$v_{2,1}\,\, $ }};
    \node [madj] (31) at (-0.25,0) {\tiny{$v_{3,1}\,\, $ }};
    \node [mystyle] (41) at (0,-1.5) {\tiny{$v_{4,1}\,\, $ }};
    
    
    \node [elim] (12) at (2,3.25) {\tiny{$v_{1,2}\,\, $ }};
    \node [mystyle] (22) at (2.25,1.75) {\tiny{$v_{2,2}\,\, $ }};
    \node [madj] (32) at (1.75,0.25) {\tiny{$v_{3,2}\,\, $ }};
    \node [mystyle] (42) at (2,-1.25) {\tiny{$v_{4,2}\,\, $ }};
    
    
    \node [madj] (13) at (4,2.75) {\tiny{$v_{1,3}\,\, $ }};
    \node [madj] (23) at (4.25,1.25) {\tiny{$v_{2,3}\,\, $ }};
    \node [current] (33) at (3.75,-0.25) {\tiny{$v_{3,3}\,\, $ }};
    \node [madj] (43) at (4,-1.75) {\tiny{$v_{4,3}\,\, $ }};
    
    
    \node [mystyle] (14) at (6,3) {\tiny{$v_{1,4}\,\, $ }};
    \node [mystyle] (24) at (6.25,1.5) {\tiny{$v_{2,4}\,\, $ }};
    \node [madj] (34) at (5.75,-0) {\tiny{$v_{3,4}\,\, $ }};
    \node [mystyle] (44) at (6,-1.5) {\tiny{$v_{4,4}\,\, $ }};
    
    \begin{scope}[on background layer]
    {
    \draw[-] 
        (11)--(12)
        (12)--(13)
        (13)--(14)
        (11)--(13)
        (11)--(14)
        (12)--(14)
        
        (21)--(22)
        (22)--(23)
        (23)--(24)
        (21)--(23)
        (21)--(24)
        (22)--(24)
        
        (31)--(32)
        (32)--(33)
        (33)--(34)
        (31)--(33)
        (31)--(34)
        (32)--(34)
        
        (41)--(42)
        (42)--(43)
        (43)--(44)
        (41)--(43)
        (41)--(44)
        (42)--(44)
        
        
        (11)--(21)
        (21)--(31)
        (31)--(41)
        (11)--(31)
        (11)--(41)
        (21)--(41)
        
        (12)--(22)
        (22)--(32)
        (32)--(42)
        (12)--(32)
        (12)--(42)
        (22)--(42)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(33)
        (13)--(43)
        (23)--(43)
        
        (14)--(24)
        (24)--(34)
        (34)--(44)
        (14)--(34)
        (14)--(44)
        (24)--(44)
        ;
        }
    \node [comp] (33comp) at (3.75,-0.25) {};
    \end{scope}
    \end{tikzpicture}
    \caption{$i=4,\alpha(i)=v_{3,3}$}
    \label{fig:RookMadjDemo1}   
  \end{subfigure}
  \hspace{1.15em}
  \begin{subfigure}[b]{0.25\textwidth}
  \begin{tikzpicture}[scale=0.5,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
    \node [elim] (11) at (0,3) {\tiny{$v_{1,1}\,\, $ }};
    \node [elim] (21) at (0.25,1.5) {\tiny{$v_{2,1}\,\, $ }};
    \node [madj] (31) at (-0.25,0) {\tiny{$v_{3,1}\,\, $ }};
    \node [madj] (41) at (0,-1.5) {\tiny{$v_{4,1}\,\, $ }};
    
    
    \node [elim] (12) at (2,3.25) {\tiny{$v_{1,2}\,\, $ }};
    \node [madj] (22) at (2.25,1.75) {\tiny{$v_{2,2}\,\, $ }};
    \node [madj] (32) at (1.75,0.25) {\tiny{$v_{3,2}\,\, $ }};
    \node [madj] (42) at (2,-1.25) {\tiny{$v_{4,2}\,\, $ }};
    
    
    \node [madj] (13) at (4,2.75) {\tiny{$v_{1,3}\,\, $ }};
    \node [current] (23) at (4.25,1.25) {\tiny{$v_{2,3}\,\, $ }};
    \node [madj] (33) at (3.75,-0.25) {\tiny{$v_{3,3}\,\, $ }};
    \node [madj] (43) at (4,-1.75) {\tiny{$v_{4,3}\,\, $ }};
    
    
    \node [madj] (14) at (6,3) {\tiny{$v_{1,4}\,\, $ }};
    \node [madj] (24) at (6.25,1.5) {\tiny{$v_{2,4}\,\, $ }};
    \node [mystyle] (34) at (5.75,-0) {\tiny{$v_{3,4}\,\, $ }};
    \node [mystyle] (44) at (6,-1.5) {\tiny{$v_{4,4}\,\, $ }};
    
    \begin{scope}[on background layer]
    {
    \draw[-] 
        (11)--(12)
        (12)--(13)
        (13)--(14)
        (11)--(13)
        (11)--(14)
        (12)--(14)
        
        (21)--(22)
        (22)--(23)
        (23)--(24)
        (21)--(23)
        (21)--(24)
        (22)--(24)
        
        (31)--(32)
        (32)--(33)
        (33)--(34)
        (31)--(33)
        (31)--(34)
        (32)--(34)
        
        (41)--(42)
        (42)--(43)
        (43)--(44)
        (41)--(43)
        (41)--(44)
        (42)--(44)
        
        
        (11)--(21)
        (21)--(31)
        (31)--(41)
        (11)--(31)
        (11)--(41)
        (21)--(41)
        
        (12)--(22)
        (22)--(32)
        (32)--(42)
        (12)--(32)
        (12)--(42)
        (22)--(42)
        
        (13)--(23)
        (23)--(33)
        (33)--(43)
        (13)--(33)
        (13)--(43)
        (23)--(43)
        
        (14)--(24)
        (24)--(34)
        (34)--(44)
        (14)--(34)
        (14)--(44)
        (24)--(44)
        ;
        }
        \node [comp] (11comp) at (0,3) {};
        \node [comp] (21comp) at (0.25,1.5) {};
        \node [comp] (12comp) at (2,3.25) {};
        \node [comp] (23comp) at (4.25,1.25) {};

    \end{scope}
    
    \end{tikzpicture}
    \caption{$i=4,\alpha(i)=v_{2,3}$}
    \label{fig:RookMadjDemo2}   
  \end{subfigure}
  \hspace{1.15em}
  \caption{
  The $K_4\square K_4$ rook's graph $G$ and an elimination ordering $\alpha$ over $G$.
  Given the steps $i\in\{1,\dots,|V|\}$, the vertex $\alpha(i)$ is drawn with a thick border. The vertices from $\alpha[1,i]$ are drawn in red, $V_{\textit{comp}_\alpha(i)}$ are highlighted with a yellow circle around them and the vertices of $\textit{madj}^+_\alpha(\alpha(i))$ are drawn in green.
  (a) depicts step 3 where $\alpha(3)=v_{1,2}$ and 
  $\alpha[1,2]= \{v_{1,1}, v_{2,1}\}$.
  (b) and (c) depict 2 different cases at step 4.
  In (b) we have $\alpha(4)=v_{3,3}$ and $\alpha(4)=v_{2,3}$ in (c).
  }
  \label{fig:RookMadjDemo}
\end{figure}
}
Let $\alpha$ be an elimination ordering over the $m\times n$ rook's graph $G$.
We begin by proving that $\textit{madj}^+_\alpha(\alpha(i))=
N_G(V_{\textit{comp}_\alpha(i)})$ for every step $i\in\{1,\dots,|V|\}$.
To do so, fix a step $i^* \in \{1, \dots, |V|\}$ and let $\alpha(i^*)=v_{r^*c^*}$, for some $r^*\in \{1,\dots,m\}$ and $c^*\in \{1,\dots,n\}$.

By definition, $N_G(\alpha(i^*))\setminus \alpha[1,i^*]$ is a subset of
$\textit{madj}^+_\alpha(\alpha(i^*))$.
So let us consider the neighbourhood of every vertex $u\in (V_{\textit{comp}_\alpha(i^*)}\setminus \{\alpha(i^*)\})$.
By definition $V_{\textit{comp}_\alpha(i^*)} \subseteq \alpha[1,i^*]$ so
$V_{\textit{comp}_\alpha(i^*)}\setminus \{\alpha(i^*)\}
\subseteq \alpha[1,i^*-1]$, i.e.,\ every vertex $u\in (V_{\textit{comp}_\alpha(i^*)}\setminus \{\alpha(i^*)\})$ is eliminated before $\alpha(i^*)$.
For every vertex $u\in V_{\textit{comp}_\alpha(i^*)}\setminus \{\alpha(i^*)\}$ there exists an $\alpha(i^*),u$-path in $G$ where all the internal vertices belong to $V_{\textit{comp}_\alpha(i^*)}\setminus \{\alpha(i^*)\}$.
This is due to the fact that $\textit{comp}_\alpha(i^*)$ is connected by definition.
Then by \cref{thm:madjLowerInbetween}, for every vertex $w\in N_G(u)$ s.t.\ $\alpha^{-1}(w)>i^*$ we have that $w\in \textit{madj}^+_\alpha(\alpha(i^*))$.
Since $\textit{comp}_\alpha(i^*)$ is the connected component of $G[\alpha[1,i^*]]$ containing $\alpha(i^*)$ we can state the following for every vertex $u\in V_{\textit{comp}_\alpha(i^*)}\setminus \{\alpha(i^*)\}$:
$$
N_G(u)\setminus \alpha[1,i^*]=
N_G(u)\setminus V_{\textit{comp}_\alpha(i^*)}
\subseteq 
\textit{madj}^+_\alpha(\alpha(i^*))
$$

This combined with the fact that 
$(N_G(\alpha(i^*))\setminus V_{\textit{comp}_\alpha(i^*)})\subseteq 
\textit{madj}^+_\alpha(\alpha(i^*))$ implies that 
$\textit{madj}^+_\alpha(\alpha(i^*))=
N_G(V_{\textit{comp}_\alpha(i^*)})$ as desired.
Note that $\textit{madj}^+_\alpha(\alpha(i^*))\not\supset N_G(V_{\textit{comp}_\alpha(i^*)})$ as this will imply (by \cref{thm:madjLowerInbetween}) that there exists a vertex $w'\notin V_{\textit{comp}_\alpha(i^*)}$ for which there exists a $w',\alpha(i^*)$-path in $G$ with all the internal vertices in $V_{\textit{comp}_\alpha(i^*)}$.
Thus showing that $w'$ belongs to $N_G(u')\setminus \alpha[1,i^*]$ for some $u\in V_{\textit{comp}_\alpha(i^*)}$ which is already covered above.
See \cref{fig:RookMadjDemo} for a demonstration.

Now let us describe $N_G(V_{\textit{comp}_\alpha(i^*)})$.
For a vertex $v_{r,c}\in V_{\textit{comp}_\alpha(i^*)}$, $N_G(v_{r,c})\setminus V_{\textit{comp}_\alpha(i^*)}$ contains every vertex from row $r$ or column $c$ that is not contained in $\alpha[1,i^*]$.
Formally, for every $v_{r,c}\in V_{\textit{comp}_\alpha(i^*)}$:
$$ 
N_G(v_{r,c})\setminus V_{\textit{comp}_\alpha(i^*)}=
% \{u|u\in N_G(v_{r,c}),u\notin V_{\textit{comp}_\alpha(i^*)}\}=
\{w|w\in M_r \textit{ or } w\in L_c\}\setminus\alpha[1,i^*] 
$$

Since 
$\textit{madj}^+_\alpha(\alpha(i^*))=
N_G(V_{\textit{comp}_\alpha(i^*)})$ and $\mathcal{L}_\alpha(i^*),\mathcal{M}_\alpha(i^*)$ are respectively the set of column and row indices spanned by $V_{\textit{comp}_\alpha(i^*)}$ we get that:
$$
\textit{madj}^+_\alpha(\alpha(i^*))=
\{v_{r,c}|c\in \mathcal{L}_\alpha(i^*) 
\textit{ \,or\, } r\in \mathcal{M}_\alpha(i^*)\}
\setminus \alpha[1,i^*]
$$

The lemma thus follows.
\end{proof}

We have provided \cref{fig:RookMadjDemo} as a demonstration for \cref{rmk:madjRooks}.
The figure shows the $K_4\square K_4$ graph $G$ and an elimination ordering $\alpha$ over $G$ where $\alpha[1,2]=\{v_{1,1}, v_{2,1}\}$.
\cref{fig:RookMadjDemo0} shows step 3 where $\alpha(3)=v_{1,2}$ and it is easy to verify that $V_{\textit{comp}_\alpha(3)}=\{v_{1,1},v_{2,1},v_{1,2}\}$.
Therefore 
$\textit{madj}^+_\alpha(\alpha(3))=
\{v_{r,c}\ |\ c\in \{1,2\} \textit{ or } r\in \{1,2\}\}\setminus\alpha[1,3]$.
In step 4, we consider 2 cases.
In \cref{fig:RookMadjDemo1} we let $\alpha(4)=v_{3,3}$. 
Since for any vertex $v\in \alpha[1,3]$ there is no $\alpha(4),v$-path in $G$ containing only vertices from $\alpha[1,3]$, we have 
$V_{\textit{comp}_\alpha(4)}=\{v_{3,3}\}$ and as a result $\textit{madj}^+_\alpha(\alpha(4))=
\{v_{r,c}\ |\ c=3 \textit{ or } r=3\} \setminus\alpha[1,3]$.
In \cref{fig:RookMadjDemo2} we let $\alpha(4)=v_{2,3}$.
Note that $v_{2,3},v_{2,1}\in E$ and more generally there exists a $\alpha(4),v$-path in $G$ containing only vertices from $\alpha[1,4]$ for every one of these vertices $v\in \{v_{1,1},v_{1,2},v_{2,1}\}$.
Consequently 
$V_{\textit{comp}_\alpha(4)}=
\alpha[1,4]=
\{v_{1,1},v_{1,2},v_{2,1},v_{2,3}\}$ and so 
$\textit{madj}^+_\alpha(\alpha(4))=
\{v_{r,c}\ | \ c\in \{1,2,3\} \textit{ or } r\in \{1,2\}\}
\setminus\alpha[1,4]$.

As a corollary to \cref{rmk:madjRooks} we have the following:

\begin{corollary}\label{cor:madjRooks}
Let $G=(V,E)$ be a $K_m\square K_n$ for $n,m\geq 2$ and $\alpha$ an elimination ordering over $G$.
For a step $i\in \{1,\dots,|V|\}$ of the elimination ordering $\alpha$ we have

$$|\textit{madj}^+_\alpha(\alpha(i))|=
nm-(m-|\mathcal{M}_\alpha(i)|)(n-|\mathcal{L}_\alpha(i)|)-|V_{\textit{comp}_\alpha(i)}|$$
\end{corollary}

\begin{proof}
Fix a step $i^*\in\{1,\dots,|V|\}$.
By \cref{rmk:madjRooks}, the set of vertices in $V$ that are not contained in  $\textit{madj}^+_\alpha(\alpha(i^*))$ is $V_{\textit{comp}_\alpha(i^*)}$ 
as well as every vertex from 
$\bigcup_{r\in (\{1,\dots,m\}\setminus \mathcal{M}_\alpha(i^*))} M_r$ or
$\bigcup_{c\in (\{1,\dots,n\}\setminus \mathcal{L}_\alpha(i^*))} L_c$.
This proves the statement of the corollary.
\end{proof}
}

% 2xn rook
{

First, let us discuss the $\tau$ parameter for $K_2\square K_n$ graphs, for $n\geq 2$.

\begin{lemma}\label{lem:2Rooktau}
Let $G$ be a $K_2\square K_n$ for $n\geq 2$.
Then $\tau(G)=0$.
\end{lemma}
\begin{proof}
Let $G$ be a $K_2\square K_n$ for $n\geq 2$.
By \cref{lem:twRook} we have that $\textit{tw}(G)=n$.
It is easy to see that $\kappa(G)=n$.
Since $G$ has treewidth and vertex connectivity of $n$, we know from \cref{lem:tw=kConnected} that there exists a minimum triangulation $H$ of $G$ with $\textit{tw}(H)=\textit{tw}(G)$.
This concludes that $\tau(G)=0$ as desired.
\end{proof}
}

% 2xn rook mfi
{

The minimum fill-in of a graph $G=K_m\square K_n$ for $n\geq 2$ is easy to determine considering that its complement only contains cycles with 5 or more vertices. 
As a result $G$ contains ${n(n-1)}/{2}$ cycles with 4 vertices that pairwise share an edge thus requiring ${n(n-1)}/{2}$ edges to triangulate.
In order to showcase the application of \cref{cor:mfiKConnectedTreewidthK}, we have proved it differently below:

\begin{corollary}
Let $G$ be a $K_2\square K_n$ graph for $n\geq 2$.
Then $\textit{mfi}(G)= \frac{n(n-1)}{2}$.
\end{corollary}

\begin{proof}
Let $G=(V,E)$ be a $K_2\square K_n$ for $n\geq 2$.
It is easy to verify that $|V|=2n$ and $|E|= n^2$.
As discussed in the proof of \cref{lem:2Rooktau}, $\textit{tw}(G)=\kappa(G)=n$.
Then by \cref{cor:mfiKConnectedTreewidthK} the number of edges in every minimum triangulation of $G$ is: $n(|V|-n)+\frac{n(n-1)}{2}$.
% 2n^2/2+(n^2-n)/2
% (2n^2-n^2-n)/2
% (n^2-n)/2
% Below we first define an elimination ordering $\alpha$ over $G$ and then show that
% $|E_{G^+_\alpha}|=n(|V|-n)+\frac{n(n-1)}{2}$. 
% Using $\alpha$ we determine the value of $\textit{mfi}(G)$.
% Let $\alpha$ eliminate the vertices $v_{1,1},\dots,v_{1,n-1}$ in this order during steps $i\in\{1,\dots,n-1\}$.
% It is simple to verify that $|\textit{madj}^+_\alpha(\alpha(i))|=n$ for every step $i\in\{1,\dots,n-1\}$ and that
% the resulting graph $G_{n-1}$ is a $K_{n+1}$.
% So in the remaining steps we let $\alpha$ be any elimination ordering over $G_{n-1}$.
% By construction we have that $\sum_{v\in V}|\textit{madj}^+_\alpha(v)|= n(|V|-n)+\frac{n(n-1)}{2}$ proving that $G^+_\alpha$ is a minimum triangulation of $G$.
As a result, we can conclude by stating that:
$$ \textit{mfi}(G)= n(|V|-n)+\frac{n(n-1)}{2} - |E| = \frac{n(n-1)}{2} $$
\end{proof}
}

% 3xn rook helper
{
The following lemma describes a property of minimum elimination ordering over the $K_3\square K_n$ graphs for $n\geq 3$. 

\begin{lemma}\label{lem:elimn3Rook}
Let $G=(V,E)$ be a $K_3\square K_n$ for $n\geq 3$.
There exists a minimum elimination ordering $\gamma$ over $G$ s.t.\ both of the following conditions hold for the set of vertices $\gamma[1,n]$:
\begin{enumerate}
    \item[(1)] For every $c\in\{1,\dots,n\}$, $|L_c\cap \gamma[1,n]|=1$.
    \item[(2)] For every $r\in\{1,2,3\}$, $|M_r\cap \gamma[1,n]|\leq \ceil{\frac{n}{3}}$.
\end{enumerate}
\end{lemma}
% \todo{\textbf{TODO}: Can the proof be extended to any m?}

\begin{proof}
% part (1)
{
Let $\alpha$ be any fixed minimum elimination ordering over $G$. By \cref{lem:niceElim} we can fix a nice minimum elimination ordering $\alpha^*$ over $G$ s.t.\ $G^+_{\alpha^*}=G^+_{\alpha}$.
If for $\alpha[1,n]$ or $\alpha^*[1,n]$ both of the conditions (1) and (2) are true, the lemma is clearly valid. 
Otherwise, we show that $\alpha^*$ can be transformed to another minimum elimination ordering where both properties (1) and (2) are valid.

By \cref{def:niceElim}, for every step $i\in\{|V|-\textit{tw}(G^+_{\alpha^*}),\dots,|V|\}$ we have
% tw= 5
% i:|V|-5 … |V|, \alpha(i) is universal
% \alpha(|V|-5) is eliminated from G_{|V|-6} that has 6 vertices
% so madj is 5
$|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=|V|-i$.
$\textit{tw}(G)=2n-1$ (by \cref{lem:twRook}) therefore $\textit{tw}(G^+_{\alpha^*})\geq 2n-1$ thus showing that $|V|-\textit{tw}(G^+_{\alpha^*})\leq n+1$.
% 3n - (2n-1+c) = n+1-c
% from step n+1 onwards every vertex simplicial
% at n+1 we eliminate from G_{n}, 2n left, so 2n-1
% (2n-1)n
This implies the following statement:
\begin{equation}\label{eq:elimn3Rook:1}
    \sum\nolimits_{v\in\alpha^*[n+1,|V|]}
    |\textit{madj}^+_{\alpha^*}(v)|
    =n(2n-1)
\end{equation}

Based on $\alpha^*$, we first define an elimination ordering $\beta$ over $G$ where $\beta[1,n]$ meets condition (1).
We then show that $\sum_{v\in V}|\textit{madj}^+_\beta(v)|\leq
\sum_{v\in V}|\textit{madj}^+_{\alpha^*}(v)|$ thus proving that $\beta$ is a minimum elimination ordering over $G$.

Begin by letting $\beta(1)={\alpha^*}(1)$.
For every following step $i\in\{2,\dots,n\}$, let $v_{r',c'}={\alpha^*}(i)$ for some $c'\in\{1,\dots,n\}$, $r'\in\{1,2,3\}$ and define $\beta(i)$ depending on which one of the following cases is true:
\begin{mycases}
    \case 
    {
    Suppose that ${\alpha^*}(i)$ is not on the same column as any of the vertices from $\beta[1,i-1]$.
    Formally $L_{c'}\cap \beta[1,i-1]=\emptyset$.
    Then in this case, let $\beta(i)={\alpha^*}(i)$.
    }
    
    \case 
    {
    Suppose that ${\alpha^*}(i)$ is on the same column as a vertex from $\beta[1,i-1]$.
    Formally $L_{c'}\cap \beta[1,i-1]=\{v_{r,c'}\}$ for some row index $r\in\mathcal{R}= \{1,2,3\}\setminus\{r'\}$.
    Since $L_{c'}$ contains at least 2 vertices from ${\alpha^*}[1,i]$, there exists some column index $c^*\in\{1,\dots,n\}$ s.t.\ $L_{c^*}\cap {\alpha^*}[1,n]=\emptyset$ and $c^*\notin \mathcal{C}$ where $\mathcal{C}$ is a set of such column indices selected so far in $\beta$.
    Then in this case add $c^*$ to $\mathcal{C}$ and let $\beta(i)=v_{r',c^*}$.
    }
\end{mycases}

In the remaining steps $i\in\{n+1,\dots,|V|\}$ we let $\beta$ be any elimination ordering over the graph $G^\beta_{n}$.
By \cref{eq:elimn3Rook:1} and the fact that $G^{\alpha^*}_n$ is a clique, regardless of how the vertices of $G^\beta_{n}$ are eliminated by $\beta$ during the steps $i\in\{n+1,\dots,|V|\}$ we can state that:

\begin{equation}\label{eq:elimn3Rook:2}
    \sum\nolimits_{v\in\beta[n+1,|V|]}|\textit{madj}^+_\beta(v)|\leq
    \sum\nolimits_{v\in{\alpha^*}[n+1,|V|]}|\textit{madj}^+_{\alpha^*}(v)|
    = n(2n-1)
\end{equation}

Next we prove that 
$\sum_{v\in \beta[1,n]}|\textit{madj}^+_\beta(v)|\leq
\sum_{v\in {\alpha^*}[1,n]}|\textit{madj}^+_{\alpha^*}(v)|$.
Obviously we have that
$|\textit{madj}^+_\beta(\beta(1))|=
|\textit{madj}^+_{\alpha^*}({\alpha^*}(1))|$ as $\beta(1)={\alpha^*}(1)$.
Therefore, let us show that $|\textit{madj}^+_\beta(\beta(i))|\leq |\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|$ for every other step $i\in\{2,\dots,n\}$.
Let $M_{r'}$, $r'\in \{1,2,3\}$, be the row containing the vertex $\alpha(i)$ as well as $\beta$.
This is due to the fact that $\beta(i)$, following our construction, is selected from a different column but belongs to the same row as $\alpha(i)$.

By construction $\beta[1,i]$ satisfies condition (1) stated in the lemma, 
then for every column index $c\in \{1,\dots,n\}$ with the vertex $v_{r',c}\in V_{\textit{comp}_\beta(i)}$ we have $L_c\cap \beta[1,i]=\{v_{r',c}\}$ (as no two eliminated vertices share the same column).
Consequently, $\textit{comp}_\beta(i)$ cannot contain vertices from any other row 
$r\in \{1,2,3\}\setminus\{r'\}$.
So $V_{\textit{comp}_\beta(i)}$ can only contain the vertices $M_{r'}\cap \beta[1,i]$.
Note that the condition (1) is not necessarily true for ${\alpha^*}[1,i]$.
Then there may exist a vertex $v_{r',c}\in V_{\textit{comp}_{\alpha^*}(i)}$
s.t.\ $\{v_{r',c},v_{r,c}\}\subseteq L_c\cap {\alpha^*}[1,i]$ for some row $r\in \mathcal{R}$ (where $\mathcal{R}=\{1,2,3\}\setminus\{r'\}$).
In this case, $\{r,r'\}\subseteq \mathcal{M}_{\alpha^*}(i)$ and we can generally state that $M_{r'}\cap {\alpha^*}[1,i]\subseteq 
V_{\textit{comp}_{\alpha^*}(i)}$.
To summarize:

\begin{equation}\label{eq:rowsAlphavsRowsBeta}
    \{r'\}=\mathcal{M}_\beta(i)\subseteq \mathcal{M}_{\alpha^*}(i)
\end{equation}

By our construction, for every vertex $v_{r',c}\in (M_{r'}\cap {\alpha^*}[1,i])$ either
$v_{r',c}\in (M_{r'}\cap \beta[1,i])$ or it can be mapped one to one, to a vertex 
$v_{r',c^*}\in (M_{r'}\cap \beta[1,i])$.
This means that ${\alpha^*}$ and $\beta$ eliminate the same number of vertices from row $r'$ during the steps 1 to $i$.
Since $M_{r'}$ is a clique in $G$, 
$(M_{r'}\cap \alpha^*[1,i])\subseteq V_{\textit{comp}_{\alpha^*}(i)}$ and for the same reason $(M_{r'}\cap \beta[1,i])\subseteq V_{\textit{comp}_{\beta}(i)}$.
Because $\beta[1,n]$ satisfies condition (1) we have that:
$(M_{r'}\cap \beta[1,i])= V_{\textit{comp}_{\beta}(i)}$ thus showing that:
$$\{c| v_{r',c}\in M_{r'}\cap \beta[1,i]\}= 
\{c| v_{r',c}\in V_{\textit{comp}_{\beta}(i)}\}=
\mathcal{L}_\beta(i)$$

However, as this condition is not necessarily satisfied for $\alpha^*[1,n]$, we would have that:
$$\{c| v_{r',c}\in M_{r'}\cap {\alpha^*}[1,i]\}\subseteq 
\{c| v_{r,c}\in V_{\textit{comp}_{\alpha^*}(i)}\} =
\mathcal{L}_{\alpha^*}(i)$$

As a consequence, we have that the number of columns spanned by $\textit{comp}_\beta(i)$ cannot exceed that of $\textit{comp}_{\alpha^*}(i)$.
In short:
\begin{equation}\label{eq:colsAlphavsBeta}
|\mathcal{L}_\beta(i)|=
|\{c|c\in \{1,\dots,n\}, v_{r',c}\in V_{comp_\beta(i)}\}| \leq
|\mathcal{L}_{\alpha^*}(i)|
\end{equation}

Using \cref{rmk:madjRooks} we outline  $\textit{madj}^+_\beta(\beta(i))$ and $\textit{madj}^+_{\alpha^*}({\alpha^*}(i))$ in the following equations:
\begin{equation}\label{eq:madjAlpha}
    \textit{madj}^+_{\alpha^*}({\alpha^*}(i))=
    \{v_{r,c}|v_{r,c}\in V, c\in \mathcal{L}_{\alpha^*}(i) \textit{ or }
    r\in \mathcal{M}_{\alpha^*}(i)\}
    \setminus{\alpha^*}[1,i]
\end{equation}

Since $\mathcal{M}_\beta(i)=\{r'\}$ by \cref{eq:rowsAlphavsRowsBeta} we have:
\begin{equation}\label{eq:madjBeta}
    \textit{madj}^+_\beta(\beta(i))=
    \{v_{r,c}|v_{r,c}\in V, c\in \mathcal{L}_\beta(i) \textit{ or }
    r=r'\}
    \setminus\beta[1,i]
\end{equation}
    
As noted before, the set ${\alpha^*}[1,i]$ and $\beta[1,i]$ contain the same number of vertices in $M_{r'}$ (that is a clique in $G$).
Then by \cref{eq:madjAlpha} and \cref{eq:madjBeta} we have
$|M_{r'}\cap  \textit{madj}^+_{\alpha^*}({\alpha^*}(i))| = |M_{r'}\cap  \textit{madj}^+_\beta(\beta(i))|$.
Consequently, in order to show that 
$|\textit{madj}^+_\beta(\beta(i))|\leq |\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|$, it suffices to compare the number of vertices $\textit{madj}^+_\beta(\beta(i))$ and $\textit{madj}^+_{\alpha^*}({\alpha^*}(i))$ have in $\bigcup_{r\in \mathcal{R}}M_r$ (where $\mathcal{R}=\{1,2,3\}\setminus\{r'\}$).
Formally, we need to prove that
$ 
|\bigcup\nolimits_{r\in \mathcal{R}}M_r \cap \textit{madj}^+_\beta(\beta(i))|\leq 
|\bigcup\nolimits_{r\in \mathcal{R}}M_r \cap \textit{madj}^+_{\alpha^*}({\alpha^*}(i))|
$.
By \cref{eq:madjBeta} and the fact that $V_{\textit{comp}_\beta(i)}=
M_{r'}\cap \beta[1,i]$ we have:
$$\bigcup\nolimits_{r\in \mathcal{R}}M_r \cap \textit{madj}^+_\beta(\beta(i))=
\{v_{r,c}| r\in \mathcal{R}\, \textit{ and } \, c\in \mathcal{L}_\beta(i)\}$$

% \todo[inline]{
% This is not clear…following \cref{eq:madjBeta} also a vertex $v_{r',c}$ where $c\notin \mathcal{L}_\beta(i)$ belongs to $\textit{madj}^+_\beta(\beta(i))$. Is it true also here?
% }
% \unsure[inline]
% {
% It is true by \cref{eq:madjBeta} that $v_{r',c}\in \textit{madj}^+_\beta(\beta(i))$ where $c\notin \mathcal{L}_\beta(i)$.
% This is because $v_{r',c}$ is from row $r'$ same row as $\alpha(i)=v_{r',c'}$.
% But in the above equation I am focusing on $\textit{madj}^+_\beta(\beta(i))$ in the rows $\mathcal{R}$ which does not contain $r'$.
% So not sure what your comment is here.\\

% I have mentioned in the above para that
% $|M_{r'}\cap  \textit{madj}^+_{\alpha^*}({\alpha^*}(i))| = 
% |M_{r'}\cap  \textit{madj}^+_\beta(\beta(i))|$
% i.e.,\ higher adjacency of $\beta(i)$ and $\alpha^*(i)$ in row $M_{r'}$ is the same, so let us only focus on rows $\mathcal{R}$.
% So we take \cref{eq:madjBeta} and ignore the ``or $r=r'$'' condition.
% This tells us that higher adjacency of $\beta(i)$ in rows $\mathcal{R}$ is: 
% $\{v_{r,c}| r\in \mathcal{R}, c\in \mathcal{L}_\beta(i)\}$
% which is the exact same equation above.
% }
% \todo[inline]{OK, this is correct -- my confusion was due to the notation, I supposed that $\mathcal{R}=\{1, 2, 3\}$…the notation should be easy…}

Then for every $c\in \mathcal{L}_\beta(i)$, $|L_c\cap \textit{madj}^+_\beta(\beta(i))|=2$ and so:
\begin{equation}\label{eq:sum2RowsBeta}
    |\bigcup\nolimits_{r\in \mathcal{R}}M_r \cap \textit{madj}^+_\beta(\beta(i))|
    =2|\mathcal{L}_\beta(i)|
\end{equation}

In order to show 
$
|\bigcup\nolimits_{r\in \mathcal{R}}M_r \cap \textit{madj}^+_\beta(\beta(i))|
\leq 
|\bigcup\nolimits_{r\in \mathcal{R}}M_r \cap \textit{madj}^+_{\alpha^*}({\alpha^*}(i))|
$ we first prove the following statement:
\begin{equation}\label{eq:sum2RowsAlpha}
    |\bigcup\nolimits_{r\in \mathcal{R}}M_r \cap \textit{madj}^+_{\alpha^*}({\alpha^*}(i))|
    \geq 2|\{c|c\in \{1,\dots,n\}, v_{r',c}\in V_{\textit{comp}_{\alpha^*}(i)}\}|
\end{equation}

For every column index $c$ such that $v_{r',c}\in V_{\textit{comp}_{\alpha^*}(i)}$ one of the following cases must be true.
We show in each case that there exist 2 distinct vertices from 
$\bigcup\nolimits_{r\in \mathcal{R}}M_r \cap \textit{madj}^+_{\alpha^*}({\alpha^*}(i))$ that correspond to  the column index $c$.

\begin{mycases}
    \case
    {
    Suppose that $|L_c\cap{\alpha^*}[1,i]|=1$, then we must have $L_c\cap{\alpha^*}[1,i]=\{v_{r',c}\}$.
    Since $v_{r',c}\in 
    V_{\textit{comp}_{\alpha^*}(i)}$ we have $c\in \mathcal{L}_{\alpha^*}(i)$ and as a result for both row indices $r\in\mathcal{R}$ we have $v_{r,c}\in \textit{madj}^+_{\alpha^*}({\alpha^*}(i))$ by \cref{rmk:madjRooks}.
    }
    
    \case
    {
    Suppose that $|L_c\cap{\alpha^*}[1,i]|=2$, then let $L_c\cap{\alpha^*}[1,i]=\{v_{r',c},v_{r'',c}\}$ for some $r''\in \mathcal{R}$.
    Since $v_{r',c}\in V_{\textit{comp}_{\alpha^*}(i)}$ we have $c\in \mathcal{L}_{\alpha^*}(i)$.
    Then by \cref{rmk:madjRooks}, $v_{r,c}\in \textit{madj}^+_{\alpha^*}({\alpha^*}(i))$ where $\{r\}=\mathcal{R}\setminus\{r''\}$.
    $v_{r,c}$ is one of the 2 vertices in $\textit{madj}^+_{\alpha^*}({\alpha^*}(i))$ corresponding to column index $c$.
    
    Since $i\leq n$ and $L_c$ contains two vertices from ${\alpha^*}[1,i]$ we can fix a column index $c^*\in \{1,\dots,n\}\setminus\{c\}$ corresponding to $c$ s.t.\ $L_{c^*}\cap {\alpha^*}[1,i]=\emptyset$ and $c^*\notin \mathcal{C}$, where the set $\mathcal C$ contains the indices of  already selected columns $c^*$.
    As $v_{r'',c}\in {\alpha^*}[1,i]$, we have that $r''\in \mathcal{M}_{\alpha^*}(i)$ and so $v_{r'',c^*}\in \textit{madj}^+_{\alpha^*}({\alpha^*}(i))$ by \cref{rmk:madjRooks}.
    To summarize, $v_{r'',c^*},v_{r,c}\in \textit{madj}^+_{\alpha^*}({\alpha^*}(i))$ correspond to column $c$.
    }
    
    \case
    {
    Suppose that $|L_c\cap{\alpha^*}[1,i]|=3$, i.e.,\ $L_c\subseteq {\alpha^*}[1,i]$.
    Since $L_c$ has all 3 vertices in ${\alpha^*}[1,i]$, same as the previous case, we can fix a column $c^*\in \{1,\dots,n\}$ corresponding to $c$ s.t.\ $L_{c^*}\cap {\alpha^*}[1,i]=\emptyset$ and $c^*\notin \mathcal{C}$ where the set $\mathcal C$ contains the indices of  already selected columns $c^*$ (this includes the ones selected in the previous case).
    Then similarly, we have $v_{r,c^*}\in \textit{madj}^+_{\alpha^*}({\alpha^*}(i))$, for both row indices $r\in\mathcal{R}$, corresponding to column $c$.
    }
\end{mycases}

This proves \cref{eq:sum2RowsAlpha} as desired. 

Note that 
$\{c|c\in \{1,\dots,n\}, v_{r',c}\in V_{\textit{comp}_{\alpha^*}(i)}\}
\subseteq \mathcal{L}_{\alpha^*}(i)$ as a result we have that 
$|\bigcup\nolimits_{r\in \mathcal{R}}M_r \cap \textit{madj}^+_{\alpha^*}({\alpha^*}(i))| \geq 2|\mathcal{L}_{\alpha^*}(i)|$.
We know from \cref{eq:colsAlphavsBeta} that $|\mathcal{L}_\beta(i)|\leq |\mathcal{L}_{\alpha^*}(i)|$ then by \cref{eq:sum2RowsBeta} we can conclude that:

$$
|\bigcup\nolimits_{r\in \mathcal{R}}M_r \cap \textit{madj}^+_{\alpha^*}({\alpha^*}(i))|\geq |\bigcup\nolimits_{r\in \mathcal{R}}M_r \cap \textit{madj}^+_\beta(\beta(i))|
$$

Consequently, $|\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|\geq |\textit{madj}^+_\beta(\beta(i))|$.
Since this statement can be proved for any step, we can conclude that 
$\sum_{v\in {\beta}[1,n]}|\textit{madj}^+_{\beta}(v)|\leq 
\sum_{v\in {\alpha^*}[1,n]}|\textit{madj}^+_\beta(v)|$.
This combined with \cref{eq:elimn3Rook:2} implies that 
$\sum_{v\in V}|\textit{madj}^+_\beta(v)|\leq
\sum_{v\in V}|\textit{madj}^+_{\alpha^*}(v)|$ showing that $\beta$ is a minimum elimination ordering over $G$.

}

% part (2)
{
So far we have constructed a minimum elimination ordering $\beta$ over $G$ s.t.\ $\beta[1,n]$ satisfies condition (1) of the lemma.
In the next step of the proof, given $\beta$ we define an elimination ordering $\gamma$ s.t.\ 
$\sum_{v\in \gamma[1,n]}|\textit{madj}^+_\gamma(v)|\leq 
\sum_{v\in \beta[1,n]}|\textit{madj}^+_\beta(v)|$ and $\gamma[1,n]$ meets both conditions (1) and (2).

For each row index $r\in\{1,2,3\}$ let $k_\beta(r)$ be the number of vertices $\beta$ eliminates from $M_r$ in the first $n$ steps.
Formally, define $k_\beta(r)=|M_r\cap \beta[1,n]|$.
We point out that:
\begin{equation}\label{eq:nsumOfK}
    \sum\nolimits_{r\in \{1,2,3\}}k_\beta(r)=
    \sum\nolimits_{r\in \{1,2,3\}}|M_r\cap \beta[1,n]|=n
\end{equation}

Fix a row index $r^*\in \{1,2,3\}$ and a vertex 
$v\in M_{r^*}\cap\beta[1,n]$.
Assume that $v$ is the $j$-th vertex to be eliminated by $\beta$ from row $r^*$, where $1\leq j \leq k_\beta(r^*)$.
Then since $\beta[1,n]$ meets condition (1), it is easy to see that $\textit{madj}^+_\beta(v)$ contains $(n-j)$ vertices from $M_{r^*}$ and $2j$ vertices in 
$\bigcup_{r\in\{1, 2, 3\}\setminus \{r^*\}} M_r$.
This shows that $|\textit{madj}^+_\beta(v)|=n-j +2j  =n+j$.
Hence, using \cref{eq:nsumOfK} we state that:
\begin{multline}\label{eq:sumBeta}
    \sum_{v\in \beta[1,n]}|\textit{madj}^+_\beta(v)|=
    \sum_{r\in \{1,2,3\}}\sum_{i=1}^{k_\beta(r)}(n+i)=
    n^2 + \sum_{r\in \{1,2,3\}}\sum_{i=1}^{k_\beta(r)}i=\\ 
    n^2 +\frac 12 \sum_{r\in \{1,2,3\}}k_\beta(r)(k_\beta(r)+1)
\end{multline}


Therefore, in order to minimize $\sum_{v\in\beta[1,n]}|\textit{madj}^+_\beta(v)|$, one can solely focus on minimizing $\sum_{r\in \{1,2,3\}}k_\beta(r)(k_\beta(r)+1)$. 

Let $x$, $y$, $z$ be natural numbers. Then it is easy to prove that
$x^2+y^2 +z^2 \geq \frac{(x+y+z)^2}{3}$, where the inequality becomes equality if $x=y=z$. 
Applying this inequality to the previous sum, we get:


% k^2 + k
% sum (k(k+1))
% 1/4 sum (4k(k+1))
% 1/4 sum (4k^2 + 4k)
% 1/4 (-3 + sum (4k^2 + 4k +1))
\begin{equation*}
\sum _{r\in \{1,2,3\}}k_\beta(r)(k_\beta(r)+1) =
\frac14 \bigl(-3+\sum _{r\in \{1,2,3\}}(2 k_\beta(r)+1)^2 \bigr)\geq
\frac 1{12} \bigl( \sum _{r\in \{1,2,3\}}(2k_\beta(r)+1)\bigr)^2 -\frac34 
\end{equation*}
and using \cref{eq:nsumOfK} this can be further simplified to:
% 1/12(sum(2k+1))^2-3/4
% 1/12(3+sum(2k))^2-3/4
% 1/12(3+2sum(k))^2-3/4
% 1/12(3+2n)^2-3/4
% 1/12(9+12n+4n^2)-3/4
% 1/4+n+1/3n^2-3/4
% n+1/3n^2-2/4

\begin{equation}\label{eq:lowbeta}
\sum_{r\in \{1,2,3\}}k_\beta(r)(k_\beta(r)+1)\geq n(\frac n3 +1)
\end{equation}
% 1/12  (sum (2k+1))^2 -3/4
% 1/12  (3 + sum 2k)^2 -3/4
% 1/12  (3 + 2sum k)^2 -3/4
% 1/12  (3 + 2n)^2 -3/4
% 1/12  (9 + 4n^2 + 12n) -3/4
% (1/4 + 3/4 n^2 + n) -3/4
% (1/3 n^2 + n) -3/4+3/4
% n(n/3 + 1)

It is easy to see that in case $n$ is divisible by 3 and $k_\beta(1)=k_\beta(2)=k_\beta(3)=\frac n3$ then  the inequality  \cref{eq:lowbeta} becomes equality. Similarly, in case $n \text{\,mod\,} 3\equiv 1$ or $n \text{\, mod\,} 3\equiv 2$ the sum $\sum_{r\in \{1,2,3\}}k_\beta(r)(k_\beta(r)+1)$ is minimum, if the difference between any
$k_\beta(i)$ and $k_\beta(j)$ is at most 1, where $i, j \in\{1, 2, 3\} $.
Based on this, we can define the elimination ordering $\gamma$ as follows: 
For $i\in\{1,\dots,\floor{\frac{n}{3}}\}$ let $\gamma(i)=v_{1,i}$, for  $i\in\{\floor{\frac{n}{3}}+1, \dots, 2\floor{\frac{n}{3}}+k\}$ let $\gamma(i)=v_{2,i}$, and for $i\in\{2\floor{\frac{n}{3}}+k+1, \dots, n\}$ let $\gamma(i)=v_{3,i}$, where $k=1$ if $n\,\text{mod}\,3 \equiv 2$ and $k=0$ if $n\,\text{mod}\,3 \equiv 1$.
% n=6: 2, 2, 2
% n=7: 2, 2, 3
% n=8: 2, 3, 3
It is easy to verify that the graph $G_n$ obtained at step $n$ of $\gamma$ is a complete graph on $2n$ vertices.
Then let $\gamma$ be any elimination ordering over $G_n$ in the remaining steps.
Note that by our construction $\gamma[1,n]$ meets both conditions (1) and (2) and since $\sum_{v\in \beta[1,n]}|\textit{madj}^+_\beta(v)|\geq 
\sum_{v\in \gamma[1,n]}|\textit{madj}^+_\gamma(v)|$, we have that $\gamma$ is a minimum elimination ordering over $G$ thus the lemma follows.
}
\end{proof}
}

% 3xn rook
{


Below, we prove that $\tau(G)=0$ given a $K_3\square K_n$ graph $G$, for $n\geq 3$.

\begin{lemma}\label{lem:3Rooktau}
Let $G=(V,E)$ be a $K_3\square K_n$ for $n\geq 3$. 
Then $\tau(G)=0$.
\end{lemma}

\begin{proof}
From \cref{lem:twRook} we have that $\textit{tw}(G)=2n-1$.
In order to show that $\tau(G)=0$, 
it suffices to find a minimum triangulation of $G$ with treewidth of $2n-1$.
By \cref{lem:twEliminationHigherAdjacency} this task translates to finding a minimum elimination ordering $\gamma$ over $G$ s.t.\
$\max_{v\in V}|\textit{madj}^+_\gamma(v)|=
\textit{tw}(G^+_\gamma)=2n-1$.

Let $\gamma$ be the minimum elimination ordering defined in the proof of \cref{lem:elimn3Rook}.
Now let us determine $\max_{v\in V}|\textit{madj}^+_\gamma(v)|$.
For every row index $r\in \{1,2,3\}$ let $k_\gamma(r)=|M_r\cap \gamma[1,n]|$ and fix a row index $r^*\in\{1,2,3\}$.
For some $i\in \{1,\dots,k_\gamma(r^*)\}$ let $v_{r^*,c}$ be the $i$-th vertex eliminated from row $r^*$ by $\gamma$ s.t.\ $\gamma^{-1}(v_{r^*,c})\leq n$.
As stated in the proof of \cref{lem:elimn3Rook}, $\textit{madj}^+_\alpha(v_{r^*,c})$ consists of $n-i$ vertices from $M_{r^*}$ and $2i$ vertices from $\bigcup\nolimits_{r\in \{1,2,3\}\setminus\{r^*\}}M_{r}$.
Then $|\textit{madj}^+_\gamma(v_{r^*,c})|=n+i$ and since 
$k_\gamma(r^*)\leq \ceil{\frac{n}{3}}$ we have that 
$\max_{v\in \gamma[1,n]} |\textit{madj}^+_\gamma(v)|= n+\ceil{\frac{n}{3}} <2n-1$.
It is easy to verify that the graph $G_n$ obtained at step $n$ of $\gamma$ is a complete graph on $2n$ vertices. 
Consequently, we get that 
$\max_{v\in V}|\textit{madj}^+_\gamma(v)|=\textit{tw}(G)=2n-1$ proving the statement of the lemma.
\end{proof}
}

% 3xn rook mfi
{
Let $G$ be a $K_3\square K_n$ graph, for $n\geq 3$, and $\gamma$ the minimum elimination ordering over $G$ defined in the proof of \cref{lem:elimn3Rook}.
Before discussing $\textit{mfi}(G)$, let first us evaluate 
$\sum_{i\in\{1,\dots,n\}} |\textit{madj}^+_\gamma(\gamma(i))|$.
By construction 
$\sum_{i\in\{1,\dots,n\}} |\textit{madj}^+_\gamma(\gamma(i))|
=n^2 +\frac 12 \sum_{r\in \{1,2,3\}}k_\gamma(r)(k_\gamma(r)+1)$ where $k_\gamma(r)=|M_r\cap \gamma[1,n]|$ for every row index $r\in\{1,2,3\}$.
Therefore, for every $k\geq 1$ we can state that:
\begin{equation}\label{eq:3rook:mfi:sum1toNGamma}
    \sum_{i\in\{1,\dots,n\}} |\textit{madj}^+_\gamma(\gamma(i))| = 
    \begin{cases}
        % n^2+ 3\sum_{i\in\{1,\dots,\frac{n}{3}\}}
        % & \text{if } n=3k\\
        % (3k)^2+ 3\sum_{i\in\{1,\dots,k\}}
        % & \text{if } n=3k\\
        % (3k)^2+ 3 (k(k+1))/2
        % & \text{if } n=3k\\
        % (3k)^2+ (3k)(k+1)/2
        % & \text{if } n=3k\\
        % (3k)[(3k)+(k+1)/2]
        % & \text{if } n=3k\\
        % (3k)[(6k)/2+(k+1)/2]
        % & \text{if } n=3k\\
        \frac{21k^2+3k}{2}
        & \text{if } n=3k\\
        
        % n^2+ 2\sum_{i\in\{1,\dots,\floor{\frac{n}{3}}\}} + \sum_{i\in\{1,\dots,\ceil{\frac{n}{3}}\}}
        % & \text{if } n=3k+1\\
        % (9k^2+6k+1)+ 
        % (3k^2+5k+2)/2
        % & \text{if } n=3k+1\\
        % (18k^2+6k+1k^2+12k+2)/2+ 
        % (3k^2+5k+2)/2
        % & \text{if } n=3k+1\\
        \frac{21k^2+17k+4}{2}
        & \text{if } n=3k+1\\
        
        % n^2+ \sum_{i\in\{1,\dots,\floor{\frac{n}{3}}\}} + 2\sum_{i\in\{1,\dots,\ceil{\frac{n}{3}}\}}
        % & \text{if } n=3k+2\\
        % (3k+2)^2+ \sum_{i\in\{1,\dots,k\}} + 2\sum_{i\in\{1,\dots,k+1\}}
        % & \text{if } n=3k+2\\
        % 9k^2+12k+4 +
        % k(k+1)/2 + 
        % 2 ((k+2)(k+1)/2)
        % & \text{if } n=3k+2\\
        % 9k^2+12k+4 +
        % k(k+1)/2 + 
        % 2 ((k+2)(k+1)/2)
        % & \text{if } n=3k+2\\
        % 9k^2+12k+4 +
        % (k^2+k+2k^2+2k+4k+4/2)
        % & \text{if } n=3k+2\\
        % 9k^2+12k+4 +
        % (3k^2+7k+4/2)
        % & \text{if } n=3k+2\\
        % 18k^2+24k+8 + 3k^2+7k+4/2
        % & \text{if } n=3k+2\\
        \frac{21k^2+31k+12}{2}
        & \text{if } n=3k+2
    \end{cases}
\end{equation}

Using this, we determine $\textit{mfi}(G)$ in the following corollary:

\begin{corollary}\label{cor:3rookmfi}
Let $G$ be a $K_3\square K_n$ graph for $n\geq 3$.
Then we have: 
\begin{equation*}
    \textit{mfi}(G) = 
    \begin{cases}
        k(15k-6)
        & \text{if } n=3k\\
        
        k(15k+4)
        & \text{if } n=3k+1\\
        
        (5k+3)(3k+1)
        & \text{if } n=3k+2 
    \end{cases}
\end{equation*}
\end{corollary}

\begin{proof}
We will prove the corollary using the minimum elimination ordering $\gamma$ defined in the proof of \cref{lem:elimn3Rook}.
Notice that since $\gamma$ is a minimum elimination ordering, the number of edges that $\gamma$ adds when eliminating the vertices of $G$ is equal to $\textit{mfi}(G)$.

We have previously determined in \cref{eq:3rook:mfi:sum1toNGamma} the value of $\sum_{i\in\{1,\dots,n\}} |\textit{madj}^+_\gamma(\gamma(i))|$ As discussed in the proof of \cref{lem:elimn3Rook}, the graph $G^\gamma_n$ is a complete graph on $2n$ vertices thus
$\sum_{i\in\{n+1,\dots,|V|\}} |\textit{madj}^+_\gamma(\gamma(i))|=
n(2n-1)$.
Obviously $|E_G|= n\frac{3(n+1)}{2}$ therefore we can conclude by stating the following for every $k\geq 1$:

\begin{equation*}
    \sum\nolimits_{i\in\{1,\dots,3n\}}
    |\textit{madj}^+_\gamma(\gamma(i))| -|E_G|= 
    \begin{cases}
        % \frac{21k^2+3k}{2}
        % +n(2n-1)-n\frac{3(n+1)}{2}
        % & \text{if } n=3k\\
        % \frac{21k^2+3k}{2}
        % +(3k)(6k-1)-(3k)\frac{3((3k)+1)}{2}
        % & \text{if } n=3k\\
        % \frac{21k^2+3k}{2}
        % +18k^2-3k-(3k)\frac{9k+3}{2}
        % & \text{if } n=3k\\
        % \frac{21k^2+3k+36k^2-6k}{2}
        % +\frac{-27k^2-9k}{2}
        % & \text{if } n=3k\\
        % \frac{30k^2-12k}{2}
        % & \text{if } n=3k\\
        k(15k-6)
        & \text{if } n=3k\\
        
        % \frac{21k^2+17k+4}{2}
        % +n(2n-1)-n\frac{3(n+1)}{2}
        % & \text{if } n=3k+1\\
        % \frac{21k^2+17k+4}{2}
        % +(3k+1)(2(3k+1)-1)-(3k+1)\frac{3((3k+1)+1)}{2}
        % & \text{if } n=3k+1\\
        % \frac{21k^2+17k+4}{2}
        % +(3k+1)(6k+2-1)-(3k+1)\frac{(9k+6)}{2}
        % & \text{if } n=3k+1\\
        % \frac{21k^2+17k+4}{2}
        % +(18k^2+3k+6k+1)-\frac{(27k^2+18k+9k+6)}{2}
        % & \text{if } n=3k+1\\
        % \frac{21k^2+17k+4}{2}
        % +(36k^2+18k+2)/2-\frac{(27k^2+27k+6)}{2}
        % & \text{if } n=3k+1\\
        % \frac{21k^2+17k+4+36k^2+18k+2-27k^2-27k-6}{2}
        % & \text{if } n=3k+1\\
        % \frac{30k^2+8k}{2}
        % & \text{if } n=3k+1\\
        k(15k+4)
        & \text{if } n=3k+1\\
        
        % \frac{21k^2+31k+12}{2}
        % +n(2n-1)-n\frac{3(n+1)}{2}
        % & \text{if } n=3k+2
        % \frac{21k^2+31k+12}{2}
        % +(3k+2)(2(3k+2)-1)-(3k+2)\frac{3((3k+2)+1)}{2}
        % & \text{if } n=3k+2
        % \frac{21k^2+31k+12}{2}
        % +(3k+2)(6k+3)-(3k+2)(9k+9)/2
        % & \text{if } n=3k+2
        % \frac{21k^2+31k+12}{2}
        % +(18k^2+9k+12k+6)-(27k^2+27k+18k+18)/2
        % & \text{if } n=3k+2
        % (21k^2+31k+12)/2
        % +(18k^2+21k+6)-(27k^2+45k+18)/2
        % & \text{if } n=3k+2
        % (21k^2+31k+12)/2
        % +(36k^2+42k+12)/2-(27k^2+45k+18)/2
        % & \text{if } n=3k+2
        % (21k^2+31k+12+36k^2+42k+12-27k^2-45k-18)/2
        % & \text{if } n=3k+2
        % (30k^2+28k+6)/2
        % & \text{if } n=3k+2 
        (5k+3)(3k+1)
        & \text{if } n=3k+2 
    \end{cases}
\end{equation*}

This concludes the statement of the corollary.
\end{proof}
}

% 4xn rook helper
{
As discussed in \cref{sec:Ch2:Sec4-grid}, for $K_n\square K_m$ rook's graph $G
$, for $n\geq m\geq 2$, is $(n+m-2)$-regular with $\kappa(G)=n+m-2$.

The following lemma shows that given a $K_n\square K_m$ graph $G$, for $n\geq m\geq 3$, and any elimination ordering $\alpha$ over $G$, at most $m$ vertices can be eliminated by $\alpha$ with degree of $n+m-2$ prior to step $|V|-(n+m-1)$.

\begin{lemma}\label{lem:minDegreeRook}
Let $G=(V,E)$ be a $K_m\square K_n$ graph, for $n\geq m\geq 3$, and $\alpha$ any elimination ordering over $G$.
For a step $i\in\{1,\dots,|V|-(n+m-1)\}$ let $\alpha(i)=v_{r',c'}$ for $r'\in \{1,\dots,m\}$ and $c'\in \{1,\dots,n\}$.
Then $|\textit{madj}^+_\alpha(\alpha(i))|=n+m-2$ iff $(L_{c'}\cup M_{r'})\cap\alpha[1,i-1]=\emptyset$.
As a consequence, $1\leq|\mathcal{V}_G(\alpha,n+m-2)|\leq m$.
\end{lemma}

\begin{proof}
Since $\kappa(G)=n+m-2$, by \cref{cor:tw=kConnected} we have that $|\textit{madj}^+_\alpha(\alpha(i))|\geq n+m-2$ for every step $i\in\{1,\dots,|V|-(n+m-2)\}$.
By the same corollary $G_{|V|-(n+m-1)}$ is a complete graph on $|V|-(n+m-1)$ vertices so $|\textit{madj}^+_\alpha\, (\alpha|V|-(n+m-2))|$ is necessarily $n+m-2$.
For this reason, we are only concerned with steps $i\in \{1,\dots,|V|-(n+m-1)\}$.

Fix a step $i^*\in \{1,\dots,|V|-(n+m-1)\}$ and let $\alpha(i^*)=v_{r^*,c^*}$ for some $r^*\in \{1,\dots,m\}$ and $c^*\in \{1,\dots,n\}$.
Assume that $(L_{c^*}\cup M_{r^*})\cap\alpha[1,i^*-1]=\emptyset$, i.e.,\ $\alpha$ has not eliminated any other vertices from column $c^*$ or row $r^*$ in the previous steps.
Then $V_{\textit{comp}_\alpha(i^*)}= \{v_{r^*,c^*}\}$ and $\textit{madj}^+_\alpha(\alpha(i^*))= (L_{c^*}\cup M_{r^*})\setminus\{v_{r^*,c^*}\}$ by \cref{rmk:madjRooks}.
Consequently, $|\textit{madj}^+_\alpha(\alpha(i^*))|=n+m-2$ proving the statement of the lemma in the `\textit{if}' direction.

Next, we prove that the statement of the lemma also holds in the `\textit{only if}' direction.
Clearly, for every step $i\in\{1,\dots,|V|\}$, $\textit{madj}^+_\alpha(\alpha(i))=N_{G_{i-1}}(\alpha(i))$ is a minimal separator in graph $G_{i-1}$.
Therefore, given that $|\textit{madj}^+_\alpha(\alpha(i))|=n+m-2$ for a step $i\in\{1,\dots,|V|-(n+m-1)\}$, we have that $N_{G_{i-1}}(\alpha(i))$ is a minimal separator of size $n+m-2$ in the graph $G_{i-1}$.
For this reason, we will be considering the set of all minimum separators (of size $n+m-2$) in the intermediate graphs obtained during $\alpha$.
Let us begin by outlining the set of minimum separators in $G$, and then discuss how this set differs from that of $G_1$.
Afterwards, we show that our argument can be repeatedly applied to any step 
$i\in \{1,\dots,|V|-(n+m-1)\}$.

Clearly, $N(v_{r,c})$ for any vertex $v_{r,c}\in V_G$ is a minimal separator (of size $n+m-2$) in $G$ as $N(v_{r,c})\setminus\{u\}$ does not disconnect $v_{r,c}$ from rest of the graph for every vertex $u\in N(v_{r,c})$.
Two vertices $v_{r,c},v_{r',c'}\in V$ are non-adjacent in $G$ iff $c,c'\in \{1,\dots,n\}$ are distinct column indices and $r,r'\in \{1,\dots,m\}$ are distinct row indices.
Every $v_{r,c},v_{r',c'}$-path in $G$ has an internal vertex from either $(L_c\cup M_r)\setminus\{v_{r,c}\}=N(v_{r,c})$ or 
$(L_{c'}\cup M_{r'})\setminus\{v_{r',c'}\}=N(v_{r',c'})$ which implies that $N(v_{r,c})$ and $N(v_{r',c'})$ are the only minimum $v_{r,c},v_{r',c'}$-separators in $G$.
By applying the same arguemenet to every other pair of non-adjacent vertices in $G$, we can conclude that the set of minimum separators of $G$ is exactly $\mathcal{S}^*_G=\{N(v)|v\in V\}$.
% Since $G$ is $(n+m-2)$-regular, every separator from $\mathcal{S}_G$ has $(n+m-2)$ vertices.\todo{There is no need to use such a strong argument about $G$ being $(n+m-2)$-regular… Obviously,  every separator from $\mathcal{S}_G$ has $(n+m-2)$ vertices.?}
Before discussing the set of minimum separators in the intermediate graphs obtained during the elimination ordering $\alpha$, we remind the reader that for every minimum separator $S\in \mathcal{S}^*_G$, $|S|=\kappa(G)=n+m-2$, i.e.\ $\mathcal{S}^*_G=\mathcal{S}^{n+m-2}_G$.

By \cref{cor:tw=kConnected} and the fact that $\kappa(G)=n+m-2$ we have that $\kappa(G_i)\geq n+m-2$ for every step $i\in\{1,\dots,|V|-(n+m-2)\}$.
Let $v_{r',c'}=\alpha(1)$ for some $r'\in \{1,\dots,m\}, c'\in \{1,\dots,n\}$.
Below we show that $\kappa(G_1)=n+m-2$ and more specifically we claim that:
\begin{equation}\label{eq:minSepRook1}
    \mathcal{S}^{n+m-2}_{G_1}= \mathcal{S}^{n+m-2}_{G}\setminus \{N_G(v_{r'',c''})|r''\in \{1,\dots,m\}, c''\in \{1,\dots,n\}, c''=c' \textit{ or } r''=r'\}
\end{equation}

% Informally, we claim that by elimination of $v_{r',c'}$ at step 1, every minimum separator $N_G(v_{r,c})\in \mathcal{S}^*_{G}$, where $v_{r,c}$ is a vertex in the same column or row as $v_{r',c'}$, is no longer a separator in the resulting graph $G_1$.

By \cref{lem:numberofMinimumSeparators} we have $\mathcal{S}^{n+m-2}_{G_1}\subseteq \mathcal{S}^{n+m-2}_G$.
Note that $G[\{v_{r',c'}\}]$ is one of the two components of $G-N_G(v_{r',c'})$ and by elimination of $v_{r',c'}$ at step 1 we have that $|\mathcal{C}_{G_1}\,(N_G(v_{r',c'}))|=1$, i.e.,\ $N_G(v_{r',c'})$ is no longer a separator in the graph $G_1$.
As a result we have that $N_G(v_{r',c'})\notin \mathcal{S}^{n+m-2}_{G_1}$.

Next fix a separator $N_G(v_{r'',c''})\in \mathcal{S}^*_G$ for a vertex $v_{r'',c''}\in (L_{c'}\cup M_{r'})\setminus\{v_{r',c'}\}$.
As $v_{r',c'}\in N_G(v_{r'',c''})$ and $v_{r',c'}\notin V_{G_1}$ we have that
$N_G(v_{r'',c''})\notin \mathcal{S}^{n+m-2}_{G_1}$.
Thus far this proves that:
\begin{equation}\label{eq:minDegreeRook:1subset}
\mathcal{S}^{n+m-2}_{G_1}\subseteq \mathcal{S}^{n+m-2}_{G}\setminus \{N_G(v_{r'',c''})|r''\in \{1,\dots,m\}, c''\in \{1,\dots,n\}, c''=c' \textit{ or } r''=r'\} 
\end{equation}

In order to prove \cref{eq:minSepRook1} we show that for every other separator $N_G(v_{r,c})\in\mathcal{S}^{n+m-2}_G$, for $r\in \{1,\dots,m\}\setminus\{r'\}$ and $c\in \{1,\dots,n\}\setminus\{c'\}$, remains a minimal separator of size $n+m-2$ in $G_1$.
By definition, $G_1$ is the graph obtained from $G$ by eliminating of the vertex $v_{r',c'}$, hence turning $N_G(v_{r',c'})=
(L_{c'}\cup M_{r'})\setminus\{v_{r',c'}\}$ is a clique.
Then for every vertex $v_{r,c}\in V_{G_1}$, $r\in \{1,\dots,m\}\setminus\{r'\}$ and $c\in \{1,\dots,n\}\setminus\{c'\}$ we have that $N_{G_1}(v_{r,c})=N_G(v_{r,c})$.
Thus $N_{G}(v_{r,c})$, for every such vertex $v_{r,c}$, is still a minimal separator in $G_1$.
Because $|N_{G}(v_{r,c})|=n+m-2$ and as shown before $\kappa(G_1)\geq n+m-2$ we can conclude that $\kappa(G_1)=n+m-2$.
This also proves \cref{eq:minSepRook1}, which can be restated as:
\begin{equation}\label{eq:separatorsG1}
    \mathcal{S}^{n+m-2}_{G_1}=\{N_G(v_{r,c})|r\in \{1,\dots,m\}\setminus\{r'\}, c\in \{1,\dots,n\}\setminus\{c'\}\}
\end{equation}

Clearly for a vertex $v_{r,c}$ in graph $G_1$ we have $\textit{deg}_{G_1}(v_{r,c})=n+m-2$ iff $N_{G_1}(v_{r,c})\in 
\mathcal{S}^{n+m-2}_{G_1}$.
By \cref{eq:separatorsG1}, $N_{G_1}(v_{r,c})$ is a separator of size $n+m-2$ in $G_1$ iff $v_{r,c}$ is not from the same row or column as $\alpha(1)=v_{r',c'}$.
Then by combining these 2 observations we can conclude that $\textit{deg}_{G_1}(v_{r,c})=n+m-2$ for a vertex $v_{r,c}\in V_{G_1}$ iff $\{\alpha(1)\}\cap (L_c\cup M_r)=\emptyset$.
So given that $|\textit{madj}^+_\alpha(\alpha(2))|=n+m-2$ we can state that $\alpha(2)$ is not from the same row and column as the previously eliminated vertex $\alpha(1)$.

Now let us briefly discuss why the above statement is applicable to any step $i\in \{2,\dots,|V|-(n+m-1)\}$ (thus proving the statement of the lemma).
It is easy to see that for any vertex $v_{r,c}\in V_{G_{i-1}}$ s.t.\ 
$\alpha[1,i-1]\cap (L_c\cup M_r)=\emptyset$ we have 
$N_{G_{i-1}}(v_{r,c})\in (\mathcal{S}^{n+m-2}_G\cap \mathcal{S}^{n+m-2}_{G_{i-1}})$ as neighbourhood of such a vertex $v_{r,c}$ remains unchanged, i.e.,\ $N_{G_{i-1}}(v_{r,c})=N_G(v_{r,c})$
Also, for any step $i\in\{2,\dots,|V|-(n+m-1)\}$, $\mathcal{S}^{n+m-2}_{G_i}$ will not contain
$N_{G}(v_{r,c})$ for every vertex $v_{r,c}$ from the same column or row as $\alpha(i)$ (since we either have $v_{r,c}=\alpha(i)$ or $\alpha(i)\in N_{G}(v_{r,c})$).
Hence, we can state for any step $i\in\{1,\dots,|V|-(n+m-1)\}$ that $N_{G_{i-1}}(\alpha(i))$ is a separator of size $n+m-2$ in $G_{i-1}$ iff $\alpha(i)$ does not share the same column or row with any of the vertices from $\alpha[1,i-1]$.
Since $m\leq n$ this implies that $|\mathcal{V}_G(\alpha,n+m-2)|\leq m$.
Furthermore, we always have that $|\textit{madj}^+_\alpha(\alpha(1))|=n+m-2$ as $G$ is $(n+m-2)$-regular thus showing that $|\mathcal{V}_G(\alpha,n+m-2)|\geq 1$.
The statement of the lemma follows as a result.
\end{proof}
}

% 4x4 rook
{
We will later show in \cref{lem:46Rooktau} that in the $4\times n$ rook's graph $G$, for $n\geq 6$, every triangulation $H$ of $G$ with $\textit{tw}(H)=\textit{tw}(G)$ cannot be a minimum triangulation of $G$ thus proving that $\tau(G)>0$.
To the best of our knowledge,
$K_4\square K_6$ is in fact the smallest instance of rook's graphs for which the $\tau$ parameter is greater than 0.
For this purpose we will be discussing the $\tau$ parameter of the $4\times n$ rook's graphs for $n\in\{4,5\}$ separately.
In \cref{lem:44Rooktau} we prove that $\tau(G)=0$ for the $4\times 4$ rook's graph $G$.
It will be pointed out after the proof of \cref{lem:44Rooktau} that our approach to discussing the $\tau$ parameter of the $4\times 4$ rook's graph must be slightly modified to be applicable to the $4\times 5$ rook's graph.

\begin{lemma}\label{lem:44Rooktau}
Let $G=(V,E)$ be a $K_4\square K_4$, then $\tau(G)=0$.
\end{lemma}

\begin{proof}
% Beta
{
By \cref{lem:twRook}, $\textit{tw}(G)=9$.
We first define an elimination ordering $\beta$ over $G$ s.t.\ $\textit{tw}(G^+_\beta)=9$.
We point out that $G^+_\beta$ is not necessarily a minimum triangulation.
Next, we use the following argument to prove that $\tau(G)=0$.

Suppose for a contradiction that $\tau(G)>0$.
Then there must exist a minimal triangulation $H$ of $G$ with $\textit{tw}(H)>9$ s.t.\ $|E_H|<|E_{G^+_\beta}|$ (where $H$ may not be a minimum triangulation).
Let $\alpha$ be a peo over one such triangulation $H$, hence $G^+_\alpha=H$ (following \cref{lem:elim}).
To summarize, $\tau(G)>0$ implies that there must exist an elimination ordering $\alpha$ over $G$ where $\textit{tw}(G^+_\alpha)>9$ and $|E_{G^+_\alpha}|<|E_{G^+_\beta}|$.
Therefore, to prove that $\tau(G)=0$, it suffices to show that $|E_{G^+_\alpha}|\geq |E_{G^+_\beta}|$ for every elimination ordering $\alpha$ over $G$ with $\textit{tw}(G^+_\alpha)>9$.
Define $\beta(i)=v_{i,i}$ for $i\in \{1,\dots,4\}$.
Using \cref{lem:minDegreeRook}, it is easy to verify that by our selection $|\textit{madj}^+_\beta(i)|= n+m-2=6$ for every step $i\in \{1,\dots,4\}$.
Let $\beta(5)=v_{1,2}$ and then $\beta(6)=v_{2,1}$.
It is easy to verify that $|\textit{madj}^+_\beta(\alpha(5))|=9$ and $|\textit{madj}^+_\beta(\alpha(6))|=8$
(see $G_4$ shown in \cref{fig:44Rooktau:G4} and $G_5$ in \cref{fig:44Rooktau:G5}).
The graph $G_6$, depicted in \cref{fig:44Rooktau:G6}, is a $K_{10}$.
Therefore, in the remaining steps $i\in\{7,\dots,16\}$ we let $\beta$ be any elimination ordering over $G_6$.
By our construction, 
$\sum_{v\in V} |\textit{madj}^+_\beta(v)|= |E_{G^+_\beta}|= 86$ which combined with the fact that $G$ has $48$ edges implies that there are 38 added edges in $G^+_\beta$.
Since
% 4(6)+9+8+(9(10))/2
$\max_{v\in V}|\textit{madj}^+_\beta(v)|= 9$,
by \cref{lem:twEliminationHigherAdjacency} we have that $G^+_\beta$ is a triangulation of $G$ with $\textit{tw}(G^+_\beta)= \textit{tw}(G)=9$.
}

% fig Beta
{
\tikzset{
mystyle/.style={draw=black,rectangle, inner sep=0pt, text width=5mm, text height=1.75 mm,  align=right, fill=white}
}
\tikzset{
mystyle1/.style={draw=black,rectangle, inner sep=0pt, text width=5mm, text height=2.25 mm,  align=right, fill=white}
}
\begin{figure}
  \centering
    \begin{subfigure}[b]{0.325\textwidth}
        \begin{tikzpicture}[scale=0.7,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        \node [label={[label distance=0.1cm]180:\scriptsize{$1\rightarrow$}}] [mystyle] (11) at (0,3) {\tiny{$v_{1,1}\,\, $ }};
        \node [mystyle] (21) at (0.25,1.5) {\tiny{$v_{2,1}\,\, $ }};
        \node [mystyle] (31) at (-0.25,0) {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5) {\tiny{$v_{4,1}\,\, $ }};
        
        \node [mystyle] (12) at (2,3.25) {\tiny{$v_{1,2}\,\, $ }};
        \node [mystyle] (22) at (2.25,1.75) {\tiny{$v_{2,2}\,\, $ }};
        \node [mystyle] (32) at (1.75,0.25) {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.25) {\tiny{$v_{4,2}\,\, $ }};
        
        
        \node [mystyle] (13) at (4,2.75) {\tiny{$v_{1,3}\,\, $ }};
        \node [mystyle] (23) at (4.25,1.25) {\tiny{$v_{2,3}\,\, $ }};
        \node [mystyle] (33) at (3.75,-0.25) {\tiny{$v_{3,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75) {\tiny{$v_{4,3}\,\, $ }};
        
        
        \node [mystyle] (14) at (6,3) {\tiny{$v_{1,4}\,\, $ }};
        \node [mystyle] (24) at (6.25,1.5) {\tiny{$v_{2,4}\,\, $ }};
        \node [mystyle] (34) at (5.75,-0) {\tiny{$v_{3,4}\,\, $ }};
        \node [mystyle] (44) at (6,-1.5) {\tiny{$v_{4,4}\,\, $ }};
        
        \begin{scope}[on background layer]
        \draw[-] 
            (11)--(12)
            (12)--(13)
            (13)--(14)
            (11)--(13)
            (11)--(14)
            (12)--(14)
            
            (21)--(22)
            (22)--(23)
            (23)--(24)
            (21)--(23)
            (21)--(24)
            (22)--(24)
            
            (31)--(32)
            (32)--(33)
            (33)--(34)
            (31)--(33)
            (31)--(34)
            (32)--(34)
            
            (41)--(42)
            (42)--(43)
            (43)--(44)
            (41)--(43)
            (41)--(44)
            (42)--(44)
            
            
            (11)--(21)
            (21)--(31)
            (31)--(41)
            (11)--(31)
            (11)--(41)
            (21)--(41)
            
            (12)--(22)
            (22)--(32)
            (32)--(42)
            (12)--(32)
            (12)--(42)
            (22)--(42)
            
            (13)--(23)
            (23)--(33)
            (33)--(43)
            (13)--(33)
            (13)--(43)
            (23)--(43)
            
            (14)--(24)
            (24)--(34)
            (34)--(44)
            (14)--(34)
            (14)--(44)
            (24)--(44)
            ;
        \end{scope}
        \end{tikzpicture}
    \caption{$G_0$}
    \label{fig:44Rooktau:G}   
    \end{subfigure}
    \hspace{1.25cm}
    \begin{subfigure}[b]{0.325\textwidth}
        \begin{tikzpicture}[scale=0.7,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (21) at (0.25,1.5) {\tiny{$v_{2,1}\,\, $ }};
        \node [mystyle] (31) at (-0.25,0) {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5) {\tiny{$v_{4,1}\,\, $ }};
        
        \node [mystyle] (12) at (2,3.25) {\tiny{$v_{1,2}\,\, $ }};
        \node [label={[label distance=0.1cm]180:\scriptsize{$2\rightarrow$}}] [mystyle] (22) at (2.25,1.85) {\tiny{$v_{2,2}\,\, $ }};
        \node [mystyle] (32) at (1.75,0.25) {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.25) {\tiny{$v_{4,2}\,\, $ }};
        
        \node [mystyle] (13) at (4,2.75) {\tiny{$v_{1,3}\,\, $ }};
        \node [mystyle] (23) at (4.25,1.25) {\tiny{$v_{2,3}\,\, $ }};
        \node [mystyle] (33) at (3.75,-0.25) {\tiny{$v_{3,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75) {\tiny{$v_{4,3}\,\, $ }};
        
        
        \node [mystyle] (14) at (6,3) {\tiny{$v_{1,4}\,\, $ }};
        \node [mystyle] (24) at (6.25,1.5) {\tiny{$v_{2,4}\,\, $ }};
        \node [mystyle] (34) at (5.75,-0) {\tiny{$v_{3,4}\,\, $ }};
        \node [mystyle] (44) at (6,-1.5) {\tiny{$v_{4,4}\,\, $ }};
        
        %\begin{scope}[on background layer]
        \draw[-] 
            (12)--(13)
            (13)--(14)
            (12)--(14)
            
            (21)--(22)
            (22)--(23)
            (23)--(24)
            (21)--(23)
            (21)--(24)
            (22)--(24)
            
            (31)--(32)
            (32)--(33)
            (33)--(34)
            (31)--(33)
            (31)--(34)
            (32)--(34)
            
            (41)--(42)
            (42)--(43)
            (43)--(44)
            (41)--(43)
            (41)--(44)
            (42)--(44)
            
            
            (21)--(31)
            (31)--(41)
            (21)--(41)
            
            (12)--(22)
            (22)--(32)
            (32)--(42)
            (12)--(32)
            (12)--(42)
            (22)--(42)
            
            (13)--(23)
            (23)--(33)
            (33)--(43)
            (13)--(33)
            (13)--(43)
            (23)--(43)
            
            (14)--(24)
            (24)--(34)
            (34)--(44)
            (14)--(34)
            (14)--(44)
            (24)--(44)
            ;
            
            \begin{scope}[on background layer]
                \draw [draw=MyColorOne!70, rounded corners=5mm, fill=MyColorOne!70, line width=0pt, fill opacity=0.5, draw opacity=0.3]
                %(21)--(12)--(14)--(41)
                (0.25,2)--(1.5,3.25)--(6.5,3)--(0,-2)--cycle;
                ;
                
                \draw [draw=MyColorOne!100, rounded corners=5mm, fill=MyColorOne!140, line width=5pt, fill opacity=0.7, draw opacity=0.7]
                %(12)--(13)--(14)
                (1.5,3.25)--(4,2.5)--(6.5,3)--cycle;
                \draw [draw=MyColorOne!100, rounded corners=5mm, fill=MyColorOne!140, line width=5pt, fill opacity=0.7, draw opacity=0.7]
                %(21)--(31)--(41)
                (0.25,2)--(-0.5,0)--(0.25,-2)--cycle;
            \end{scope}
        %\end{scope}
        \end{tikzpicture}
    \caption{$G_1$}
    \label{fig:44Rooktau:G1}   
    \end{subfigure}
    \vspace{1cm}
    \hfill\\
    \begin{subfigure}[b]{0.325\textwidth}
        \begin{tikzpicture}[scale=0.7,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (21) at (0.25,1.5) {\tiny{$v_{2,1}\,\, $ }};
        \node [mystyle] (31) at (-0.25,0) {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5) {\tiny{$v_{4,1}\,\, $ }};
        
        \node [mystyle] (12) at (2,3.25) {\tiny{$v_{1,2}\,\, $ }};
        \node [mystyle] (32) at (1.75,0.25) {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.25) {\tiny{$v_{4,2}\,\, $ }};
        
        \node [mystyle] (13) at (4,2.75) {\tiny{$v_{1,3}\,\, $ }};
        \node [mystyle] (23) at (4.25,1.25) {\tiny{$v_{2,3}\,\, $ }};
        \node [label={[label distance=-0.05cm]0:\scriptsize{$\leftarrow 3$}}] [mystyle] (33) at (3.85,-0.35) {\tiny{$v_{3,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75) {\tiny{$v_{4,3}\,\, $ }};
        
        
        \node [mystyle] (14) at (6,3) {\tiny{$v_{1,4}\,\, $ }};
        \node [mystyle] (24) at (6.25,1.5) {\tiny{$v_{2,4}\,\, $ }};
        \node [mystyle] (34) at (5.75,-0) {\tiny{$v_{3,4}\,\, $ }};
        \node [mystyle] (44) at (6,-1.5) {\tiny{$v_{4,4}\,\, $ }};
        
        %\begin{scope}[on background layer]
        \draw[-] 
            (12)--(13)
            (13)--(14)
            (12)--(14)
            
            (23)--(24)
            (21)--(23)
            (21)--(24)
            
            (31)--(32)
            (32)--(33)
            (33)--(34)
            (31)--(33)
            (31)--(34)
            (32)--(34)
            
            (41)--(42)
            (42)--(43)
            (43)--(44)
            (41)--(43)
            (41)--(44)
            (42)--(44)
            
            (21)--(31)
            (31)--(41)
            (21)--(41)
            
            (32)--(42)
            (12)--(32)
            (12)--(42)
            
            (13)--(23)
            (23)--(33)
            (33)--(43)
            (13)--(33)
            (13)--(43)
            (23)--(43)
            
            (14)--(24)
            (24)--(34)
            (34)--(44)
            (14)--(34)
            (14)--(44)
            (24)--(44)
            ;
            \begin{scope}[on background layer]
                \draw [draw=MyColorOne!70, rounded corners=5mm, fill=MyColorOne!70, line width=0pt, fill opacity=0.5, draw opacity=0.3]
                %(21)--(12)--(14)--(41)
                (0.25,2)--(1.5,3.25)--(6.5,3)--(0,-2)--cycle;
                ;
                
                \draw [draw=MyColorOne!100, rounded corners=5mm, fill=MyColorOne!140, line width=5pt, fill opacity=0.7, draw opacity=0.7]
                %(12)--(13)--(14)
                (1.5,3.25)--(4,2.5)--(6.5,3)--cycle;
                \draw [draw=MyColorOne!100, rounded corners=5mm, fill=MyColorOne!140, line width=5pt, fill opacity=0.7, draw opacity=0.7]
                %(21)--(31)--(41)
                (0.25,2)--(-0.5,0)--(0.25,-2)--cycle;
                
                
                \draw [draw=red!50, rounded corners=5mm, fill=red!50, line width=0pt, fill opacity=0.5, draw opacity=0.5]
                %(12)--(24)--(42)--(21)
                (1.85,3.5)--(6.75,1.4)--(1.85,-1.5)--(-0.15,1.4)--cycle;
                ;
                
                \draw [draw=red!90, rounded corners=5mm, fill=red!90, line width=5pt, fill opacity=0.5, draw opacity=0.6]
                %(21)--(23)--(24)
                (-0.25,1.4)--(4.25,1.15)--(6.85,1.4)--cycle;
                ;
                \draw [draw=red!90, rounded corners=5mm, fill=red!90, line width=5pt, fill opacity=0.5, draw opacity=0.6]
                %(12)--(32)--(42)
                (1.85,3.65)--(1.65,0.25)--(1.85,-1.65)--cycle;
                ;
            \end{scope}
        %\end{scope}
        \end{tikzpicture}
    \caption{$G_2$}
    \label{fig:44Rooktau:G2}   
    \end{subfigure}
    \hspace{1.25cm}
    \begin{subfigure}[b]{0.325\textwidth}
        \begin{tikzpicture}[scale=0.7,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (21) at (0.25,1.5) {\tiny{$v_{2,1}\,\, $ }};
        \node [mystyle] (31) at (-0.25,0) {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5) {\tiny{$v_{4,1}\,\, $ }};
        
        \node [label={[label distance=0.1cm]180:\scriptsize{$5\rightarrow$}}] [mystyle] (12) at (2,3.25) {\tiny{$v_{1,2}\,\, $ }};
        \node [mystyle] (32) at (1.75,0.25) {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.25) {\tiny{$v_{4,2}\,\, $ }};
        
        
        \node [mystyle] (13) at (4,2.75) {\tiny{$v_{1,3}\,\, $ }};
        \node [mystyle] (23) at (4.25,1.25) {\tiny{$v_{2,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75) {\tiny{$v_{4,3}\,\, $ }};
        
        
        \node [mystyle] (14) at (6,3) {\tiny{$v_{1,4}\,\, $ }};
        \node [mystyle] (24) at (6.25,1.5) {\tiny{$v_{2,4}\,\, $ }};
        \node [mystyle] (34) at (5.75,-0) {\tiny{$v_{3,4}\,\, $ }};
        
        %\begin{scope}[on background layer]
        \draw[-] 
            (12)--(13)
            (13)--(14)
            (12)--(14)
            
            (23)--(24)
            (21)--(23)
            (21)--(24)
            
            (31)--(32)
            (31)--(34)
            (32)--(34)
            
            (41)--(42)
            (42)--(43)
            (41)--(43)
            
            (21)--(31)
            (31)--(41)
            (21)--(41)
            
            (32)--(42)
            (12)--(32)
            (12)--(42)
            
            (13)--(23)
            (13)--(43)
            (23)--(43)
            
            (14)--(24)
            (24)--(34)
            (14)--(34)
            ;

            \begin{scope}[on background layer]
                \draw [draw=MyColorOne!70, rounded corners=5mm, fill=MyColorOne!70, line width=0pt, fill opacity=0.5, draw opacity=0.3]
                %(21)--(12)--(14)--(41)
                (0.25,2)--(1.5,3.25)--(6.5,3)--(0,-2)--cycle;
                ;
                
                \draw [draw=MyColorOne!100, rounded corners=5mm, fill=MyColorOne!140, line width=5pt, fill opacity=0.7, draw opacity=0.7]
                %(12)--(13)--(14)
                (1.5,3.25)--(4,2.5)--(6.5,3)--cycle;
                \draw [draw=MyColorOne!100, rounded corners=5mm, fill=MyColorOne!140, line width=5pt, fill opacity=0.7, draw opacity=0.7]
                %(21)--(31)--(41)
                (0.25,2)--(-0.5,0)--(0.25,-2)--cycle;
                
                
                \draw [draw=red!50, rounded corners=5mm, fill=red!50, line width=0pt, fill opacity=0.5, draw opacity=0.5]
                %(12)--(24)--(42)--(21)
                (1.85,3.5)--(6.75,1.4)--(1.85,-1.5)--(-0.15,1.4)--cycle
                ;
                
                \draw [draw=red!90, rounded corners=5mm, fill=red!90, line width=5pt, fill opacity=0.5, draw opacity=0.6]
                %(21)--(23)--(24)
                (-0.25,1.4)--(4.25,1.15)--(6.85,1.4)--cycle;
                \draw [draw=red!90, rounded corners=5mm, fill=red!90, line width=5pt, fill opacity=0.5, draw opacity=0.6]
                %(12)--(32)--(42)
                (1.85,3.65)--(1.65,0.25)--(1.85,-1.65)--cycle;
                
                
                \draw [draw=blue!50, rounded corners=5mm, fill=blue!50, line width=0pt, fill opacity=0.5, draw opacity=0.5]
                %(31)--(13)--(34)--(43)
                (-0.45,0)--(4,3)--(6.15,-0)--(4,-2)--cycle;
                ;
                
                \draw [draw=blue!90, rounded corners=5mm, fill=red!90, line width=5pt, fill opacity=0.6, draw opacity=0.7]
                %(13)--(23)--(43)
                (4,3)--(4.25,1.25)--(4,-2)--cycle;
                ;
                \draw [draw=blue!90, rounded corners=5mm, fill=red!90, line width=5pt, fill opacity=0.6, draw opacity=0.7]
                %(31)--(32)--(34)
                (-0.45,0)--(1.75,0.25)--(6.15,-0)--cycle;
                ;
                
                
                \draw [draw=darkgray!50, rounded corners=5mm, fill=darkgray!50, line width=0pt, fill opacity=0.4, draw opacity=0.4]
                %(41)--(14)--(34)--(43)
                (-.15,-1.5)--(6,3.5)--(5.75,-0.5)--(4.35,-1.65)--cycle;
                ;
                
                \draw [draw=darkgray!90, rounded corners=5mm, fill=darkgray!90, line width=5pt, fill opacity=0.7, draw opacity=0.6]
                %(14)--(24)--(34)
                (6,3.5)--(6.25,1.5)--(5.75,-0.5)--cycle;
                ;
                \draw [draw=darkgray!90, rounded corners=5mm, fill=darkgray!90, line width=5pt, fill opacity=0.7, draw opacity=0.6]
                %(41)--(42)--(43)
                (-.15,-1.5)--(1.85,-1.15)--(4.35,-1.65)--cycle;
                ;
                
            \end{scope}
        %\end{scope}
        \end{tikzpicture}
    \caption{$G_4$}
    \label{fig:44Rooktau:G4}   
    \end{subfigure}
    \vspace{1cm}
    \hfill\\
    \begin{subfigure}[b]{0.325\textwidth}
        \begin{tikzpicture}[scale=0.7,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        \node [label={[label distance=0.1cm]180:\scriptsize{$6\rightarrow$}}] [mystyle] (21) at (0.25,1.5) {\tiny{$v_{2,1}\,\, $ }};
        \node [mystyle] (31) at (-0.25,0) {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5) {\tiny{$v_{4,1}\,\, $ }};
        
        \node [mystyle] (32) at (1.75,0.25) {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.25) {\tiny{$v_{4,2}\,\, $ }};
        
        \node [mystyle] (13) at (4,2.75) {\tiny{$v_{1,3}\,\, $ }};
        \node [mystyle] (23) at (4.25,1.25) {\tiny{$v_{2,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75) {\tiny{$v_{4,3}\,\, $ }};
        
        \node [mystyle] (14) at (6,3) {\tiny{$v_{1,4}\,\, $ }};
        \node [mystyle] (24) at (6.25,1.5) {\tiny{$v_{2,4}\,\, $ }};
        \node [mystyle] (34) at (5.75,-0) {\tiny{$v_{3,4}\,\, $ }};
        
        
        %\begin{scope}[on background layer]
        \draw[-] 
            (13)--(14)
            
            (23)--(24)
            (21)--(23)
            (21)--(24)
            
            (31)--(32)
            (31)--(34)
            (32)--(34)
            
            (41)--(42)
            (42)--(43)
            (41)--(43)
            
            (21)--(31)
            (31)--(41)
            (21)--(41)
            
            (32)--(42)
            
            (13)--(23)
            (13)--(43)
            (23)--(43)
            
            (14)--(24)
            (24)--(34)
            (14)--(34)
            ;
            
            
            \begin{scope}[on background layer]
                \draw [draw=blue!50, rounded corners=5mm, fill=blue!50, line width=0pt, fill opacity=0.3, draw opacity=0.3]
                %(31)--(13)--(34)--(43)
                (-0.45,0)--(4,3)--(6.15,-0)--(4,-2)--cycle;
                ;
                
                \draw [draw=blue!90, rounded corners=5mm, fill=red!90, line width=5pt, fill opacity=0.5, draw opacity=0.6]
                %(13)--(23)--(43)
                (4,3)--(4.25,1.25)--(4,-2)--cycle;
                ;
                \draw [draw=blue!90, rounded corners=5mm, fill=red!90, line width=5pt, fill opacity=0.5, draw opacity=0.6]
                %(31)--(32)--(34)
                (-0.45,0)--(1.75,0.25)--(6.15,-0)--cycle;
                ;
                
                
                \draw [draw=darkgray!50, rounded corners=5mm, fill=darkgray!50, line width=0pt, fill opacity=0.3, draw opacity=0.3]
                %(41)--(14)--(34)--(43)
                (-.15,-1.5)--(6,3.5)--(5.75,-0.5)--(4.35,-1.65)--cycle;
                ;
                \draw [draw=darkgray!90, rounded corners=5mm, fill=darkgray!90, line width=5pt, fill opacity=0.6, draw opacity=0.7]
                %(14)--(24)--(34)
                (6,3.5)--(6.25,1.5)--(5.75,-0.5)--cycle;
                ;
                \draw [draw=darkgray!90, rounded corners=5mm, fill=darkgray!90, line width=5pt, fill opacity=0.6, draw opacity=0.7]
                %(41)--(42)--(43)
                (-.15,-1.5)--(1.85,-1.15)--(4.35,-1.65)--cycle;
                ;
                
                
                \draw [draw=orange!50, rounded corners=5mm, fill=orange!50, line width=0pt, fill opacity=0.4, draw opacity=0.5]
                %(13)--(14)--(24)--(42)--(41)--(31)--(21)
                (4,3)--(6,3.5)--(6.75,1.4)--(1.85,-1.5)--(0,-2)--(-0.45,0)--(-0.15,1.4)--cycle;
                \draw [draw=orange!100, rounded corners=5mm, fill=orange!100, line width=5pt, fill opacity=0.7, draw opacity=0.6]
                % (21)--(31)--(41)--(42)--(32)
                 (0.25,2)--(-0.65,-0.25)--(-.35,-2)--(2.25,-1.5)--(2,0.35)--cycle;
                ;
                \draw [draw=orange!100, rounded corners=5mm, fill=orange!100, line width=5pt, fill opacity=0.7, draw opacity=0.6]
                % (13)--(14)--(24)--(23)
                 (3.5,3)--(6.35,3.25)--(6.65,1.25)--(3.75,1)--cycle;
                ;
                
            %\end{scope}
        \end{scope}
        \end{tikzpicture}
    \caption{$G_5$}
    \label{fig:44Rooktau:G5}   
    \end{subfigure}
    \hspace{1.25cm}
    \begin{subfigure}[b]{0.325\textwidth}
        \begin{tikzpicture}[scale=0.7,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (31) at (-0.25,0) {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5) {\tiny{$v_{4,1}\,\, $ }};
        
        \node [mystyle] (32) at (1.75,0.25) {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.25) {\tiny{$v_{4,2}\,\, $ }};
        
        \node [mystyle] (13) at (4,2.75) {\tiny{$v_{1,3}\,\, $ }};
        \node [mystyle] (23) at (4.25,1.25) {\tiny{$v_{2,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75) {\tiny{$v_{4,3}\,\, $ }};
        
        \node [mystyle] (14) at (6,3) {\tiny{$v_{1,4}\,\, $ }};
        \node [mystyle] (24) at (6.25,1.5) {\tiny{$v_{2,4}\,\, $ }};
        \node [mystyle] (34) at (5.75,-0) {\tiny{$v_{3,4}\,\, $ }};
        
        
        %\begin{scope}[on background layer]
        \draw[-] 
            (13)--(14)
            
            (23)--(24)
            
            (31)--(32)
            (31)--(34)
            (32)--(34)
            
            (41)--(42)
            (42)--(43)
            (41)--(43)
            
            (31)--(41)
            
            (32)--(42)
            
            (13)--(23)
            (13)--(43)
            (23)--(43)
            
            (14)--(24)
            (24)--(34)
            (14)--(34)
            ;
            
            
            \begin{scope}[on background layer]
                \draw [draw=blue!50, rounded corners=5mm, fill=blue!50, line width=0pt, fill opacity=0.3, draw opacity=0.3]
                %(31)--(13)--(34)--(43)
                (-0.45,0)--(4,3)--(6.15,-0)--(4,-2)--cycle;
                ;
                
                \draw [draw=blue!90, rounded corners=5mm, fill=red!90, line width=5pt, fill opacity=0.5, draw opacity=0.6]
                %(13)--(23)--(43)
                (4,3)--(4.25,1.25)--(4,-2)--cycle;
                ;
                \draw [draw=blue!90, rounded corners=5mm, fill=red!90, line width=5pt, fill opacity=0.5, draw opacity=0.6]
                %(31)--(32)--(34)
                (-0.45,0)--(1.75,0.25)--(6.15,-0)--cycle;
                ;
                
                \draw [draw=darkgray!50, rounded corners=5mm, fill=darkgray!50, line width=0pt, fill opacity=0.3, draw opacity=0.3]
                %(41)--(14)--(34)--(43)
                (-.15,-1.5)--(6,3.5)--(5.75,-0.5)--(4.35,-1.65)--cycle;
                ;
                \draw [draw=darkgray!90, rounded corners=5mm, fill=darkgray!90, line width=5pt, fill opacity=0.6, draw opacity=0.7]
                %(14)--(24)--(34)
                (6,3.5)--(6.25,1.5)--(5.75,-0.5)--cycle;
                ;
                \draw [draw=darkgray!90, rounded corners=5mm, fill=darkgray!90, line width=5pt, fill opacity=0.6, draw opacity=0.7]
                %(41)--(42)--(43)
                (-.15,-1.5)--(1.85,-1.15)--(4.35,-1.65)--cycle;
                ;
                
                \draw [draw=orange!50, rounded corners=5mm, fill=orange!50, line width=0pt, fill opacity=0.5, draw opacity=0.5]
                %(13)--(14)--(24)--(42)--(41)--(31)
                (4,3)--(6,3.5)--(6.75,1.4)--(1.85,-1.5)--(0,-2)--(-0.45,0)--cycle;
                \draw [draw=orange!100, rounded corners=5mm, fill=orange!100, line width=5pt, fill opacity=0.7, draw opacity=0.6]
                %(31)--(41)--(42)--(32)
                 (-0.5,0.15)--(-.35,-1.75)--(2.25,-1.65)--(2,0.5)--cycle;
                \draw [draw=orange!100, rounded corners=5mm, fill=orange!100, line width=5pt, fill opacity=0.7, draw opacity=0.6]
                % (13)--(14)--(24)--(23)
                 (3.5,3)--(6.35,3.25)--(6.65,1.25)--(3.75,1)--cycle;
                
            %\end{scope}
        \end{scope}
        \end{tikzpicture}
    \caption{$G_6$}
    \label{fig:44Rooktau:G6}   
    \end{subfigure}
    \caption{
    Elimination ordering $\beta$ over the $4\times 4$ rook's graph $G$.
    In every figure (a)-(f) the graph $G_{i}$ is shown and the vertex $\alpha(i+1)$ pointed out with its label.
    (b) depicts the graph $G_1$ where $N_{G_0}(\alpha(1))$ is a clique.
    For simplicity, we have not drawn the added edges $\textit{fill}_{G_0}\,(N_{G_0}(\alpha(1)))$ and instead highlighted $N_{G_0}(\alpha(1))$ in light green.
    (c) depicts $G_2$ and the clique $N_{G_1}(\alpha(2))$ is highlighted in red.
    (d) the graph $G_4$ where the cliques $N_{G_2}(\alpha(3))$ and $N_{G_3}(\alpha(4))$ are highlighted in blue and grey respectively.
    Note that $\alpha(5)$ is adjacent to every vertex from $N_{G_0}(\alpha(1))\cup N_{G_1}(\alpha(2))$ (drawn in red and green) thus $\textit{deg}_{G_4}(\alpha(5))=9$.
    (e) similarly shows $G_5$ where $N_{G_4}(\alpha(5))$ is shown in orange.
    It is easy to see that $\textit{deg}_{G_5}(\alpha(6))=8$ as $N_{G_5}(\alpha(6))= N_{G_4}(\alpha(5))\setminus \{\alpha(6)\}$.
    (f) the $K_{10}$ graph $G_6$.
    }
    \label{fig:44Rooktau:Beta}
\end{figure}
}

% Alpha
{
Suppose for a contradiction that $\tau(G)>0$.
Then by definition, for every minimum elimination ordering $\alpha$ over $G$ we have that $\textit{tw}(G^+_{\alpha})>9$ and 
$\sum_{v\in V}|\textit{madj}^+_{\alpha}(v)|<\sum_{v\in V}|\textit{madj}^+_\beta(v)|$.
Let $\alpha$ be one such minimum elimination ordering over $G$ where $\textit{tw}(G^+_{\alpha})$ is minimized among all minimum elimination orderings.
By \cref{lem:niceElim}, we can fix a nice elimination ordering $\alpha^*$ over $G$ where $G^+_{\alpha^*}=G^+_\alpha$.
Since $\alpha^*$ is also a minimum elimination ordering, we have that:
\begin{equation}\label{eq:44RookSumAlpha}
    \sum\nolimits_{v\in V}|\textit{madj}^+_{\alpha^*}(v)|<
    \sum\nolimits_{v\in V}|\textit{madj}^+_\beta(v)|=86
\end{equation}

Let $\textit{tw}(G^+_{\alpha^*})=9+k$ for some $k\geq 1$.
Because ${\alpha^*}$ is a nice elimination ordering and $\omega(G^+_{\alpha^*})=\textit{tw}(G^+_{\alpha^*})+1= 10+k$, by \cref{def:niceElim} we have that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=|V|-i$ for every step $i\in\{|V|-(10+k),\dots,16\}$ (as $\alpha^*(i)$ is a universal vertex in $G_{i-1}$).
% k is min =1 so from step 6 till end 
% k is higher = 2 so from step 16-(9+2)= 5 …
% but we are sure that from 6 till end we do simplicial
Thus, we can conclude that $\sum_{v\in\alpha^*[6,16]} |\textit{madj}^+_{\alpha^*}(v)|= 55$.
This combined with \cref{eq:44RookSumAlpha} implies:
\begin{equation}\label{eq:44RookSumAlpha15}
    \sum\nolimits_{v\in {\alpha^*}[1,5]}|\textit{madj}^+_{\alpha^*}(v)|=
    \sum\nolimits_{v\in V}|\textit{madj}^+_{\alpha^*}(v)|-\frac{10(10+1)}{2}<31
\end{equation}

\cref{cor:tw=kConnected} and the fact that $\kappa(G)=6$ imply that $|\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|\geq 6$ for every step $i\in\{1,\dots,10\}$, therefore we can state that:
\begin{equation}\label{eq:4rookMinMadj1to5}
    \min\nolimits_{i\in\{1,\dots,5\}}|\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|\geq 6
\end{equation}

By \cref{lem:minDegreeRook} the number of vertices ${\alpha^*}$ can eliminate with degree 6 prior to step $|V|-(6+1)=9$ is at most 4 as $G$ is a $K_4\square K_4$.
Formally, we have that $|\mathcal{V}_G({\alpha^*},6)|\leq 4$.
Which combined with \cref{eq:4rookMinMadj1to5} implies that at most 4 vertices in ${\alpha^*}[1,5]$ are eliminated with degree 6 and the remaining vertices are eliminated in ${\alpha^*}$ with degree at least 7.
To summarize, we can state that:
\begin{equation}\label{eq:4rookMinMadj1to5Sum}
    \sum\nolimits_{v\in {\alpha^*}[1,5]}|\textit{madj}^+_{\alpha^*}(v)|\geq (4\times 6)+(1\times 7)=31
\end{equation}
This contradicts \cref{eq:44RookSumAlpha15} implying that 
$\sum_{v\in V}|\textit{madj}^+_{\alpha^*}(v)|\geq\sum_{v\in V}|\textit{madj}^+_\beta(v)|$.
This consequently proves that $\tau(G)=0$ as desired.
}
\end{proof}
}

% 4x4 rook mfi experimental is 38
{
In the proof of \cref{lem:44Rooktau}, the number of added edges in the triangulation $G^+_\beta$ is clearly an upper bound for 
$\textit{mfi}(K_4\square K_4)$.
This value matches $\textit{mfi}(K_4\square K_4)$ obtained from our experimental work presented in \cref{tab:4rookMfi}.
As a result, we can state the following remark (which is not formally proved):

\begin{remark}\label{rmk:mfi44Rook}
Let $G$ be a $K_4\square K_4$.
Then $\textit{mfi}(G)=38$.
\end{remark}
}

% 4x5 rook helper
{
We will be determining the $\tau$ parameter of the $4\times 5$ rook's graph using a similar approach.
More specifically, we will first define an elimination ordering $\beta$ over the $K_4\times K_5$ graph $G$ s.t.\ $\textit{tw}(G^+_\beta)=\textit{tw}(G)$ and then show that $|E_{G^+_\alpha}|\geq |E_{G^+_\beta}|$ for every elimination ordering $\alpha$ over $G$ with $\textit{tw}(G^+_\alpha)>\textit{tw}(G^+_\alpha)$.
Similar to \cref{lem:44Rooktau}, in order to show that $|E_{G^+_\alpha}|\geq |E_{G^+_\beta}|$, we will be comparing the number of edges added in $\beta$ and $\alpha$ over a fixed set of steps.
However, unlike the $4\times 4$ rook's graph, this value for $\alpha$ is not as high relative to that of $\beta$.
Therefore, in the proof of \cref{lem:45Rooktau} we will need to consider every possible scenario $\alpha$ can eliminate the vertices of $G$.
Furthermore, we will be using the following lemma showing that given any elimination ordering $\alpha$ over the $m\times n$ rook's graph $G$, for $n\geq m\geq 2$, there exists a nice elimination ordering $\gamma^*$ where $G^+_\alpha=G^+_{\gamma^*}$ and $\gamma^*$ has an additional property:

\begin{lemma}\label{lem:minDegreeRookFirst}
Let $G$ be a $K_m\square K_n$ rook's graph for $n\geq m\geq 2$ and $\alpha$ any elimination ordering over $G$.
Then there exists a nice elimination ordering $\gamma^*$ over $G$ s.t.\ $G^+_{\gamma^*}=G^+_\alpha$ and 
$\mathcal{V}_G({\gamma^*},n+m-2)=
\gamma^*[1,|\mathcal{V}_G(\gamma^*,n+m-2)|]$
(where the vertex set $\mathcal{V}_G(\gamma^*, n+m-2)$ is defined in \cref{def:f}).
\end{lemma}

\begin{proof}
By \cref{lem:niceElim} we can fix a nice elimination ordering $\alpha^*$ over $G$ where $G^+_{\alpha^*}=G^+_\alpha$.
Consider the set
$\mathcal{V}_G({\alpha^*},n+m-2)$ and suppose that it is not equal to the set
$\alpha^*[1,|\mathcal{V}_G(\alpha^*,n+m-2)|]$.
It means that we can fix a vertex $v_{r',c'}\in\mathcal{V}_G({\alpha^*},n+m-2)$ s.t.\
$v_{r',c'}\notin \alpha^*[1,|\mathcal{V}_G(\alpha^*,n+m-2)|]$, i.e.,\
${\alpha^*}^{-1}(v_{r',c'})>|\mathcal{V}_G({\alpha^*},n+m-2)|$.

% Then one of the following cases must be true:
% \begin{mycases}
%     \case
%     {
%     There exists a vertex $v\in\mathcal{V}_G({\alpha^*},n+m-2)$ s.t.\ $v\notin \alpha^*[1,|\mathcal{V}_G(\alpha^*,n+m-2)|]$.
%     }
    
%     \case
%     {
%     There exists a vertex $u\in \alpha^*[1,|\mathcal{V}_G(\alpha^*,n+m-2)|]$ s.t.\ $u\notin \mathcal{V}_G({\alpha^*},n+m-2)$.
%     }
% \end{mycases}

% Given that Case 2 is true, not all vertices from $\mathcal{V}_G({\alpha^*},n+m-2)$ are eliminated during steps 1 to $|\mathcal{V}_G(\alpha^*,n+m-2)|$.
% Therefore ${\alpha^*}^{-1}(v)>|\mathcal{V}_G({\alpha^*},n+m-2)|$ for some vertex $v\in\mathcal{V}_G({\alpha^*},n+m-2)$ (which is equivalent case 1).
% \todo{this is not clear?}
% \unsure{is it clear now? I really don't think it is so hard to see.}
% For this purpose we can assume w.l.o.g.\ that the first case is true, otherwise the statement of the lemma follows as $\mathcal{V}_G({\alpha^*},n+m-2)=
% \bigcup_{i\in\{1,\dots,|\mathcal{V}_G(\alpha^*,n+m-2)|\}} \alpha^*(i)$.\todo{not clear}
% % \unsure[inline]{
% % Updated\\
% % We have a subset of vertices $X\subset V$.
% % We claim that all of $X$ are eliminated during steps 1 to $|X|$, i.e.,\ $X=\alpha[1,|X|]$.
% % If this is not true, then either:\\
% % (1) $\alpha[1,|X|]\subset X$. 
% % This means that there is a vertex in $X$ that is not in eliminated prior to step $|X|$.
% % \textbf{So there exists a vertex $x\in X$ s.t.\ $x\notin \alpha[1,|X|]$.}\\

% % (2) $X\subset \alpha[1,|X|]$. 
% % meaning that there exists a vertex $y\in\alpha[1,|X|]$, that is eliminated before step $|X|$ s.t.\ $y\notin X$.
% % Since $\alpha$ is an ordering of $V$ and all of $V$ (including $X$) must be eliminated at some step, we can state that:
% % $y$ takes the place of a vertex $x\in X$ in $\alpha$ that could have been eliminated before step $|X|$.
% % I.e.,\ there exists a vertex $x\in X$ s.t.\ $\alpha^{-1}(x)>|X|$.
% % \textbf{So there exists a vertex $x\in X$ s.t.\ $x\notin \alpha[1,|X|]$.}\\

% % Both cases lead to same statement. Should add a discussion like this?
% % }

First, we prove that there exists a nice elimination ordering ${\beta^*}$ over $G$ where $G^+_{\beta^*}=G^+_{\alpha^*}$ and $v_{r',c'}$ is the first vertex to be eliminated in ${\beta^*}$.
Let $i$ be the step at which $v_{r',c'}$ is eliminated in $\alpha^*$, i.e.,\ $i={\alpha^*}^{-1}(v_{r',c'})$.
Then by selection and the fact that $v_{r',c'}\in\mathcal{V}_G(\alpha^*,n+m-2)$ (defined in \cref{def:f}) we have that:
\begin{equation}\label{eq:minDegreeRookFirsteq1}
    |\mathcal{V}_G({\alpha^*},n+m-2)|+1\leq i\leq |V|-(n+m-1)
\end{equation}

We define the elimination ordering ${\beta^*}$ as follows.
Let ${\beta^*}(1)={\alpha^*}(i)=v_{r',c'}$, for $j\in\{2,\dots,i\}$ let ${\beta^*}(j)={\alpha^*}(j-1)$ and for $j\in\{i+1,\dots,|V|\}$ let ${\beta^*}(j)={\alpha^*}(j)$.
Informally, the only difference between ${\alpha^*}$ and ${\beta^*}$ is that $v_{r',c'}$ is the first vertex to be eliminated in $\beta^*$.
In order to show that $G^+_{\beta^*},G^+_{\alpha^*}$ are identical graphs, it suffices to prove that $E_{G^+_{\alpha^*}}=E_{G^+_{\beta^*}}$ as these two graphs are defined over the same vertex sets.

Since the vertex $v_{r',c'}$ eliminated at step $i$ in $\alpha^*$ belongs to $\mathcal{V}_G({\alpha^*},n+m-2)$, by \cref{lem:minDegreeRook} we have that 
$
%\textit{madj}^+_{\alpha^*}({\alpha^*}(i))=
(L_{c'}\cup M_{r'})\cap \alpha^*[1,i-1]=\emptyset$.
Then by construction of $\beta^*$, $\textit{madj}^+_{\beta^*}({\beta^*}(1))=
\textit{madj}^+_{\alpha^*}({\alpha^*}(i))=
(L_{c'}\cup M_{r'})\setminus \{v_{r',c'}\}$
Therefore
$|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|
=|\textit{madj}^+_{\beta^*}(\beta^*(1))|
=n+m-2$.
% Also since $v_{r',c'}\in\mathcal{V}_G({\alpha^*},n+m-2)$, by \cref{def:f} we have that $i\leq |V|-(n+m-1)$.
% Then we can state using \cref{lem:minDegreeRook} that $\alpha^*[1,i-1]\cap (L_{c'}\cup M_{r'})=\emptyset$.
% As a result we have:
% $$
% \textit{madj}^+_{\alpha^*}({\alpha^*}(1))= 
% (L_{c'}\cup M_{r'})\setminus\{v_{r',c'}\} = \textit{madj}^+_{\beta^*}({\beta^*}(1))
% $$\todo{it this correct? Should it be $({\alpha^*}(i))$? }

By our construction of $\beta^*$ and the fact that
$(L_{c'}\cup M_{r'})\cap \alpha^*[1,i-1]=\emptyset$, we have that ${\beta^*}(j)\notin (L_{c'}\cup M_{r'})$ for every step $j\in\{2,\dots,i\}$.
Then by \cref{cor:madjNonAdjacent}, for every step $j\in\{2,\dots,i\}$, $\textit{madj}^+_{\beta^*}({\beta^*}(j))=
\textit{madj}^+_{\alpha^*}({\alpha^*}(j-1))$.
Since $\alpha^*[1,i]=\beta^*[1,i]$
and $\bigcup_{v\in \alpha^*[1,i]}\textit{madj}^+_{\alpha^*}(v)
=\bigcup_{v\in \beta^*[1,i]}\textit{madj}^+_{\beta^*}(v)$, 
we can state that the graphs $G^{\beta^*}_i,G^{\alpha^*}_i$ are identical.
Recall that by our construction $\alpha^*(j)=\beta^*(j)$ and for every later step $j\in \{i+1,\dots,|V|\}$.
Then because $G^{\beta^*}_i,G^{\alpha^*}_i$ are identical we can state that $\textit{madj}^+_{\beta^*}({\beta^*}(j))=\textit{madj}^+_{\alpha^*}({\alpha^*}(j))$ for every step $j\in \{i+1,\dots,|V|\}$.
By summarizing all above observations, we can state that:
$$
E_{G^+_{\beta^*}}
=\bigcup\nolimits_{v\in V}\textit{madj}^+_{\beta^*}(v)
=\bigcup\nolimits_{v\in V}\textit{madj}^+_{\alpha^*}(v)
=E_{G^+_{\alpha^*}}
$$

This proves that $G^+_{\beta^*}=G^+_{\alpha^*}$ as desired.
To summarize, $\beta^*$ is an elimination ordering over $G$ resulting in an identical triangulation to $\alpha^*$ with the only change that $v_{r',c'}$ (which by selection is a vertex from $\mathcal{V}_G({\alpha^*},n+m-2)$ s.t.\ ${\alpha^*}^{-1}(v_{r',c'})>|\mathcal{V}_G({\alpha^*},n+m-2)|$) is the first vertex to be eliminated in ${\beta^*}$.

Next, let us show that $\beta^*$ is a nice elimination ordering.
Since $\alpha^*$ is a nice elimination ordering, from \cref{def:niceElim} we know that there exists exactly one step $j\in\{|V|-(\textit{tw}(G^+_{\alpha^*})),\dots,|V|\}$ where $|\textit{madj}^+_{\alpha^*}(\alpha^*(j))|=n+m-2$.
% j <-      |V|-tw, …, |V|-0
% madj(j)=  |V|-(|V|-i)=i
It is easy to see that this step is $j=|V|-(n+m-2)$ so by
% i <= |V|-(n+m-1) = |V|-n-m+1
% j = |V|-(n+m-2) = |V|-n-m+2
% i<j
\cref{eq:minDegreeRookFirsteq1} we have that $i<j$ and so  $i<|V|-(\textit{tw}(G^+_{\alpha^*}))$.
It is already shown that for $j\in\{i+1,\dots,|V|\}$, $\textit{madj}^+_{\beta^*}(\beta^*(j))=
\textit{madj}^+_{\alpha^*}(\alpha^*(j))$ thus proving that $\beta^*$ is, same as $\alpha^*$, a nice elimination ordering.
% \unsure[inline]
% {
% Should I add some informal explanation here?\\
% We know that $\textit{tw}(G^+_{\alpha^*})=\textit{tw}(G^+_{\beta^*})$ as the 2 triangulations are identical.
% The step in $\alpha^*$ where we have made a change is step $i$ selected s.t. $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=n+m-2$.
% Since $\alpha^*$ is nice we have that 
% $|\textit{madj}^+_{\alpha^*}\, (\alpha^*(|V|-(n+m-2)))|= n+m-2$ and we cannot have
% $|\textit{madj}^+_{\alpha^*}\, (\alpha^*(j)))|= n+m-2$
% for every later step $j\in\{|V|-(n+m-3),\dots,|V|\}$.
% So we have not made any changes in the final steps $j\in\{|V|-(n+m-2),\dots,|V|\}$ of $\alpha^*$.
% }

By exhaustively applying the above arguments, we can obtain a nice elimination ordering $\gamma^*$ over $G$ where $G^+_{\gamma^*}=G^+_{\alpha^*}=G^+_\alpha$ and for every vertex $v\in \mathcal{V}_G(\gamma^*,n+m-2)$ we have ${\gamma^*}^{-1}(v)\leq |\mathcal{V}_G(\gamma^*,n+m-2)|$.
The lemma thus follows.
\end{proof}
}

% 4x5 rook
{
Now let us determine the value of $\tau$ parameter for the $4\times 5$ rook's graph.

\begin{lemma}\label{lem:45Rooktau}
Let $G=(V,E)$ be a $K_4\square K_5$, then $\tau(G)=0$.
\end{lemma}
\begin{proof}
We know from \cref{lem:twRook} that $\textit{tw}(G)=11$.
By the same argument used in the proof of \cref{lem:44Rooktau}, in order to show that $\tau(G)=0$ it suffices to first define an elimination ordering $\beta$ over $G$ s.t.\ $\textit{tw}(G^+_\beta)=11$ and then prove that $|E_{G^+_\alpha}|\geq |E_{G^+_\beta}|$ for every elimination ordering $\alpha$ over $G$ with $\textit{tw}(G^+_\alpha)>11$.

Define the elimination ordering $\beta$ as follows.
Let $\beta(i)=v_{i,i}$ for $i\in \{1,\dots,4\}$.
By this selection and \cref{lem:minDegreeRook} we have that $|\textit{madj}^+_\beta(\beta(i))|=n+m-2=7$ for every one of these steps $i\in \{1,\dots,4\}$.
Next, let $\beta(5)=v_{1,2}$ and $\beta(6)=v_{3,4}$.
It is simple to verify that $|\textit{madj}^+_\beta(\beta(i))|=11$ for $i\in\{5,6\}$.
Afterwards, let $\beta(7)=v_{2,1}$ and $\beta(8)=v_{4,3}$.
We point out that by this selection $|\textit{madj}^+_\beta(\beta(i))|=10$ for $i=\{7,8\}$.
The resulting $G^\beta_8$ is a $K_{12}$ so in the remaining steps we let $\beta$ be any elimination ordering over $G^\beta_8$.
By our construction, we have $\sum_{v\in V}|\textit{madj}^+_\beta(v)|=136$ which combined with the fact that $|E_G|=70$ implies that there are 66 edges added in $G^+_\beta$.
We also note that by our construction $\max_{v\in V}
|\textit{madj}^+_\beta(v)|=
\textit{tw}(G^+_\beta)=11$.
% n+m-2= 9-2=7
% 4(7)+2(11)+2(10)+(12(11))/2 = 136

Suppose for a contradiction that $\tau(G)>0$.
Then for every minimum elimination ordering ${\alpha}$ over $G$ we have $\textit{tw}(G^+_{\alpha})>11$ and 
$\sum_{v\in V}|\textit{madj}^+_{\alpha}(v)|<\sum_{v\in V}|\textit{madj}^+_\beta(v)|$.
Fix a minimum elimination ordering $\alpha$ over $G$ s.t.\ $\textit{tw}(G^+_{\alpha})$ is minimized.
By \cref{lem:minDegreeRookFirst}, we can fix a nice elimination ordering $\alpha^*$ over $G$ where $G^+_{\alpha^*}=G^+_\alpha$ and the following condition is true:
\begin{equation}\label{eq:45rooktau:1}
    {\alpha^*}^{-1}(v)\leq|\mathcal{V}_G({\alpha^*},7)| \,\textit{ for every vertex }\, v\in\mathcal{V}_G(\alpha^*,7)
\end{equation}

Since $G^+_{\alpha^*}=G^+_\alpha$, $\alpha^*$ is also a minimum triangulation and consequently $\sum_{v\in V}|\textit{madj}^+_{\alpha^*}(v)|<\sum_{v\in V}|\textit{madj}^+_\beta(v)|$.
Additionally, we have that $\textit{tw}(G^+_{\alpha^*})=\textit{tw}(G^+_\alpha)>\textit{tw}(G^+_\beta)=11$.

Let $\textit{tw}(G^+_{\alpha^*})=11+k$ for some $k\geq 1$.
Since ${\alpha^*}$ is a nice elimination ordering and $\textit{tw}(G^+_{\alpha^*})\geq 12$, we have that $|\textit{madj}^+_{\alpha^*}
(\alpha^*(i))|=|V|-i$ for every step $i\in\{8,\dots,20\}$ (following \cref{def:niceElim}).
% tw is at least 12, so G_{|V|-13} is a K_{13}
% so during steps |V|-12=8 to 20 we are eliminating a K_13
% therefore 12(13)/2 is a number of added edges from step 8 onwards
Then $\sum_{v\in{\alpha^*}[8,20]} |\textit{madj}^+_{{\alpha^*}}(v)|=
\frac{12(12+1)}{2}$ and combined with the fact that 
$\sum_{v\in V} |\textit{madj}^+_{{\alpha^*}}(v)| < 
\sum_{v\in V} |\textit{madj}^+_\beta(v)|= 136$ we can state that:
% 78 + sum 1 to 7 < 136
% sum 1 to 7 < 58
\begin{equation}\label{eq:45RookAlpha17}
    \sum\nolimits_{v\in{\alpha^*}[1,7]}|\textit{madj}^+_{\alpha^*}(v)|=
    \sum\nolimits_{v\in V}|\textit{madj}^+_{\alpha^*}(v)|-\frac{12(12+1)}{2}<58
\end{equation}

Let $t=|\mathcal{V}_G({\alpha^*},7)|$.
Since $G$ is a $K_4\square K_5$, by \cref{lem:minDegreeRook} we have that 
$1\leq t\leq 4$.
By \cref{eq:45rooktau:1} we have that $\alpha^*[1,t]=\mathcal{V}_G({\alpha^*},7)$, consequently for every step $i\in\{1,\dots,t\}$ we have $|\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|=7$.
Clearly, for every step $i\in\{t+1,\dots,7\}$ we have that $|\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|>7$.
By \cref{lem:minDegreeRook}, for every such step $i\in\{t+1,\dots,7\}$, ${\alpha^*}(i)$ must be adjacent to at least one vertex from the vertex set ${\alpha^*}[1,i-1]$ in the graph $G^{\alpha^*}_{i-1}$.
This clearly implies that $|V_{\textit{comp}_{\alpha^*}(i)}|\geq 2$ so either $|\mathcal{M}_{\alpha^*}(i)|\geq 2$ or $|\mathcal{L}_{\alpha^*}(i)|\geq 2$ (or both).
In \cref{tab:madj45Rook}, we have considered all possible values for $|V_{\textit{comp}_{\alpha^*}(i)}|,|\mathcal{M}_{\alpha^*}(i)|$ and $|\mathcal{L}_{\alpha^*}(i)|$ for any step $i\in\{t+1,\dots,7\}$.
We will use this table and \cref{cor:madjRooks} in order to evaluate $|\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|$.

Below we consider every possible value of $t$ (note that $t\in\{1,\dots,4\}$ as previously discussed), and in every case we prove that $\sum_{v\in{\alpha^*}[1,7]}|\textit{madj}^+_{\alpha^*}(v)|\geq 58$ thus contradicting \cref{eq:45RookAlpha17}.

\begin{mycases}
    \case
    {
    Suppose that $t=1$.
    This implies that $|\textit{madj}^+_{\alpha^*}(\alpha^*(1))|=7$, and we will now determine the value of $\sum_{v\in{\alpha^*}[2,7]}
    |\textit{madj}^+_{\alpha^*}(v)|$.
    As discussed before, for every step $i\in\{t+1,\dots,7\}$, $|V_{\textit{comp}_{\alpha^*}(i)}|\geq 2$.
    Then by \cref{tab:madj45Rook}, for every vertex $v\in{\alpha^*}[2,7]$ we have $|\textit{madj}^+_{\alpha^*}(v)|\geq 9$.
    % 7+ 6(9) = 61  
    This implies that $\sum_{v\in{\alpha^*}[2,7]}|\textit{madj}^+_{\alpha^*}(v)|\geq 54$ and consequently $\sum_{v\in{\alpha^*}[1,7]}|\textit{madj}^+_{\alpha^*}(v)|\geq 61$ contradicting \cref{eq:45RookAlpha17}.
    }
    
    \case
    {
    Suppose that $t=2$.
    Therefore, $\sum_{v\in{\alpha^*}[1,2]}|\textit{madj}^+_{\alpha^*}(v)|=14$, and we will now determine the value of $\sum_{v\in{\alpha^*}[3,7]}
    |\textit{madj}^+_{\alpha^*}(v)|$.
    We know that for every step $i\in\{t+1,\dots,7\}$, $|V_{\textit{comp}_{\alpha^*}(i)}|\geq 2$.
    By \cref{tab:madj45Rook}, for every vertex $v\in{\alpha^*}[3,7]$ we have $|\textit{madj}^+_{\alpha^*}(v)|\geq 9$ thus showing that $\sum_{v\in{\alpha^*}[3,7]}|\textit{madj}^+_{\alpha^*}(v)|\geq 45$.
    % 5(9)
    Since $\sum_{v\in{\alpha^*}[1,2]}|\textit{madj}^+_{\alpha^*}(v)|=14$, we can state that $\sum_{v\in{\alpha^*}[1,7]}|\textit{madj}^+_{\alpha^*}(v)|\geq 59$ contradicting \cref{eq:45RookAlpha17}.
    }
    
    \case
    {
    Suppose that $t=3$.
    Then we have $\sum_{v\in{\alpha^*}[1,3]}|\textit{madj}^+_{\alpha^*}(v)|=21$ so let us evaluate $\sum_{v\in{\alpha^*}[4,7]}
    |\textit{madj}^+_{\alpha^*}(v)|$.
    
    As discussed in the previous case, the fact that $|V_{\textit{comp}_{\alpha^*}(i)}|\geq 2$ for every step $i\in\{4,\dots,7\}$ implies that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|\geq 9$ 
    (following \cref{tab:madj45Rook}).
    We claim that there exist at most 2 steps $i\in\{4,\dots,7\}$ where $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=9$.
    Suppose for a contradiction that we can fix 3 distinct steps $i_1,i_2,i_3\in\{4,\dots,7\}$ where $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=9$ for every step $i\in\{i_1,i_2,i_3\}$.
    W.l.o.g.\ assume that $i_1<i_2<i_3$. 
    Since $t=3$, we have $\alpha^*[1,3]=\mathcal{V}_G(\alpha^*,7)$ and using \cref{lem:minDegreeRook} we can write $\alpha^*[1,3]=\{v_{r_1,c_1},v_{r_2,c_2},v_{r_3,c_3}\}$ for unique row indices $r_1,r_2,r_3\in\{1,\dots,4\}$ and unique column indices $c_1,c_2,c_3\in\{1,\dots,5\}$.
    Let $\{c_4,c_5\}=\{1,\dots,5\}\setminus\{c_1,c_2,c_3\}$, then for a column index $c\in\{1,\dots,5\}$ we have $L_c\cap\alpha^*[1,3]=\emptyset$ iff $c\in\{c_4,c_5\}$.
    By \cref{tab:madj45Rook} we can deduce that for a step $i\in\{4,\dots,7\}$, $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=9$ iff $|\mathcal{M}_{\alpha^*}(i)|=1$ and $|\mathcal{L}_{\alpha^*}(i)|=2$ (which corresponds to row 1 of \cref{tab:madj45Rook}).
    In other words, $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=9$ iff
    $V_{\textit{comp}_{\alpha^*}(i)}$ is contained within a single row, and no two vertices from it (including $\alpha^*(i)$) share the same column.
    Then w.l.o.g.\ we can assume that $\alpha^*(i_1)\in L_{c_4}$ and $\alpha^*(i_2)\in L_{c_5}$.
    However, as $G$ has 5 columns, we have that $\alpha^*(i_3)$ necessarily shares the same column with a vertex from $\alpha^*[1,i_3-1]$ proving that $|\textit{madj}^+_{\alpha^*}\,(\alpha^*(i_3))|>9$, a contradiction.
    Consequently, there can exist at most 2 steps $i\in\{4,\dots,7\}$ where $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=9$ and for every other step we necessarily have that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|\geq 10$.
    
    As a consequence of the above observation, we can state that $\sum_{v\in\alpha^*[4,7]}
    |\textit{madj}^+_{\alpha^*}(v)|\geq 
    2\times 9+2\times 10$.
    Since $\sum_{v\in{\alpha^*}[1,3]}|\textit{madj}^+_{\alpha^*}(v)|=21$ we conclude that $\sum_{v\in\alpha^*[1,7]}|\textit{madj}^+_{\alpha^*}(v)|\geq 59$ contradicting \cref{eq:45RookAlpha17}.
    }

    \case
    {
    Suppose that $t=4$.
    Therefore, $\sum_{v\in{\alpha^*}[1,4]}|\textit{madj}^+_{\alpha^*}(v)|=28$, so it remains for us to evaluate $\sum_{v\in{\alpha^*}[5,7]}
    |\textit{madj}^+_{\alpha^*}(v)|$.

    Since $t=4$, we have $\alpha^*[1,4]=\mathcal{V}_G(\alpha^*,7)$ and by \cref{lem:minDegreeRook} we can let $\alpha^*[1,4]=\{v_{r_1,c_1},v_{r_2,c_2},v_{r_3,c_3},v_{r_4,c_4}\}$ for unique row indices $r_1,r_2,r_3,r_4\in\{1,\dots,4\}$ and unique column indices $c_1,c_2,c_3,c_4\in\{1,\dots,5\}$.
    Let $c_5=\{1,\dots,5\}\setminus\{c_1,\dots,c_4\}$, i.e.,\ $c_5$ is the column index where $L_{c_5}\cap \alpha^*[1,4]=\emptyset$.
    First, we need to prove the following statements:
    \begin{itemize}
        \item[(a)]
        {
        There exists at most one step $i\in\{5,\dots,7\}$ s.t.\ $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=9$.
        }
        
        \item[(b)]
        {
        There exists at most one step $i\in\{5,\dots,7\}$ s.t.\ $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=10$.
        }
    \end{itemize}
    
    % (a)
    {
    In order to prove statement (a), suppose for a contradiction that there exists 2 steps $i_1,i_2\in\{5,\dots,7\}$ s.t.\ $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_1))|=
    |\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))|=9$.
    W.l.o.g.\ let $i_1<i_2$.
    By \cref{tab:madj45Rook}, $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=9$ for a step $i\in\{5,\dots,7\}$ iff $|\mathcal{M}_{\alpha^*}(i)|=1$ and $|\mathcal{L}_{\alpha^*}(i)|=2$ (row 1 of \cref{tab:madj45Rook}).
    This means that every vertex from $V_{\textit{comp}_{\alpha^*}(i_1)}$ is from the same row and no two vertices from this set (including $\alpha^*(i)$) share the same column.
    Since $i_1<i_2$ we must have $\alpha^*(i_1)\in L_{c_5}$ which implies that $\alpha^*(i_2)$ neccessarily shares a column with a vertex from $\alpha^*[1,i_2-1]$.
    As a result, $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))|>9$, a contradiction.
    This proves statement (a) as desired.
    }
    
    % (b)
    {
    In order to prove statement (b), let us consider all possible cases where we can have $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=10$ for a step $i\in\{5,\dots,7\}$.
    As seen in \cref{tab:madj45Rook} there are 3 such cases (rows 2, 8, and 17).
    Below we prove that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=10$ iff $|V_{\textit{comp}_{\alpha^*}(i)}|=4$, $|\mathcal{M}_{\alpha^*}(i)|=2$ and $|\mathcal{L}_{\alpha^*}(i)|=2$ 
    (i.e.,\ row 8 of \cref{tab:madj45Rook}) by showing that the other 2 cases, listed below in subcases (i) and (ii), are not possible.
    
    \begin{subcases}
        \subcase 
        {
        For a step $i\in\{5,\dots,7\}$, $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=10$ if $|V_{\textit{comp}_{\alpha^*}(i)}|=2$, $|\mathcal{M}_{\alpha^*}(i)|=2$ and $|\mathcal{L}_{\alpha^*}(i)|=1$ (row 2 of \cref{tab:madj45Rook}).
        Since $i>4$ and $\alpha^*[1,4]$ has a vertex from every row, $\textit{comp}_{\alpha^*}(i)$ necessarily spans across 2 or more columns, formally $|\mathcal{L}_{\alpha^*}(i)|\geq2$.
        As a result, we can conclude that this case is not possible.
        }
        
        \subcase 
        {
        For a step $i\in\{5,\dots,7\}$, $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=10$ if $|V_{\textit{comp}_{\alpha^*}(i)}|=6$, $|\mathcal{M}_{\alpha^*}(i)|=2$ and $|\mathcal{L}_{\alpha^*}(i)|=3$ (row 17 of \cref{tab:madj45Rook}).
        W.l.o.g.\ assume that $\mathcal{M}_{\alpha^*}(i)=\{r_1,r_2\}$.
        Since $i\leq 7$ we have that 
        $V_{\textit{comp}_{\alpha^*}(i)}\subset \alpha^*[1,7]$ and because $|V_{\textit{comp}_{\alpha^*}(i)}|=6$ we have that 
        $|\alpha^*[1,7]\setminus V_{\textit{comp}_{\alpha^*}(i)}|=1$.
        Let us assume w.l.o.g.\ that this vertex 
        $\{v\}=(\alpha^*[1,7]\setminus V_{\textit{comp}_{\alpha^*}(i)})$ belongs to row $r_3$.
        As a result, $\alpha^*[1,7]$ cannot contain any vertices from row $r_4$.
        This results in a contradiction as $\alpha^*[1,4]\subset \alpha^*[1,7]$ and $\alpha^*[1,4]$ contains a vertex from every row of $G$.
        We can thus conclude that this case is also not possible.
        }
    \end{subcases}
    
    This proves that for a step $i\in\{5,\dots,7\}$ we have $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=10$ iff $|V_{\textit{comp}_{\alpha^*}(i)}|=4$, $|\mathcal{M}_{\alpha^*}(i)|=2$ and $|\mathcal{L}_{\alpha^*}(i)|=2$.
    To prove statement (b), suppose for a contradiction that we can fix 2 steps $i_1,i_2\in\{5,\dots,7\}$ s.t.\ $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_1))|=
    |\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))|=10$.
    W.l.o.g.\ let us assume that $i_1<i_2$.
    As previously discussed, 
    $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=10$ for a step $i\in\{5,\dots,7\}$ iff
    $|V_{\textit{comp}_{\alpha^*}(i)}|=4$, $|\mathcal{M}_{\alpha^*}(i)|=2$ and $|\mathcal{L}_{\alpha^*}(i)|=2$.
    Therefore, it is easy to verify that $V_{\textit{comp}_{\alpha^*}(i_1)}\cap V_{\textit{comp}_{\alpha^*}(i_2)}=\emptyset$.
    The fact that $i_2>i_1$ and $|V_{\textit{comp}_{\alpha^*}(i_1)}|=|V_{\textit{comp}_{\alpha^*}(i_2)}|=4$ implies that $i_2\geq 8$ as $\alpha^*[1,i_2]$ must contain all 8 vertices of $V_{\textit{comp}_{\alpha^*}(i_1)}\cup V_{\textit{comp}_{\alpha^*}(i_2)}$.
    This contradicts the fact that $i_2\in\{5,\dots,7\}$ proving statement (b) as a result.
    }
    
    By combining statements (a) and (b) we can state that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|\geq11$ for at least 1 step $i\in\{5,\dots,7\}$ hence showing that $\sum_{v\in\alpha^*[5,7]}|\textit{madj}^+_{\alpha^*}(v)|\geq 9+10+11$.
    Together with the fact that $\sum_{v\in\alpha^*[1,4]}|\textit{madj}^+_{\alpha^*}(v)|=28$ we have that $\sum_{v\in\alpha^*[1,7]}|\textit{madj}^+_{\alpha^*}(v)|\geq 58$ contradicting \cref{eq:45RookAlpha17} in the case where $t=4$.
    }
\end{mycases}

\begin{table}
    \centering
    \begin{tabular}{
    @{\makebox[3em][c]{\rownumber\space\space\space}} cccc}
        \toprule
        $|V_{\textit{comp}_{\alpha^*}(i)}|$ & 
        $|\mathcal{M}_{\alpha^*}(i)|$ & 
        $|\mathcal{L}_{\alpha^*}(i)|$ & $|\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|$ 
        \gdef\rownumber{\stepcounter{magicrownumbers}\arabic{magicrownumbers}} \\%
        % \multirow{2}{*}[-1em]{Models} & \multicolumn{3}{c}{Metric 1} & Metric 2\\
        % \addlinespace[10pt]
        % \cmidrule(lr){2-4} \cmidrule(lr){5-5} \\
        % col1 & precision & recall & F-score  & R@10 \\
        \midrule
        2&1&2&9\\\midrule
         2&2&1&10\\\midrule
         3&1&3&11\\\midrule
         3&2&2&11\\\midrule
         3&3&1&13\\\midrule
         4&1&4&13\\\midrule
         4&2&3&12\\\midrule
         4&2&2&10\\\midrule
         4&3&2&13\\\midrule
         4&4&1&16\\\midrule
         5&1&5&15\\\midrule
         5&2&3&11\\\midrule
         5&2&4&13\\\midrule
         5&3&2&12\\\midrule
         5&3&3&13\\\midrule
         5&4&2&15\\\midrule
         6&2&3&10\\\midrule
         6&2&4&12\\\midrule
         6&2&5&14\\\midrule
         6&3&2&11\\\midrule
         6&3&3&12\\\midrule
         6&3&4&13\\\midrule
         6&4&2,3&14\\\midrule
         7&2&4&11\\\midrule
         7&2&5&13\\\midrule
         7&3&3&11\\\midrule
         7&3&4&12\\\midrule
         7&3&5&13\\\midrule
         7&4&2,3,4&13\\
        \bottomrule
    \end{tabular}
    \vspace{0.25cm}
    
    \caption{
    Given the nice elimination ordering $\alpha^*$ over the $K_4\square K_5$ graph $G$ (defined in \cref{lem:45Rooktau}) the table demonstrates the value of $|\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|$ for a step $i\in\{t+1,\dots,7\}$ by considering all possible values of $|\mathcal{M}_{\alpha^*}(i)|$, $|\mathcal{L}_{\alpha^*}(i)|$ and $|V_{\textit{comp}_{\alpha^*}(i)}|$.
    Note that since $i\leq 7$ we have $|V_{\textit{comp}_{\alpha^*}(i)}|\leq 7$.}\label{tab:madj45Rook}
\end{table}

We have thus shown that every possible value of $t=|\mathcal{V}_G({\alpha^*},7)|$ results in a contradiction with \cref{eq:45RookAlpha17}.
This implies that $\sum_{v\in V}|\textit{madj}^+_{\alpha^*}(v)|\geq
\sum_{v\in V}|\textit{madj}^+_\beta(v)|$.
By selection, $\textit{tw}(G^+_\beta)=\textit{tw}(G)=11$ which by definition shows that $\tau(G)=0$ as desired.
\end{proof}
}

% 4x5 rook mfi experimental is 66
{
A similar statement to \cref{rmk:mfi44Rook} can also be stated for the $4\times 5$ rook's graph following the proof of \cref{lem:45Rooktau}.
This is due to the fact that the number of added edges in $G^+_\beta$ is inline with the value obtained for $\textit{mfi}(K_4\square K_5)$ from our experimental work presented in \cref{tab:4rookMfi}.
We again point out that the following statement is not formally proved:

\begin{remark}\label{rmk:mfi45Rook}
Let $G$ be a $K_4\square K_5$.
Then $\textit{mfi}(G)=66$.
\end{remark}
}

% 4xn n>=6 rook helper
{
Let $G$ be an $m\times n$, for $n\geq m\geq 2$, rook's graph.
We point out that there exists a nice elimination ordering $\alpha^*$ over $G$ satisfying both the following conditions:
\begin{itemize}
    \item[(a)]
    {
    $\textit{tw}(G^+_{\alpha^*})=\textit{tw}(G)$
    }

    \item[(b)]
    {
    $\mathcal{V}_G(\alpha^*,n+m-2)=\alpha^*[1,|\mathcal{V}_G(\alpha^*,n+m-2)|]$
    }
\end{itemize}

To do so, begin with an elimination ordering $\alpha$ over $G$ with $\textit{tw}(G^+_\alpha)=\textit{tw}(G)$.
$\alpha$ clearly exists by \cref{lem:twEliminationHigherAdjacency}.
Then by \cref{lem:minDegreeRookFirst} we can fix a nice elimination ordering $\alpha^*$ over $G$ where $G^+_{\alpha^*}=G^+_\alpha$ and $\alpha^*$ satisfies condition (b).
Then because $G^+_{\alpha^*}=G^+_\alpha$, we have that $\textit{tw}(G^+_{\alpha^*})=\textit{tw}(G^+_{\alpha})=\textit{tw}(G)$ showing that $\alpha^*$ also satisfies condition (a) as desired.
We will use this fact in order to show that $\tau(G)>0$ for the $4\times n$ rook's graph $G$, $n\geq 6$.

Before proceeding to describe our approach, we point out that to the best of our knowledge every graph class that was previously shown to have $\tau>0$, was constructed to have such a property.
In our case, we study a set of well-established graph classes and then show that there are rook's graphs with $\tau>0$.
Therefore, our approach to determining the $\tau$ parameter is itself one of the novelties of our research, as no previous literature studied the same problem.
However, our method is unique to rook's graph and is not easily applicable to all graph classes.

In the next two lemmas, we will consider the $4\times n$ rook's graph $G$, for $n\geq 4$, and a nice elimination ordering $\alpha^*$ over $G$ where $\textit{tw}(G^+_{\alpha^*})=\textit{tw}(G)$ and $\mathcal{V}_G(\alpha^*,n+m-2)=\alpha^*[1,|\mathcal{V}_G(\alpha^*,n+m-2)|]$.
Informally, in \cref{lem:46helper1} we obtain a lower bound for the number of edges added by $\alpha^*$ when eliminating a subset of vertices spanning across 2 rows of $G$.
Similarly, in \cref{lem:46helper2} we consider the case where this subset of eliminated vertices spans 3 rows and then prove a lower bound on the number of edges added by $\alpha^*$.
We then combine the statements of \cref{lem:46helper1} and \cref{lem:46helper2} in \cref{lem:46Rooktau} so to prove a lower bound on the number of edges in any triangulation $H$ of $G$ selected s.t.\ $\textit{tw}(H)=\textit{tw}(G)$.
Ultimately, we show that this lower bound can be beaten by a triangulation $H'$ of $G$ with $\textit{tw}(H')>\textit{tw}(G)$ thus proving that $\tau(G)>0$ as desired.

\begin{lemma}\label{lem:46helper1}
Let $G=(V,E)$ be a $K_4\square K_n$ for $n\geq 4$ and $\alpha^*$ a nice elimination ordering over $G$ s.t.\ $\mathcal{V}_G(\alpha^*,n+2)=
\alpha^*[1,|\mathcal{V}_G(\alpha^*,n+2)|]$ and $\textit{tw}(G^+_{\alpha^*})=\textit{tw}(G)$.
Then for any step $j\in\{|\mathcal{V}_G(\alpha^*,n+2)|+1,\dots,2n-2\}$ 
such that $|\mathcal{M}_{\alpha^*}(j)|=2$, the following statement holds (where we denote $X=V_{\textit{comp}_{\alpha^*}(j)}$):
\[
    \sum\nolimits_{v\in X}
    |\textit{madj}^+_{\alpha^*}(v)|\geq
\begin{cases}
    % 2n+4+
    % \ceil*{\frac{|X|-2}{2}}(2n+1)+
    % \floor*{\frac{|X|-2}{2}}2n,
    2n(|X|-1)+\ceil*{\frac{|X|}{2}}+3,
    & \text{if } 
    |\mathcal{V}_G(\alpha^*,n+2)\cap X|=2\\
    2n(|X|-1)+\ceil*{\frac{|X|}{2}}+5,              
    & \text{otherwise}
\end{cases}
\]
\end{lemma}

% \todo[inline]
% {
% To summarize: firstly $\alpha^*$ remove $|\mathcal{V}_G(\alpha^*,n+2)|$ vertices (4 in this case) with strategy that from each column/row at most one vertex is eliminated…then for sure between the step $|\mathcal{V}_G(\alpha^*,n+2)|+1 $  and the step $n+1$ (in the worst case scenario we  eliminate  vertices from different columns)  $\alpha^*$ must eliminate a vertex $j$ with property $|\mathcal{M}_{\alpha^*}(j)|=2$ (hence we eliminate two vertices from the same column)….  
% }
% \unsure[inline]
% {
% Note, the focus here is no existence of such step $j$.
% This is just a helper lemma for $4\times n$, $n\geq 6$.
% In the proof of \cref{lem:46Rooktau}, I want to take a nice elimination ordering $\alpha^*$ that has the above-mentioned properties and I want to obtain a lower bound on number of edges in $G^+_{\alpha^*}$.
% For this I suppose different scenarios:\\

% (a) exists a step $j$, $|\mathcal{V}_G(\alpha^*,n+2)|+1\leq j\leq 2n-2$, with $|\mathcal{M}_{\alpha^*}(j)|=2$\\
% (b) exists a step $j$, $|\mathcal{V}_G(\alpha^*,n+2)|+1\leq j\leq 2n-2$, with $|\mathcal{M}_{\alpha^*}(j)|=3$

% I have noted why at least one of these 2 cases must happen in proof of \cref{lem:46Rooktau} ($2n-2$ vertices are eliminated from $n$ columns, just simple pigeonhole).
% In \cref{lem:46helper1} and \cref{lem:46helper2}, as mentioned previously also, I just want to obtain lower bounds for $\sum_{v\in V_{\textit{comp}_{\alpha^*}(j)}} |\textit{madj}^+_{\alpha^*}(v)|$.
% }
% \todo[inline]{Yes, I can see that, but it must be written clearly…}
\begin{proof}
We have shown prior to the statement of the lemma that for every $m\times n$ rook's graph $G$, where $m\geq n\geq 2$, there exists a nice elimination ordering 
$\alpha^*$ where $\textit{tw}(G^+_{\alpha^*})=\textit{tw}(G)$ and $\mathcal{V}_G(\alpha^*,n+m-2)=
\alpha^*[1,|\mathcal{V}_G(\alpha^*,n+m-2)|]$.
Therefore, given the $4\times n$ rook's graph $G$, where $n\geq 4$, we can fix a nice elimination ordering $\alpha^*$ satisfying the conditions of the lemma.

% Let us begin by showing that there exists a nice elimination ordering over $G$ satisfying both conditions stated in the lemma (as it was briefly mentioned before the lemma).
% Clearly we can fix an elimination ordering $\alpha$ over $G$ where $\textit{tw}(G^+_\alpha)=\textit{tw}(G)$.
% By \cref{lem:minDegreeRookFirst}, we can fix a nice elimination ordering $\alpha^*$ over $G$ s.t.\ $\mathcal{V}_G(\alpha^*,n+2)=
% \alpha^*[1,|\mathcal{V}_G(\alpha^*,n+2)|]$ and $G^+_{\alpha^*}= G^+_\alpha$.
% This shows that $\textit{tw}(G^+_{\alpha^*})= \textit{tw}(G^+_\alpha)= \textit{tw}(G)$ as desired.

% \todo[inline]{
% \cref{lem:minDegreeRookFirst} holds in a general case—so is it true that the discussion before \cref{46helper1}—holds in general case? If yes, it could be mentioned there and here applied only on special case $4x n$….
% }
% \unsure[inline]{
% \cref{lem:minDegreeRookFirst} holds for $n,m\geq 3$.\\
% The discussion before \cref{lem:46helper1} is stated for $4\times n$ rook's graphs, as we already took care of $3\times n$.
% And yes if you are wondering it clearly holds for $3\times n$.\\

% Not sure what you want me to add here?
% }
% \todo[inline]{See the comments before Lemma 26}

By \cref{lem:twRook}, $\textit{tw}(G)=\textit{tw}(G^+_{\alpha^*})=2n+1$ and by \cref{lem:twEliminationHigherAdjacency} we can state the following about $\alpha^*$:
\begin{equation}\label{eq:4nConTw}
    \max\nolimits_{v\in V}
    |\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|\leq 2n+1
\end{equation}

Fix a step $j\in\{|\mathcal{V}_G(\alpha^*,n+2)|+1,\dots,2n-2\}$ such that $|\mathcal{M}_{\alpha^*}(j)|=2$, let  $X=V_{\textit{comp}_{\alpha^*}(j)}$. Obviously because $|\mathcal{M}_{\alpha^*}(j)|=2$, $|X|\geq 2$.
Let $\mathcal{M}_{\alpha^*}(j)=\{r, r'\}$  and let $i_1$, $i_2$ be the first two steps in $\alpha^*$ s.t.\ $\{\alpha^*(i_1),\alpha^*(i_2)\}\subseteq X$, $1\leq i_1<i_2\leq j$.
Since any two vertices in $M_r$ (similarly $M_r'$) are adjacent by an edge in $G$, we can conclude that $\alpha^*(i_1)$ is the first vertex to be eliminated by $\alpha^*$ from $M_r\cup M_{r'}$.
Furthermore, it is easy to see that $\alpha^*(i_1)$ cannot share a column with any of the  previously eliminated.
Hence, $|\textit{madj}^+_{\alpha^*}(i_1)|=n+2$ by \cref{cor:madjRooks} and then necessarily $\alpha^*(i_1)\in \mathcal{V}_G(\alpha^*,n+2)$.

Therefore, we have $\alpha^*(i_1)\in(X\cap\mathcal{V}_G(\alpha^*,n+2))$.
By \cref{lem:minDegreeRook} and the fact that the vertices of $X$ span across exactly 2 rows of $G$, we have that  $|X\cap\mathcal{V}_G(\alpha^*,n+2)|\leq 2$.
Below we provide a lower bound for $\sum_{i\in \{i_1,i_2\}}
|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|$ by considering 2 complementary cases:

\begin{mycases}
    \case{Suppose that $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=2$.
    Since $i_2$ is the next step at which $\alpha^*$ eliminates a vertex from $X$, and we must have  $\mathcal{V}_G(\alpha^*,n+2)\cap X = 
    \{\alpha^*(i_1), \alpha^*(i_2)\}$.

    As a result
    $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))| =n+2$ which implies 
    $\sum_{i\in \{i_1,i_2\}}
    |\textit{madj}^+_{\alpha^*}(\alpha^*(i))|= 2n+4$.
    }
    
    \case{
    Suppose that $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=1$.
    Then in this case $\mathcal{V}_G(\alpha^*,n+2)\cap X = \{\alpha^*(i_1)\}$.
    Below we prove that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))| \geq n+4$.
    The fact that $\alpha^*(i_2)\notin \mathcal{V}_G(\alpha^*,n+2)$ 
    and selection of $\alpha^*(i_2)$ as the second vertex eliminated from $X$ implies that $\alpha^*(i_2)$ must be in the same row
    or column as  $\alpha^*(i_1)$, i.e.,\
    $V_{\textit{comp}_{\alpha^*}(i_2)}=\{\alpha^*(i_2),\alpha^*(i_1)\}$.

   Below, we consider 2 complementary subcases:
    
    \begin{subcases}
        \subcase {
        Suppose that $\alpha^*(i_1),\alpha^*(i_2)$ are in the same column.
        Then $|\mathcal{L}_{\alpha^*}(i_2)|=1$ and $|\mathcal{M}_{\alpha^*}(i_2)|=
        |V_{\textit{comp}_{\alpha^*}(i_2)}|=2$ as a result by \cref{cor:madjRooks} we have that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))|= 2n$.
        }
        
        \subcase {
        Suppose that $\alpha^*(i_1),\alpha^*(i_2)$ are in the same row.
        Then $|\mathcal{M}_{\alpha^*}(i_2)|=1$ and $|\mathcal{L}_{\alpha^*}(i_2)|=
        |V_{\textit{comp}_{\alpha^*}(i_2)}|=2$ so by \cref{cor:madjRooks} we have that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))|= n+4$.
        }
    \end{subcases}
    
    By combining the above subcases we can state that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))| \geq n+4$, hence
    $\sum\nolimits_{i\in \{i_1,i_2\}}
    |\textit{madj}^+_{\alpha^*}(\alpha^*(i))|
    \geq 2n+6$.
    }
\end{mycases}

The following statement summarizes our observations from the above 2 cases:
\begin{equation}\label{eq:46helper1:i1i2}
    \sum\nolimits_{i\in \{i_1,i_2\}}
    |\textit{madj}^+_{\alpha^*}(\alpha^*(i))| \geq
    \begin{cases}
        2n+4, &\text{if $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=2$}\\
        2n+6, &\text{if $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=1$.}
    \end{cases}
\end{equation}

% hidden old proof
\iffalse{
Obviously because $|\mathcal{M}_{\alpha^*}(j)|=2$, we have that $|X|\geq 2$.
Let $\mathcal{M}_{\alpha^*}(j)=\{r,r'\}$ for $r,r'\in\{1,\dots,4\}$ and define the steps $i_1,i_2$, where $1\leq i_1<i_2\leq j$, be the earliest steps in $\alpha^*$ s.t.\ $\{\alpha^*(i_1),\alpha^*(i_2)\}\subseteq X$.
Since $X$ spans across row $r,r'$ and the vertex set of each of these rows is a clique in $G$, we can conclude that $\alpha^*(i_1)$ is the first vertex to be eliminated from $M_r\cup M_{r'}$.
% \unsure[inline]{
% Suppose there exists a step $i<i_1$ s.t.\ $\alpha^*(i)\in \bigcup_{r\in\{r_1,r_2\}} M_r$ and $\alpha^*(i)\notin X$.
% Then because rows $r_1,r_2$ are cliques and $X$ spans across both of these rows, we necessarily have that $\alpha^*(i)\in X$ contradicting selection of $i_1,i_2$.

% I have also discussion because $r_1,r_2$ are clique, no other vertex can be eliminated from them.
% }
\todo[inline]{
Why the first vertex which is removed from $M_r\cup M_{r'}$ must belong to $X$? 
Due to the properties of $\alpha^*$, we know how the first $|\mathcal{V}_G(\alpha^*,n+2)|$ steps look like, which seems to be used in the proof. Therefore, there should not be some more assumptions be given about $i_1$?
}
\unsure[inline]
{
I don't want to add any more conditions for $i_1,i_2$.
I just need them to be the first steps where we eliminated vertices from $X$.
My goal in this proof is to obtain a lower bound for 
$\sum_{v\in X} |\textit{madj}^+_{\alpha^*}(v)|$.
To do so, first I provide a lower bound for the first 2 vertices eliminated from $X$ (i.e.,\ 
$\sum_{i\in \{i_1,i_2\}} |\textit{madj}^+_{\alpha^*}(\alpha^*(i))|$) and then provide a lower bound for the rest of the vertices eliminated from $X$ (i.e., $\sum_{v\in (X\setminus\{\alpha^*(i_1),\alpha^*(i_2)\})} |\textit{madj}^+_{\alpha^*}(v)|$).
So as you can see I don't want $i_1,i_2$ to have any other conditions apart from them being first steps where we eliminated from $X$.

Now to explain my argument in more detail and let me know if I should put this above in the proof:\\

We let $\mathcal{M}_{\alpha^*}(j)=\{r,r'\}$ for some $r,r'\in\{1,\dots,4\}$, i.e.,\ $X=V_{\textit{comp}_{\alpha^*}(j)}$ is a connected component spanning across both rows $M_r$ and $M_{r'}$.
We also fix $1\leq i_1<i_2\leq j$ to be the earliest steps in $\alpha^*$ s.t.\ $\{\alpha^*(i_1),\alpha^*(i_2)\}\subseteq X$.

Likewise, we claim that $i_1,i_2$ are the firsts steps in $\alpha^*$ where we have eliminated vertices from $M_r\cup M_{r'}$.
First, let us show this for $i_1$.
Suppose for a contradiction that there exists an earlier step $i$, where $1\leq i<i_1$, s.t.\ $\alpha^*(i)\in M_r\cup M_{r'}$ and $\alpha^*(i)\notin X$.
Since $\mathcal{M}_{\alpha^*}(j)=\{r,r'\}$, $i<j$ and $M_r$, $M_{r'}$ are both cliques in $G$, we have that $\alpha^*(i)\in X$ contradicting the selection of step $i_1$.

Now let us show that $i_2$ is the second vertex eliminated in $\alpha^*$ from $M_r\cup M_{r'}$.
Suppose for a contradiction that there exists a step $i'$, where $i_1<i'<i_2$, s.t.\ $\alpha^*(i')\in M_r\cup M_{r'}$ and $\alpha^*(i')\notin X$.
By the same logic as before, we have that $\alpha^*(i')\in X$ and is eliminated after $i_1$ yet before $i_2$.
This contradicts the selection of step $i_2$.
}

Clearly $\alpha^*(i_1)$ does not share a row and a column with any vertex from $\alpha^*[1,i_1-1]$ proving that $|\textit{madj}^+_{\alpha^*}(i_1)|=n+2$.
By our selection $i_1<j\leq 2n-2<|V|-(n+3)$ therefore we necessarily have that $\alpha^*(i_1)\in \mathcal{V}_G(\alpha^*,n+2)$ (following \cref{def:f}). 
We point out that because $\mathcal{V}_G(\alpha^*,n+2)=
\alpha^*[1,|\mathcal{V}_G(\alpha^*,n+2)|]$ by our selection of $\alpha^*$, we necessarily have that $i_1<|\mathcal{V}_G(\alpha^*,n+2)|$.
\unsure{Updated. Not sure if last sentence is used}

By \cref{lem:minDegreeRook} and the fact that the vertices of $X$ span across 2 rows of $G$, we have that $1\leq |X\cap\mathcal{V}_G(\alpha^*,n+2)|\leq 2$ (as shown before $\alpha^*(i_1)\in(X\cap\mathcal{V}_G(\alpha^*,n+2))$).
Below we provide a lower bound for $\sum_{i\in \{i_1,i_2\}}
|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|$ by considering 2 complementary cases:
\begin{mycases}
    \case{Suppose that $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=2$.
    Since $i_2$ is the next step at which $\alpha^*$ eliminates a vertex from $X$, and we have that $\mathcal{V}_G(\alpha^*,n+2)\cap X = 
    \{\alpha^*(i_1), \alpha^*(i_2)\}$.
    \unsure[inline]
    {
    Is this easy to see that 
    $\mathcal{V}_G(\alpha^*,n+2)\cap X = 
    \{\alpha^*(i_1), \alpha^*(i_2)\}$?
    
    Suppose that is not the case. 
    We have previously shown that $\alpha^*(i_1)\in \mathcal{V}_G(\alpha^*,n+2)\cap X$.
    Let $\alpha^*(i)$ for $i_1<i\leq j$ be the other vertex eliminated from $X$ with degree of $n+2$, i.e.,\ 
    $\{\alpha^*(i)\}=
    (X\cap\mathcal{V}_G(\alpha^*,n+2))
    \setminus\{\alpha^*(i_1)\}$.
    If our statement above is not correct, there must exist another step $i'$ (that is possibly same as $i_2$), where $i_1<i'<i\leq j$, in which we have to eliminate a vertex $\alpha^*(i')\in X$ that has $|\textit{madj}^+_{\alpha^*}(\alpha^*(i'))| >n+2$ and then later at $i$ we have $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))| =n+2$.
    
    By selection $\alpha^*(i)$ is eliminated with degree $n+2$ at a step $i\leq j<3n-3$ thus showing that 
    $\alpha^*(i)\in \mathcal{V}_G(\alpha^*,n+2)$.
    However, by selection of $\alpha^*$ we have that all vertices from $\mathcal{V}_G(\alpha^*,n+2)$ are eliminated first which contradicts the existence of such step $i'$.
    }
    Consequently
    $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))| =n+2$ which concludes that 
    $\sum_{i\in \{i_1,i_2\}}
    |\textit{madj}^+_{\alpha^*}(\alpha^*(i))|= 2n+4$ when $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=2$.
    }
    \case{Suppose that $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=1$.
    In this case, $\mathcal{V}_G(\alpha^*,n+2)\cap X = \{\alpha^*(i_1)\}$.
    Below we prove that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))| \geq n+4$.
    The fact that $\alpha^*(i_2)\notin \mathcal{V}_G(\alpha^*,n+2)$ together with \cref{lem:minDegreeRook} implies that $\alpha^*(i_2)$ shares a column of a row with a vertex from $\alpha^*[1,i_2-1]$.
    By selection, this vertex must be $\alpha^*(i_1)$, i.e.,\
    $V_{\textit{comp}_{\alpha^*}(i_2)}=\{\alpha^*(i_2),\alpha^*(i_1)\}$.
    \unsure
    {
    Is this easy to see?
    }
    Below, we consider 2 complementary subcases:
    
    \begin{subcases}
        \subcase {
        Suppose that $\alpha^*(i_1),\alpha^*(i_2)$ are in the same column.
        Then $|\mathcal{L}_{\alpha^*}(i_2)|=1$ and $|\mathcal{M}_{\alpha^*}(i_2)|=
        |V_{\textit{comp}_{\alpha^*}(i_2)}|=2$ as a result by \cref{cor:madjRooks} we have that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))|= 2n$.
        }
        
        \subcase {
        Suppose that $\alpha^*(i_1),\alpha^*(i_2)$ are in the same row.
        Then $|\mathcal{M}_{\alpha^*}(i_2)|=1$ and $|\mathcal{L}_{\alpha^*}(i_2)|=
        |V_{\textit{comp}_{\alpha^*}(i_2)}|=2$ so by \cref{cor:madjRooks} we have that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))|= n+4$.
        }
    \end{subcases}
    
    By combining the above subcases, we can state that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_2))| \geq n+4$.
    This combined with the fact that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i_1))|=n+2$ implies that
    $\sum\nolimits_{i\in \{i_1,i_2\}}
    |\textit{madj}^+_{\alpha^*}(\alpha^*(i))|
    \geq 2n+6$ when $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=1$.
    }
\end{mycases}

The following statement summarizes our observations from the above 2 cases:
\begin{equation}\label{eq:46helper1:i1i2}
    \sum\nolimits_{i\in \{i_1,i_2\}}
    |\textit{madj}^+_{\alpha^*}(\alpha^*(i))| \geq
    \begin{cases}
        2n+4 &\text{if $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=2$}\\
        2n+6 &\text{if $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=1$}
    \end{cases}
\end{equation}
}
\fi

% \todo{
% $X$ can have only 2 vertices, so maybe the assumption should be added, that this value will be determined for all $X$ of size at least 3
% } 
% \unsure{Why should it have 2 vertices? Can have $2n$ even.}
% \todo[inline]{
% yes, there is no problem with that, but at the beginning of the proof due to the lemma's assumptions there is mentioned that $|X|$ is at least 2....and I haven't noticed that it would be mentioned some other assumption about $X$ so far...so this comment was only a a small one, that the calculations below have no sense for $X$ of size 2, so we can suppose further $X$ has at least 3 elements….
% }

In the case where $|X|=2$, the statement of the lemma clearly follows from \cref{eq:46helper1:i1i2} so let us suppose that $|X|>2$.
In the next part of the proof, we determine the value of $\sum_{v\in (X\setminus \{\alpha^*(i_1),\alpha^*(i_2)\})}
|\textit{madj}^+_{\alpha^*}(v)|$.
To do so, we first show the following statement is true:
\begin{equation}\label{eq:46helper1:VvsL}
    |\mathcal{L}_{\alpha^*}(i)|= \ceil*{\frac{|V_{\textit{comp}_{\alpha^*}(i)}|}{2}} 
    \, \textit{ for every step } \, 
    i\in\{i_2+1,\dots,j\} \,
    \textit{ s.t.\ } \,
    \alpha^*(i)\in X
\end{equation}

For every step
$i\in\{i_2+1,\dots,j\}$ s.t. $\alpha^*(i)\in X$ we have that $|\mathcal{L}_{\alpha^*}(i)|\geq \ceil*{|V_{\textit{comp}_{\alpha^*}(i)}|/2}$ due to the fact that $|\mathcal{M}_{\alpha^*}(i)|\leq 2$.
Thus suppose for a contradiction that we can fix one such step $i\in\{i_2+1,\dots,j\}$ where $\alpha^*(i)\in X$ and $|\mathcal{L}_{\alpha^*}(i)|> \ceil*{|V_{\textit{comp}_{\alpha^*}(i)}|/2}$.
Let $|\mathcal{L}_{\alpha^*}(i)|= \ceil*{|V_{\textit{comp}_{\alpha^*}(i)}|/2}+k$, for some $k\geq 1$.
Below we consider 2 complementary cases and show that both cases lead to a contradiction as needed:

\begin{mycases}
    \case 
    {
    Suppose that $|\mathcal{M}_{\alpha^*}(i)|=2$.
    By \cref{cor:madjRooks} we have that $|\textit{madj}^+_{\alpha^*}({\alpha^*}(i))|=
    2n+2\ceil*{|V_{\textit{comp}_{\alpha^*}(i)}|/2}+
    2k-|V_{\textit{comp}_{\alpha^*}(i)}|$ 
    % 4n-2(n-\ceil{V/2}-k)-V
    % 4n-2n+2\ceil{V/2}+k-V
    % 2n+2\ceil{V/2}+2k-V
    which is clearly greater than $2n+1$.
    This contracts \cref{eq:4nConTw} as needed.
    }

    \case 
    {
    Suppose that $|\mathcal{M}_{\alpha^*}(i)|=1$.
    Let $i'\in\{i+1,\dots,j\}$ be the first step where ${\alpha^*}(i')\in X$
    % $V_{\textit{comp}_{\alpha^*}(i)}\subset V_{\textit{comp}_{\alpha^*}(i')}$
    and $\mathcal{M}_{\alpha^*}(i')=\{r,r'\}$.
    This step clearly exists as ${\alpha^*}(j)\in X$ and $\mathcal{M}_{\alpha^*}(j)=\{r,r'\}$.
    We point out that $i'$ is not necessarily different to $j$.

    Recall that $1\leq |\mathcal{V}_G(\alpha^*,n+2)\cap X|\leq 2$, so below we consider 2 complementary subcases.
    In both cases we show that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i'))|>2n+1$, contradicting \cref{eq:4nConTw} as needed:
    
    \begin{subcases}
        \subcase{
        Suppose that $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=2$.
        Then as discussed before
        $\mathcal{V}_G(\alpha^*,n+2)\cap X=
        \{\alpha^*(i_1),\alpha^*(i_2)\}$ so $\alpha^*(i_1)$ and $\alpha^*(i_2)$ must be from different rows of $\mathcal{M}_{\alpha^*}(j)=\{r,r'\}$.
        Since $\alpha^*(i)\in X$ and $i>i_2$, $\alpha^*(i)$ must be from the same row as either $\alpha^*(i_1)$ or $\alpha^*(i_2)$.
        W.l.o.g.\ assume that 
        $\alpha^*(i),\alpha^*(i_1)\in M_r$ and as a result 
        $\alpha^*(i_2)\in M_{r'}$.
        Then $\alpha^*(i_2)$ must be from a different column than both vertices $\alpha^*(i),\alpha^*(i_1)$ otherwise $\alpha^*(i_2)\in V_{\textit{comp}_{\alpha^*}(i)}$ implying that $\mathcal{M}_{\alpha^*}(i)=\{r,r'\}$, contradicting $|\mathcal{M}_{\alpha^*}(i)|=1$.
        Since $\mathcal{M}_{\alpha^*}(i')=\{r,r'\}$ we have that $(V_{\textit{comp}_{\alpha^*}(i)}\cup\{\alpha^*(i_2)\})\subset V_{\textit{comp}_{\alpha^*}(i')}$ as a result
        $|\mathcal{L}_{\alpha^*}(i')|\geq 3$.
        Moreover, since $i'$ is the first step where ${\alpha^*}(i')\in X$ and $|\mathcal{M}_{\alpha^*}(i')|=2$ we get that $|V_{\textit{comp}_{\alpha^*}(i')}|= |\mathcal{L}_{\alpha^*}(i')|+1$.
        This combined with \cref{cor:madjRooks} implies that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i'))|=
        2n+|\mathcal{L}_{\alpha^*}(i')|-1>2n+1$.
        % V_comp = \mathcal{L}+1 >=3
        % V_comp-1 = \mathcal{L}
        % \mathcal{R} = 2
        % madj = 4n - 2(n-\mathcal{L}) - (\mathcal{L}+1)
        % madj = 2n + 2\mathcal{L} - \mathcal{L} -1
        }
        
        \subcase{
        Suppose that $|\mathcal{V}_G(\alpha^*,n+2)\cap X|=1$, hence $\mathcal{V}_G(\alpha^*,n+2)\cap X=
        \{\alpha^*(i_1)\}$.
        Then in this case, $\alpha^*(i_2)$ either shares a column or a row with $\alpha^*(i_1)$.
        By selection, $i>i_2$ and $|\mathcal{M}_{\alpha^*}(i)|=1$ in this case, therefore $\alpha^*(i_2)$ cannot belong to the same column as $\alpha^*(i_1)$.
        So assume w.l.o.g.\ that $\alpha^*(i_1)$ and $\alpha^*(i_2)$ both belong to row $r$.
        Furthermore, $\alpha^*(i)$ cannot belong to row $r'$ as it will imply that $\mathcal{M}_{\alpha^*}(i)=\{r,r'\}$ or $\alpha^*(i)\in\mathcal{V}_G(\alpha^*,n+2)$ both of which leading to a contradiction.
        This shows that 
        $\alpha^*(i_1),\alpha^*(i_2),\alpha^*(i)\in M_r$ implying that $|\mathcal{L}_{\alpha^*}(i)|\geq 3$.
        As discussed in the previous subcase, since $i'$ is the first step where $|\mathcal{M}_{\alpha^*}(i')|=2$ we have that $|V_{\textit{comp}_{\alpha^*}(i')}|= |\mathcal{L}_{\alpha^*}(i')|+1$.
        Then because $V_{\textit{comp}_{\alpha^*}(i)}\subset V_{\textit{comp}_{\alpha^*}(i')}$, we necessarily have that $|\mathcal{L}_{\alpha^*}(i')|\geq 3$.
        So we can conclude using \cref{cor:madjRooks} that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i'))|=
        2n+|\mathcal{L}_{\alpha^*}(i')|-1>2n+1$.
        }
    \end{subcases}
    }
\end{mycases}

We have thus shown that both of the above cases lead to a contradiction with \cref{eq:4nConTw} thus proving \cref{eq:46helper1:VvsL}.

In order to determine $\sum_{v\in (X\setminus \{\alpha^*(i_1),\alpha^*(i_2)\})}
|\textit{madj}^+_{\alpha^*}(v)|$, fix a vertex $v\in (X\setminus \{\alpha^*(i_1),\alpha^*(i_2)\})$ and let $i$ be the step at which $v$ is eliminated in $\alpha^*$.
Note that by selection $i_2+1\leq i\leq j$ and $|V_{\textit{comp}_{\alpha^*}(i)}|\geq 2$ as $v\notin \mathcal{V}_G(\alpha^*,n+2)$.
By \cref{eq:46helper1:VvsL} we must have that $|\mathcal{M}_{\alpha^*}(i)|=2$, otherwise $|\mathcal{L}_{\alpha^*}(i)|=|V_{\textit{comp}_{\alpha^*}(i)}|$ which contradicts \cref{eq:46helper1:VvsL}.
% \todo[inline]{
% The proof is OK,
% the only change I would suggest is here:
% ``By \cref{eq:46helper1:VvsL} we must have that $|\mathcal{M}_{\alpha^*}(i)|=2$.'' [and remove the rest of the sentence—we already know that (6.25) is true, so it can be used here directly, the rest is fine!]
% }

Therefore, every vertex from $\alpha^*[1,i-1]\cap X$ must be contained within $V_{\textit{comp}_{\alpha^*}(i)}$.
This together with the fact that $|V_{\textit{comp}_{\alpha^*}(i_2)}|=2$ is even
shows that the number of such vertices $v\in (X\setminus \{\alpha^*(i_1),\alpha^*(i_2)\})$ where $|V_{\textit{comp}_{\alpha^*}(i)}|$ is even cannot exceed those where $|V_{\textit{comp}_{\alpha^*}(i)}|$ is odd.
This observation will be needed shortly, but first consider the following complementary cases in regard to $|V_{\textit{comp}_{\alpha^*}(i)}|$:
\begin{mycases}
    \case
    {
    Suppose that $|V_{\textit{comp}_{\alpha^*}(i)}|$ is odd.
    In this case, \cref{eq:46helper1:VvsL} implies that $|\mathcal{L}_{\alpha^*}(i)|= (|V_{\textit{comp}_{\alpha^*}(i)}|+1)/2$ and using \cref{cor:madjRooks} we can state that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=
    4n-2(n-(|V_{\textit{comp}_{\alpha^*}(i)}|+1)/2)-|V_{\textit{comp}_{\alpha^*}(i)}|
    =2n+1$.
    % 4n-2(n-(V+1)/2)-V=
    % 4n-2n+2(V+1)/2-V=
    % 4n-2n+V+1-V=
    }
    
    \case
    {
    Suppose that $|V_{\textit{comp}_{\alpha^*}(i)}|$ is even.
    Then by \cref{eq:46helper1:VvsL} we have that $|\mathcal{L}_{\alpha^*}(i)|= |V_{\textit{comp}_{\alpha^*}(i)}|/2$.
    Also, using \cref{cor:madjRooks} we can state that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=
    4n-2(n-|V_{\textit{comp}_{\alpha^*}(i)}|/2)-|V_{\textit{comp}_{\alpha^*}(i)}|
    =2n$.
    % 4n-2(n-(V/2))-2(V/2)=4n-2n+2(V/2)-2(V/2)
    }
\end{mycases}

By combining all above observations, we that:
$$
\sum_{v\in (X\setminus \{\alpha^*(i_1),\alpha^*(i_2)\})}
|\textit{madj}^+_{\alpha^*}(v)|=
\ceil*{\frac{|X|-2}{2}}(2n+1)+
\floor*{\frac{|X|-2}{2}}2n=
%2n(\ceil{(|X|-2)/2}+\floor{(|X|-2)/2}) + \ceil{(|X|-2)/2}
%2n(\ceil{|X|/2}+\floor{|X|/2}-2) + \ceil{(|X|-2)/2}
%2n(|X|-2) + \ceil{(|X|-2)/2}
%2n(|X|-2) + \ceil{|X|/2}-1
2n(|X|-2)+\ceil*{\frac{|X|}{2}}-1
$$

This together with \cref{eq:46helper1:i1i2} proves the statement of the lemma.
\end{proof}
}

% 4x6 helper 2
{
\begin{lemma}\label{lem:46helper2}
Let $G=(V,E)$ be a $K_4\square K_n$ for $n\geq 4$ and $\alpha^*$ be a nice elimination ordering over $G$ where $\mathcal{V}_G(\alpha^*,n+2)=
\alpha^*[1,|\mathcal{V}_G(\alpha^*,n+2)|]$ and $\textit{tw}(G^+_{\alpha^*})=\textit{tw}(G)$.
If there exists a step $j\in\{|\mathcal{V}_G(\alpha^*,n+2)|+1,\dots,2n-2\}$ s.t.\ $|\mathcal{M}_{\alpha^*}(j)|=3$ then we have $\sum_{v\in \alpha^*[1,2n-2]}|\textit{madj}^+_{\alpha^*}(v)|\geq 4n^2-6n+4$
\end{lemma}

\begin{proof}
As discussed prior to the proof of \cref{lem:46helper1}, given any $m\times n$ rook's graph $G$, for any $n\geq m\geq 2$, there exists a nice elimination ordering $\alpha^*$ over $G$ s.t.\ $\mathcal{V}_G(\alpha^*,n+m-2)=
\alpha^*[1,|\mathcal{V}_G(\alpha^*,n+m-2)|]$ and $\textit{tw}(G^+_{\alpha^*})=\textit{tw}(G)$.
Then clearly we can fix one such nice elimination ordering $\alpha^*$ over $G$ satisfying the statement of the lemma.

We know from \cref{lem:twRook} that $\textit{tw}(G)=2n+1$.
By \cref{lem:twEliminationHigherAdjacency}, the fact that $\textit{tw}(G^+_{\alpha^*})=\textit{tw}(G)=2n+1$ implies that:
\begin{equation}\label{eq:4n2ConTw}
    \max\nolimits_{v\in V}|\textit{madj}^+_{\alpha^*}(v)|
    \leq 2n+1
\end{equation}

In the first part of the proof, we provide some boundaries on  $|\mathcal{L}_{\alpha^*}(i)|, |\mathcal{M}_{\alpha^*}(i)|$ and $|V_{\textit{comp}_{\alpha^*}(i)}|$ for any step $i\in\{1,\dots,2n-2\}$.
Then, using these bounds, we proceed to prove the statement of the lemma.

First, we claim the following to be true:
\begin{equation}\label{eq:4n2ConAnyi}
    |\mathcal{L}_{\alpha^*}(i)|\leq n-1
    \textit{\,,\,\,}
    |\mathcal{M}_{\alpha^*}(i)|\leq 3
    \textit{\,\,and\,\,}
    |V_{\textit{comp}_{\alpha^*}(i)}|\leq 2n-2
    \textit{ \, for every $i\in\{1,\dots,2n-2\}$}
\end{equation}

It is easy to see that since $i\leq 2n-2$, we necessarily have that $|V_{\textit{comp}_{\alpha^*}(i)}|\leq 2n-2$.
To prove the rest, suppose for a contradiction that $|\mathcal{L}_{\alpha^*}(i)|=n$ or $|\mathcal{M}_{\alpha^*}(i)|=4$ for a fixed step $i\in\{1,\dots,2n-2\}$.
Then by \cref{cor:madjRooks} we get that $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=
4n-|V_{\textit{comp}_{\alpha^*}(i)}|\geq 2n+2$ contradicting \cref{eq:4n2ConTw}.
This proves \cref{eq:4n2ConAnyi} as needed.
% 4n-(2n-2)= 2n+2

Next let $i\in\{3,\dots,2n-2\}$ be a fixed step in $\alpha^*$ where $|\mathcal{M}_{\alpha^*}(i)|=3$ (clearly we cannot have $i<3$).
Let $i'\in\{3,\dots,i\}$ be the first step where $\mathcal{M}_{\alpha^*}(i')=\mathcal{M}_{\alpha^*}(i)$.
Note that by selection $i'$ is the first step in $\alpha^*$ where $|\mathcal{M}_{\alpha^*}(i')|=3$.
This is because for any earlier step $i''$,
$3\leq i''< i'$, s.t.\
$|\mathcal{M}_{\alpha^*}(i'')|=3$ we must have $V_{\textit{comp}_{\alpha^*}(i'')}\subset V_{\textit{comp}_{\alpha^*}(i')}$ therefore $\mathcal{M}_{\alpha^*}(i'')=\mathcal{M}_{\alpha^*}(i)$ contradicting the selection of step $i'$.

Since $|\mathcal{M}_{\alpha^*}(i')|=3$, using \cref{cor:madjRooks} and \cref{eq:4n2ConTw} we can state the following lower bound on $|V_{\textit{comp}_{\alpha^*}(i')}|$:
% n-1+L<=V
\begin{equation}\label{eq:46helper2:Li'andV:1}
    |V_{\textit{comp}_{\alpha^*}(i')}|\geq n-1+|\mathcal{L}_{\alpha^*}(i')|
\end{equation}

Next, let us determine an upper bound on $|V_{\textit{comp}_{\alpha^*}(i')}|$.
Since $i'$ is the first step with $|\mathcal{M}_{\alpha^*}(i')|=3$, there clearly can exist at most one column index $c^*\in\mathcal{L}_{\alpha^*}(i')$ s.t.\ $|L_{c^*}\cap V_{\textit{comp}_{\alpha^*}(i')}|=3$.
For every other column index $c\in (\mathcal{L}_{\alpha^*}(i')\setminus\{c^*\})$ we have $|L_{c}\cap V_{\textit{comp}_{\alpha^*}(i')}|\leq 2$.
As a result, we have that:
\begin{equation}\label{eq:46helper2:Li'andV:2}
    |V_{\textit{comp}_{\alpha^*}(i')}|\leq 2|\mathcal{L}_{\alpha^*}(i')|+1
\end{equation}

By combining \cref{eq:46helper2:Li'andV:1} and \cref{eq:46helper2:Li'andV:2} we have that $\mathcal{L}_{\alpha^*}(i')\geq n-2$.
% V>=n-1+L && V>=2L => 2L>=n-1+L =>L>=n-1
% V>=n-1+L && V>=2L+1 => 2L+1>=n-1+L =>L+1>=n-1 =>L>=n-2
%
% n-1+L <= 2L+1
% n-1 <= L+1
% n-2 <= L
%
Recall that $i\in\{3,\dots,2n-2\}$ was any fixed step in $\alpha^*$ where $|\mathcal{M}_{\alpha^*(i)}|=3$ and $i'\in\{3,\dots,i\}$ was the first step with  $\mathcal{M}_{\alpha^*(i')}=\mathcal{M}_{\alpha^*(i)}$ then we that
$\alpha^*(i')\in V_{\textit{comp}_{\alpha^*}(i)}$.
This implies that 
$V_{\textit{comp}_{\alpha^*}(i')}\subseteq V_{\textit{comp}_{\alpha^*}(i)}$ and so
$|\mathcal{L}_{\alpha^*}(i')|\leq |\mathcal{L}_{\alpha^*}(i)|$.
This combined with \cref{eq:4n2ConAnyi} implies that 
$n-2\leq |\mathcal{L}_{\alpha^*}(i)| \leq n-1$.
% n-2<= L<= n-1

Below we consider two possible cases in regard to $|\mathcal{L}_{\alpha^*}(i)|$ in order to discuss the value of $|V_{\textit{comp}_{\alpha^*}(i)}|$:
\begin{mycases}
    \case
    {
    % madj = 4n-(n-(n-2))-V<=2n+1
    % madj = 4n-2-V<=2n+1
    % madj = 2n-2-V<=1
    % madj = 2n-3<=V
    Suppose that $|\mathcal{L}_{\alpha^*}(i)|=n-2$.
    By \cref{cor:madjRooks}, $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=
    4n-2-|V_{\textit{comp}_{\alpha^*}(i)}|$ and by \cref{eq:4n2ConTw} we have that $|V_{\textit{comp}_{\alpha^*}(i)}|\geq 2n-3$.
    This combined with \cref{eq:4n2ConAnyi} implies that $2n-3\leq |V_{\textit{comp}_{\alpha^*}(i)}|\leq 2n-2$.
    }
    
    \case
    {
    % madj = 4n-(n-(n-1))-V<=2n+1
    % madj = 4n-1-V<=2n+1
    % madj = 2n-1-V<=1
    % madj = 2n-2<=V
    Suppose that $|\mathcal{L}_{\alpha^*}(i)|=n-1$.
    By \cref{cor:madjRooks} $|\textit{madj}^+_{\alpha^*}(\alpha^*(i))|=
    4n-1-|V_{\textit{comp}_{\alpha^*}(i)}|$ and by \cref{eq:4n2ConTw} we have that $|V_{\textit{comp}_{\alpha^*}(i)}|\geq 2n-2$.
    This combined with \cref{eq:4n2ConAnyi} necessarily implies that $|V_{\textit{comp}_{\alpha^*}(i)}|=2n-2$.
    }
\end{mycases}

The following statement summarizes our above observations:
\begin{equation}\label{eq:4n2Coni}
    \begin{split}
        & ( |\mathcal{L}_{\alpha^*}(i)|=n-1 \textit{\,\,and\,\,} |V_{\textit{comp}_{\alpha^*}(i)}|=2n-2 ) \\
        & \textit{or\,\,} 
        ( |\mathcal{L}_{\alpha^*}(i)|=n-2 \textit{\,\,and\,\,} 2n-3\leq|V_{\textit{comp}_{\alpha^*}(i)}|\leq2n-2 )\\
        & \textit{for any step\,\,} i\in\{3,\dots,2n-2\} \textit{\,\,s.t.\,\,}
        |\mathcal{M}_{\alpha^*}(i)|=3
    \end{split}
\end{equation}

Note that the selection of one such step $i$ in $\alpha^*$ with $|\mathcal{M}_{\alpha^*}(i)|=3$ is indeed very restricted due to the above conditions (i.e. $2n-3\leq i\leq 2n-2$).

Let $j$ be the fixed step in the statement of the lemma.
Since $|\mathcal{M}_{\alpha^*}(j)|=3$ the condition stated in \cref{eq:4n2Coni} must also hold for step $j$.
So in order to prove the statement of the lemma, we consider the following complementary cases:

\begin{mycases}
    \case
    {
    Suppose that $|\mathcal{L}_{\alpha^*}(j)|=n-2$.
    Let $\mathcal{M}_{\alpha^*}(j)=\{r_1,r_2,r_3\}$ and 
    $\mathcal{L}_{\alpha^*}(j)=\{c_1,\dots,c_{n-2}\}$ for distinct row indices $r_1,r_2,r_3\in\{1,\dots,4\}$ and column indices $c_1,\dots,c_{n-2}\in\{1,\dots,n\}$.
    By \cref{eq:4n2Coni} we have that $2n-3\leq |V_{\textit{comp}_{\alpha^*}(j)}|\leq 2n-2$.
    Below, we consider 2 complementary subcases and provide a lower bound for 
    $\sum_{v\in \alpha^*[1,2n-2]}
    |\textit{madj}^+_{\alpha^*}(v)|$:
    \begin{subcases}
    % Vj=2n-3, Lj=n-2, Mj=3
        \subcase
        {Suppose that $|V_{\textit{comp}_{\alpha^*}(j)}|=2n-3$.
        We first show that $j$ is the first step in $\alpha^*$ s.t.\ $|\mathcal{M}_{\alpha^*}(j)|=3$.
        To show this, suppose for a contradiction that there exists a step $i\in\{3,\dots,j-1\}$ s.t.\ $|\mathcal{M}_{\alpha^*}(i)|=3$.
        As discussed in the paragraph before \cref{eq:46helper2:Li'andV:1}, this implies that $\mathcal{M}_{\alpha^*}(i)= \mathcal{M}_{\alpha^*}(j)$ and so $V_{\textit{comp}_{\alpha^*}(i)}\subset V_{\textit{comp}_{\alpha^*}(j)}$.
        Consequently, $|V_{\textit{comp}_{\alpha^*}(i)}|\leq 2n-4$ 
        % and $|\mathcal{L}_{\alpha^*}(i)|\leq |\mathcal{L}_{\alpha^*}(j)|\leq n-2$
        which contradicts \cref{eq:4n2Coni} as desired.
        
        This shows that there are $(2n-4)$ vertices in 
        $V_{\textit{comp}_{\alpha^*}(j)}\setminus \{\alpha^*(j)\}$ spanned across at most $(n-2)$ columns and 3 rows with the recently proved condition that $j$ is the first step s.t.\ $|\mathcal{M}_{\alpha^*}(j)|=3$.
        It is then easy to see that there must exist a row index $r^*\in\{r_1,r_2,r_3\}$ s.t.\ $M_{r^*}\cap (V_{\textit{comp}_{\alpha^*}(j)}\setminus \{\alpha^*(j)\})=\emptyset$.
        % Fitting 2n-4 vertices in n-2 columns at most 2 rows 
        Assume w.l.o.g.\ that $r^*=r_3$ therefore $V_{\textit{comp}_{\alpha^*}(j)}\setminus \{\alpha^*(j)\}=
        \{v_{r,c}|r\in\{r_1,r_2\},c\in\{c_1,\dots,c_{n-2}\}\}$.
        
        Let $l\in\{1,\dots,j-1\}$ be the latest step in $\alpha^*$ where $\alpha^*(l)\in V_{\textit{comp}_{\alpha^*}(j)}$.% $i$
        By this selection, we have $V_{\textit{comp}_{\alpha^*}(l)}=
        V_{\textit{comp}_{\alpha^*}(j)}\setminus \{\alpha^*(j)\}=
        \{v_{r,c}|r\in\{r_1,r_2\},c\in\{c_1,\dots,c_{n-2}\}\}$ therefore $|\mathcal{M}_{\alpha^*}(l)|=2$.
        Therefore, by \cref{lem:minDegreeRook}, $\alpha^*(l)\notin \mathcal{V}_G(\alpha^*,n+2)$ and by selection of $\alpha^*$ we have that $l>|\mathcal{V}_G(\alpha^*,n+2)|$. 
        Hence, we can use \cref{lem:46helper1} to state that
        $\sum_{v\in V_{\textit{comp}_{\alpha^*}(l)}}
        |\textit{madj}^+_{\alpha^*}(v)|\geq 4n^2-9n+1$.
        % Mi=2 Vi=2n-4 Li=n-2
        % madj >= 2n(V-1)+\ceil{V/2}+3
        % madj >= 2n(2n-4-1)+\ceil{2n-4/2}+3
        % madj >= 2n(2n-5)+\ceil{n-2}+3
        % madj >= 2n(2n-5)+n-2+3
        % madj >= 2n(2n-5)+n+1
        % madj >= 4n^2-10n+n+1
        % madj >= 4n^2-9n+1
        % 2n+4+\ceil[((2n-4)-2)/2](2n+1)+\floor[((2n-4)-2)/2]2n
        % 2n+4+\ceil[(2n-6)/2](2n+1)+\floor[(2n-6)/2]2n
        % 2n+4+(n-3)(2n+1)+(n-3)2n
        % 2n+4+2n^2+n-6n-3+2n^2-6n
        % 2n+4+4n^2+n-6n-3-6n
        % 4+4n^2+n-6n-3-4n
        % 4+4n^2+n-3-10n
        % 4+4n^2-3-9n
        % 4n^2-9n+1
        Also, by \cref{cor:madjRooks} we have that $|\textit{madj}^+_{\alpha^*}(\alpha^*(j)|=2n+1$ as a result $\sum_{v\in V_{\textit{comp}_{\alpha^*}(j)}}
        |\textit{madj}^+_{\alpha^*}(v)|\geq 4n^2-7n+2$.

        Since $|V_{\textit{comp}_{\alpha^*}(j)}|=2n-3$ there exists exactly one step $i'\in\{1,\dots,2n-2\}$ where 
        $\alpha^*(i')\notin V_{\textit{comp}_{\alpha^*}(j)}$.
        Let $v_{r,c}=\alpha^*(i')$ for some row index $r\in\{1,\dots,4\}$ and column index $c\in\{1,\dots,n\}$.
        By \cref{eq:4n2ConAnyi}, $|\mathcal{M}_{\alpha^*}(i')|\neq 4$ thus either 
        $\{r\}=\{1,\dots,4\}\setminus\{r_1,r_2,r_3\}$ and $c\in \{1,\dots,n\}\setminus\{c_1,\dots,c_{n-2}\}$ in which case $|\textit{madj}^+_{\alpha^*}(v_{r,c})|\geq n+2$ or $r\in\{r_1,r_2,r_3\}$ where it is easy to check using \cref{cor:madjRooks} that $|\textit{madj}^+_{\alpha^*}(v_{r,c})|\geq 2n$.
        In conclusion, we have that $\sum_{v\in \alpha^*[1,2n-2]}|\textit{madj}^+_{\alpha^*}(v)|\geq 4n^2-6n+4$.
        % Vi'=2n-2, Li'=n-2 or Li'=n-1, Mi'=3
        % madji'= 4n-2-(2n-2) or
        % madji'= 4n-1-(2n-2)
        % madji'= 4n-2-2n+2 or
        % madji'= 4n-1-2n+2
        % madji'= 2n or
        % madji'= 2n+1
        }
        
        \subcase
        {
        % Vj=2n-2 Lj=n-2 Mj=3
        Suppose that $|V_{\textit{comp}_{\alpha^*}(j)}|=2n-2$.
        We note that this combined with the fact that $j\leq 2n-2$ implies that $j=2n-2$ and so $V_{\textit{comp}_{\alpha^*}(j)}= \alpha^*[1,2n-2]$.
        
        Contrary to the previous subcase, because $|V_{\textit{comp}_{\alpha^*}(j)}|=2n-2$, $|\mathcal{L}_{\alpha^*}(j)|=n-2$ and $|\mathcal{M}_{\alpha^*}(j)|=3$, it is easy to see that 
        $G[V_{\textit{comp}_{\alpha^*}(j)}\setminus \{\alpha^*(j)\}]$ is a connected subgraph with a vertex in every row from $\mathcal{M}_{\alpha^*}(j)=\{r_1,r_2,r_3\}$.
        In other words, we have that $|\mathcal{M}_{\alpha^*}(j-1)|=|\mathcal{M}_{\alpha^*}(j)|=3$.
        Clearly $|V_{\textit{comp}_{\alpha^*}(j-1)}|=
        |V_{\textit{comp}_{\alpha^*}(j)}|-1=2n-3$ and
        $|\mathcal{L}_{\alpha^*}(j-1)|\leq
        |\mathcal{L}_{\alpha^*}(j)|$.
        We cannot have $|\mathcal{L}_{\alpha^*}(j-1)|<|\mathcal{L}_{\alpha^*}(j)|=n-2$ as this contradicts \cref{eq:4n2Coni} so necessarily we have that $|\mathcal{L}_{\alpha^*}(j-1)|=n-2$.
        
        To recap, at step $j-1$ we have $\mathcal{M}_{\alpha^*}(j-1)=\mathcal{M}_{\alpha^*}(j)$,
        $|V_{\textit{comp}_{\alpha^*}(j-1)}|=2n-3$ and
        $|\mathcal{L}_{\alpha^*}(j-1)|=n-2$ which is the exact same premise of step $j$ in subcase (i) of case 1. 
        Therefore, we can state that $\sum_{v\in V_{\textit{comp}_{\alpha^*}(j-1)}}
        |\textit{madj}^+_{\alpha^*}(v)|\geq 4n^2-7n+2$.
        This, combined with the fact that $|\textit{madj}^+_{\alpha^*}(\alpha^*(j))|=2n$ (by \cref{cor:madjRooks}) implies that
        $\sum_{v\in V_{\textit{comp}_{\alpha^*}(j)}}
        |\textit{madj}^+_{\alpha^*}(v)|\geq 
        4n^2-5n+2$.
        Since $V_{\textit{comp}_{\alpha^*}(j)}=\alpha^*[1,2n-2]$ we have that
        $\sum_{v\in \alpha^*[1,2n-2]}|\textit{madj}^+_{\alpha^*}(v)|\geq 4n^2-5n+2$.
        }
    \end{subcases}
    
    The following statement summarizes our observation from the above 2 subcases:
    \begin{equation}\label{eq:4n2ConLjn2}
        \sum\nolimits_{v\in \alpha^*[1,2n-2]}|\textit{madj}^+_{\alpha^*}(v)|\geq
        4n^2-6n+4
        \textit{ \,\,if\,\, }
        |\mathcal{L}_{\alpha^*}(j)|=n-2
    \end{equation}
    }
    
    \case 
    {Suppose that $|\mathcal{L}_{\alpha^*}(j)|=n-1$.
    %madj=4n-1-V<=2n+1
    %then 2n-1-V<=1
    %then 2n-2<=V
    Then by \cref{cor:madjRooks} and \cref{eq:4n2ConTw} we have that 
    $|V_{\textit{comp}_{\alpha^*}(j)}|\leq 2n-2$ which combined with \cref{eq:4n2ConAnyi} implies that $|V_{\textit{comp}_{\alpha^*}(j)}|=2n-2$.
    By selection, $j\leq 2n-2$ which combined with the fact that  $|V_{\textit{comp}_{\alpha^*}(j)}|=2n-2$ implies that $j=2n-2$ and so $V_{\textit{comp}_{\alpha^*}(j)}= \alpha^*[1,2n-2]$.
    % Lj=n-1, Mj=3, Vj=2n-2
    
    %Lj-1<=n-1, Mj-1<=3, Vj-1<=2n-3
    %
    %(1) Lj-1=n-2, Mj-1=3, Vj-1=2n-3
    %(2) Lj-1<=n-1, Mj-1<3, Vj-1<=2n-3
    Clearly $|V_{\textit{comp}_{\alpha^*}(j-1)}|\leq 2n-3$ and by \cref{eq:4n2Coni} one of the following subcases must be true about $j-1$: 
    \begin{subcases}
        \subcase
        {$|\mathcal{M}_{\alpha^*}(j-1)|=3$, $|\mathcal{L}_{\alpha^*}(j-1)|=n-2$ and $|V_{\textit{comp}_{\alpha^*}(j-1)}|=2n-3$.
        It is previously shown (in subcase (i) of Case 1) that
        $\sum_{v\in V_{\textit{comp}_{\alpha^*}(j-1)}}
        |\textit{madj}^+_{\alpha^*}(v)|
        \geq 4n^2-7n+2$.
        Since $|\textit{madj}^+_{\alpha^*}(j)|=2n+1$ (by \cref{cor:madjRooks}) we can state that $\sum_{v\in\alpha^*[1,2n-2]}|\textit{madj}^+_{\alpha^*}(v)|
        \geq 4n^2-5n+3$.
        }

        \subcase
        {
% V_j = 2n-2
% L_j = n-1
% M_j = 3
% M_{j-1} is in less than 3 rows and has at most 2n-3 vertices
%
        $|\mathcal{M}_{\alpha^*}(j-1)|<3$,
        $|\mathcal{L}_{\alpha^*}(j-1)|\leq n-1$ and
        $|V_{\textit{comp}_{\alpha^*}(j-1)}|\leq 2n-3$.
        Let $\mathcal{L}_{\alpha^*}(j)=\{c_1,\dots,c_{n-1}\}$ and $\mathcal{M}_{\alpha^*}(j)=\{r_1,r_2,r_3\}$ for distinct column indices $c_1,\dots,c_{n-1}\in\{1,\dots,n\}$ and row indices $r_1,r_2,r_3\in\{1,\dots,4\}$.
        Since 
        $V_{\textit{comp}_{\alpha^*}(j-1)}\subset
        V_{\textit{comp}_{\alpha^*}(j)}$ it is easy to verify that one of the following scenarios must be true:
        \begin{itemize}
            \item[(a)] 
            $V_{\textit{comp}_{\alpha^*}(j-1)}\subset 
            \{v_{r,c}|r\in\{r_1,r_2\}, c\in\{c_1,\dots,c_{n-1}\}\}$
            
            \item[(b)] 
             $V_{\textit{comp}_{\alpha^*}(j-1)}=
            \{v_{r_3,c_{n-1}}\}\cup \{v_{r,c}|r\in\{r_1,r_2\}, c\in\{c_1,\dots,c_{n-2}\}\}$
        \end{itemize}
        
        By \cref{lem:46helper1} we have 
        $\sum_{v\in V_{\textit{comp}_{\alpha^*}(j-1)}}
        |\textit{madj}^+_{\alpha^*}(v)|\geq 4n^2-7n+2$ when (a) is true and 
        $\sum_{v\in V_{\textit{comp}_{\alpha^*}(j-1)}}
        |\textit{madj}^+_{\alpha^*}(v)|\geq 4n^2-8n+3$ given that (b) holds.
        % sum >= 2n+4+\ceil[((2n-3)-2)/2](2n+1)+
        % \floor[((2n-3)-2)/2]2n
        % sum >= 2n+4+\ceil[(2n-5)/2](2n+1)+
        % \floor[(2n-5)/2]2n
        % sum >= 2n+4+(2n-4)/2(2n+1)+
        % (2n-6)/2*2n
        % sum >= 2n+4+(n-2)(2n+1)+(n-3)*2n
        % sum >= 2n+4+(2n^2+n-4n-2)+(2n^2-6n)
        % sum >= 2n+4+2n^2+n-4n-2+2n^2-6n
        % sum >= 2n+4+4n^2+n-4n-2-6n
        % sum >= 3n+4+4n^2-4n-2-6n
        % sum >= 2+4n^2-4n-3n
        % sum >= 4n^2-7n+2
        %
        % sum >= 2n+4+\ceil[((2n-4)-2)/2](2n+1)+
        % \floor[((2n-4)-2)/2]2n+(n+4-2)
        % sum >= 2n+4+\ceil[(2n-6)/2](2n+1)+
        % \floor[(2n-6)/2]2n+(n+4-2)
        % sum >= 2n+4+(n-3)(2n+1)+(n-3)2n+(n+4-2)
        % sum >= 2n+4+(2n^2+n-6n-3)+2n^2-6n+n+2
        % sum >= 2n+2n^2+n-6n+2n^2-6n+n+3
        % sum >= 2n+4n^2+n-6n-6n+n+3
        % sum >= 4n^2+4n-12n+3
        % sum >= 4n^2-8n+3
        This, combined with the fact that $|\textit{madj}^+_{\alpha^*}(\alpha^*(j))|=2n+1$ 
        implies that 
        $\sum_{v\in\alpha^*[1,j]}
        |\textit{madj}^+_{\alpha^*}(v)|=
        \sum_{v\in\alpha^*[1,2n-2]}
        |\textit{madj}^+_{\alpha^*}(v)|
        \geq
        4n^2-6n+4$.
        }
    \end{subcases}
    
    Combining the above subcases, we can say that:
    \begin{equation}\label{eq:4n2ConLjn1}
        \sum\nolimits_{v\in \alpha^*[1,2n-2]}|\textit{madj}^+_{\alpha^*}(v)|\geq
        4n^2-6n+4
        \textit{ \,\,if\,\, }
        |\mathcal{L}_{\alpha^*}(j)|=n-1
    \end{equation}
    }
\end{mycases}
The statement of the lemma follows by combining \cref{eq:4n2ConLjn2} and \cref{eq:4n2ConLjn1}.
\end{proof}
}

% 4xn n>=6 rook
{
In contrast to the previous graphs discussed in this chapter, we show in the following theorem that the $\tau$ parameter is greater than 0 for the $4\times n$ rooks graphs, when $n\geq 6$.

\begin{theorem}\label{lem:46Rooktau}
Let $G=(V,E)$ be a $K_4\square K_n$ for $n\geq 6$.
Then there does not exit any minimum triangulation $H^*$ of $G$ with $\textit{tw}(H^*)=\textit{tw}(G)$.
As a consequence, we have that $\tau(G)>0$.
\end{theorem}

\begin{proof}
Since $G$ is a $4\times n$ rook's graph 
% $\kappa(G)=n+2$\todo{is $\kappa(G)$ mentioned/used somewhere in the proof?} and by \cref{lem:twRook} we have that $\textit{tw}(G)=2n+1$.

We begin the proof by defining an elimination ordering $\beta$ over $G$ s.t.\ $\textit{tw}(G^+_{\beta})>2n+1$.
Let us describe below how we aim to prove the statement of the theorem using $\beta$.

Suppose for a contradiction that there exists a minimum triangulation $H^*$ of $G$ with $\textit{tw}(H^*)=\textit{tw}(G)$.
Then we can fix a minimal triangulation $H$ of $G$ where $\textit{tw}(H)=2n+1$ and $|E_H|\leq|E_{G^+_{\beta}}|$ (note that $H$ is not necessarily a minimum triangulation of $G$).
Let $\alpha$ be a peo over $H$ therefore $G^+_\alpha=H$ and $|E_{G^+_\alpha}|=|E_H|\leq|E_{G^+_\beta}|$.
So in order to prove the statement of the theorem, it suffices to show that for every elimination ordering $\alpha$ over $G$ s.t.\ $\textit{tw}(G^+_{\alpha})=2n+1$, the triangulation $G^+_{\alpha}$ has more edges than $G^+_{\beta}$.
It is important to note that we do not claim $\beta$ to be a minimum elimination ordering, as we are only interested in showing that $|E_{G^+_\alpha}|>|E_{G^+_\beta}|$.

For every step $i\in\{1,\dots,\ceil*{\frac{n}{2}}-1\}$ let $\beta(i)=v_{1,i}$
% eliminate v_{1,1} to v_{1,\ceil((n-2)/2)}
% e.g. for 4x6: v_{1,1} to v_{1,2}
% e.g. for 4x7: v_{1,1} to v_{1,3}
and for $i\in\{\ceil*{\frac{n}{2}},\dots,n-2\}$ let $\beta(i)=v_{2,i}$.
% eliminate v_{2,\ceil((n-2)/2)}+1 to v_{2,n-2}
% e.g. for 4x6: v_{2,3} to v_{2,4}
% e.g. for 4x7: v_{2,4} to v_{2,5}
Next during the steps $i\in\{n-1,\dots,2(n-2)\}$ let $\beta$ eliminate the following vertices in this order:
$$ v_{2,1},\dots,v_{2,\ceil*{\frac{n}{2}}-1},
v_{1,\ceil*{\frac{n}{2}}},\dots,v_{1,n-2} $$

Afterwards let $\beta(2n-3)=v_{3,n-1}$ and $\beta(2n-2)=v_{4,n}$ and observe that the graph $G^\beta_{2n-2}$ is a complete graph on $2n+2$ vertices so let $\beta$ be any elimination ordering over $G^\beta_{2n-2}$ in the remaining vertices.

We have demonstrated $\beta$ over the $K_4\square K_6$ graph in \cref{fig:4nRooktau:Beta}. 

% fig Beta
{
\tikzset{
mystyle/.style={draw=black,rectangle, inner sep=0pt, text width=5mm, text height=1.75 mm,  align=right, fill=white}
}
\tikzset{
mystyle1/.style={draw=black,rectangle, inner sep=0pt, text width=5mm, text height=2.25 mm,  align=right, fill=white}
}
\begin{figure}
  \centering
    % \hspace{-2em}
    \begin{subfigure}[b]{0.45\textwidth}
        \begin{tikzpicture}[scale=0.65,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        \node [mystyle] (11) at (0,3)       {\tiny{$v_{1,1}\,\, $ }};
        \node [mystyle] (21) at (0.15,1.5)  {\tiny{$v_{2,1}\,\, $ }};
        \node [mystyle] (31) at (0.15,0)   {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5)    {\tiny{$v_{4,1}\,\, $ }};
        
        \node [mystyle] (12) at (2,3.15)       {\tiny{$v_{1,2}\,\, $ }};
        \node [mystyle] (22) at (2.15,1.65)  {\tiny{$v_{2,2}\,\, $ }};
        \node [mystyle] (32) at (1.85,0.15)   {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.35)    {\tiny{$v_{4,2}\,\, $ }};
        
        \node [mystyle] (13) at (4,2.75)       {\tiny{$v_{1,3}\,\, $ }};
        \node [mystyle] (23) at (4.15,1.25)  {\tiny{$v_{2,3}\,\, $ }};
        \node [mystyle] (33) at (3.85,-0.25)   {\tiny{$v_{3,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75)    {\tiny{$v_{4,3}\,\, $ }};
        
        \node [mystyle] (14) at (6,3.25)       {\tiny{$v_{1,4}\,\, $ }};
        \node [mystyle] (24) at (6.15,1.75)  {\tiny{$v_{2,4}\,\, $ }};
        \node [mystyle] (34) at (5.85,0.25)   {\tiny{$v_{3,4}\,\, $ }};
        \node [mystyle] (44) at (6,-1.25)    {\tiny{$v_{4,4}\,\, $ }};
        
        \node [mystyle] (15) at (8,2.85)       {\tiny{$v_{1,5}\,\, $ }};
        \node [mystyle] (25) at (8.15,1.35)  {\tiny{$v_{2,5}\,\, $ }};
        \node [mystyle] (35) at (7.85,-0.15)   {\tiny{$v_{3,5}\,\, $ }};
        \node [mystyle] (45) at (8,-1.65)    {\tiny{$v_{4,5}\,\, $ }};
        
        \node [mystyle] (16) at (10,3)       {\tiny{$v_{1,6}\,\, $ }};
        \node [mystyle] (26) at (10.15,1.5)  {\tiny{$v_{2,6}\,\, $ }};
        \node [mystyle] (36) at (10.15,0)   {\tiny{$v_{3,6}\,\, $ }};
        \node [mystyle] (46) at (10,-1.5)    {\tiny{$v_{4,6}\,\, $ }};

        
        \begin{scope}[on background layer]
            % \draw [draw=MyColorOne!70, rounded corners=5mm, fill=MyColorOne!70, line width=0pt, fill opacity=0.5, draw opacity=0.3]
            % %(21)--(12)--(14)--(41)
            % (0.25,2)--(1.5,3.25)--(6.5,3)--(0,-2)--cycle;
            
            
            % \draw [draw=MyColorOne!100, rounded corners=5mm, fill=MyColorOne!140, line width=5pt, fill opacity=0.7, draw opacity=0.7]
            % %(12)--(13)--(14)
            % (1.5,3.25)--(4,2.5)--(6.5,3)--cycle;
            % \draw [draw=MyColorOne!100, rounded corners=5mm, fill=MyColorOne!140, line width=5pt, fill opacity=0.7, draw opacity=0.7]
            % %(21)--(31)--(41)
            % (0.25,2)--(-0.5,0)--(0.25,-2)--cycle;
            
            \draw[-] 
                (11)--(21)
                (11)--(31)
                (11)--(41)
                (21)--(31)
                (21)--(41)
                (31)--(41)
                
                (12)--(22)
                (12)--(32)
                (12)--(42)
                (22)--(32)
                (22)--(42)
                (32)--(42)
                
                (13)--(23)
                (13)--(33)
                (13)--(43)
                (23)--(33)
                (23)--(43)
                (33)--(43)
                
                (14)--(24)
                (14)--(34)
                (14)--(44)
                (24)--(34)
                (24)--(44)
                (34)--(44)
                
                (15)--(25)
                (15)--(35)
                (15)--(45)
                (25)--(35)
                (25)--(45)
                (35)--(45)
                
                (16)--(26)
                (16)--(36)
                (16)--(46)
                (26)--(36)
                (26)--(46)
                (36)--(46)
                
                (11)--(12)
                (11)--(13)
                (11)--(14)
                (11)--(15)
                (11)--(16)
                (12)--(13)
                (12)--(14)
                (12)--(15)
                (12)--(16)
                (13)--(14)
                (13)--(15)
                (13)--(16)
                (14)--(15)
                (14)--(16)
                (15)--(16)
                
                (21)--(22)
                (21)--(23)
                (21)--(24)
                (21)--(25)
                (21)--(26)
                (22)--(23)
                (22)--(24)
                (22)--(25)
                (22)--(26)
                (23)--(24)
                (23)--(25)
                (23)--(26)
                (24)--(25)
                (24)--(26)
                (25)--(26)
                
                (31)--(32)
                (31)--(33)
                (31)--(34)
                (31)--(35)
                (31)--(36)
                (32)--(33)
                (32)--(34)
                (32)--(35)
                (32)--(36)
                (33)--(34)
                (33)--(35)
                (33)--(36)
                (34)--(35)
                (34)--(36)
                (35)--(36)
                
                (41)--(42)
                (41)--(43)
                (41)--(44)
                (41)--(45)
                (41)--(46)
                (42)--(43)
                (42)--(44)
                (42)--(45)
                (42)--(46)
                (43)--(44)
                (43)--(45)
                (43)--(46)
                (44)--(45)
                (44)--(46)
                (45)--(46)
                ;
            
        \end{scope}
        \end{tikzpicture}
    \caption{$G$}
    \label{fig:4nRookTau:G}   
    \end{subfigure}
    \hspace{3em}
    % \hfill\\
    \begin{subfigure}[b]{0.45\textwidth}
        \begin{tikzpicture}[scale=0.65,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        
        \node [mystyle] (21) at (0.15,1.5)  {\tiny{$v_{2,1}\,\, $ }};
        \node [mystyle] (31) at (-0.15,0)   {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5)    {\tiny{$v_{4,1}\,\, $ }};
        
        \node [mystyle] (22) at (2.15,1.65)  {\tiny{$v_{2,2}\,\, $ }};
        \node [mystyle] (32) at (1.85,0.15)   {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.35)    {\tiny{$v_{4,2}\,\, $ }};
        
        \node [mystyle] (13) at (4,2.75)       {\tiny{$v_{1,3}\,\, $ }};
        \node [mystyle] (23) at (4.15,1.25)  {\tiny{$v_{2,3}\,\, $ }};
        \node [mystyle] (33) at (3.85,-0.25)   {\tiny{$v_{3,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75)    {\tiny{$v_{4,3}\,\, $ }};
        
        \node [mystyle] (14) at (6,3.25)       {\tiny{$v_{1,4}\,\, $ }};
        \node [mystyle] (24) at (6.15,1.75)  {\tiny{$v_{2,4}\,\, $ }};
        \node [mystyle] (34) at (5.85,0.25)   {\tiny{$v_{3,4}\,\, $ }};
        \node [mystyle] (44) at (6,-1.25)    {\tiny{$v_{4,4}\,\, $ }};
        
        \node [mystyle] (15) at (8,2.85)       {\tiny{$v_{1,5}\,\, $ }};
        \node [mystyle] (25) at (8.15,1.35)  {\tiny{$v_{2,5}\,\, $ }};
        \node [mystyle] (35) at (7.85,-0.15)   {\tiny{$v_{3,5}\,\, $ }};
        \node [mystyle] (45) at (8,-1.65)    {\tiny{$v_{4,5}\,\, $ }};
        
        \node [mystyle] (16) at (10,3)       {\tiny{$v_{1,6}\,\, $ }};
        \node [mystyle] (26) at (10.15,1.5)  {\tiny{$v_{2,6}\,\, $ }};
        \node [mystyle] (36) at (10.15,0)   {\tiny{$v_{3,6}\,\, $ }};
        \node [mystyle] (46) at (10,-1.5)    {\tiny{$v_{4,6}\,\, $ }};

        
        \begin{scope}[on background layer]
            \draw [draw=MyColorOne!70, rounded corners=4mm, fill=MyColorOne!70, line width=0pt, fill opacity=0.5, draw opacity=0.3]
            %       (13)--(14)--(16)--(42)--(41)--(21)
            (4,2.75)--(6,3.25)--(10.5,3)--(2,-1.35)--(0,-1.5)--(0.15,1.5)--cycle;
            
            
            \draw [draw=MyColorOne!100, rounded corners=4mm, fill=MyColorOne!140, line width=9pt, fill opacity=0.7, draw opacity=0.7]
            %       (13)--(14)--(16)--(15)
            (4,2.75)--(6,3.25)--(10.5,3)--(8,2.85)--cycle;
            \draw [draw=MyColorOne!100, rounded corners=4mm, fill=MyColorOne!140, line width=3pt, fill opacity=0.7, draw opacity=0.7]
            %       (21)--(31)--(41)--(42)--(22)
            (-0.15,1.75)--(-0.5,0)--(-0.25,-1.75)--(2.35,-1.5)--(2.35,1.85)--cycle;
            
            \draw[-]
                (21)--(31)
                (21)--(41)
                (31)--(41)

                (22)--(32)
                (22)--(42)
                (32)--(42)
                
                (13)--(23)
                (13)--(33)
                (13)--(43)
                (23)--(33)
                (23)--(43)
                (33)--(43)
                
                (14)--(24)
                (14)--(34)
                (14)--(44)
                (24)--(34)
                (24)--(44)
                (34)--(44)
                
                (15)--(25)
                (15)--(35)
                (15)--(45)
                (25)--(35)
                (25)--(45)
                (35)--(45)
                
                (16)--(26)
                (16)--(36)
                (16)--(46)
                (26)--(36)
                (26)--(46)
                (36)--(46)

                (13)--(14)
                (13)--(15)
                (13)--(16)
                (14)--(15)
                (14)--(16)
                (15)--(16)
                
                (21)--(22)
                (21)--(23)
                (21)--(24)
                (21)--(25)
                (21)--(26)
                (22)--(23)
                (22)--(24)
                (22)--(25)
                (22)--(26)
                (23)--(24)
                (23)--(25)
                (23)--(26)
                (24)--(25)
                (24)--(26)
                (25)--(26)
                
                (31)--(32)
                (31)--(33)
                (31)--(34)
                (31)--(35)
                (31)--(36)
                (32)--(33)
                (32)--(34)
                (32)--(35)
                (32)--(36)
                (33)--(34)
                (33)--(35)
                (33)--(36)
                (34)--(35)
                (34)--(36)
                (35)--(36)
                
                (41)--(42)
                (41)--(43)
                (41)--(44)
                (41)--(45)
                (41)--(46)
                (42)--(43)
                (42)--(44)
                (42)--(45)
                (42)--(46)
                (43)--(44)
                (43)--(45)
                (43)--(46)
                (44)--(45)
                (44)--(46)
                (45)--(46)
                ;
            
        \end{scope}
        \end{tikzpicture}
    \caption{$G_2$}
    \label{fig:4nRookTau:G2}   
    \end{subfigure}
    \hspace{0.5em}
    \hfill\\
    \begin{subfigure}[b]{0.45\textwidth}
        \begin{tikzpicture}[scale=0.65,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        
        \node [mystyle] (21) at (0.15,1.5)  {\tiny{$v_{2,1}\,\, $ }};
        \node [mystyle] (31) at (-0.15,0)   {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5)    {\tiny{$v_{4,1}\,\, $ }};
        
        \node [mystyle] (22) at (2.15,1.65)  {\tiny{$v_{2,2}\,\, $ }};
        \node [mystyle] (32) at (1.85,0.15)   {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.35)    {\tiny{$v_{4,2}\,\, $ }};
        
        \node [mystyle] (13) at (4,2.75)       {\tiny{$v_{1,3}\,\, $ }};
        \node [mystyle] (33) at (3.85,-0.25)   {\tiny{$v_{3,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75)    {\tiny{$v_{4,3}\,\, $ }};
        
        \node [mystyle] (14) at (6,3.25)       {\tiny{$v_{1,4}\,\, $ }};
        \node [mystyle] (34) at (5.85,0.25)   {\tiny{$v_{3,4}\,\, $ }};
        \node [mystyle] (44) at (6,-1.25)    {\tiny{$v_{4,4}\,\, $ }};
        
        \node [mystyle] (15) at (8,2.85)       {\tiny{$v_{1,5}\,\, $ }};
        \node [mystyle] (25) at (8.15,1.35)  {\tiny{$v_{2,5}\,\, $ }};
        \node [mystyle] (35) at (7.85,-0.15)   {\tiny{$v_{3,5}\,\, $ }};
        \node [mystyle] (45) at (8,-1.65)    {\tiny{$v_{4,5}\,\, $ }};
        
        \node [mystyle] (16) at (10,3)       {\tiny{$v_{1,6}\,\, $ }};
        \node [mystyle] (26) at (10.15,1.5)  {\tiny{$v_{2,6}\,\, $ }};
        \node [mystyle] (36) at (10.15,0)   {\tiny{$v_{3,6}\,\, $ }};
        \node [mystyle] (46) at (10,-1.5)    {\tiny{$v_{4,6}\,\, $ }};

        
        \begin{scope}[on background layer]
            \draw [draw=MyColorOne!70, rounded corners=4mm, fill=MyColorOne!70, line width=4pt, fill opacity=0.5, draw opacity=0.3]
            %       (13)--(14)--(16)--(42)--(41)--(21)
            (3.75,2.75)--(6,3.25)--(10.5,3)--(2,-1.35)--(0,-1.5)--(0.15,1.5)--cycle;
            
            \draw [draw=MyColorOne!100, rounded corners=4mm, fill=MyColorOne!140, line width=9pt, fill opacity=0.7, draw opacity=0.7]
            %       (13)--(14)--(16)--(15)
            (4,2.75)--(6,3.25)--(10.5,3)--(8,2.85)--cycle;
            \draw [draw=MyColorOne!100, rounded corners=4mm, fill=MyColorOne!140, line width=3pt, fill opacity=0.7, draw opacity=0.7]
            %       (21)--(31)--(41)--(42)--(22)
            (-0.15,1.75)--(-0.5,0)--(-0.25,-1.75)--(2.35,-1.5)--(2.35,1.85)--cycle;
            
            
            \draw [draw=red!40, rounded corners=4mm, fill=red!40, line width=0pt, fill opacity=0.5, draw opacity=0.3]
            %       (13)--(14)--(26)--(44)--(43)--(21)
            (4,2.75)--(6,3.15)--(10.15,1.5)--(6,-1.25)--(4,-1.75)--(0.15,1.5)--cycle;
            
            
            \draw [draw=red!80, rounded corners=4mm, fill=red!100, line width=9pt, fill opacity=0.7, draw opacity=0.7]
            %       (21)--(22)--(26)--(25)
            (-0.15,1.5)--(2.15,1.65)--(10.5,1.5)--(8.5,1.35)--cycle;
            \draw [draw=red!80, rounded corners=4mm, fill=red!100, line width=8pt, fill opacity=0.7, draw opacity=0.7]
            %       (13)--(14)--(44)--(43)
            (4,2.85)--(6,3.35)--(6,-1.45)--(4,-1.95)--cycle;
            
            \draw[-]
                (21)--(31)
                (21)--(41)
                (31)--(41)

                (22)--(32)
                (22)--(42)
                (32)--(42)
                
                (13)--(33)
                (13)--(43)
                (33)--(43)
                
                (14)--(34)
                (14)--(44)
                (34)--(44)
                
                (15)--(25)
                (15)--(35)
                (15)--(45)
                (25)--(35)
                (25)--(45)
                (35)--(45)
                
                (16)--(26)
                (16)--(36)
                (16)--(46)
                (26)--(36)
                (26)--(46)
                (36)--(46)

                (13)--(14)
                (13)--(15)
                (13)--(16)
                (14)--(15)
                (14)--(16)
                (15)--(16)
                
                (21)--(22)
                (21)--(25)
                (21)--(26)
                (22)--(25)
                (22)--(26)
                (25)--(26)
                
                (31)--(32)
                (31)--(33)
                (31)--(34)
                (31)--(35)
                (31)--(36)
                (32)--(33)
                (32)--(34)
                (32)--(35)
                (32)--(36)
                (33)--(34)
                (33)--(35)
                (33)--(36)
                (34)--(35)
                (34)--(36)
                (35)--(36)
                
                (41)--(42)
                (41)--(43)
                (41)--(44)
                (41)--(45)
                (41)--(46)
                (42)--(43)
                (42)--(44)
                (42)--(45)
                (42)--(46)
                (43)--(44)
                (43)--(45)
                (43)--(46)
                (44)--(45)
                (44)--(46)
                (45)--(46)
                ;
            
        \end{scope}
        \end{tikzpicture}
    \caption{$G_4$}
    \label{fig:4nRookTau:G4}   
    \end{subfigure}
    \hspace{3em}
    % \hfill\\
    \begin{subfigure}[b]{0.45\textwidth}
        \begin{tikzpicture}[scale=0.65,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        
        \node [mystyle] (31) at (-0.15,0)   {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5)    {\tiny{$v_{4,1}\,\, $ }};

        \node [mystyle] (32) at (1.85,0.15)   {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.35)    {\tiny{$v_{4,2}\,\, $ }};
        
        \node [mystyle] (13) at (4,2.75)       {\tiny{$v_{1,3}\,\, $ }};
        \node [mystyle] (33) at (3.85,-0.25)   {\tiny{$v_{3,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75)    {\tiny{$v_{4,3}\,\, $ }};
        
        \node [mystyle] (14) at (6,3.25)       {\tiny{$v_{1,4}\,\, $ }};
        \node [mystyle] (34) at (5.85,0.25)   {\tiny{$v_{3,4}\,\, $ }};
        \node [mystyle] (44) at (6,-1.25)    {\tiny{$v_{4,4}\,\, $ }};
        
        \node [mystyle] (15) at (8,2.85)       {\tiny{$v_{1,5}\,\, $ }};
        \node [mystyle] (25) at (8.15,1.35)  {\tiny{$v_{2,5}\,\, $ }};
        \node [mystyle] (35) at (7.85,-0.15)   {\tiny{$v_{3,5}\,\, $ }};
        \node [mystyle] (45) at (8,-1.65)    {\tiny{$v_{4,5}\,\, $ }};
        
        \node [mystyle] (16) at (10,3)       {\tiny{$v_{1,6}\,\, $ }};
        \node [mystyle] (26) at (10.15,1.5)  {\tiny{$v_{2,6}\,\, $ }};
        \node [mystyle] (36) at (10.15,0)   {\tiny{$v_{3,6}\,\, $ }};
        \node [mystyle] (46) at (10,-1.5)    {\tiny{$v_{4,6}\,\, $ }};

        
        \begin{scope}[on background layer]
        % \draw [draw=MyColorOne!70, rounded corners=4mm, fill=MyColorOne!70, line width=4pt, fill opacity=0.5, draw opacity=0.3]
        % %       (13)--(14)--(16)--(42)--(41)--(21)
        % (3.75,2.75)--(6,3.25)--(10.5,3)--(2,-1.35)--(0,-1.5)--(0.15,1.5)--cycle;
        % \draw [draw=red!40, rounded corners=4mm, fill=red!40, line width=0pt, fill opacity=0.5, draw opacity=0.3]
        % %       (13)--(14)--(26)--(44)--(43)--(21)
        % (4,2.75)--(6,3.15)--(10.15,1.5)--(6,-1.25)--(4,-1.75)--(0.15,1.5)--cycle;
        \draw [draw=blue!40, rounded corners=4mm, fill=blue!40, line width=0pt, fill opacity=0.5, draw opacity=0.3]
        %           (31)--(41)--(43)--(44)--(26)--(16)--(14)--(13)
        (-0.35,0.25)--(-0.25,-1.75)--(4,-1.75)--(6,-1.5)--(10.35,1.25)--(10.25,3.25)--(6,3.25)--(4,2.75)--cycle;
            
        % \draw [draw=MyColorOne!100, rounded corners=4mm, fill=MyColorOne!140, line width=9pt, fill opacity=0.7, draw opacity=0.7]
        % %       (13)--(14)--(16)--(15)
        % (4,2.75)--(6,3.25)--(10.5,3)--(8,2.85)--cycle;
        % \draw [draw=MyColorOne!100, rounded corners=4mm, fill=MyColorOne!140, line width=3pt, fill opacity=0.7, draw opacity=0.7]
        % %       (21)--(31)--(41)--(42)--(22)
        % (-0.15,1.75)--(-0.5,0)--(-0.25,-1.75)--(2.35,-1.5)--(2.35,1.85)--cycle;
        
        % \draw [draw=red!80, rounded corners=4mm, fill=red!100, line width=9pt, fill opacity=0.7, draw opacity=0.7]
        % %       (21)--(22)--(26)--(25)
        % (-0.15,1.5)--(2.15,1.65)--(10.5,1.5)--(8.5,1.35)--cycle;
        % \draw [draw=red!80, rounded corners=4mm, fill=red!100, line width=8pt, fill opacity=0.7, draw opacity=0.7]
        % %       (13)--(14)--(44)--(43)
        % (4,2.85)--(6,3.35)--(6,-1.45)--(4,-1.95)--cycle;
        \draw [draw=blue!100, rounded corners=4mm, fill=blue!100, line width=0pt, fill opacity=0.6, draw opacity=0.6]
        %       (13)--(14)--(16)--(26)--(25)
        (3.25,2.75)--(6,3.5)--(10.5,3.25)--(10.5,1.25)--(8,1.15)--cycle;
        \draw [draw=blue!100, rounded corners=4mm, fill=blue!100, line width=0pt, fill opacity=0.6, draw opacity=0.6]
        %       (31)--(41)--(43)--(44)--(34)--(32)
        (-0.65,0.35)--(-0.45,-1.75)--(4.5,-2)--(6.45,-1.6)--(6.15,0.65)--(1.85,0.45)--cycle;
            
            \draw[-]
                (31)--(41)
                
                (32)--(42)
                
                (13)--(33)
                (13)--(43)
                (33)--(43)
                
                (14)--(34)
                (14)--(44)
                (34)--(44)
                
                (15)--(25)
                (15)--(35)
                (15)--(45)
                (25)--(35)
                (25)--(45)
                (35)--(45)
                
                (16)--(26)
                (16)--(36)
                (16)--(46)
                (26)--(36)
                (26)--(46)
                (36)--(46)

                (13)--(14)
                (13)--(15)
                (13)--(16)
                (14)--(15)
                (14)--(16)
                (15)--(16)
                
                (25)--(26)
                
                (31)--(32)
                (31)--(33)
                (31)--(34)
                (31)--(35)
                (31)--(36)
                (32)--(33)
                (32)--(34)
                (32)--(35)
                (32)--(36)
                (33)--(34)
                (33)--(35)
                (33)--(36)
                (34)--(35)
                (34)--(36)
                (35)--(36)
                
                (41)--(42)
                (41)--(43)
                (41)--(44)
                (41)--(45)
                (41)--(46)
                (42)--(43)
                (42)--(44)
                (42)--(45)
                (42)--(46)
                (43)--(44)
                (43)--(45)
                (43)--(46)
                (44)--(45)
                (44)--(46)
                (45)--(46)
                ;
            
        \end{scope}
        \end{tikzpicture}
    \caption{$G_6$}
    \label{fig:4nRookTau:G6}   
    \end{subfigure}
    \hfill\\
    \begin{subfigure}[b]{0.45\textwidth}
        \begin{tikzpicture}[scale=0.65,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        
        \node [mystyle] (31) at (-0.15,0)   {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5)    {\tiny{$v_{4,1}\,\, $ }};

        \node [mystyle] (32) at (1.85,0.15)   {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.35)    {\tiny{$v_{4,2}\,\, $ }};
        
        \node [mystyle] (33) at (3.85,-0.25)   {\tiny{$v_{3,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75)    {\tiny{$v_{4,3}\,\, $ }};
        
        \node [mystyle] (34) at (5.85,0.25)   {\tiny{$v_{3,4}\,\, $ }};
        \node [mystyle] (44) at (6,-1.25)    {\tiny{$v_{4,4}\,\, $ }};
        
        \node [mystyle] (15) at (8,2.85)       {\tiny{$v_{1,5}\,\, $ }};
        \node [mystyle] (25) at (8.15,1.35)  {\tiny{$v_{2,5}\,\, $ }};
        \node [mystyle] (35) at (7.85,-0.15)   {\tiny{$v_{3,5}\,\, $ }};
        \node [mystyle] (45) at (8,-1.65)    {\tiny{$v_{4,5}\,\, $ }};
        
        \node [mystyle] (16) at (10,3)       {\tiny{$v_{1,6}\,\, $ }};
        \node [mystyle] (26) at (10.15,1.5)  {\tiny{$v_{2,6}\,\, $ }};
        \node [mystyle] (36) at (10.15,0)   {\tiny{$v_{3,6}\,\, $ }};
        \node [mystyle] (46) at (10,-1.5)    {\tiny{$v_{4,6}\,\, $ }};

        
        \begin{scope}[on background layer]
        \draw [draw=blue!40, rounded corners=4mm, fill=blue!40, line width=0pt, fill opacity=0.5, draw opacity=0.3]
        %           (31)--(41)--(43)--(44)--(26)--(16)--(15)
        (-0.35,0.25)--(-0.25,-1.75)--(4,-1.75)--(6,-1.5)--(10.35,1.25)--(10.25,3.25)--(8,2.85)--cycle;
            
        \draw [draw=blue!100, rounded corners=4mm, fill=blue!100, line width=0pt, fill opacity=0.6, draw opacity=0.6]
        %       (15)--(16)--(26)--(25)
        (7.65,3.15)--(10.5,3.25)--(10.5,1.25)--(7.65,1)--cycle;
        \draw [draw=blue!100, rounded corners=4mm, fill=blue!100, line width=0pt, fill opacity=0.6, draw opacity=0.6]
        %       (31)--(41)--(43)--(44)--(34)--(32)
        (-0.65,0.35)--(-0.45,-1.75)--(4.5,-2)--(6.45,-1.6)--(6.15,0.65)--(1.85,0.45)--cycle;
            
            \draw[-]
                (31)--(41)
                
                (32)--(42)
                
                (33)--(43)
                
                (34)--(44)
                
                (15)--(25)
                (15)--(35)
                (15)--(45)
                (25)--(35)
                (25)--(45)
                (35)--(45)
                
                (16)--(26)
                (16)--(36)
                (16)--(46)
                (26)--(36)
                (26)--(46)
                (36)--(46)

                (15)--(16)
                
                (25)--(26)
                
                (31)--(32)
                (31)--(33)
                (31)--(34)
                (31)--(35)
                (31)--(36)
                (32)--(33)
                (32)--(34)
                (32)--(35)
                (32)--(36)
                (33)--(34)
                (33)--(35)
                (33)--(36)
                (34)--(35)
                (34)--(36)
                (35)--(36)
                
                (41)--(42)
                (41)--(43)
                (41)--(44)
                (41)--(45)
                (41)--(46)
                (42)--(43)
                (42)--(44)
                (42)--(45)
                (42)--(46)
                (43)--(44)
                (43)--(45)
                (43)--(46)
                (44)--(45)
                (44)--(46)
                (45)--(46)
                ;
            
        \end{scope}
        \end{tikzpicture}
    \caption{$G_8$}
    \label{fig:4nRookTau:G8}   
    \end{subfigure}
    \hspace{3em}
    \begin{subfigure}[b]{0.45\textwidth}
        \begin{tikzpicture}[scale=0.65,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        
        \node [mystyle] (31) at (-0.15,0)   {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5)    {\tiny{$v_{4,1}\,\, $ }};

        \node [mystyle] (32) at (1.85,0.15)   {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.35)    {\tiny{$v_{4,2}\,\, $ }};
        
        \node [mystyle] (33) at (3.85,-0.25)   {\tiny{$v_{3,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75)    {\tiny{$v_{4,3}\,\, $ }};
        
        \node [mystyle] (34) at (5.85,0.25)   {\tiny{$v_{3,4}\,\, $ }};
        \node [mystyle] (44) at (6,-1.25)    {\tiny{$v_{4,4}\,\, $ }};
        
        \node [mystyle] (15) at (8,2.85)       {\tiny{$v_{1,5}\,\, $ }};
        \node [mystyle] (25) at (8.15,1.35)  {\tiny{$v_{2,5}\,\, $ }};
        \node [mystyle] (45) at (8,-1.65)    {\tiny{$v_{4,5}\,\, $ }};
        
        \node [mystyle] (16) at (10,3)       {\tiny{$v_{1,6}\,\, $ }};
        \node [mystyle] (26) at (10.15,1.5)  {\tiny{$v_{2,6}\,\, $ }};
        \node [mystyle] (36) at (10.15,0)   {\tiny{$v_{3,6}\,\, $ }};
        \node [mystyle] (46) at (10,-1.5)    {\tiny{$v_{4,6}\,\, $ }};

        
        \begin{scope}[on background layer]
        \draw [draw=blue!40, rounded corners=4mm, fill=blue!40, line width=0pt, fill opacity=0.5, draw opacity=0.3]
        %           (31)--(41)--(43)--(44)--(26)--(16)--(15)
        (-0.35,0.25)--(-0.25,-1.75)--(4,-1.75)--(6,-1.5)--(10.35,1.25)--(10.25,3.25)--(8,2.85)--cycle;
            
        \draw [draw=blue!100, rounded corners=4mm, fill=blue!100, line width=0pt, fill opacity=0.6, draw opacity=0.6]
        %       (15)--(16)--(26)--(25)
        (7.65,3.15)--(10.5,3.25)--(10.5,1.25)--(7.65,1)--cycle;
        \draw [draw=blue!100, rounded corners=4mm, fill=blue!100, line width=0pt, fill opacity=0.6, draw opacity=0.6]
        %       (31)--(41)--(43)--(44)--(34)--(32)
        (-0.65,0.35)--(-0.45,-1.75)--(4.5,-2)--(6.45,-1.6)--(6.15,0.65)--(1.85,0.45)--cycle;
        
        
        \draw [draw=orange!40, rounded corners=4mm, fill=orange!40, line width=0pt, fill opacity=0.5, draw opacity=0.3]
        %           (31)--(15)--(36)--(45)
        (-0.15,0)--(8,2.85)--(10.15,0)--(8,-1.65)--cycle;
        
        \draw [draw=orange!100, rounded corners=4mm, fill=orange!100, line width=5pt, fill opacity=0.9, draw opacity=0.8]
        %       (31)--(32)--(34)--(36)--(35)--(33)
       (-1,0)--(1.85,0.35)--(5.85,0.5)--(10.75,0)--(7.8,-0.5)--(3.85,-0.5)--cycle;
        \draw [draw=orange!100, rounded corners=4mm, fill=orange!100, line width=5pt, fill opacity=0.9, draw opacity=0.8]
        %       (15)--(25)--(45)
       (7.9,3.15)--(8.4,1.65)--(7.9,-2.15)--cycle;
            
        %darkgray
            \draw[-]
                (31)--(41)
                
                (32)--(42)
                
                (33)--(43)
                
                (34)--(44)
                
                (15)--(25)
                (15)--(45)
                (25)--(45)
                
                (16)--(26)
                (16)--(36)
                (16)--(46)
                (26)--(36)
                (26)--(46)
                (36)--(46)

                (15)--(16)
                
                (25)--(26)
                
                (31)--(32)
                (31)--(33)
                (31)--(34)
                (31)--(36)
                (32)--(33)
                (32)--(34)
                (32)--(36)
                (33)--(34)
                (33)--(36)
                (34)--(36)
                
                (41)--(42)
                (41)--(43)
                (41)--(44)
                (41)--(45)
                (41)--(46)
                (42)--(43)
                (42)--(44)
                (42)--(45)
                (42)--(46)
                (43)--(44)
                (43)--(45)
                (43)--(46)
                (44)--(45)
                (44)--(46)
                (45)--(46)
                ;
            
        \end{scope}
        \end{tikzpicture}
    \caption{$G_9$}
    \label{fig:4nRookTau:G9}   
    \end{subfigure}
    \hfill\\\hfill\\
    \begin{subfigure}[b]{0.45\textwidth}
        \begin{tikzpicture}[scale=0.65,every node/.style={draw=black,rectangle, inner sep=0pt, text width=7mm, text height=1.75 mm,  align=right}]
        
        \node [mystyle] (31) at (-0.15,0)   {\tiny{$v_{3,1}\,\, $ }};
        \node [mystyle] (41) at (0,-1.5)    {\tiny{$v_{4,1}\,\, $ }};

        \node [mystyle] (32) at (1.85,0.15)   {\tiny{$v_{3,2}\,\, $ }};
        \node [mystyle] (42) at (2,-1.35)    {\tiny{$v_{4,2}\,\, $ }};
        
        \node [mystyle] (33) at (3.85,-0.25)   {\tiny{$v_{3,3}\,\, $ }};
        \node [mystyle] (43) at (4,-1.75)    {\tiny{$v_{4,3}\,\, $ }};
        
        \node [mystyle] (34) at (5.85,0.25)   {\tiny{$v_{3,4}\,\, $ }};
        \node [mystyle] (44) at (6,-1.25)    {\tiny{$v_{4,4}\,\, $ }};
        
        \node [mystyle] (15) at (8,2.85)       {\tiny{$v_{1,5}\,\, $ }};
        \node [mystyle] (25) at (8.15,1.35)  {\tiny{$v_{2,5}\,\, $ }};
        \node [mystyle] (45) at (8,-1.65)    {\tiny{$v_{4,5}\,\, $ }};
        
        \node [mystyle] (16) at (10,3)       {\tiny{$v_{1,6}\,\, $ }};
        \node [mystyle] (26) at (10.15,1.5)  {\tiny{$v_{2,6}\,\, $ }};
        \node [mystyle] (36) at (10.15,0)   {\tiny{$v_{3,6}\,\, $ }};

        
        \begin{scope}[on background layer]
        \draw [draw=blue!40, rounded corners=4mm, fill=blue!40, line width=0pt, fill opacity=0.5, draw opacity=0.3]
        %           (31)--(41)--(43)--(44)--(26)--(16)--(15)
        (-0.35,0.25)--(-0.25,-1.75)--(4,-1.75)--(6,-1.5)--(10.35,1.25)--(10.25,3.25)--(8,2.85)--cycle;
            
        \draw [draw=blue!100, rounded corners=4mm, fill=blue!100, line width=0pt, fill opacity=0.6, draw opacity=0.6]
        %       (15)--(16)--(26)--(25)
        (7.65,3.15)--(10.5,3.25)--(10.5,1.25)--(7.65,1)--cycle;
        \draw [draw=blue!100, rounded corners=4mm, fill=blue!100, line width=0pt, fill opacity=0.6, draw opacity=0.6]
        %       (31)--(41)--(43)--(44)--(34)--(32)
        (-0.65,0.35)--(-0.45,-1.75)--(4.5,-2)--(6.45,-1.6)--(6.15,0.65)--(1.85,0.45)--cycle;
        
        \draw [draw=orange!40, rounded corners=4mm, fill=orange!40, line width=0pt, fill opacity=0.5, draw opacity=0.3]
        %           (31)--(15)--(36)--(45)
        (-0.15,0)--(8,2.85)--(10.15,0)--(8,-1.65)--cycle;
        
        \draw [draw=orange!100, rounded corners=4mm, fill=orange!100, line width=5pt, fill opacity=0.9, draw opacity=0.8]
        %       (31)--(32)--(34)--(36)--(35)--(33)
       (-1,0)--(1.85,0.35)--(5.85,0.5)--(10.75,0)--(7.8,-0.5)--(3.85,-0.5)--cycle;
        \draw [draw=orange!100, rounded corners=4mm, fill=orange!100, line width=5pt, fill opacity=0.9, draw opacity=0.8]
        %       (15)--(25)--(45)
       (7.9,3.15)--(8.4,1.65)--(7.9,-2.15)--cycle;
       
        \draw [draw=darkgray!50, rounded corners=4mm, fill=darkgray!50, line width=0pt, fill opacity=0.6, draw opacity=0.4]
        %           (41)--(42)--(44)--(16)--(26)--(36)
        %--(45)--(43)
        (-0.25,-1.5)--(2,-1.15)--(6,-1)--(10,3.5)--(10.15,1.5)--(10.15,0)
        --(8.25,-1.85)--(4,-2)--cycle;
        
        \draw [draw=darkgray!80, rounded corners=4mm, fill=darkgray!80, line width=2pt, fill opacity=0.8, draw opacity=0.8]
        %           (41)--(42)--(44)--(45)--(43)
        (-0.75,-1.5)--(2,-1.15)--(6,-1)--(8.65,-1.85)--(4,-2)--cycle;
        \draw [draw=darkgray!80, rounded corners=4mm, fill=darkgray!80, line width=2pt, fill opacity=0.8, draw opacity=0.8]
        %       (16)--(26)--(36)
        (9.85,3.65)--(10.5,1.5)--(9.85,-0.65)--cycle;
            
        %darkgray
            \draw[-]
                (31)--(41)
                
                (32)--(42)
                
                (33)--(43)
                
                (34)--(44)
                
                (15)--(25)
                (15)--(45)
                (25)--(45)
                
                (16)--(26)
                (16)--(36)
                (26)--(36)

                (15)--(16)
                
                (25)--(26)
                
                (31)--(32)
                (31)--(33)
                (31)--(34)
                (31)--(36)
                (32)--(33)
                (32)--(34)
                (32)--(36)
                (33)--(34)
                (33)--(36)
                (34)--(36)
                
                (41)--(42)
                (41)--(43)
                (41)--(44)
                (41)--(45)
                (42)--(43)
                (42)--(44)
                (42)--(45)
                (43)--(44)
                (43)--(45)
                (44)--(45)
                ;
            
        \end{scope}
        \end{tikzpicture}
    \caption{$G_{10}$}
    \label{fig:4nRookTau:G10}   
    \end{subfigure}
    \caption{
    (a) depicts the $4\times 6$ rook's graph $G$ and the following figures demonstrate how the elimination ordering $\beta$, defined in \cref{lem:46Rooktau}, eliminates the vertices of $G$.
    (b) depicts the graph $G_2$ obtained from $G$ by elimination of vertices $v_{1,1},v_{1,2}$, thus turning $N_G(\{v_{1,1},v_{1,2}\})$ into a clique.
    For simplicity, we have not drawn the added edges $\textit{fill}_G\,(N_G(\{v_{1,1},v_{1,2}\}))$ and instead highlighted $N_G(\{v_{1,1},v_{1,2}\})$ in light green.
    (c) depicts $G_4$ where the clique $N_{G_2}(\{v_{2,3},v_{2,4}\})$ is highlighted in red.
    (d) depicts $G_6$ where the clique $N_{G_4}(\{v_{2,1},v_{2,2}\})$ is highlighted in blue.
    (e) shows $G_8$ with the clique $N_{G_6}(\{v_{1,3},v_{1,4}\})$ in blue.
    (f) demonstrates the graph $G_9$ obtained from $G_8$ by elimination of $v_{3,5}$ and the clique $N_{G_8}(v_{3,5})$ is in orange.
    Finally, in (g) we have the graph $G_{10}$ obtained from $G_9$ by elimination of $v_{4,6}$ and the clique $N_{G_9}(v_{4,6})$ is in grey.
    }
    \label{fig:4nRooktau:Beta}
\end{figure}
}

Let us first determine $\textit{tw}(G^+_\beta)$ and $|E_{G^+_\beta}|$.
It is easy to see that $\mathcal{M}_{\beta}(i)=\{1\}$ for every step $i\in\{1,\dots,\ceil*{\frac{n}{2}}-1\}$, i.e.,\ $V_{\textit{comp}_\beta(i)}$ is contained within $M_1$.
This clearly implies that $V_{\textit{comp}_\beta(i)}=\beta[1,i]$ and $|V_{\textit{comp}_\beta(i)}|=|\mathcal{L}_{\beta}(i)|$.
So using \cref{cor:madjRooks} we can state that 
$|\textit{madj}^+_\beta(\beta(i))| = 3i+n-i$.
By getting the sum over the first $(\ceil*{\frac{n}{2}}-1)$ steps, we can state that 
$\sum_{v\in \beta[1,\ceil*{\frac{n}{2}}-1]}
|\textit{madj}^+_{\beta}(v)|=
\sum_{i=1}^{\ceil*{\frac{n}{2}}-1}(2i+n)=
% n(\ceil*{\frac{n}{2}}-1) + \sum_{i=1}^{\ceil*{\frac{n}{2}}-1}(2i)=
% n(\ceil*{\frac{n}{2}}-1) + 2\sum_{i=1}^{\ceil*{\frac{n}{2}}-1}i=
% n(\ceil*{\frac{n}{2}}-1) + (\ceil*{\frac{n}{2}}-1)\ceil*{\frac{n}{2}}=
(\ceil*{\frac{n}{2}}-1)(n+\ceil*{\frac{n}{2}})
$.
Note that by construction
$\max_{v\in \beta[1,\ceil*{\frac{n}{2}}-1]}
|\textit{madj}^+_{\beta}(v)|=
2(\ceil*{\frac{n}{2}}-1)+n
% if n is odd: 2((n+1)/2 -1)+n = ((n+1) -2)+n = (n -1)+n = 2n-1
% if n is even: 2(n/2 -1)+n = (n-2)+n = 2n-2
\leq 2n-1$.

Using the same logic as above, we have that
$\sum_{v\in \beta[\ceil*{\frac{n}{2}},n-2]}
|\textit{madj}^+_{\beta}(v)|=
\sum_{i=1}^{\floor*{\frac{n}{2}}-1}(2i+n)=
% n(\floor*{\frac{n}{2}}-1)+\sum_{i=1}^{\floor*{\frac{n}{2}}-1}(2i)=
% n(\floor*{\frac{n}{2}}-1)+2\sum_{i=1}^{\floor*{\frac{n}{2}}-1}i=
% n(\floor*{\frac{n}{2}}-1)+(\floor*{\frac{n}{2}}-1)\floor*{\frac{n}{2}}=
(\floor*{\frac{n}{2}}-1)(n+\floor*{\frac{n}{2}})
$ and 
$\max_{v\in \beta[\ceil*{\frac{n}{2}},n-2]}
|\textit{madj}^+_{\beta}(v)|=
2(\floor*{\frac{n}{2}}-1)+n\leq 2n-2$.

By construction $\beta(n-1)=v_{2,1}$ which shares a column with $\beta(1)=v_{1,1}$ and a row with $\beta(\ceil{\frac{n}{2}})=v_{2,\ceil{\frac{n}{2}}}$.
Then because every row in $G$ is a clique, $V_{\textit{comp}_{\beta}(i)}$, for every step $i\in\{n-1,\dots,2n-4\}$, will contain every previously eliminated vertex from rows 1 and 2.
Formally, for any fixed step $i\in\{n-1,\dots,2n-4\}$ we have that:
$\mathcal{M}_\beta(i)=\{1,2\}$, $\mathcal{L}_\beta(i)=\{1,\dots,n-2\}$ and $V_{\textit{comp}_{\beta}(i)}=\beta[1,i]$.
As a consequence, using \cref{cor:madjRooks} we can state that $|\textit{madj}^+_\beta(\beta(i))|=4n-4-i$ for every such step.
% madji = 4n-(m-2)(n-(n-2))-|V_{\textit{comp}_{\beta}(i)}|= 4n-4-i
Then by getting the sum over steps $n-1$ to $2n-4$ we have that 
$\sum_{v\in \beta[n-1,2n-4]}|\textit{madj}^+_\beta(v)|=
\sum_{i=0}^{n-3}(2n+i)=
% 2n + \sum_{i=1}^{n-3}(2n+i)=
% 2n + 2n(n-3) + \sum_{i=1}^{n-3}(i)=
% 2n + 2n^2-6n + \sum_{i=1}^{n-3}(i)=
% 2n^2-4n + (n-3)(n-2)/2=
2n^2-4n +\frac{(n-3)(n-2)}{2}$.
This is due to the fact that when $i=n-1$ we get that $|\textit{madj}_\beta^+(\beta(i))|=2n+n-3$ and when
$i=2n-4$ we have that $|\textit{madj}_\beta^+(\beta(i))|=2n+0$.
We also have that 
$\max_{v\in\beta[n-1,\dots,2n-4]}
|\textit{madj}^+_\beta(v)|=
|\textit{madj}^+_\beta(\beta(n-1))|=
3n-3$.
Due to \cref{lem:twEliminationHigherAdjacency} and the fact that $n\geq 6$, we have that $\textit{tw}(G^+_\beta)=3n-2>\textit{tw}(G)=2n+1$ as discussed earlier.

By construction, $\beta(i)$ for any step $i\in\{2n-3,2n-2\}$ does not share a row or a column with any of the previously eliminated vertices, i.e.,\ $|\mathcal{M}_\beta(i)|=|\mathcal{L}_\beta(i)|=|V_{\textit{comp}_\beta(i)}|=1$.
So by \cref{cor:madjRooks} we have that
$\sum_{v\in\beta[2n-3,2n-2]}|\textit{madj}^+_\beta(v)|=2(n+2)$ and $\max_{v\in\beta[2n-3,2n-2]}|\textit{madj}^+_\beta(v)|=n+2$.

As previously mentioned, the graph $G^\beta_{2n-2}$ is a $K_{2n+2}$ so 
$\sum_{v\in\beta[2n-1,4n]}
|\textit{madj}^+_\beta(v)|=
\sum_{i=1}^{2n+1}i=
% \frac{(2n+1)(2n+2)}{2}=
(2n+1)(n+1)
$ 
and 
$\max_{v\in\beta[2n-1,4n]}
|\textit{madj}^+_\beta(v)|
=2n+1$.

We summarize our construction of $\beta$ by stating that 
$\max_{v\in V}
|\textit{madj}^+_\beta(v)|= 
3n-3> 2n+1=
\textit{tw}(G)
$ and:


\begin{equation}\label{eq:4nLemmaSumBeta}
\sum\nolimits_{v\in V}
|\textit{madj}^+_\beta(v)|=
|E_{G^+_\beta}|= 
    \begin{cases}
    % (2((n/2)-1)(n+(n/2)))+(2n^2-4n+((n-3)(n-2)/2))+(2(n+2))+((2n+1)(n+1))
    % \text{\,\, if $n$ is even}
    % (2((n/2)-1)(n+(n/2)))+(2n^2-4n+((n-3)(n-2)/2))+(2(n+2))+((2n+1)(n+1))
    % \text{\,\, if $n$ is even}
    % (2((n-2)/2)(3n/2))+(2n^2-4n+((n^2-5n+6)/2))+(2n+4)+(2n^2+3n+1)
    % \text{\,\, if $n$ is even}
    % ((3n^2-6n)/2)+((4n^2-8n+n^2-5n+6)/2)+((4n+8)/2)+((4n^2+6n+2)/2)
    % \text{\,\, if $n$ is even}
    % (3n^2-6n+4n^2-8n+n^2-5n+6+4n+8+4n^2+6n+2)/2
    % \text{\,\, if $n$ is even}
    % (12n^2-9n+16)/2
    % \text{\,\, if $n$ is even}
    % 6n^2+(-8n-n)/2 +8
    % \text{\,\, if $n$ is even}
    6n^2-4n-\frac{n}{2} +8
    \text{\,\, if $n$ is even}
    % 4n^2+2n+2-\frac{n}{2} \text{\,\, if $n$ is even}
    \\
    % ((n+1)/2 -1)(n+ (n+1)/2) + ((n-1)/2 -1)(n+ (n-1)/2) +
    % 2n^2-4n+ (n-3)(n-2)/2 + 2(n+2) + (2n+1)(n+1)
    % \text{\,\, otherwise}
    % ((n-1)/2)((3n+1)/2) + ((n-3)/2)((3n-1)/2) +
    % (4n^2-8n)/2 + ((n^2-5n+6)/2) + (4n+8)/2 + (4n^2+6n+2)/2
    % \text{\,\, otherwise}
    % ((3n^2+n-3n-1)/4) + ((3n^2-10n+3)/4) +
    % (8n^2-16n)/4 + ((2n^2-10n+12)/4) + (8n+16)/4 + (8n^2+12n+4)/2
    % \text{\,\, otherwise}
    % (3n^2+n-3n-1+3n^2-10n+3+8n^2-16n+2n^2-10n+12+8n+16+8n^2+12n+4)/4
    % \text{\,\, otherwise}
    % (24n^2-18n+34)/4
    % \text{\,\, otherwise}
    % (12n^2-9n+17)/2
    % \text{\,\, otherwise}
    % 6n^2+ (-8n-n+16+1)/2
    % \text{\,\, otherwise}
    6n^2-4n-\frac{n-1}{2}+8
    \text{\,\, if $n$ is odd}
    \end{cases}
\end{equation}

% 4n(4+n)/2-4n
% 2n(n+4)-4n
% 2n^2+8n-4n
% 2n^2+4n
% 2n(n+2)

% Since 
% $\sum_{v\in\beta[2n-1,4n]}=
% 2n^2+3n+1
% $ we can state the following, which will be needed for the rest of the proof:
% \begin{equation}
% \sum\nolimits_{v\in \beta[1,2n-2]}
%     |\textit{madj}^+_\beta(v)|=
%     \begin{cases}
%     4n^2-7n-\frac{n}{2}+7
%     \text{\,\, if $n$ is even}
%     \\
%     4n^2-7n-\frac{n-1}{2}+7
%     \text{\,\, otherwise}
%     \end{cases}
% \end{equation}

As discussed before, in order to prove that $\tau(G)>0$ it suffices to show that for every elimination ordering $\alpha$ over $G$ s.t.\ $\textit{tw}(G^+_\alpha)=\textit{tw}(G)$ we have that $|E_{G^+_\alpha}|>|E_{G^+_\beta}|$.
Suppose for a contradiction that we can fix one such elimination ordering $\alpha$ over $G$ with $\textit{tw}(G^+_\alpha)=\textit{tw}(G)$ and $|E_{G^+_\alpha}|\leq|E_{G^+_\beta}|$.
By \cref{lem:minDegreeRookFirst} we can fix a nice elimination ordering $\alpha^*$ over $G$ where $G^+_{\alpha^*}=G^+_\alpha$ and for every vertex $v\in\mathcal{V}_G(\alpha^*,n+2)$ we have ${\alpha^*}^{-1}\leq|\mathcal{V}_G(\alpha^*,n+2)|$.
Clearly we must have that $\textit{tw}(G^+_{\alpha^*})=2n+1$ then using \cref{lem:twEliminationHigherAdjacency} we can state that:
 \begin{equation}\label{eq:4nLemmaMaxAlpha}
    \max\nolimits_{v\in V}|\textit{madj}^+_{\alpha^*}(v)|\leq 2n+1
 \end{equation}
 
Furthermore, since $G^+_{\alpha^*}=G^+_\alpha$ we have that $|E_{G^+_{\alpha^*}}|\leq|E_{G^+_\beta}|$, implying that:
\begin{equation}\label{eq:4nLemmaSumAlphavsBeta}
    \sum\nolimits_{v\in V}|\textit{madj}^+_{\alpha^*}(v)|<
    \sum\nolimits_{v\in V}|\textit{madj}^+_{\beta}(v)|
\end{equation}

Since $\alpha^*$ is a nice elimination ordering,
$\sum_{v\in\alpha^*[2n-1,4n]}
|\textit{madj}^+_{\alpha^*}(v)|
=\sum_{v\in\beta[2n-1,4n]}
|\textit{madj}^+_{\beta}(v)|
=(2n+1)(n+1)$ (following \cref{def:niceElim}).
This together with \cref{eq:4nLemmaSumBeta}
and \cref{eq:4nLemmaSumAlphavsBeta} implies that:
\begin{equation}\label{eq:4nLemmaSumAlpha}
    \sum\nolimits_{v\in {\alpha^*}[1,2n-2]}
    |\textit{madj}^+_{\alpha^*}(v)|<
    \begin{cases}
    4n^2-7n-\frac{n}{2}+7
    \text{\,\, if $n$ is even}
    \\
    4n^2-7n-\frac{n-1}{2}+7
    \text{\,\, if $n$ is odd}
    \end{cases}
\end{equation}

For every step $i\in\{1,\dots,2n-2\}$ we must necessarily have that $|\mathcal{M}_{\alpha^*}(i)|\leq 3$ otherwise by \cref{cor:madjRooks} we get that $\textit{madj}^+_{\alpha^*}(\alpha^*(i))=
4n-|V_{\textit{comp}_{\alpha^*}}(i)|\geq 2n+2$ contradicting \cref{eq:4nLemmaMaxAlpha}.
Moreover, there necessarily exists a step $i\in\{1,\dots,2n-2\}$ in $\alpha^*$ s.t.\ $|\mathcal{M}_{\alpha^*}(i)|\geq 2$.
This is due to the fact that we eliminate $2n-2$ vertices and $G$ is a $4\times n$ rook's graph for $n\geq 6$.
% 2n-2>=10 vertices from n>=6 columns then\todo{Then} by the Pigeonhole principle there exists a column index $c\in\{1,\dots,n\}$ s.t.\ $|L_c\cap\alpha^*[1,2n-2]|\geq 2$.
As a consequence of these facts, $\max_{i\in\{1,\dots,2n-2\}}|\mathcal{M}_{\alpha^*}(i)|$ is either 2 or 3.
% Informally, the induced graph $G[\alpha^*[1,2n-2]]$ must have a connected component whose vertex set spans across 2 or 3 rows of $G$.
So let us consider the following complementary cases and show that they both result in a contradiction with \cref{eq:4nLemmaSumAlpha}.


\begin{mycases}
    \case 
    {
    Suppose that 
    $\max_{i\in\{1,\dots,2n-2\}}|\mathcal{M}_{\alpha^*}(i)|=3$.
    Then we can fix a step $j\in\{1,\dots,2n-2\}$ s.t.\ $|\mathcal{M}_{\alpha^*}(j)|=3$.
    Then in this case
    \cref{lem:46helper2} implies that 
    $\sum\nolimits_{v\in {\alpha^*}[1,2n-2]}
    |\textit{madj}^+_{\alpha^*}(v)|\geq 
    4n^2-6n+4$.
    % n+n/2 > 3
    This clearly contradicts \cref{eq:4nLemmaSumAlpha} as desired.
    }
    
    \case
    {
    Suppose that 
    $\max_{i\in\{1,\dots,2n-2\}}|\mathcal{M}_{\alpha^*}(i)|=2$, it means there exists a connected component $C$ of in $G[\alpha^*[1,2n-2]]$ that has its vertices, $V_C$, in exactly two rows of $G$.
    Additionally, because $G$ is a $4\times n$ rook's graph and every row is a clique, there may exist another  connected component $C'$ in $G[\alpha^*[1,2n-2]]$ s.t.\ $V_{C'}$ spans across two different rows of $G$.
    So let us consider the following subcases:


    \begin{subcases}
        \subcase
        {
        Suppose that $G[\alpha^*[1,2n-2]]$ has 2 connected components $C,C'$ each spanning across 2 rows of $G$.
        Let $j,j'\in\{1,\dots,2n-2\}$ be the latest steps in $\alpha^*$ s.t.\ $\alpha^*(j)\in C$ and $\alpha^*(j')\in C'$.
        By this selection $V_{\textit{comp}_{\alpha^*}(j)}=C$, $V_{\textit{comp}_{\alpha^*}(j')}=C'$ and $|\mathcal{M}_{\alpha^*}(j)|=
        |\mathcal{M}_{\alpha^*}(j')|=2$.
        We point out that 
        $\mathcal{M}_{\alpha^*}(j)\cap \mathcal{M}_{\alpha^*}(j')=\emptyset$ and $\mathcal{L}_{\alpha^*}(j)\cap \mathcal{L}_{\alpha^*}(j')=\emptyset$ otherwise because every row and column of $G$ is a clique, $C,C'$ cannot be distinct connected components of $G[\alpha^*[1,2n-2]]$.
        % W.l.o.g.\ assume that $\mathcal{M}_{\alpha^*}(j)=\{1,2\}$ and $\mathcal{M}_{\alpha^*}(j')=\{3,4\}$.
        Using \cref{lem:46helper1} we can state that:
        $$
        \sum_{v\in C} |\textit{madj}^+_{\alpha^*}(v)| \geq
        2n(|C|-1)+\ceil*{\frac{|C|}{2}}+3 
        \textit{ \, and \, }
        \sum_{v\in C'} |\textit{madj}^+_{\alpha^*}(v)| \geq
        2n(|C'|-1)+\ceil*{\frac{|C'|}{2}}+3
        $$

        Since every row of $G$ is a clique, $G[\alpha^*[1,2n-2]]$ has exactly the 2 connected components $C$ and $C'$.
        As a result, $|C|+|C'|=2n-2$ and we point out that $\ceil*{|C|/2}+\ceil*{|C'|/2}\geq n-1$.
        % n=8, 2n-2=14, C=3, C'=11, \ceil*{|C|/2}+\ceil*{|C'|/2}=2+6=8
        % n=8, 2n-2=14, C=2, C'=12, \ceil*{|C|/2}+\ceil*{|C'|/2}=1+6=7
        Furthermore, we have that
        $\sum_{v\in C} |\textit{madj}^+_{\alpha^*}(v)|+
        \sum_{v\in C'} |\textit{madj}^+_{\alpha^*}(v)|=
        \sum_{v\in {\alpha^*}[1,2n-2]}
        |\textit{madj}^+_{\alpha^*}(v)|$ so as a result we can summarize by saying that:
        $$
        \sum_{v\in {\alpha^*}[1,2n-2]}
        |\textit{madj}^+_{\alpha^*}(v)|\geq
        2n(|C|+|C'|-2)+\ceil*{\frac{|C|}{2}}+\ceil*{\frac{|C'|}{2}}+6\geq
        % 2n(2n-4)+\ceil*{\frac{|C|}{2}}+\ceil*{\frac{|C'|}{2}}+6=
        % 4n^2-8n+6+\ceil*{\frac{|C|}{2}}+\ceil*{\frac{|C'|}{2}}=
        % 4n^2-8n+6+n-1=
        4n^2-7n+5
        % 4n^2-8n+6+n-1= 4n^2-7n+5
        $$
        % n is even: 4n^2-7n+5 vs 4n^2-7n-(n/2)+7
        % n is even: (n/2) > 2 
        % n is odd: 4n^2-7n+5 vs 4n^2-7n-(n-1/2)+7
        % n is odd: (n-1/2) vs 2 
        % n is at least 7 so 6/2=3 > 2
        
        This clearly contradicts \cref{eq:4nLemmaSumAlpha} as $n\geq 6$.
        }
        
        \subcase
        {
        Suppose that $G[\alpha^*[1,2n-2]]$ has only 1 connected components $C$ spanning across 2 rows of $G$.
        Let $j\in\{1,\dots,2n-2\}$ be the latest step in $\alpha^*$ s.t.\ $\alpha^*(j)\in V_C$.
        Then $V_{\textit{comp}_{\alpha^*}(j)}=V_C$ and $|\mathcal{M}_{\alpha^*}(j)|=2$.
        Assume w.l.o.g.\ that $\mathcal{M}_{\alpha^*}(j)=\{1,2\}$.
        Since $C$ spans across rows 1,2 and rows 3,4 are cliques in $G$, there can exist at most 2 other connected components in $G[\alpha^*[1,2n-2]]$.
        Then there are 3 distinct possibilities regarding the connected components of $G[\alpha^*[1,2n-2]]$ and we need to discuss all of them in order to determine a lower bound for $\sum_{v\in {\alpha^*}[1,2n-2]}
        |\textit{madj}^+_{\alpha^*}(v)|$.
        
        Begin by supposing that $C$ is the only connected component of $G[\alpha^*[1,2n-2]]$.]
        Then we have $V_C=\alpha^*[1,2n-2]$ and \cref{lem:46helper1} we can state that: 
        \begin{equation}\label{eq:46Rook:ConlyComp}
            \sum\nolimits_{v\in {\alpha^*}[1,2n-2]}
            |\textit{madj}^+_{\alpha^*}(v)|\geq
            4n^2-5n+2 \textit{ \, if \, } \alpha^*[1,2n-2]=V_C
        \end{equation}
        
        Next, suppose that $C$ is not the only connected component of $G[\alpha^*[1,2n-2]]$.
        Then clearly $V_C\subset \alpha^*[1,2n-2]$ so let us define the vertex set $R= \alpha^*[1,2n-2]\setminus V_C$.
        Note that by definition, $|V_C|=2n-2-|R|$.
        
        No two vertices from $R$ can share the same column otherwise $C$ is not the only connected component of $G[\alpha^*[1,2n-2]]$ spanning across 2 rows, a contradiction.
        Then there are $|R|$ column indices $c\in\{1,\dots,n\}$ each containing a vertex from $R$.
        Furthermore, we must have
        $\mathcal{L}_{\alpha^*}(j)\cap 
        \{c|c\in\{1,\dots,n\} 
        \textit{\, s.t.\ } 
        L_c\cap R\neq \emptyset\}=\emptyset$ otherwise there exists a vertex $r\in R$ that is also a vertex of $C$, contradicting the selection of $R$.
        This proves that $C$ spans across at most $n-|R|$ columns, formally 
        $|\mathcal{L}_{\alpha^*}(j)|\leq n-|R|$.
        Since $C$ spans across 2 rows, we can conclude that $|V_C|\leq 2(n-|R|)$.
        This, combined with the fact that $|V_C|=2n-2-|R|$, implies that $|R|=|\alpha^*[1,2n-2]\setminus V_C|\leq 2$.
        Informally, there are at most 2 vertices eliminated before step $2n-2$ in $\alpha^*$ that are not vertices of the connected component $C$.
        
        First, suppose that $|\alpha^*[1,2n-2]\setminus V_C|=1$.
        W.l.o.g.\ assume that this vertex belongs to row 3, i.e.,\ let $\alpha^*[1,2n-2]\setminus V_C= \{v_{3,c}\}$ for some column index $c\in (\{1,\dots,n\}\setminus \mathcal{L}_{\alpha^*}(j))$.
        Since $v_{3,c}$ does not share a row or a column with any previously eliminated vertex, we can state using \cref{cor:madjRooks} that $|\textit{madj}^+_{\alpha^*}(v_{3,c})| =n+2$.
        Since $|\alpha^*[1,2n-2]\setminus V_C|=1$ we have that $|V_C|=2n-3$ and using \cref{lem:46helper1} we can state that 
        $\sum_{v\in V_C} |\textit{madj}^+_{\alpha^*}(v)|\geq
        % 2n(2n-3-1)+\ceil{(2n-3)/2}+3
        % =2n(2n-4)+(2n-2)/2+3
        % =2n(2n-4)+(n-1)+3
        % =4n^2-8n+n-1+3
        4n^2-7n+2
        $
        Since $V_C\cup\{v_{3,c}\}= \alpha^*[1,2n-2]$ we can conclude that:
        \begin{equation}\label{eq:46Rook:Candv}
            \sum\nolimits_{v\in {\alpha^*}[1,2n-2]}
            |\textit{madj}^+_{\alpha^*}(v)|\geq
            4n^2-6n+4 \textit{ \, if \, } |\alpha^*[1,2n-2]\setminus V_C|=1
        \end{equation}
        
        Finally, suppose that $|\alpha^*[1,2n-2]\setminus V_C|=2$.
        Let us label these vertices with $\{v,v'\}=\alpha^*[1,2n-2]\setminus V_C$ and let $i_v,i_{v'} \in\{1,\dots,2n-2\}$ be respectively the steps at which $v,v'$ are eliminated in $\alpha^*$.
        Note that $v,v'$ cannot belong to the same column, and they cannot share the same row with any of the vertices in $V_C$, therefore $v,v'\in M_3\cup M_4$.
        W.l.o.g.\ assume that $v\in M_3$ and that $i_v<i_{v'}$.
        Then, because $v$ does not share a row or a column with any of the previously eliminated vertices, we can state using \cref{cor:madjRooks} that $|\textit{madj}^+_{\alpha^*}(v)| =n+2$.
        We either have that $v'\in M_3$ resulting in
        $V_{\textit{comp}_{\alpha^*}(i_{v'})}= \{v,v'\}$, $|\mathcal{M}_{\alpha^*}(i_{v'})|=1$ and $|\mathcal{L}_{\alpha^*}(i_{v'})|=2$ implying that
        $|\textit{madj}^+_{\alpha^*}(v')|=
        % 4n-3(n-2)-2 = 4n-3n+6-2= n+4
        n+4$.
        Or we have that $v'\in M_4$ then $v'$ does not share a column or a row with any of the previously eliminated vertices implying that $|\textit{madj}^+_{\alpha^*}(v')| =n+2$.
        We can sum up by saying that
        $|\textit{madj}^+_{\alpha^*}(v)|+|\textit{madj}^+_{\alpha^*}(v')|\geq 2n+4$.
        Since $|\alpha^*[1,2n-2]\setminus V_C|=2$ we have that $|V_C|=2n-4$ so using \cref{lem:46helper1} we can state that
        $\sum_{v\in V_C} |\textit{madj}^+_{\alpha^*}(v)| \geq
        % 2n(2n-4-1)+(2n-4)/2+3
        % 2n(2n-5)+(n-2)+3
        % 4n^2-10n+n-2+3
        4n^2-9n+1
        $
        Recall that $\alpha^*[1,2n-2]= V_C\cup\{v,v'\}$ as a result we have that:
        \begin{equation}\label{eq:46Rook:Candvv}
            \sum\nolimits_{v\in {\alpha^*}[1,2n-2]}
            |\textit{madj}^+_{\alpha^*}(v)|\geq
            4n^2-7n+5 \textit{ \, if \, } |\alpha^*[1,2n-2]\setminus V_C|=2
        \end{equation}
        
        Let us now summarize our observations in this subcase.
        By combining \cref{eq:46Rook:ConlyComp}, \cref{eq:46Rook:Candv} and \cref{eq:46Rook:Candvv} we have that:
        $$ \sum\nolimits_{v\in {\alpha^*}[1,2n-2]}
            |\textit{madj}^+_{\alpha^*}(v)|\geq
            4n^2-7n+5
        $$
        
        Since $n\geq 6$, it is easy to see that this contradicts \cref{eq:4nLemmaSumAlpha} as needed.
        }
    \end{subcases}
    }
\end{mycases}

The statement of the theorem ultimately follows, as we have proved a contradiction with \cref{eq:4nLemmaSumAlpha} in all possible cases.
This proves that $|E_H|>|E_{G^+_\beta}|$ for every triangulation $H$ of $G$ with $\textit{tw}(H)=\textit{tw}(G)$.
Since $\textit{tw}(G^+_\beta)>\textit{tw}(G)$ we can conclude that for every minimum triangulation $H^*$ of $G$, $\textit{tw}(H^*)>\textit{tw}(G)$.
This in turn proves that $\tau(G)>0$ by \cref{def:tau}.
\end{proof}
}

% 4xn n>=6 rook mfi
{
Unlike \cref{rmk:mfi44Rook} and \cref{rmk:mfi45Rook}, we can only state an upper bound for $\textit{mfi}(K_4\square K_n)$ for any $n\geq 6$:

\begin{remark}\label{rmk:46rookMfi}
Let $G$ be a $K_4\square K_n$ for $n\geq 6$ and $G^+_\beta$ the triangulation defined in the proof of \cref{lem:46Rooktau}.
It is easy to verify that the number of edges in $G$ is 
%
$2n^2+4n$ therefore using \cref{eq:4nLemmaSumBeta} we can state that:

\begin{equation}\label{eq:mfi46upper bound}
\textit{mfi}(G)\leq 
|E_{G^+_\beta}|-|E_G|=
    \begin{cases}
    % 6n^2-4n-\frac{n}{2} +8
    4n^2-8n-\frac{n}{2} +8
    \text{\,\, if $n$ is even}
    \\
    % 6n^2-4n-\frac{n-1}{2}+8
    % 6n^2-4n-\frac{n-1}{2}+8-2n^2+4n
    4n^2-8n-\frac{n-1}{2}+8
    \text{\,\, if $n$ is odd}
    \end{cases}
\end{equation}
\end{remark}

We point out that the upper bound shown in \cref{rmk:46rookMfi} is not tight, considering the values obtained by our experimental work that is presented in \cref{tab:4rookMfi}.
}
}





==> content/tfm0.tex <==
\section{The $\tau$ Parameter: General Results}\label{sec:tfm:General}

% tau greater than 0
{
Let us begin by proving that the $\tau$ parameter can be arbitrarily large.
For this purpose, we will be using the construction provided in \cite{Dar2019}.

\begin{theorem}\label{rmk:tauArbLarge}
Given any positive integer $l$, there exists an infinite family of graphs $\mathcal{G}$ where for each graph $G\in\mathcal{G}$, $\tau(G)=l$.
\end{theorem}
\begin{proof}
Let $l$ be a fixed positive integer and $\mathcal{G}$ the graph class containing every graph $G$ defined using the following construction.
Begin by letting $G$ be the cycle $(a,b_1,c,b_2,a)$.
Next replace each of the vertices $a,b,c,d$ with non-empty cliques $A,B_1,B_2,C$ respectively under the restriction that $|A|+l=|B_1|=|B_2|<|C|$ and $|B_1|^2<|A||C|$.
See \cref{fig:tauArbLarge:1} for a demonstration.

% proof not using minimal elimination
{
Following its construction, $G$ has two distinct minimal traingulations, one minimising the number of added edges and the other minimising the clique size of the resulting traignulation.
These have been previously discussed in \cite{Dar2019} and we have included a proof for this here for completion.

Considering our observation following \cref{lem:elim}, there must exist a minimum elimination ordering over $G$ that adds $\textit{mfi}(G)$ many edges.
It is easy to see that every elimination ordering (hence also minimum elimination ordering) over $G$ either starts by eliminating a vertex $v\in (B_1\cup B_2)$ or a vertex $v\in (A\cup C)$. 
So let $\alpha$ and $\beta$ be any elimination orderings selected s.t.\ $\alpha(1)\in (B_1\cup B_2)$ and $\beta(1)\in (A\cup C)$.
We will use $F_\alpha$ and $F_\beta$ while referring to the added edges in the triangulations $G^+_\alpha$ and $G^+_\beta$.

Since $\alpha(1)\in(B_1\cup B_2)$ we have that $\textit{fill}_G(N_G\,(\alpha(1)))=
\{ac|a\in A, c\in C\}$.
These missing edges will be added to $G$ by elimination of $\alpha(1)$.
It is easy to see that the graph $G_1^\alpha$ is chordal.
% Define $F_{\alpha(1)}$ to be the chords added in the corresponding triangulations $G^\alpha_1$.
% \unsure[inline]{
% This sentence is not correct.
% $G^\alpha_1$ is the graph obtained from $G$ by addition of $\textit{fill}_G(N_G\,(\alpha(1)))$ and then removal of $\alpha(1)$.
% This means that $G^\alpha_1$ (and similarly $G^\beta_1$ \textbf{***}) are not supergraph nor subgraph of $G$.
% Therefore, they \textbf{are not a triangulation of G}.
% The graph $G^+_\alpha$ however is a chordal supergraph of $G$ and is a triangulation, so I think you meant to say:\\
% The graph $G\oplus \textit{fill}_G(N_G\,(\alpha(1)))$ is a triangulation (demonstrated in \cref{fig:tauArbLarge:2}).
% And if $\alpha$ is a peo over $G^\alpha_1$ we have that $G^+_\alpha=G\oplus \textit{fill}_G(N_G\,(\alpha(1)))$.\\
% }
By construction, $\omega(G^\alpha_1)=|A|+|B_1|+|C|$ we also note that $|\textit{fill}_G\,(N_G(\alpha(1)))|=|A||C|$.
As a result, $\textit{tw}(G^+_\alpha)\geq \omega(G^\alpha_1)-1=|A|+|B_1|+|C|-1$ and $|F_\alpha|\geq |A||C|$.
Supposing that $\alpha$ is a peo over $G^\alpha_1$ (note that this is possible by \cref{thm:chordalIffPeo} as $G^\alpha_1$ is chordal) in the remaining steps we have that $\textit{tw}(G^+_\alpha)=|A|+|B_1|+|C|-1$ and $|F_\alpha|=|A||C|$.
In either case, the triangulation $G\oplus \textit{fill}_G(N_G\,(\alpha(1)))$ is demonstrated in \cref{fig:tauArbLarge:2}.


Regardless of whether $\beta(1)\in A$ or $\beta(1)\in C$, the set of missing edges
$\textit{fill}_G\,(N_G(\beta(1)))=\textit{fill}_G(B_1\cup B_2)$ is added by elimination of $\beta(1)$.
Similar to the previous case, the graph $G_1^\beta$ is chordal.
Since $B_1\cup B_2$ is a clique in $G^\beta_1$ we have that $\omega(G^\beta_1)=2|B_1|+|C|$ as $|A|<|C|$.
We also note that $|\textit{fill}_G\,(N_G(\beta(1)))|=|B_1|^2$.
Then $\textit{tw}(G^+_\beta)\geq \omega(G^\beta_1)-1=2|B_1|+|C|-1$ and $|F_\beta|\geq |B_1|^2$.
Again we point out that if $\beta$ is a peo over $G^\beta_1$ we will have:
$\textit{tw}(G^+_\beta)=2|B_1|+|C|-1$ and $|F_\beta|=|B_1|^2$.
The triangulation $G\oplus \textit{fill}_G(N_G\,(\beta(1)))$ is demonstrated in \cref{fig:tauArbLarge:3}.

By construction of $G$, $|B_1|>|A|$ so we have that
$\textit{tw}(G\oplus \textit{fill}_G(N_G\,(\beta(1))))=2|B_1|+|C|-1
>|A|+|B_1|+|C|-1=\textit{tw}(G\oplus \textit{fill}_G(N_G\,(\alpha(1))))$, hence $\textit{tw}(G)\leq |A|+|B_1|+|C|-1$.
Next, we prove that the clique size of any triangulation of $G$ is at least $|A|+|B_1|+|C|$.
Let $H=(V,E\cup F)$ be any triangulation of $G$.
Below we consider 2 complementary cases and prove in each case that $\omega(H)\geq |A|+|B_1|+|C|$:
\begin{mycases}
    \case
    {
    Suppose that $A\cup C$ is a clique in $H$.
    Then $A\cup B_1\cup C$ is a clique in $H$ showing that $\omega(H)\geq |A|+|B_1|+|C|$ as desired.
    }
    
    \case
    {
    Suppose that $A\cup C$ is not a clique in $H$.
    Then there exists two vertices $a\in A$ and $c\in C$ s.t.\ $ac\notin F$.
    For every selection of vertices $b_1\in B$ and $b_2\in B_2$, the cycle $C=(a,b_1,c,b_2,a)$ must have the chord $b_1b_2\in F$ otherwise $C$ is a chordless cycle in $H$, a contradiction.
    Therefore, $B_1\cup B_2$ is a clique in $H$ implying that $\omega(H)\geq 2|B_1|+|C|$.
    Since $|B_1|>|A|$ we have that $\omega(H)> |A|+|B_1|+|C|$ as needed.
    }
\end{mycases}

This proves that the minimum clique size over all triangulations of $G$ is $|A|+|B_1|+|C|$ and using \cref{lem:twEliminationHigherAdjacency} we can state the following: 
$$\textit{tw}(G)=\textit{tw}(G\oplus \textit{fill}_G\,(N_G(\alpha(1))))=|A|+|B_1|+|C|-1$$

Furthermore, because $|F_\beta|\geq|B_1|^2$, $|F_\alpha|\geq|A||C|$ and $|B_1|^2<|A||C|$ we can conclude that $G^+_\beta$ can be a minimum elimination ordering.
This is indeed the case if $\beta$ is a peo over $G^\beta_1$ in the remaining steps.
By \cref{def:tau} we have that $\tau(G)=|C|+2|B_1|-1-(|A|+|B_1|+|C|-1)=|B_1|-|A|=l$ as desired.
}

\iffalse
% proof using minimal elimination
{
\unsure[inline]{
Below is old proof using minimal elimination ordering. 
Can I please ask why this proof is bad?
}
\todo[inline]
{
There is nothing like `bad' proof—the proof is either correct or not. 
Some proofs can be correct, but may sometimes use arguments which are often overcomplicated—there is of course nothing wrong with that, but the reader has to verify some additional properties which are not necessary. 
In this case, the reader has to see the connections between minimal elimination schemes and min-fill/TW and additional to verify that defined elimination schemes are minimal one with the required properties.
In my view, the first proof is straightforward and very natural, does not require any additional information.
}
\unsure[inline]
{
OK, I understand your argument.
My understanding is however that we have discussed the connection between minimal elimination ordering and these parameters previously, so now we can use it to make the proof shorter.
If you think the above proof is easier to read than mines, then we can remove it.
}

% previously done by citing \cite{BouchitteWeaklyChordal}
Let us begin by determining the value of the treewidth and the minimum fill-in parameter of $G$.
As pointed out in our discussion, following \cref{lem:elim}, in order to find out $\textit{mfi}(G)$ we can restrict ourselves to minimal triangulations over $G$.
The same statement holds for $\textit{tw}(G)$ as shown by \cref{lem:minimalTwAndMfi}.
\unsure
{
This used to be a cite to \cite{BouchitteWeaklyChordal} (page 199 after Definition 3) but it was not fully proven in that paper.
}
For this reason, we will consider all possible minimal elimination orderings of $G$.
It is easy to see that every elimination ordering (also minimal elimination ordering) over $G$ either starts by eliminating a vertex $v\in (B_1\cup B_2)$ or a vertex $v\in (A\cup C)$.
So let $\alpha$ and $\beta$ be any minimal elimination orderings selected s.t.\ $\alpha(1)\in (B_1\cup B_2)$ and $\beta(1)\in (A\cup C)$.
Define $F_\alpha,F_\beta$ to be the chords added in the corresponding minimal triangulations $G^+_\alpha$ and $G^+_\beta$.

Since $\alpha(1)\in(B_1\cup B_2)$ we have that $\textit{fill}_G(N_G\,(\alpha(1)))=
\{ac|a\in A,c\in C\}$.
These missing edges will be added to $G$ by elimination of $\alpha(1)$.
It is easy to see that the graph $G_1^\alpha$ is chordal (then by \cref{thm:chordalIffPeo}, there exists a perfect elimination ordering over $G^\alpha_1$).
By selection, $\alpha$ is a minimal elimination ordering over $G$, thus $\alpha$ is perfect elimination ordering of $G_1^\alpha$ in the remaining steps.
Formally $\alpha(i)$ for $i\in\{2,\dots,|V|\}$ is a simplicial vertex in the graph $G_{i-1}^\alpha$.
The minimal triangulation $G^+_\alpha$ is demonstrated in \cref{fig:tauArbLarge:2}.
By construction, $\omega(G^+_\alpha)=|A|+|B_1|+|C|$ we also note that, $|F_\alpha|=|A||C|$.

Regardless of whether $\beta(1)\in A$ or $\beta(1)\in C$, the set of missing edges $\textit{fill}_G(N_G(\beta(1)))=\textit{fill}_G(B_1\cup B_2)$ is added by elimination of $\beta(1)$.
Similar to the previous case, the graph $G_1^\beta$ is chordal, therefore $\beta$ is a perfect elimination ordering over $G_1^\beta$ in the remaining steps (see \cref{fig:tauArbLarge:3} for a demonstration of the graph $G^+_\beta$).
Since $B_1\cup B_2$ is a clique in $G^+_\beta$ we have that $\omega(G^+_\beta)=|C|+2|B_1|$ as $|A|<|C|$ and we note that $|F_\beta|=|B_1|^2$.

By construction of $G$, $|F_\beta|=|B_1|^2<|A||C|=|F_\alpha|$ and since $|B_1|>|A|$ we have that
$\omega(G^+_\beta)=|C|+2|B_1|>|A|+|B_1|+|C|=\omega(G^+_\alpha)$.
Consequently, $G^+_\beta$ is necessarily the minimum triangulation of $G$ with $\textit{tw}(G^+_\beta)=|C|+2|B_1|-1$.
Also, $G^+_\alpha$ is the minimum clique size triangulation of $G$ showing that $\textit{tw}(G)=\textit{tw}(G^+_\alpha)=|A|+|B_1|+|C|-1$.
By \cref{def:tau} we have that $\tau(G)=|C|+2|B_1|-1-(|A|+|B_1|+|C|-1)=|B_1|-|A|=l$ as desired.
}
\fi

% tau=l image
{
\usetikzlibrary{shapes, backgrounds}
\tikzset{
a/.style={draw=black,ellipse,minimum width=10pt, inner sep=3pt, text width=4mm, text height=2 mm,  align=center, fill=white}
}
\tikzset{
b/.style={draw=black,ellipse,minimum width=50pt, inner sep=7.5pt, text width=3mm, text height=1.5 mm,  align=center, fill=white}
}
\tikzset{
c/.style={draw=black,ellipse,minimum width=175pt, inner sep=10pt, text width=3mm, text height=1.5 mm,  align=center, fill=white}
}
\begin{figure}
\centering
    \begin{subfigure}{0.4\textwidth}
        \begin{tikzpicture}
            [scale=0.4,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
            {
            \node [a] (a) at (0,4) {A};
            \node [b] (b1) at (-4,0) {$B_1$};
            \node [b] (br) at (4,0) {$B_2$};
            \node [c] (c) at (0,-4) {C};
            }
            \begin{scope}[on background layer]
                \draw[-]
                    (a)--(-5,1)
                    (a)--(-2.1,0)
                    
                    (a)--(5,1)
                    (a)--(2.1,0)
                    
                    (5.9,0)--(7.5,-4)
                    (-3.5,0)--(7,-3.58)
                    
                    (-5.9,0)--(-7.5,-4)
                    (3.5,0)--(-7,-3.58)
                    ;
            \end{scope}
        \end{tikzpicture}
        \caption{$G$}
        \label{fig:tauArbLarge:1}   
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.4\textwidth}
        \begin{tikzpicture}
            [scale=0.4,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
            {
            \node [a] (a) at (0,4) {A};
            \node [b] (b1) at (-4,0) {$B_1$};
            \node [b] (br) at (4,0) {$B_2$};
            \node [c] (c) at (0,-4) {C};
            }
            \begin{scope}[on background layer]
                \draw[-]
                    (a)--(-5,1)
                    (a)--(-2.1,0)
                    
                    (a)--(5,1)
                    (a)--(2.1,0)
                    
                    (5.9,0)--(7.5,-4)
                    (-3.5,0)--(7,-3.58)
                    
                    (-5.9,0)--(-7.5,-4)
                    (3.5,0)--(-7,-3.58)
                    ;
            \end{scope}
            
                \draw [draw=MyColorOne, rounded corners=5mm, fill=MyColorOne, draw=MyColorOne, line width=2pt, opacity=0.3]
                (-0.5,4.5)--(-6.5,0)--(-8,-4.3)--(-3.5,-5.5)--(3.5,-5.5)--(8.3,-4.3)--(-2,0)--(1.25,4.5)--cycle;
                \draw[dashed, draw=red, thick, opacity=0.8]
                (a)--(-7.5,-4)
                (a)--(-5.5,-4)
                (a)--(-3.5,-4)
                (a)--(-1.5,-4)
                (a)--(1.5,-4)
                (a)--(3.5,-4)
                (a)--(5.5,-4)
                (a)--(7.5,-4)
                ;
        \end{tikzpicture}
        \caption{$G^+_\alpha$}
        \label{fig:tauArbLarge:2}   
    \end{subfigure}
    \vspace{0.5cm}
    \begin{subfigure}{0.4\textwidth}
        \begin{tikzpicture}
            [scale=0.4,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
            {
            \node [a] (a) at (0,4) {A};
            \node [b] (b1) at (-4,0) {$B_1$};
            \node [b] (br) at (4,0) {$B_2$};
            \node [c] (c) at (0,-4) {C};
            }
            \begin{scope}[on background layer]
                \draw[-]
                    (a)--(-5,1)
                    (a)--(-2.1,0)
                    (a)--(5,1)
                    (a)--(2.1,0)
                    (5.9,0)--(7.5,-4)
                    (-3.5,0)--(7,-3.58)
                    (-5.9,0)--(-7.5,-4)
                    (3.5,0)--(-7,-3.58);
            \end{scope}
            \draw [draw=MyColorOne, rounded corners=5mm, fill=MyColorOne, draw=MyColorOne, line width=2pt, opacity=0.3]
            (-6.5,0)--(-5,1.5)--(5,1.5)--(6.5,0)--(8,-4.5)--(3.5,-5.5)--(-3.5,-5.5)--(-8,-4.5)--cycle;
            \draw[dashed, draw=red, thick, opacity=0.8]
            (3.5,1.25)--(-3.5,1.25)
            (3.5,-1.25)--(-3.5,-1.25)
            (3,-0.75)--(-3,-0.75)
            (3,0.75)--(-3,0.75)
            (2.75,-0.25)--(-2.75,-0.25)
            (2.75,0.25)--(-2.75,0.25)
            ;
        \end{tikzpicture}
        \caption{$G^+_\beta$}
        \label{fig:tauArbLarge:3}   
    \end{subfigure}
\caption
{
(a) the graph $G$. 
The vertices in the cliques $A,B_1,B_2,C$ alongside the edges in between them are grouped together for simplicity.
(b),(c) respectively demonstrate the minimal triangulations $G^+_\alpha$ and $G^+_\beta$.
The maximum clique in each graph is highlighted with green and the added edges are drawn in red.
} 
\label{fig:tauArbLarge}
\end{figure}
}
\end{proof}

It is easy to see that a statement similar to \cref{rmk:tauArbLarge} also holds for the parameter $\phi$.
}

% tau 0 simple examples
{
Let us now discuss some classes of graphs where the $\tau$ parameter is 0.
Clearly, $\tau(G)=0$ for a chordal graph $G$.
This follows from \cref{def:tau} and the fact that $G$ is itself a minimum triangulation with treewidth equal to $\textit{tw}(G)$.

% cocktail party
{
For another easy example, we prove that \textit{cocktail party} graphs, which are not chordal, have $\tau=0$.
Formally a graph $G=(V,E)$ is a cocktail party if $V$ can be partitioned into two subsets $X,Y$ satisfying the following conditions: 
$X=\{x_1,\dots,x_r\}$ and $Y=\{y_1,\dots,y_r\}$ for $r\geq 1$ and $E=\{x_iv|i\in\{1,\dots,r\},v\in V\setminus\{x_i,y_i\}\}\cup \{y_iv|i\in\{1,\dots,r\},v\in V\setminus\{x_i,y_i\}\}$.
We point out that a cocktail party graph with $2r$ vertices can be obtained from the $K_{2r}$ by removal of a perfect matching.

\begin{lemma}\label{lemma:cocktailParty}
Let $G=(V,E)$ be a cocktail party graph.
Then $\tau(G)=0$.
\end{lemma}
\begin{proof}
A cocktail party graph has a unique (up to ismorphism) minimal triangulation which is a solution to both problems \textsc{Minimum Fill-In} and \textsc{Treewidth}.
To prove this and the statement of the lemma, we begin by determining $\textit{mfi}(G)$ and $\textit{tw}(G)$.
We then define a minimum triangulation $H^*=(V,E\cup F^*)$ of $G$  where $\textit{tw}(H^*)=\textit{tw}(G)$.
Since $G$ is a cocktail party graph we can partition $V$ into the vertex sets $\{x_1,\dots,x_r\}$ and $\{y_1,\dots,y_r\}$, for $r\geq 1$, s.t.\ $E=\{x_iv|i\in\{1,\dots,r\},v\in V\setminus\{x_i,y_i\}\}\cup \{y_iv|i\in\{1,\dots,r\},v\in V\setminus\{x_i,y_i\}\}$.

First, we claim that $\textit{mfi}(G)\geq r-1$.
To prove this, suppose for a contradiction that there exists a triangulation $H=(V,E\cup F)$ of $G$  s.t.\ $|F|\leq r-2$.
Notice that the set of missing edges of $G$ is  $\textit{fill}_G(V)=\{x_iy_i|i\in\{1,\dots,r\}\}$.
Then by selection of $H$, we can fix two missing edges $x_iy_i,x_jy_j\in\textit{fill}_H(V)$ for distinct $i,j\in\{1,\dots,r\}$.
Moreover, by definition of cocktail party graphs we have that $x_j,y_j\in N_G(x_i)\cap N_G(y_i)$ so we can fix a cycle $C=(x_i,x_j,y_i,y_j,x_i)$ in the triangulation $H$.
Since $x_iy_i,x_jy_j\notin E\cup F$, $C$ is a chordless cycle, contradicting the assumption that $H$ is a triangulation of $G$.
This proves that $\textit{mfi}(G)\geq r-1$.
Now, define the edge set $F^*=\{x_iy_i|i\in\{1,\dots,r-1\}\}$ and consider the graph $H^*=(V,E\cup F^*)$.
It is easy to see that $H^*$ is chordal, as it is a complete graph minus one edge showing that $\textit{mfi}(G)=r-1$.

It is easy to see that $\omega(H^*)=2r-1$ and consequently $\textit{tw}(H^*)=2r-2$.
By definition of the treewidth parameter, $\textit{tw}(H^*)$ is an upperbound on $\textit{tw}(G)$, so $\textit{tw}(G)\leq 2r-2$.
Since $\textit{mfi}(G)=r-1$, every triangulation of $G$ is either a complete graph or a complete graph without a single edge.
This obviously implies that $\textit{tw}(G)\geq 2r-1$ which consequently proves that $\textit{tw}(G)=2r-2$.

By \cref{def:tau}, $\tau(G)=0$ if there exists a minimum triangulation with treewidth of $2r-2$.
Clearly, the minimum triangulation $H^*$, defined earlier, satisfies this condition as $\textit{tw}(H^*)=2r-2=\textit{tw}(G)$ thus showing that $\tau(G)=0$ as desired.
\end{proof}

%old note
{
% We point out that the above lemma proves a stronger property of cocktail party graphs:
% Given a graph $G$ and any elimination ordering $\alpha$ over $G$, $G^+_\alpha$ is a minimum triangulation with $\textit{tw}(G^+_\alpha)=\textit{tw}(G)$.
% In order to see this, observe that the graph $G_1$ obtained from $G$ by elimination of any vertex is a complete graph.
% Thus $\alpha$ is a peo over $G_1$ in the remaining steps and as discusses in the proof of \cref{lemma:cocktailParty}, the number of edges added by $\alpha$ is exactly equal to $\textit{mfi}(G)$.
% Since $G$ is $(|V|-1)$-regular, it is easy to see that 
% $\textit{tw}(G^+_\alpha)=|V|-2=\textit{tw}(G)$.
% In \cref{sec:tfm:Ktrees} we will discuss a large class of graphs that share a similar property.
% \unsure[inline]{
% This part is updated, is the justification sufficient? 
% Also shall I note that cycles have this property too? 
% I.e.,\ any elimination ordering $\alpha$ over a cycle $G$ produces a minimum triangulation $G^+_\alpha$ with $\textit{tw}(G^+_\alpha)=\textit{tw}(G)$.
% }
}

We point out that the cocktail party graphs are not the only the example of graphs with $\tau=0$.
As mentioned in the proof of \cref{lemma:cocktailParty}, we note that cocktail party graphs have a special property:
Any minimal triangulation $H$ of a cocktail party graph $G$ is also minimum triangulation with $\textit{tw}(H)=\textit{tw}(G)$.
Equivalently, any minimal elimination ordering $\alpha$ over $G$, the graph $G^+_\alpha$ is a minimum triangulation with $\textit{tw}(G^+_\alpha)=\textit{tw}(G)$.
In order to see this, observe that the graph $G_1$ obtained from $G$ by elimination of any vertex is a complete graph.
Thus, $\alpha$ is a peo over $G_1$ in the remaining steps.
It is easy to see that the number of edges added during $\alpha$ is exactly $|\textit{fill}_G\,(N_G(\alpha(1)))|=r-1$ which is equal to the $\textit{mfi}(G)$
% (as determined in the proof of \cref{lemma:cocktailParty})
.
Furthermore, since $\omega(G^+_\alpha)=2r-1$ we can conclude that $\alpha$ is an elimination ordering resulting in a minimum triangulation $G^+_\alpha$ with $\textit{tw}(G^+_\alpha)=\textit{tw}(G)$ as desired.
We also point out that cycles share the same property.

In \cref{sec:tfm:Ktrees} we will discuss the $\tau$ parameter of a large class of graphs and observe that they share a similar but less strict property:
Every minimal triangulation is a minimum triangulation with treewidth equal to the treewidth of the input graph, thus proving that these graphs have $\tau=0$.
}
}

% lemma showing when tau=0, used in grids
{
The following result, demonstrating a criterion for graphs to have $\tau$ value of 0, will be frequently used to prove our results in \cref{chp:grid}:

\begin{theorem}\label{lem:tau0Elim}
Let $G=(V,E)$ be a graph.
Then $\tau(G)=0$ if there exists an integer $k\in\{1,\dots,|V|-1\}$ and an elimination ordering $\alpha$ over $G$ s.t.\ all the following conditions are satisfied:
\begin{itemize}
     \item[(1)] For every step $i\in\{1,\dots,k\}$, the vertex $\alpha(i)$ satisfies one of the following conditions (A) or (B) ($F^{\alpha(i)}$ is the set of edges defined using Algorithm~\ref{alg:Fv}):
        \begin{itemize}
            \item[(A)] $\alpha(i)$ is a simplicial in $G_{i-1}$ or $G_{i-1}\oplus F^{\alpha(i)}$.
            
            \item[(B)] $\textit{deg}_{G_{i-1}}(\alpha(i))=
            \kappa(G_{i-1})$ and $\alpha(i)$ is almost simplicial in $G_{i-1}$ or $G_{i-1}\oplus F^{\alpha(i)}$.
        \end{itemize}
    \item[(2)] $\alpha$ is any minimum elimination ordering over the graph $G_k$.
    
    \item[(3)] $\max_{v\in V}|\textit{madj}^+_\alpha(v)|\leq \textit{tw}(G)$
\end{itemize}
\end{theorem}
\begin{proof}
By \cref{lem:safeVertexRepeatedly}, $\alpha$ is a minimum elimination ordering over $G$ given that it satisfies both conditions \textit{(1)} and \textit{(2)}.
Similarly, by \cref{lem:twEliminationHigherAdjacency}, $\textit{tw}(G^+_\alpha)\leq \textit{tw}(G)$ given that $\alpha$ satisfies condition \textit{(3)}.
Hence, $G^+_\alpha$ is a minimum triangulation of $G$ with treewidth of at most $\textit{tw}(G)$ proving that $\tau(G)=0$ (following \cref{def:tau}).
\end{proof}

The following corollary slightly extends the statement of \cref{lem:tau0Elim} using the concept of clique minimal separator decomposition:

\begin{corollary}\label{cor:tau0Elim}
Let $G$ be a graph and $\mathcal{A}_G$ the set of atoms of $G$ (as defined using Algorithm \ref{alg:cliqueMinimalSeparator}).
Then $\tau(G)=0$ if for every atom $A\in\mathcal{A}_G$ there exists an elimination ordering $\alpha$ over $A$ satisfying all conditions (1)--(3) of \cref{lem:tau0Elim}.
\end{corollary}

Before proceeding to the next section, discussing the $\tau$ parameter of graphs with bounded treewidth, we point out a general property of this parameter.
For short, \cref{rmk:tauSubSup} shows that the value of the $\tau$ parameter can change between a graph, its supergraphs, and subgraphs.
Thus, unlike some other graph parameters, $\tau$ does not have such hereditary properties.

\begin{remark}\label{rmk:tauSubSup}
Let $G=(V,E)$ be a graph from the graph class $\mathcal{G}$ defined in the proof of \cref{rmk:tauArbLarge}.
As previously shown, $\tau(G)>0$.
Let $H$ be the graph obtained from $G$ by addition $\textit{fill}_G(V)$, thus making $H$ a complete graph on $V$.
Clearly $H$ is a supergraph of $G$ and since it is already chordal we have that $\tau(H)=0$.
This proves that there is no correlation for the $\tau$ parameter between a graph and its supergraph.

In the opposite direction, let $X\subset V$ be a clique in $G$ and define the induced subgraph $Q=G[X]$.
Since $Q$ is a complete graph we have that $\tau(Q)=0$ yet for its supergraph we have that $\tau(G)>0$.
\end{remark}
}




==> content/tfm1.tex <==
\section{The Treewidth and Minimum Fill-In Problem}\label{sec:tfm:Intro}

% Intro
{
In this section, we will discuss a related but more general problem, namely the \textsc{Treewidth and Fill-In Minimization} problem (TFM problem for short).
We begin with some graph notations and a related problem, then discuss the $\tau$ parameter within the context of the TFM problem.
Later we will provide some initial results.

\textit{Interval} graphs are defined as intersection graphs of the intervals on the real line, where every vertex corresponds to an interval and an edge between 2 vertices maps to the intersection between their intervals.
% In order to discuss the relationship between Interval graphs and chordal graphs, we need to review the notion of AT-free graphs.
% Given a graph $G=(V,E)$, three pairwise non-adjacent vertices $x_1,x_2,x_3\in V$ form an \textit{asteroidal triple} (abbreviated as AT) if for every pair of vertices $x_i,x_j\in\{x_1,x_2,x_3\}$ there exists a $x_ix_j$-path in $G$ without any internal vertices from $N_G(x_l)$ where $x_l=\{x_1,x_2,x_3\}\setminus\{x_i,x_j\}$.
% A graph is \textit{AT-free} if it does not contain an AT, and a chordal graph is an \textit{interval} graph if and only if it is AT-free.
Interval graphs were first introduced in \cite{IntervalGraphs} where it is shown that every graph can be turned into an interval graph by addition of edges.
The connection between pathwidth, treewidth and interval graphs has been shown in \cite{BODLAENDER19981}.
Formally, given a graph $G=(V,E)$ and an interval supergraph $H^*=(V,E\cup F^*)$ of $G$ where $\omega(H^*)$ is minimized, $\omega(H^*)-1=\textit{tw}(H^*)=\textit{pw}(H^*)=\textit{tw}(G)=\textit{pw}(G)$.
As briefly mentioned in \cref{sec:perliminaries:general},
$\textit{pw}(G)$ equals to the minimum width of all the tree decomposition of $G$ with a path as the tree of the decomposition.
In \cite{Dar2019}, the authors consider the multi-criteria problem \textsc{Pathwidth and Profile Minimization}, abbreviated as \textsc{PPM}.
Given a graph and integers $k$ and $c$, the \textsc{PPM} problem asks whether there exists an interval supergraph with the clique size of $k+1$ that has at most $c$ many edges.
In \cite{Dar2019} it is proven that given an integer $t$ at most equal to pathwidth of the graph added by 1, there exists an interval supergraph that minimizes clique size and the number of edges respectively within a factor of $1+\frac{2}{t}$ and $t+2$ of their minimum values. 
The next problem discussed in \cite{Dar2019} is the \textsc{Treewidth and Fill-In Minimization} problem or \textsc{TFM} for short.
Given a graph and two parameters $k,c$, the goal of the \textsc{TFM} problem is to find a triangulation that is up to additive constants $k$, $c$ ``close'' to the optimal value of the minimum fill-in and treewidth.

% We begin this chapter by observing some basic properties of the \textsc{TFM} problem.
% However, our main focus will be on a more specific problem of answering if given a graph, does there exist a minimum triangulation with clique size equal to the treewidth of the input graph plus 1.
% It is known that the answer to this problem is not trivially yes since \cite{kloks1994treewidth,manciniPhd,Dar2019} have all constructed distinct graphs where there does not exist any minimum triangulation with clique size equal to treewidth of the graph plus 1.
% In this section, we will actually use a similar construction to that of \cite{Dar2019} for our results.

We note that in terms of graph searching (discussed in \cref{chp:ins}), the \textsc{PPM} problem is equivalent to finding a standard node searching strategy over a graph s.t.\ the number of searchers and the cost of search is minimized simultaneously.
Similarly, the \textsc{TFM} problem is concerned with finding an inert node searching strategy over a given graph, s.t.\ the number of searchers and guard cost are minimized at the same time.
}

% def of TFM
{
Below, we have a formal definition for the \textsc{TFM} problem:

\begin{enumerate}
    \item[] The \textsc{TFM} problem (Treewidth and Fill-in Minimization):
    \item[] \textbf{Input:} A graph $G = (V,E)$, integers $k$ and $c$.
    \item[] \textbf{Question:} Is there a chordal supergraph $H=(V,E\cup F)$ s.t.\ $\textit{tw}(H)-\textit{tw}(G)\leq k$ and $|F|-\textit{mfi}(G)\leq c$?
\end{enumerate}

% We point out that the goal of the TFM problem is to minimize both parameters $k$ and $c$.
% However \cite{Dar2019} which introduces this problem (as well as the PPM) does not clearly specify how the two parameters should be minimized.
% This is mainly due to the fact that there exists classes of graphs where the parameters $k,c$ cannot be simultaneously minimized\unsure{needs clarification? Means we cannot have $k<\tau$ and $c<\phi$} (see \cref{lem:tfm} for the TFM problem and \cite{Dar2019} for a similar result for the PPM problem).
% Additionally, in this section we are only concerned with the decision version of this problem.
}

% \todo{I am afraid, this para is not written well, TFM is not well established problem—just defined in this one paper. The informal motivation and the idea behind this definition explained before, so it may be better to don't touch this area at all and remove the whole para. Everything has a sense without it, too….}

% tau phi in relation to tfm
{

% For short, the \textsc{TFM} problem for a graph $G$ and $c=0$ has a yes answer if $k\geq \tau(G)$.
% Analogously, the \textsc{TFM} problem for a graph $G$ and $k=0$ has a yes answer if $c\geq \phi(G)$.

Recall that by \cref{def:tau} and \cref{def:phi}, $\phi(G)>0$ if and only if $\tau(G)>0$ for a graph $G $.
The following statement puts these two parameters within the context of the TFM problem.

\begin{lemma}\label{lem:tfm_when_tau=0}
Let $G$ be a graph. 
If $\tau(G)=0$ then the TFM problem has a yes answer for every $k,c\geq 0$.
Otherwise, the TFM problem has a yes answer if:
\begin{itemize}
    \item[(i)] $c\geq \phi(G)$ and $k\geq 0$
    \item[(ii)]$k\geq \tau(G)$ and $c\geq 0$
\end{itemize}
\end{lemma}

\begin{proof}
Let $G=(V,E)$ be a graph.
Begin by assuming that $\tau(G)=0$.
By \cref{def:tau}, there exists a minimum triangulation $H=(V,E\cup F)$ of $G$ where $\textit{tw}(H)=\textit{tw}(G)$.
Then it is easy to see that for any $k\geq \textit{tw}(H)-\textit{tw}(G)= 0$ and $c\geq |F|-\textit{mfi}(G)= 0$ the TFM problem has a yes answer.
Thus suppose that $\tau(G)>0$.
Let $H'=(V,E\cup F')$ be a minimum triangulation of $G$ selected s.t.\ $\omega(H')$ is minimized.
Then by \cref{def:tau}, for every $k\geq \textit{tw}(H')-\textit{tw}(G)= \tau(G)$ and $c\geq |F'|-\textit{mfi}(G)= 0$ the TFM problem has a yes answer which corresponds to part (i).
Next, let $H^*=(V,E\cup F^*)$ be a triangulation of $G$ with $\textit{tw}(H^*)=\textit{tw}(G)$ selected s.t.\ $|F^*|$ is minimized.
Similarly, by \cref{def:phi}, for every $c\geq |F^*|-\textit{mfi}(G)= \phi(G)$ and $k\geq \textit{tw}(H^*)-\textit{tw}(G)= 0$ the TFM problem has a yes answer corresponding to part (ii).
\end{proof}

We point out that 
% given a graph $G$ with $\tau(G)>0$, 
\cref{lem:tfm_when_tau=0} does not outline every possible $k,c$ values for which the TFM problem has a yes answer.
% More specifically, it is not known if there exists a graph $G$ with $\tau(G)>0$ where the TFM problem for $k<\tau(G)$ and $c<\phi(G)$ has a yes solution.
On the other hand, the following Theorem shows that there exists a graph class where for every graph $G$ the TFM problem has a no answer given every $k<\tau(G)$ and $c<\phi(G)$:

% We point out that if $G$ is chordal, then $\tau(G)=0$.
% To prove the below theorem we have slightly extended the construction from \cite{Dar2019} to show that there exists an infinite family of graphs where for every graph $G$, $\tau(G)>0$, and we will later discuss the behaviour of the \textsc{TFM} problem for these graphs.
% Before the end of this chapter, we will discuss a ``well established'' class of graphs where the value of $\tau$ is greater than 0.

% For the following theorem, we will again use the same construction from \cref{rmk:tauArbLarge}:

\begin{theorem}\label{lem:tfm}
There exists an infinite family of graphs $\mathcal G$ such that for any $G\in \mathcal G$, $\tau(G)>0$ and the answer to the \textsc{TFM} problem is `no' for every $k<\tau(G)$ and $c<\phi(G)$.
% $k,c$ if and only if $k,c$ have  the following properties:
% \begin{enumerate}
%     \item[\textit{1}.] $c\geq \phi(G)$ and $k\geq \tau(G)$
%     \item[\textit{2}.] $0\leq k <\tau(G)$ and $c\geq\phi(G)$
%     \item[\textit{3}.] $k\geq\tau(G)$ and $0\leq c<\phi(G)$
% \end{enumerate}
\end{theorem}
\begin{proof}
Let $\mathcal G$ be the graph class defined in the proof of \cref{rmk:tauArbLarge}.
So let $G=(V,E)$ be a graph from $\mathcal{G}$ and $A, B_1, B_2, C$ the non-empty vertex subsets making up $V$ satisfying the conditions stated in the proof of \cref{rmk:tauArbLarge}.
We have already proved (in the same place) the following facts:
$\textit{mfi}(G)=|B_1|^2$, $\textit{tw}(G)=|A|+|B_1|+|C|-1$, $\tau(G)=|B_1|-|A|$.
Additionally, is easy to see considering the triangulation $G\oplus \textit{fill}_G\,(N_G(\alpha(1)))$ (also defined in \cref{rmk:tauArbLarge}) that $\phi(G)= |\textit{fill}_G\,(N_G(\alpha(1))|-\textit{mfi}(G)= |A||C|-|B_1|^2$.

% proof moved to arbitrarily large tau
\iffalse
{
% To show that $\tau(G)>0$ we need to determine the value of $\textit{tw}(G)$ and show that there does not exist a minimum triangulation $H^*$ of $G$ s.t.\ $\textit{tw}(H^*)=\textit{tw}(G)$.
% In order to find the value of $\textit{tw}(G)$ we can restrict ourselves to minimal elimination orderings as discussed in \cite{BouchitteWeaklyChordal}.
% Clearly every elimination ordering over $G$ either starts by eliminating a vertex $v\in B_i$ for some $i\in \{1,\dots,r\}$ or a vertex $v\in (A\cup C)$.
% Let us consider two minimal elimination orderings $\alpha$ and $\beta$ s.t.\ $\alpha(1)\in B_i$ for some $i\in \{1,\dots,r\}$ and $\beta(1)\in (A\cup C)$.
% Let $F_\alpha,F_\beta$ to be the chords added in the corresponding minimal triangulations $G^+_\alpha,G^+_\beta$ respectively.

% $N_G(\alpha(1))=A\cup (B_i\setminus\{\alpha(1)\}) \cup C$ and by \cref{def:elimGalpha}, $\textit{fill}_G(N_G(\alpha(1)))=\{uv|u\in A,v\in C\}$ is added in the graph $G_1^\alpha$ obtained by elimination of $\alpha(1)$.
% It is easy to see that the graph $G_1^\alpha$ is chordal.
% Then no more edges are added in the remaining steps of $\alpha$.
% Formally $\alpha(i)$ for $i\in\{2,\dots,|V|\}$ must be a simplicial vertex in the graph $G_{i-1}^\alpha$.
% This follows from the fact that $\alpha$ is a minimal elimination ordering.
% Hence $\alpha$ is a perfect elimination ordering of $G_1^\alpha$ in the remaining steps.
% The graph $G^+_\alpha$ is demonstrated in \cref{fig:tauNot0:Galpha}.
% By definition of $\alpha$, $\omega(G^+_\alpha)=|A|+|B_i|+|C|=|A|+|B_1|+|C|$ we also note that , $|F_\alpha|=|A||C|$.

% Considering $\beta$ we have that $\textit{fill}_G(N_G(\beta(1)))=\textit{fill}_G(\bigcup_{1\leq i\leq r}B_i)$ is added as chords in the graph $G_1^\beta$ obtained by elimination of $\beta(1)$.
% Similar to the previous case, the graph $G_1^\beta$ is chordal therefore $\beta$ is a perfect elimination ordering of $G_1^\beta$ in the remaining steps (see \cref{fig:tauNot0:Gbeta} for a demonstration of the graph $G^+_\beta$).
% Then by the definition of $\beta$ and the fact that $\bigcup_{1\leq i\leq r}B_i$ is a clique in $G^+_\beta$ we have $\omega(G^+_\beta)=|C|+r|B_1|$ as $|A|<|C|$. We note that $|F_\beta|=\frac{r(r-1)|B_1|^2}{2}$.

% By construction of $G$, $(r-1)|B_1|>|A|$ so we have that
% $\omega(G^+_\beta)=|C|+r|B_1|>|A|+|B_1|+|C|=\omega(G^+_\alpha)$.
% Furthermore $|F_\beta|=\frac{r(r-1)|B_1|^2}{2}<|A||C|=|F_\alpha|$.
% As previously noted, for every other minimal elimination ordering $\gamma$ over $G$ either $\gamma(1)\in(A\cup C)$ then $\omega(G^+_\gamma)=|C|+r|B_1|$ and $|F_\gamma|=\frac{r(r-1)|B_1|^2}{2}$ or $\gamma(1)\in B_i$ for some $i\in\{1,\dots,r\}$ then $\omega(G^+_\gamma)=|A|+|B_1|+|C|$ and $|F_\gamma|=|A||C|$.
% Thus we have that $\textit{tw}(G)=|A|+|B_1|+|C|-1$ and $\textit{mfi}(G)=\frac{r(r-1)|B_1|^2}{2}$.
% Since there are only two possible minimal triangulations and $G^+_\beta$ is the minimum triangulation, by \cref{def:tau} we have that $\tau(G)=(|C|+r|B_1|)-(|A|+|B_1|+|C|)=(r-1)|B_1|-|A|$.
% Consequently $\tau(G)>0$ as by definition of $G$ we have that $|B_1|(r-1)>|A|$.

% \usetikzlibrary{shapes, backgrounds}
% \tikzset{
% a/.style={draw=black,ellipse,minimum width=10pt, inner sep=3pt, text width=4mm, text height=2 mm,  align=center, fill=white}
% }
% \tikzset{
% b/.style={draw=black,ellipse,minimum width=50pt, inner sep=7.5pt, text width=3mm, text height=1.5 mm,  align=center, fill=white}
% }
% \tikzset{
% c/.style={draw=black,ellipse,minimum width=175pt, inner sep=10pt, text width=3mm, text height=1.5 mm,  align=center, fill=white}
% }
% \begin{figure}
% \centering
%     \hspace{0.5cm}
%     \begin{subfigure}[b]{0.4\textwidth}
%         \begin{tikzpicture}
%             [scale=0.4,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
%             {
%             \node [a] (a) at (0,4) {A};
%             \node [b] (b1) at (-4,0) {$B_1$};
%             \node [b] (br) at (4,0) {$B_r$};
%             \node [c] (c) at (0,-4) {C};
%             \draw [line width=2pt, line cap=round, dash pattern=on 0pt off 2\pgflinewidth]
%                 (-0.7,0)--(1.1,0);
%             }
%             \begin{scope}[on background layer]
%                 \draw[-]
%                     (a)--(-5,1)
%                     (a)--(-2.1,0)
                    
%                     (a)--(5,1)
%                     (a)--(2.1,0)
                    
%                     (5.9,0)--(7.5,-4)
%                     (-3.5,0)--(7,-3.58)
                    
%                     (-5.9,0)--(-7.5,-4)
%                     (3.5,0)--(-7,-3.58)
%                     ;
%             \end{scope}
%         \end{tikzpicture}
%         \caption{$G$}
%         \label{fig:tauNot0:G}   
%     \end{subfigure}
%     \hspace{0.5cm}
%     \begin{subfigure}[b]{0.4\textwidth}
%         \begin{tikzpicture}
%             [scale=0.4,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
%             {
%             \node [a] (a) at (0,4) {A};
%             \node [b] (b1) at (-4,0) {$B_1$};
%             \node [b] (br) at (4,0) {$B_r$};
%             \node [c] (c) at (0,-4) {C};
%             \draw [line width=2pt, line cap=round, dash pattern=on 0pt off 2\pgflinewidth]
%                 (-0.7,0)--(1.1,0);
%             }
%             \begin{scope}[on background layer]
%                 \draw[-]
%                     (a)--(-5,1)
%                     (a)--(-2.1,0)
                    
%                     (a)--(5,1)
%                     (a)--(2.1,0)
                    
%                     (5.9,0)--(7.5,-4)
%                     (-3.5,0)--(7,-3.58)
                    
%                     (-5.9,0)--(-7.5,-4)
%                     (3.5,0)--(-7,-3.58)
%                     ;
%             \end{scope}
%             \draw [draw=green, rounded corners=5mm, fill=green, line width=0.1pt, opacity=0.2]
%             (-0.25,4.5)--(-6.5,0)--(-8,-4.3)--(-3.5,-5.5)--(3.5,-5.5)--(8.3,-4.3)--(-2,0)--(1.25,4.5)--cycle;
%             \draw[dashed, draw=red, thick, opacity=0.6]
%             (a)--(-7.5,-4)
%             (a)--(-5.5,-4)
%             (a)--(-3.5,-4)
%             (a)--(-1.5,-4)
%             (a)--(1.5,-4)
%             (a)--(3.5,-4)
%             (a)--(5.5,-4)
%             (a)--(7.5,-4)
%             ;
%         \end{tikzpicture}
%         \caption{$G^+_\alpha$}
%         \label{fig:tauNot0:Galpha}   
%     \end{subfigure}
%     \vspace{0.5cm}
%     \begin{subfigure}[b]{0.4\textwidth}
%         \begin{tikzpicture}
%             [scale=0.4,every node/.style={draw=black,rectangle, inner sep=0pt, text width=6mm, text height=1.75 mm,  align=right}]
%             {
%             \node [a] (a) at (0,4) {A};
%             \node [b] (b1) at (-4,0) {$B_1$};
%             \node [b] (br) at (4,0) {$B_r$};
%             \node [c] (c) at (0,-4) {C};
%             \draw [line width=2pt, line cap=round, dash pattern=on 0pt off 2\pgflinewidth]
%                 (-0.7,0)--(1.1,0);
%             }
%             \begin{scope}[on background layer]
%                 \draw[-]
%                     (a)--(-5,1)
%                     (a)--(-2.1,0)
%                     (a)--(5,1)
%                     (a)--(2.1,0)
%                     (5.9,0)--(7.5,-4)
%                     (-3.5,0)--(7,-3.58)
%                     (-5.9,0)--(-7.5,-4)
%                     (3.5,0)--(-7,-3.58);
%             \end{scope}
%             \draw [draw=green, rounded corners=5mm, fill=green, line width=0.1pt, opacity=0.2]
%             (-6.5,0)--(-5,1.5)--(5,1.5)--(6.5,0)--(8,-4.5)--(3.5,-5.5)--(-3.5,-5.5)--(-8,-4.5)--cycle;
%             \draw[dashed, draw=red, thick, opacity=0.6]
%             (3.5,1.25)--(-3.5,1.25)
%             (3.5,-1.25)--(-3.5,-1.25)
%             (3,-0.75)--(-3,-0.75)
%             (3,0.75)--(-3,0.75)
%             (2.75,-0.25)--(-2.75,-0.25)
%             (2.75,0.25)--(-2.75,0.25)
%             ;
%         \end{tikzpicture}
%         \caption{$G^+_\beta$}
%         \label{fig:tauNot0:Gbeta}   
%     \end{subfigure}
% \caption
% {
% (a) the graph $G$ from the class of graphs $\mathcal{G}$ is demonstrated and the vertices in the cliques $A,B_1,\dots,B_r,C$ alongside the edges in between them are grouped together for simplicity.
% (b),(c) respectively demonstrate the minimal triangulations $G^+_\alpha$ and $G^+_\beta$.
% The maximum clique in each graph is highlighted with green and the added edges are drawn in red.
% } 
% \label{fig:tauNot0}
% \end{figure}
}
\fi

Suppose for a contradiction that the answer to the \textsc{TFM} problem is yes for some $k<\tau(G)$ and $c<\phi(G)$.
Then we can fix a triangulation $H^*=(V,E\cup F^*)$ of $G$ s.t.\ $\textit{tw}(H^*)-{(|A|+|B_1|+|C|-1)} % -|A|-|B_1|-|C|+1
< {|B_1|-|A|}= \tau(G)$ and $|F^*|- {|B_1|^2}< {|A||C|-|B_1|^2} =\phi(G)$.
As a result, both of the following conditions must hold for $H^*$:
\begin{equation}\label{eq:lem:tfm:tw}
    \textit{tw}(H^*)<2|B_1|+|C|-1
\end{equation}
\begin{equation}\label{eq:lem:tfm:mfi}
    |F^*|<|A||C|
\end{equation}

It is shown in the proof of \cref{rmk:tauArbLarge} that for every triangulation $H$ of $G$ one of the following cases must hold:
\begin{mycases}
    \case 
    {
    $\textit{fill}_G(B_1\cup B_2)$ is added in $H$, resulting in at least $|B_1|^2$ many fill edges and treewidth of at least $2|B_1|+|C|-1$.
    Therefore, $H$ does not satisfy \cref{eq:lem:tfm:tw}.
    }
    
    \case
    {
    $\textit{fill}_G(A\cup C)$ is added in $H$, resulting in at least $|A||C|$ many fill edges and treewidth of at least $|A|+|B_1|+|C|-1$.
    Hence, $H$ does not satisfy \cref{eq:lem:tfm:mfi}.
    }
\end{mycases}

This results in a contradiction, as $G$ cannot have a triangulation $H^*$ satisfying both \cref{eq:lem:tfm:tw} and \cref{eq:lem:tfm:tw}.
We can then conclude that the answer to the \textsc{TFM} problem for every $k<\tau(G)$ and $c<\phi(G)$ is no, as desired.

% This implies that there must exist an elimination ordering $\gamma$ over $G$ where $\omega(G^+_\gamma)<2|B_1|+|C|$ and $\sum_{v\in V}|\textit{madj}^+_\gamma(v)|<|A||C|$.
% As shown in the proof of \cref{rmk:tauArbLarge}, every elimination ordering $\gamma$ over $G$ either has $\gamma(1)\in (B_1\cup B_2)$ adding at least $|A||C|$ many chords or $\gamma(1)\in (A\cup C)$ resulting in clique size of $2|B_1|+|C|$, a contradiction.

% Then by applying \cref{lem:tfm_when_tau=0}, the only other values of $k,c$ for which the answer to the \textsc{TFM} problem is `yes' is $0\leq k <\tau(G)$ and $c\geq\phi(G)$ or $k\geq\tau(G)$ and $0\leq c<\phi(G)$ proving the statement of the theorem.
\end{proof}
}
